Sum-of-Squares Lower Bounds for Independent Set in Ultra-Sparse Random Graphs

We prove that for every $D \in \N$, and large enough constant $d \in \N$, with high probability over the choice of $G \sim G(n,d/n)$, the \Erdos-\Renyi random graph distribution, the canonical degree $2D$ Sum-of-Squares relaxation fails to certify that the largest independent set in $G$ is of size $o(\frac{n}{\sqrt{d} D^4})$. In particular, degree $D$ sum-of-squares strengthening can reduce the integrality gap of the classical \Lovasz theta SDP relaxation by at most a $O(D^4)$ factor. This is the first lower bound for $>4$-degree Sum-of-Squares (SoS) relaxation for any problems on \emph{ultra sparse} random graphs (i.e. average degree of an absolute constant). Such ultra-sparse graphs were a known barrier for previous methods and explicitly identified as a major open direction (e.g.,~\cite{deshpande2019threshold, kothari2021stressfree}). Indeed, the only other example of an SoS lower bound on ultra-sparse random graphs was a degree-4 lower bound for Max-Cut. Our main technical result is a new method to obtain spectral norm estimates on graph matrices (a class of low-degree matrix-valued polynomials in $G(n,d/n)$) that are accurate to within an absolute constant factor. All prior works lose $\poly log n$ factors that trivialize any lower bound on $o(\log n)$-degree random graphs. We combine these new bounds with several upgrades on the machinery for analyzing lower-bound witnesses constructed by pseudo-calibration so that our analysis does not lose any $\omega(1)$-factors that would trivialize our results. In addition to other SoS lower bounds, we believe that our methods for establishing spectral norm estimates on graph matrices will be useful in the analyses of numerical algorithms on average-case inputs.

==> edgeval.tex <==
 \section{Tight matrix norm bounds: vertex encoding cost and edge-value assigment}
%We will bound the trace on each length-2 block by, \[ 
%\max_{\calL:\text{ labeling of the edges}, |F|\geq |R|} \val(\calL)\cdot \cnt(\calL)
%\]
As illustrated in our toy-examples, our starting point here is edge-labeling,
\begin{definition}[Edge labeling]
	 A labeling $\calL$ for a walk assigns each edge in the length-$q$ walk a label in $\{F,R, H\}$, with \begin{itemize}
		\item $F$: a (forward) edge appears for the first time in the walk;
		\item $H$: a (high-mul) edge appears for neither the first nor the last time in the walk; 
		\item $R$: a (return) edge appears for the last time in the walk;
	\end{itemize}
	By default, we assume $\calL$ assigns the labels according to the traversal from $U_\al$ to $V_\al$; analogously, we denote $\calL^T$ if we traverse $\calL$ in a reverse direction from $V_\al$ to $U_\al$.
\end{definition}
\begin{remark}
	With some abuse of notation, we will also use $\calL$ (and analogously $\calL^T)$ to denote the labeling of a walk restricted to a a single block. 
\end{remark}
% \begin{observation}
% 	Any edge that is $F$ under $\calL$ becomes $R$ in $\calL^T$, and any edge that is $R$ under $\calL$ becomes $F$ in $\calL^T$; any $H$ edge remains the same.
% \end{observation}
%\begin{proposition}[Label value]
%	Each edge contributes a fixed value to the trace under a given label, \begin{itemize}
%		\item $F$: each $F$ leg corresponds to some edge appearing the first time, and contributes value of at most \[  \sqrt{\frac{n}{d}}\cdot \frac{d}{n}\cdot \singdecay \ll \sqrt{\frac{d}{n}}\cdot \exp(-d)\]
%		\item $R$: each $R$ leg corresponds to some edge appearing the second time, and contributes value of at most \[
%		 \sqrt{\frac{n}{d}}\cdot \frac{1}{\singdecay} 
%		 \]
%		 \item $H$: each $H$ leg corresponds some edge appearing high-mul, and contributes value of at most \[ 
%		 \sqrt{\frac{n}{d}} 
%		 \]
%%		 \item $S$: each $S$ leg corresponds to some edge appearing the first time, and we additionally charge the cost required in indicating the unforced return caused by the surprise visit to its edge value, and we have \[
%%		 \sqrt{\frac{n}{d}}\cdot \frac{d}{n}\cdot \singdecay\cdot (2|V(\al)|q)		  \]
%	\end{itemize}
%\end{proposition}
%Assuming each edge appears in the walk for at least twice, we can ignore the singleton decay and redistribute the factors as the following,
%\begin{proposition}[Label-value ignoring singleton decay]
%	Each edge contributes a fixed value to the trace under a given label, \begin{itemize}
%		\item $F$: each $F$ leg corresponds to some edge appearing the first time, and contributes value of at most \[ 
%		\frac{1}{\sqrt{n}}
%		\]
%		\item $R$: each $R$ leg corresponds to some edge appearing the second time, and contributes value of at most \[
%		 \sqrt{n}
%		 		 \]
%		 \item $H$: each $H$ leg corresponds some edge appearing high-mul, and contributes value of at most \[ 
%		 \sqrt{\frac{n}{d}} 
%		 \]
%%		 \item $S$: each $S$ leg corresponds to some edge appearing the first time, and we additionally charge the cost required in indicating the unforced return caused by the surprise visit to its edge value, and we have \[
%%		 \sqrt{\frac{n}{d}}\cdot \frac{d}{n}\cdot \singdecay\cdot (2|V(\al)|q)		  \]
%	\end{itemize}
%
%\end{proposition}

%\begin{definition}
%	Given a length-$2$ block and a labeling $\calL$, let $S\subseteq V(\al), S'\subseteq V(\al^T)$ be the set of vertices incident to some edge receiving $H$ label, and furthermore, we let \begin{itemize}
%		\item $S_L$ be the set of vertices reachable from $U_\al$ without passing through any other vertex in $S$;
%		\item $S'_{R^T}$ be the set of vertices reachable from $V_\al$ without passing through any vertex in $S'$. 
%	\end{itemize} 
%\end{definition}
We now describe our encoding scheme given the edge-labeling. The encoding works by maintaining a set $W_t$ of the vertices in the current block revealed to us already, and walk along edges greedily to expand $W_t$ until all vertices in the walk are encoded, i.e., $W_t =V((\al\circ \al^T)^q)  $ . In this section, we determine the cost of each encoding according to the cut edge used in encoding the vertex. 


%
%
%\subsection{Vertex encoding scheme}
%
% We first observe that for any shape $\al$, we can decompose the shape into $\al = \tilde{\al} \cup \branch(\al) \dang(\branch)$ where $\tilde{\al} $ is a shape obtained from $\al$ by removing any dangling branch, and $\branch(\al)$ is the collection of dangling branches in $\al$. With this decomposition, our encoding proceeds in the following two-step process \begin{enumerate}
%	\item Step 1: Encode the constraint graph restricted to the non-dangling part of \emph{length $q$};
%	\item Step 2:  Fix an order to traverse and attach dangling branches, then follow the fixed order to encode the dangling branches and attach them to the non-dangling constraint graph.
%\end{enumerate}
%In either step, we appeal to the following greedy vertex-encoding procedure for identifying vertices in the corresponding constraint-graph (i.e., assigning them labels in $[n]$).
%
%For a fixed set $W_t$ at time-stamp $t$, and a given shape $\al$, we consider the edges across the cut produced by $W_t$, let $B_t\subseteq V((\al\circ \al^T)^q)\setminus W_t$ be the set of unknown vertices incident to some cut edge, and let $(i,j)$ be some edge across the cut with $i\in W_t, j\notin W_t$,
%
%\begin{mdframed}[frametitle = {Vertex encoding procedure }]
%
%\begin{enumerate}
%	\item By default, we set $W_0=U_\al$: any vertex in $U_\al$ is the starting point revealed to us from the last block, hence no encoding needed;
%	\item  \label{enu:return} if there's an $R$ edge $(i,j)$ across the cut, we expand $W$ along this edge o.w.;
%	\item  \label{enu:long-high-mul-path} if there is a path of $H$ edges connected to $W$ across the cut of length at least $\log_d 2q|V(\al)|$, split the path into chunks of length at most $\kappa$ and encode each chunk's boundary in $2q|V(\al)|$ with an extra constant in $[2]$ indicating cycle orientation using $2$-cycle freeness;
%	\item \label{enu:doubly-constrained} if there is some vertex $v\in B_t$ that has (at least) two paths of $H$ edges connected to $W$, the vertex is doubly-constrained (unless the path crosses $U_\al$ or $V_\al$), and all vertices along this path can be encoded using a label in $[2]$ to indicate the orientation of the cycle altogether by using $2$-cycle freeness; (specifically, if the path has a combined length of $\ell \gg \kappa$, we need to encode additional vertices in $|2qV(\al)|$ with a label in $[2]$ for every $\kappa$ vertices to identify the entire cycle, however, this is $(1+o(1))$ per vertex on average); o.w.,
%	\item if there are multiple high-mul paths crossing $U_\al$ or $V_\al$, and it is a mirror copy, we expand  along these high-mul paths until the entire mirror copy is encoded into $W$; o.w.,
%	\item if there is an $H$ edge $(i,j)$ across the cut, we expand $W$ along this edge;
%	\item \label{enu:surprise-visit} if there is an $F$ edge $(i,j)$ across the cut for $j\notin U_\al\cup V_\al $, and $j$ is incident to some $H$ edge or $R$ edge outside the cut, or $j\in U_\al\cup V_\al$ while $j$ is incident to some $H$ edge outside the cut, we expand along this edge; o.w.,
%	\item expand along the $F$ edges;
%	\item we additionally require all vertices in the current length-$2$ block to be decoded before decoding vertices in the new block (except the vertices decoded by doubly-constrained vertices crossing the boundary or by mirror copy);
%	\item (Excess $F$ edge clean-up) for each length-$2$ block, if there is any $F$ edge that does not get encoded as the cut edge, we assign an extra label in $|2qV(\al)|$ for each such edge indicating their second-time being used (if any). 
%  \end{enumerate}
% \end{mdframed}
% \begin{remark}
% 	The above encoding scheme applies in a straightforward way for traversing walks in a reversed direction from $V_\al$ to $U_\al$.
% \end{remark}
%

%
%\subsection{Return is forced}
%Consider the invariant that any $H_v$ component at the boundary (throughout the growth of $H_v$ component), sees (on the boundary) at most $1+ 2\cdot s(H_v)$ unclosed $F$ edges where $s(H_v)$ is the number of surprised visits arriving at vertices in $H_v$. 
%
%
%
%Let $v$ be the current vertex at time $t$, let $H_t(v)$ be the component reachable from the boundary at time $t$ in the walk using $H$ edges. Notice $H_t(v)$ is a vertex component that is grown from some vertex not necessarily $v$ throughout the walk, and we can keep track its growth as the following:
%\begin{enumerate}
%	\item Starting from $v_0$ some vertex, it may have $1$ unclosed $F$ edge (the one that explores $v_0$), and at time $0$ we have $V_{t=0} (H_t(v)) = \{v_0 \}$;
%	\item  
%\end{enumerate}
%
% and let $F_t(H_t(v))$ be the number of distinct unclosed $F$ edges
%
%\subsubsection{Return is forced}
%\begin{claim}
%	For a vertex $v$ on the boundary of encoding process at time $t$, let $F_t(v)$ be the number of unclosed $F$ edges incident to $v$ at time $t$, and let $S_t(v)$ the number of surprise visits arriving at $v$, \[ 
%	F_t(v)\leq 1 + 2\cdot S_t(v) 
%	\]
%	More generally, let $H_v$ be the component of edges reachable from $v$ using $H$ edges, and let $F_t(H_v)$ be the number of unclosed $F$ edges incident to any vertex in $H_v$, and define $S_t(H)$ be the number of unclosed surprise visits arriving at vertices in $H_v$ at time $t$, we have \[ 
%	F_t(H_v) \leq 1+ 2\cdot S_t(H_v)
%	\]
%\end{claim}
%\begin{proof}
%	 We prove by induction. This is immediate for the base case, and when there is no surprise visit at all (as the walk is a tree with potentially repeated branches). Suppose we are currently at boundary vertex $u$ and the hypothesis holds so far in the walk by time $t$, and suppose in the next step we move on to $v$, and it suffices for us tho show this holds for $H_v$ after this move. Let $t_v$ be the most recent time some vertex in $H_v$ is on the boundary prior to this move, 
%	 
%	 Before we start, we first observe that we have to leave an $H_v$ component via some $F$ edge, as using $R$ edge from $H_v$ automatically pushes the new vertex into $H_v$ (if not already).
%	 
%	  We case on the status of the leg $u\rightarrow v$, and it suffices for us to focus on $F/R$ edge as $H$ is automatically accounted for by definition,
%	 \begin{enumerate}
% 	\item Innovative $F$ edge: this is immediate as $H_u=\{u\}$ and both sides are $1$;
% 	\item Surprise $F$ edge: if $u$ and $v$ are in the same $H$ component prior to this move, applying the hypothesis on $H_u$ prior to the move, we pick up an $1$ on the LHS via the new $F$ edge and a $2$ on the RHS; 	otherwise, applying the hypothesis on $F_{t_v}(H_v)$, since we depart from $H_v$ at $t_v$, $F_t(H_v)\leq 2+ F_{t_v}(H_v)$, while we pick up at a gain of $2$ on RHS via the new surprise visit; 	 	
% 	\item $R$ edge: if $u$ and $v$ are not in the same $H$ component prior to this move, and the $R$ edge now merges two $H$ components. Notice before the $u\rightarrow v$ edge is used, \[
% 	F_{t}(H_u) \leq 1+ s_t(H_u)  
% 	 \]  
% 	and the component $H_v$ is incident to at most \[ 
% 	F_{t_v}(H_v) + 1
% 	\]
% 	unclosed $F$ edges (via our inductive hypothesis at $t_v$ and we may depart $F_v$ by an additional $F$ edge). That said, notice the $u\rightarrow v$ edge at time $t$ contributes to both of the above as an unclosed $F$ edge, and it gets closed after the $u\rightarrow v$ leg is used,
% 	 \begin{align*}
% 		F_{t+1}(H_{v}) &\leq F_{t_v}(H_v)  + F_t(H_u) + 1 - 2 \\
% 		&= 1+ 2\cdot S_{t_v}(H_v) + 1+ 2\cdot S_t(H_u) + 1 - 2\\
% 		&\leq  1+ 2\cdot \left(S_{t+1}(H_v)+ (S_{t+1}(H_u)\right)\\
% 		&= 1+ 2(S_{t+1}(H_v))
% 	\end{align*}
% 	 \end{enumerate}
% \end{proof}
%
%Since the number of unforced return from any $H$ component is at most the number of \emph{distinct} $F$ edges witnessed by  $v$ when it is on the boundary, summing over all vertices gives us a bound of \[ 
%r \leq 3s
%\]
%where $r$ is the number of unforced returns throughout the walk, and $s$ the number of surprise visits.
%
%\subsubsection{(Non-dangling) Second-use is forced}
%
%	
%In this subsection, we bound the vertex factors of vertices arrived along some $R$ edge. In particular, our bound is most important for non-dangling $R$ edges where we show no vertex factor is needed for vertices arrived along such edges.
%
%Consider the following invariant, \begin{proposition}[No dangling factor]
%	By assigning each surprise visit at most $2$ return time-marks, the $H$ component of the boundary vertex, has at most $1$ unclosed $F$ edge with unspecified return-time mark; moreover, any $H$ component that can be reached without using new $F$ edges has at most $1$ unclosed $F$ edge with unspecified return-time mark if arrived on the boundary.
%\end{proposition}
%
%\begin{proof}
%	Notice this is immediate if there is no surprise visit for the entire walk and also the base case. Suppose we are currently at boundary $v$ and let $H_v$ be the component reachable, notice the hypothesis is immediate if we leave $H_v$ to explore a new vertex using a novel edge, as the new $H$ component at the boundary is solely the new vertex. That said, it suffices for us to consider departing from the current $H_v$ component, potentially to a new vertex, and then back to the $H_v$. Via our invariant, by the ti\end{proof}
%
% \begin{claim}[Vertex-factors for $R$] \label{claim:non-dangling-return-is-forced}
%		Each vertex arrived along a non-dangling $R$ leg (appearing for the last time) does not contribute any vertex factor; each vertex arrived along a dangling $R$ leg can be specified at a vertex cost of $d$; each floating component incident to some $R$ leg can be identified at a cost of at most $2|V(\al)|q$.
%\end{claim} 
%
%We start with the following observation and proposition.
%\begin{observation}
%	If a vertex is non-dangling, any cut edge that encodes the vertex is non-dangling.
%\end{observation}
%
%	We call an $F$ leg closed if there it has been used for the second time; otherwise, we call it unclosed. And recall that a vertex is dangling if it is not on any simple path from $U_\al\setminus V_\al$ to $V_\al\setminus U_\alpha $; analogously, we call an edge dangling if it is not on any simple path from $U_\al\setminus V_\alpha $ to $V_\al \setminus U_\al$. 
%
%\begin{proposition}
%	Any vertex on the boundary incident to an $R$ edge across the cut is incident to at most 1 unclosed (non-dangling) $F$ edge  with unspecified return time-mark, except dangling $F$ edges or non-dangling $F$ edges whose other endpoints are already encoded in the current block. 
%\end{proposition}
%\begin{proof}
%	We prove by induction for any non-dangling vertex $v$. Suppose this is true for vertex $v$ in the beginning of the current block. Note the claim is immediate if $v$ has not appeared in the previous blocks. We discuss by cases depending on whether $v$ produces multiple non-dangling $F$ edges in the last block it appears in the boundary.
%	
%	 If not, $v$ produces at most one non-dangling $F$ edge (with unspecified return-time) and gets bumped out of the boundary after the other endpoint of the indicative edge is encoded. In this case, in order to include $v$ into the boundary of our current block, it is either already in $U_\alpha$ in which case the claim is trivial by the inductive hypothesis, or we have to arrive at $v$ across some cut edge, and we now discuss by cases.
%%	  If we arrive at $v$ along some H edge, this does not open up new (non-excessive) F edge incident to $v$ (it might open up new F edge but they would either have to be excessive as they are not used to indicate the label of $v$, or they lead to new vertices whose endpoints are encoded in the current block); otherwise, 
%%	  If we arrive along some $F$ edge, this is either along the first edge leading to $v$, or a surprise visit which comes with a specified return time-mark. 
%	  By our inductive hypothesis, vertex $v$ can be incident to at most $2$ non-dangling $F$ edges with unspecified time-mark in the beginning of the current block (one from the inductive hypothesis when $v$ gets encoded into the boundary, and one from the potentially new indicative edge it opens up the last time it appears on the boundary). The claim is immediate if we arrive at $v$ along some $R$ edge as it would close an non-dangling $F$ edge incident to $v$. Otherwise, if we arrive along some $F$ edge or $H$ edge, we claim all but one ''unforced'' non-dangling $F$ edges at vertex $v$ receive a hardwired return time-mark. 
%	   and hence when $v$ gets encoded in the current block, it would have at most $1$ unclosed non-dangling $F$ edge incident to it. 
%%	   If we are arrive at $v$ along an $F$ edge, this is a surprise visit, and it is sufficient for us to hardwire the edge-choice for the next ''unforced'' return at $v$ when the surprise visit is created. Analogously, if we arrive at $v$ along an $H$ edge, consider the path from the last time $v$ appears in the boundary to the current boundary, we note that there must be a surprise visit on this path and again we can hardwire the edge-choice for the first ''unforced'' return when the surprise visit is created. 
%	\begin{claim}
%		[Each surprise visit creates at most $1$ ''unforced'' return] For each vertex $v$, let $m_v$ be the number of surprise visits that get charged to ''unforced'' return at $v$, and $r_v$ the number of unforced return at $v$,\[ 
%	r_v\leq m_v	
%		\]
%	\end{claim}
%	\begin{proof}
%	Consider the path induced by the walk from the last time $v$ appears in the boundary to the current boundary, and we first assume each vertex on the path only opens up at most $1$ non-dangling $F$ edge in the boundary. For each unforced return at $v$, we note that there must be a surprise visit we can charge to depending on how we arrive at $v$, \begin{enumerate}
%			\item If we arrive along an $F$ edge, this is a surprise visit and we can charge to this edge;
%			\item If we arrive at $v$ along an $H$ edge, consider the invariant that $H_v$ the current component reachable from $v$ via $H$ edges is incident to at most $1$ unspecified-return (non-dangling) $F$ edge:\begin{itemize}
%				\item if we arrive via an $H$ edge, the invariant is preserved from the last vertex (that they are in the same $H$ component);
%				\item if we arrive via an $R$ edge, this may merge two $H$ components $H_u$ and $H_v$.  Observe that $H_v$ is incident to at most $2$ unspecified $R$ edge before the current $R$ edge being used, and applying the invariant on $H_u$, we know it has at most $1$ unspecified $R$ edge. We now case on whether the $R$ edge receives a fixed time-mark: if not, $H_{u\cup v}$ is incident to at most $1$ unspecified $F$ after the $R$ edge being used; otherwise, if the $R$ edge receives a fixed time-mark, $H_{u\cup v}$ is incident to at most $3$ unspecified $F$ edges, that being said, we can charge $2$ of them to the surprised visit between $H_{u}$ and $H_{v}$, and an $O(1)$ bound is preserved; 
%				\item if we arrive via an $F$ edge, $H_v$ originally has at most $2$ unspecified $F$ edges, and this is a surprise visit, we can charge both $2$ of the previous unspecified $F$ edges to this surprise visit.
%			\end{itemize}
%			
%					\end{enumerate} 
%%		Analogously, if we arrive at $v$ along an $H$ edge, consider the path from the last time $v$ appears in the boundary to the current boundary, we note that there must be a surprise visit on this path and again we can hardwire the edge-choice for the first ''unforced'' return when the surprise visit is created. 
%%
%	To generalize to arbitrary path, we note that each vertex that opens up multiple $F$ edges across the cut must be a mirror copy, or there is a surprise visit or excess $F$ edge, both of which come with a hardwired label.
%	\end{proof}
%	
%	If $v$ opens up multiple (non-dangling) F edges with unspecified time-mark the last time it is on the boundary, before $v$ gets encoded into the boundary of the current block, these non-dangling $F$ edges will all have to be closed by some (non-dangling) $R$ edge already unless there is a surprise visit or excess $F$ edge before the next time $v$ appears in the boundary. 
%\begin{claim} \label{claim: multiple-path-mirror}
%	If there are multiple paths from $v\in V(\al)$ to $v^T\in V(\al^T)$ starting with $F$ edges, each path must be a mirror path unless there is an excessive $F$ edge or surprise visit in all but one of the paths.\end{claim}
%\begin{proof}
%	Let $P_1, P_2$ be two paths from $v$ to $v^T$ s.t. the first edge of each path incident to $v$ is F. Fix one path, if it is not a mirror copy, then we can assume $v^T$ would receive a different a label in $v$, otherwise there is a surprise visit on this path. However, suppose $v^T$ receive a different label, we now consider the second path. Again, each edge on the second path pointing to $v^T$ must be an $F$ edge, o.w., there is be a surprise visit in the second path alone, however, we would have produced a cycle of $F$ edges from $v$ to $v^T$, resulting in excess $F$ edges. 
%	
%	Finally, fixing one path, if any, that does not have surprise visit or excess $F$ edge and applying this argument with any other path gives the desired claim
%\end{proof}
%From the above claim, unless in the adjacent block is there an excessive $F$ edge, any path from $v$ starting with an $F$ edge is a mirror-copy, and hence each of the $F$ indicative edge from $v$ that gets opened up in the current block would also be closed in the second block when $v$ gets encoded into the boundary; hence, by our induction hypothesis, when $v$ is in the boundary, it would still be incident to at most one unclosed $F$ edge with unspecified time-mark.
%	\end{proof}
%From the above, we show that when a vertex $v$ when gets encoded into the boundary, it can be incident to at most $1$ non-dangling $F$ edge with unspecified return time-mark. 
%%\begin{corollary}[Encoding cost for \ref{enu:return}] 
%%	If vertex $v$ is not incident to any dangling edge, then any second-use edge from $v$ does not require any encoding cost in addition to specifying the edge-type; more generally, for a vertex incident to $t$ dangling edges, the cost of identifying second-use edges from $v$ is at most $d^{t}$. 
%%\end{corollary}
%%\begin{proof}
%%	The first part is immediate; to see the second part, whenever a vertex is incident to both dangling $F$ edges and a non-dangling $F$ edge, we follow the principle that to identify a return leg using dangling $F$ edge, we can use a label in $[d]$ while presume the return is using the non-dangling $F$ edge if no extra label is provided.
%%\end{proof}
%\begin{proof}[Proof to claim~\ref{claim:non-dangling-return-is-forced}]	
%Note that without loss of generality, we can exchange the vertex cost for indicating the destination of a leg's second appearance with the last appearance in our charging scheme.
%Moreover, we can adopt the principle that to identify a return leg using dangling $F$ edge, we can use a label in $[d]$ while presuming the return is using the non-dangling $F$ edge if no extra label is provided, and our claim now follows from the above proposition.
%\end{proof}
%
%Finally, despite the above section focuses on the second-use of a leg, we note that without loss of generality, we can exchange the vertex cost for indicating the destination of a leg's second appearance with the last appearance in our charging scheme, and this yields us the main claim of this subsection.
%
% \begin{claim}[Vertex-factors for $R$] \label{claim:non-dangling-return-is-forced}
%		Each vertex arrived along a non-dangling $R$ leg (appearing for the last time) does not contribute any vertex factor; each vertex arrived along a dangling $R$ leg can be specified at a vertex cost of $d$; each floating component incident to some $R$ leg can be identified at a cost of at most $2|V(\al)|q$.
%\end{claim} 

%\input{sparse_trace_method/order-return.tex}

\input{sparse_trace_method/return-factor.tex}

\subsection{(Local) $2$-cycle-freeness can be useful}
\begin{proposition} \label{prop:long-high-mul-path}
	Given the starting vertex, a path of $H$ edges of length $t$ can be encoded at a cost of \[ 
	(2\cdot 2q|V(\al)|)^{\lceil \frac{t}{\kappa}\rceil }
	\]
\end{proposition}
\begin{proof}
	Since the graph is $2$-cycle-free at every $\kappa$ neighborhood, it suffices to split the long walk into $\lceil \frac{t}{\kappa} \rceil$ chunks, and encode the vertex at the end of each chunk; additionally, since there are at most $2$ paths between the start and end of each chunk, a label in $[2]$ to identify the orientation of the cycle is sufficient to recover the entire path.
\end{proof}
\begin{proposition}
	For any un-encoded vertex that has at least two paths of $H$ edges to some known vertices, the vertex is doubly-constrained, and the entire paths can be encoded at a cost of \[ 
	2\cdot (2\cdot 2q|V(\al)|)^{\lfloor \frac{t}{\kappa}\rfloor }
	\]
	\end{proposition}
\begin{proof}
	The proof is identical to the above, except we no longer need to identify an extra endpoint for the end of the last chunk to use local $2$-cycle-freeness.
\end{proof}
\begin{remark}
	Throughout our work, we will take $2q\cdot|V(\al)|\approx n^\epsilon$ and $\kappa\approx 0.3\log_d n$, which would give us \[
	(2q\cdot|V(\al)|)^{1/\kappa }\leq c
	 \]
	 for some constant $c>0$ independent of $d$ provided $\eps<O(\frac{1}{\log d}) $ where we take \[ 
	 q=\Theta(\sqrt{|U_\al||V_\al|} \log^2 n)
	 \]
\end{remark}

In addition to the main claim that gives an additional factor of $d$ for each dangling vertex, we observe $2$-cycle freeness can be exploited to improve that bound.

\begin{proposition}[Improved vertex factor for dangling $R$ vertices]
Let $\al$ be a given shape, and let $S$ be a separator for some irreducible locally optimal labeling, we let $\dang(\al\setminus S)$ be the dangling factor for $S$,
	\[ 
	\dang(\al\setminus S) \leq \prod_{i\in \branch(\al\setminus S)} \min(2|V(\al)|q, d^{|\branch(i)|})
	\]
\end{proposition}
Observe that by possibly removing some edges incident to some dangling vertex if necessary, $\dang(\al\setminus S)$ can be partitioned into a collection of trees rooted at some non-dangling vertex in $\al$, and moreover, we call each vertex dangling in $\dang(\al\setminus S)$ a branch point if it is either a leaf, or has degree bigger than $1$. For each branching point $i\in \branch(\al\setminus S)$, let $\branch(i)$ denote the vertices on the path from last branching point (or the nearest non-dangling vertex) to $i$.  We are now ready to prove the proposition.


\begin{proof}
	Notice for each branch, a label in $2|V(\al)|q$ is sufficient using Proposition~\ref{prop:long-high-mul-path}; alternatively, a label in $d$ is sufficient for identifying each ''explored'' dangling vertex.
\end{proof}

%	 The above is almost sufficient to give us the desired proposition, except we note that the factors inside the proposition comes with an extra square root. To see this, we case on whether the vertex-factor is used to indicate a second-use path or a high-mul path. 
%
%
%	For the last appearance of an edge that lead to dangling vertices/branches, recall that we exchange the vertex factor for the second-use and the last appearance of an edge, the factor of $2|V(\al)|q$ or the factors of $d$ is only needed when the edge is being visited the second time (that it is not needed when it first appears),  hence taking the average with when the edge appears for the first time gives us the desired square root.
%	
%	For the case of middle appearances, notice each edge comes with a value of $\sqrt{\frac{n}{d}}^{\branch(i)}$, while each time a label in $2|V(\al)|q$ or a sequence of labels in $d$ is needed, giving us a total of \begin{align*}
%		\sqrt{\frac{n}{d}}^{\branch(i)}\min(2|V(\al)|q, d^{\branch(i)}) &\leq 
%	\sqrt{n}^{\branch(i)} \min(\frac{2|V(\al)q}{\sqrt{d}^{\branch(i)} }, \sqrt{d}^{\branch(i)}) \\&\leq \sqrt{n}^{\branch(i)}\min(\sqrt{2|V(\al)|q} ,\sqrt{d}^{\branch(i)})
%	\end{align*}
%	Recall that the factors of $\sqrt{n}^{\branch(i)}$ is already taken into account by the vertex factors of $\sqrt{n}$ for each vertex outside the separator, hence, each block's dangling blow-up is still at most $\min(\sqrt{2|V(\al)|q} ,\sqrt{d}^{\branch(i)})$ for each branch. Combining the argument for all dangling branches gives us the desired proposition.






\paragraph{Balance in $d$}
A priori, we need to show for each high-mul (non-separator) leg in the walk, only a $\sqrt{d}$ cost is sufficient for encoding, so that we can assign a cost of at most $\sqrt{n}$ for each step as \[
\sqrt{\frac{n}{d}}\cdot \sqrt{d} = \sqrt{n} \]
%\begin{proposition} [\textbf{Local $d$-balance}] For each mirror high-mul walk, each vertex in the path can receive a label in $[d]$ until it crosses the boundary, hence the vertices in the mirror walk can also be encoded in $\sqrt{d}$ per vertex on average; 
%\end{proposition}
%\begin{proof}
%	Since the vertices in $V(\al^T)$ are promised to receive the same labels in $V(\al)$ as their counterparts, it suffices to encode the vertices till $V_\al$, each of which requires a cost of $d$; hence, overall a cost of $\sqrt{d}$ is sufficient for each vertex in the path except $v^T$, which does not require any label given the start $v$.
%\end{proof}

\paragraph{Potential function for individual walker} Let's start with a potential function argument for individual walker.

\begin{proposition}[\textbf{$\sqrt{d}$-balance}] Each $H$ edge requires at most a label in $\sqrt{d}$ for identifying its destination vertex.
\end{proposition}
\begin{proof}
	First, we notice it suffices for us to consider an interval of walk of using $H$ edges, and let $s$ be the starting point of the interval and $t$ the destination. Observe that $t$, as it is reached by $H$ edge at the end of the current interval, can be specified with a label in $2|V_\al|q$, and for any interval of length $0.1\log_d n$, the non-backtracking path from $s$ to $t$ is fixed using $2$-cycle freeness. The length $0.1\log_d n$ is picked so that we can specify the destination vertex for free as $\left(2|V(\al)|q_\al\right)^{1/0.1 \log_d n}<O(1)$ for $|V(\al)|\leq n^\delta$. That said, we can decompose the upcoming interval of $H$ edges as either walking on the main-path (non-backtracking segment from $s$ to $t$), and off-track path attached the main-path (backtracking segment). Each $H$ edge on the main-path does not require any encoding cost, and each $H$ edge on the backtracking segment contributes $d$ when it is heading outward of the main-path and $O(1)$ when heading inwards.
\end{proof}

\paragraph{Assigning potential function for group of people taking the walk}
In the trace-walk, we may have arms splitting out from \emph{branching} vertices, and similarly, arms merging as well. In other words, this corresponds to walker being born and die in the walk. We now show the potential function argument for individual walker applies well for this general setting.

For starters, recall that constraint graph can be linearized and decomposed as the following, 
\begin{mdframed}[frametitle = {Decomposing (linearized) constraint graph into path-segments}]
\begin{enumerate}
	\item We start with at most $U_\al=V_\al$ \emph{directed} vertex-disjoint paths from $U_1$ to $V_q$;
	\item Attach  \emph{directed} path-segments from a \emph{branching} vertex to a vertex on a revealed path-segment, or a vertex in $V_q$.
	\item Attach path-segments between vertices in the same block;
	\item Attach \emph{directed}(dangling) path-segment from an anchor vertex to a dangling vertex in the same block.
\end{enumerate}
\end{mdframed}

Notice it suffices for the encoder to know such assignment of potential function. For each walker, if it remains alive at the end of its subsequent $\kappa$-interval, i.e., it does not intercept other revealed path-segments, then the potential function can be assigned as an individual walker. 

On the other hand, for a walker that intercepts a revealed path-segment, it suffices for us partition the segment into $\kappa$-intervals again, and it suffices for us to restrict our attention to a short-lived walker, that it only takes a walk in an interval of length much less than $\kappa$, i.e., we do not have sufficient edge-decay to identify a label in $2|V(\al)|q_\al$. However, we note that by delayed-encoding, the edge-set of non-backtracking $H$ edges can be identified in $O(1)$ via our wedge-bundling argument, and this fixes the potential function for the short-lived walker before it \emph{dies}, i..e., joins another walker's segment.

%
%\begin{proposition}[\textbf{Global $d$-balance}] For each (non-dangling) vertex that gets encoded along a high-mul edge that is not part of any high-mul mirror walk, a cost of $\sqrt{d}$ is sufficient per vertex. 
%\end{proposition}
%\begin{proof}
%Our encoding scheme relies upon the conditioning of no $2$-cycle in $\kappa$ neighborhood, and whenever our encoding fails, there is some forbidden edge that comes wit extra decay. We now restrict our attention to high-mul walk (a walk that uses high-mul edges), and it suffices for us to say we only need a label in $d$ in average every two move. Split each high-mul walk into intervals of $\kappa/2$ edges from vertices $s$ and $t$. 
% For starters, we will assume all the edges in the following upcoming interval are revealed to the decoder (edges already traversed in the walk by the current high-mul interval), hence the decoder may identify $r$ a midpoint of the shortest path from $s$ to $t$, and a label in $2Vq$ is sufficient. After identifying the midpoint, the encoder may simply run BFS from $r$ to assign each vertex in the $\kappa$ neighborhood of $t$ a depth label (using the shortest path distance to $r$) s.t.
%\begin{center}
% 	each vertex is incident to at most $2$ vertices of lower/equal depth, and at most $d$ vertices of higher depth. 
%\end{center}
%	With such a depth label in hand, a label in $d$ is only needed if the step is going towards a higher-depth neighbor, otherwise a label in $2$ suffices. Furthermore, notice since $r$ is picked as the midpoint of the shortest path from $s$ and $t$, we have \[
%	|\depth(s)-\depth(t)|\leq 1
%	 \]
%	 and hence to encode the walk on the high-mul interval from $s$ to $t$, a cost of $\sqrt{d}$ is sufficient per move. 
%\begin{claim}
%	Let $v$ be a vertex in  2-cycle free subgraph, the BFS from $v$ assigns each vertex a depth s.t. each vertex is incident to at most $2$ vertices of lower/equal depth, and at most $d$ vertices of higher depth. 
%\end{claim}
%\begin{proof}
%Each vertex $u$ incident to more than $2$ vertices of lower/equal depth witnesses a local $3$ cycle, as there are at least $3$ distinct paths (that are allowed to share vertices) from $s$ to $v$. 
%\end{proof}
%To handle high-mul interval starting at $s$ that does not necessarily use all edges revealed to $s$ at the beginning of the interval, we observe that it suffices for us to pay an extra constant for each edge to indicate the direction when a new vertex is encoded.
%\end{proof}
%



%\subsection{Surprise visit takes a time-mark}
%\begin{proposition}[Encoding cost for \ref{enu:surprise-visit} ]
%For a vertex incident to some $H$ edge outside the cut, a cost of $2|V(\al)|q$ is sufficient; for a vertex outside $U_\al\cup V_\al$ incident to an $R$ edge outside the cut, a cost of $2|V(\al)|q$ is also sufficient.
%\end{proposition}
%\begin{proof}
%	Each vertex incident to some $H$ edge must appear in previous blocks; similarly, for a vertex not on the boundary, it must also appear in previous blocks if it is incident to some $R$ edge by local injectivity. 
%\end{proof}
%
%\subsubsection{Auxiliary data for surprise visit}
%	For each surprised visit, it may incur potential unforced return (potentially later in the walk or earlier in the walk via missed-immediate-return), however, it can be shown that each surprise visit is not being charged with too many $\pur$ factors.
%	\begin{proposition} Let $P_\al$ be a trace-walk for shape $\al$,
%We can assign $\pur(P_\al) \coloneqq \sum_{H_{v,q}: \text{H-component at time }q} \pur(H_{v,q})$ factors to surprise visit such that \begin{enumerate}
%	\item each surprise visit is only charged $O(1)$ $\pur$ factors;
%	\item all but $\frac{|U_\al|+|V_\al|}{2} $ many $\pur$ factors are assigned to some surprise visit.
%\end{enumerate} each surprise visit is only charged $O(1)$ $\pur$ factors.
%\end{proposition}
% \subsection{Edge-value assignment}

% We now proceed to unpack the value of a given walk, and let $S$ be the set of singleton edges (that only appears once in $\calP$), and $T$ the rest of the edges. For the following section, let $\chi_e$ be the $p$-biased Fourier character, and let $g_e$ be the corresponding $ \{0,1\}$ indicator variable for whether an edge appears in the random graph sample $G$, and notice up to $(1+\frac{1}{n}) $ factor, \[ 
% 	\chi_e \approx (g_e-\frac{d}{n})\cdot \sqrt{\frac{n}{d}}
% 	\]
% 	For our convenience, we will consider $J\subseteq S$ to be the set of singleton edges that appear in the random graph sample, $\jbar\coloneqq S\setminus J$ those that do not; similarly,  let $W\subseteq T$ be the set of edges that appear in the random graph sample, and define $\wbar$ analogously. 
% 	\begin{proposition}\label{prop: walk-value-factor} 
% 	For some constant $c_0>0$, let $m$ be number of surprise visits in the walk that lead to visited vertices in the walk $\calP$, and 
% 	\begin{align*}
% 		&\left|\E_{G\sim G_{n,d/n}} \left[\val(P)\cdot \cycle \cdot \bdd  \right]\right|\\ &\leq 2^T \sqrt{\frac{n}{d}}^{S+\mul(T)}\max_{W\subseteq T}  (\frac{d}{n})^{|S|+|T|+(\mul(\wbar)-|\wbar|) }\max\left(C(\log n)^2n^{-0.7(\frac{|S|}{\ell}-\cl(S\cup W) ) }, 
%     d^{-c_0\cdot d|S|/\log d + c_0(2q\cdot E-m) }    \right)
% 	\end{align*}	
% 	\end{proposition}
% 	\begin{proof}
% 		This follows by direct expansion,  \begin{align*}
% 	&	\left|\E_{G\sim G_{n,d/n}} \left[\val(P)\cdot \cycle \cdot \bdd  \right]\right|\\&=
% 		\left| \E_G\left[\prod_{e\in S\cup T} \chi_e^{\mul(e)}\cdot \cycle \cdot\bdd \right]  \right|
% \\ &= \left|\E_G\left[\left((\chi_e-\frac{d}{n})\cdot \sqrt{\frac{n}{d}}\right)^{\mul(e)}\cdot \cycle\cdot \bdd  \right]  \right| \\
% &=\left(\sqrt{\frac{n}{d}}\right)^{|S|+\mul(T)}  \left|\E\left[\sum_{W\subseteq T, J\subseteq S} (1-\frac{d}{n})^{\mul(W)+\wbar}(\frac{d}{n})^{W+\mul(\wbar)}(-1)^{\mul(\wbar)+\jbar } (1-\frac{d}{n})^{J+\jbar}(\frac{d}{n})^{J+\jbar}\cdot \cycle \cdot \bdd |G_{W\cup J}=1, G_{\wbar\cup\jbar}=0 \right]  \right|\\
%  &\leq \sqrt{\frac{n}{d}}^{S+\mul(T)} \sum_{W\subseteq T} (\frac{d}{n})^{W+\mul(\wbar)} \left|\E\left[ \sum_{J\subseteq S}(1-\frac{d}{n})^{J+\jbar}(\frac{d}{n})^{J+\jbar}(-1)^{\jbar}\cdot\cycle\cdot \bdd |G_{W\cup J}=1, G_{\wbar\cup\jbar}=0  \right] \right|  \\
%     &\leq   2^{T}\sqrt{\frac{n}{d}}^{S+\mul(T)}\max_{W\subseteq T}(\frac{d}{n})^{W+\mul(\wbar)} \left|\E\left[ \sum_{J\subseteq S}(1-\frac{d}{n})^{|S|}(\frac{d}{n})^{|S|} (-1)^{\jbar}\cdot \cycle|G_{W\cup J}=1, G_{\wbar\cup\jbar}=0  \right] \right| \\
%     &= 2^{T}\sqrt{\frac{n}{d}}^{S+\mul(T)}\max_{W\subseteq T}  (\frac{d}{n})^{W+\mul(\wbar)}(\frac{d}{n})^{|S|} \left| \sum_{J\subseteq S}(-1)^{\jbar}\Pr_G[\calE(G)\land \calF(G) |G_{W\cup J}=1, G_{\wbar\cup\jbar}=0] \right|\\
%     &\leq 2^T \sqrt{\frac{n}{d}}^{S+\mul(T)}\max_{W\subseteq T}  (\frac{d}{n})^{|S|+|T|+(\mul(\wbar)-|\wbar|) }\max\left(Cn^\delta n^{-0.7(\frac{|S|}{\ell}-\cl(S\cup W) ) }, 
%     d^{-c_0\cdot d|S|/\log d + c_0(2q\cdot E-m)/d }    \right)
% 			\end{align*}
% 				where we use singleton-decay from the appendix.
% 	\end{proof}
% 	Observing the guarantee from the proposition, we notice each edge has the following contribution, \begin{enumerate}
% 	\item if it appears exactly twice in the walk, it contributes a value $1$ as it contributes $2$ factors to $\mul(T)$ and $1$ factor to $|T|$, altogether giving us $(\sqrt{\frac{n}{d}})^2\cdot \frac{d}{n}=1$  ;
% 	\item if it appears only once in the walk, it contributes a factor of $1$ to $S$, picking up a value of $\sqrt{\frac{n}{d}}\cdot \frac{d}{n}\cdot\singdecay$;
% 	\item it it appears $t>2$ times in the walk, it contributes a factor of $\sqrt{\frac{n}{d}}^{t}\cdot \frac{d}{n}\leq  \left( \sqrt{\frac{n}{d}} \right)^{t-2} $; 
% \end{enumerate} 
%	This prompts us to partition the set of $F$ legs, \begin{enumerate}
%		\item Let $F_{\exc}$ be the set of $F$ legs that correspond to edges leading to visited vertices;
%		\item Let $F_{\single}$ be the set of $F$ legs that correspond to singleton edges (if not leading to visited vertices);
%		\item With some abuse of notation, we let $F$ be the remaining of $F$ legs.
%	\end{enumerate}
%	It suffices for us to upper bound \begin{align*}
%		\sqrt{\frac{n}{d}}^{|S|+2\cdot |T|}\cdot (\frac{d}{n})^{|S|+|T|}\cdot \singdecay^{|S|}&\leq \left(\sqrt{\frac{n}{d}}\cdot \frac{d}{n} \cdot \singdecay \right)^{|S_{\text{non-surprise}|}}			\end{align*}
%	We can now consider the following edge-value assignment scheme, \begin{enumerate}
%		\item For an $T$ edge (whose first leg does not lead to visited vertices), its first two multiplicities contribute a factor $1$ altogether to the final trace, and we can assign a value of $\frac{1}{\sqrt{n}}$ for the $F$ leg, and a value of $\sqrt{n}$ of the corresponding $R$ leg;
%		\item For an $T$ edge (whose first leg leads to visited vertices), we assign a factor $1$ to its corresponding $F_\exc$ and $R_\exc$ leg;
%		\item For an $S$ leg that does not lead to visited vertices, we assign the full factor of $\sqrt{\frac{n}{d}}\cdot \frac{d}{n}\cdot \singdecay$ to the $F_\single$ leg;
%		\item For an $S$ leg that leads to visited vertices, we upper bound (loosely) its contribution by $1$;
%	\end{enumerate}
%	This culminates in the following assignment scheme for edge-value depending on edge-labels,
%	\paragraph{Edge-value assignment scheme}
%	\begin{mdframed}
%	\begin{enumerate}
%		\item $F$: each corresponds to some edge appearing for the first time,
%		\begin{itemize}
%			\item $F_\single$: the corresponding edge does not lead to visited vertices, while it is going to appear only once in the walk, and it gets assigned a factor $\sqrt{\frac{d}{n}}\cdot \frac{d}{n}\cdot \singdecay $;
%			\item $F$: the corresponding edge leads to a new vertex, and it appears at least twice throughout the entire walk. This gets assigned a factor of $1$;
%		\end{itemize} 
%		\item $H$: each corresponds to middle appearance of some high-mul edge, and each contributes a factor of $\sqrt{\frac{n}{d}}$.
%		\item $R$: each corresponds to some edge appearing for the last time, and we assign a factor of  $1$.
%	\end{enumerate}
%	\end{mdframed}
% 	\begin{enumerate}
% 		\item $F$: each corresponds to some edge appearing for the first time,
% 		\begin{itemize}
% 			\item $F_\exc$: the corresponding edge leading to some visited vertices, and we assign it a factor $1$;
% 			\item $F_\single$: the corresponding edge does not lead to visited vertices, while it is going to appear only once in the walk, and it gets assigned a factor $\sqrt{\frac{d}{n}}\cdot \frac{d}{n}\cdot \singdecay $;
% 			\item $F$: the corresponding edge leads to a new vertex, and it appears at least twice throughout the entire walk. This gets assigned a factor of $\frac{1}{\sqrt{n}}$.
% 		\end{itemize} 
% 		\item $R$: each corresponds to some edge appearing for the second time,
% 		\begin{itemize}
% 			\item If the corresponding $F$ edge is in $F_\exc$, we assign a factor $1$;
% 			\item Otherwise, we assign a factor of $\sqrt{n}$;
% 		\end{itemize}
% 		\item $H$: each corresponds to some edge appearing the third time or onwards, and contributes a factor of $\sqrt{\frac{n}{d}}$.
% 	\end{enumerate}



%	At the heart of charging argument is the above proposition, ignoring the $\max$ term that captures our singleton-decay and the $2^T$ term handled by edge-decay, for a fix $W\subseteq T$, we notice the factors in $\sqrt{\frac{d}{n}}$ can be rearranged as \begin{align*}
%		\left(\sqrt{\frac{n}{d}}\right)^{S+\mul(W)+\mul(\wbar)}\left(\frac{d}{n}\right)^{|S|+|T|+(\mul(\wbar)-|\wbar|) }&= \left(\sqrt{\frac{d}{n}}\right)^{|S|+|T|}  \left(\sqrt{\frac{n}{d}} \right)^{\mul(W)-|W|}\cdot \left(\sqrt{\frac{d}{n}}\right)^{\mul(\wbar)-|\wbar| }  	\end{align*}
%\begin{remark}
%We advise the readers to think of $W=T$ as any edge in $\wbar$ would be an edge forbidden in the random graph sample, giving a $\sqrt{\frac{d}{n}}$ decay each time it appears in the trace. 
%\end{remark}
%From our rearranging above, we can now motivate our charging strategy,\begin{enumerate}
%	\item Each time an edge appears for the first time, it comes with a $\sqrt{\frac{n}{d}}$ from the normalization into $p$-biased Fourier basis, but we also pay a $\frac{d}{n}$ for the probability the edge appears in the random graph sample, and combining these two factors gives us $\sqrt{\frac{d}{n}}$, which is captured by the first term on RHS;
%	\item Each subsequent use of an edge either contributes $\sqrt{\frac{n}{d}}$ or a $\sqrt{\frac{d}{n}}$ to the trace depending on whether the edge appears in the random graph sample, and this is captured by the last two terms.
%\end{enumerate}
%We now shift gear to the $\max$ term, and restrict attention to the term $n^{-0.7\frac{|S|} {\ell}}$, and $d^{-c_0d|S|/\log d}$ term, as the rest can be handled by decay from the extra excesses in the combinatorial factor and edge-decay over long walks.
%\begin{observation}
%	Splitting the singleton decay factor evenly over singleton edges, each singleton-edge comes with a decay of  \[
%	\singdecay \leq d^{-c_0d/\log d}
%	 \]
%\end{observation}
%
%
%	An edge contributes to the trace a certain value as a random variable and the contribution depends on its multiplicity: in the simple setting where each edge is an independent random variable, its contribution the trace is is simply
%\[ 
%\E[\chi_{e}] = 0, \E[\chi_{e}^2]=1, \E[\chi_{e}^t] \leq \left(\sqrt{\frac{n}{d}}\right)^{t-2}
%\]	
%However, the contribution is slightly complicated when we work with the bounded degree model in which we break the independence of edges due to conditioning, however, we can observe that each edge in \cref{prop:walk-value-factor}, \begin{enumerate}
%	\item if it appears exactly twice in the walk, it contributes a value $1$ as it contributes $2$ factors to $\mul(T)$ and $1$ factor to $|T|$, altogether giving us $(\sqrt{\frac{n}{d}})^2\cdot \frac{d}{n}=1$  ;
%	\item if it appears only once in the walk, it contributes a factor of $1$ to $S$, picking up a value of $\sqrt{\frac{n}{d}}\cdot \frac{d}{n}\cdot\singdecay$;
%	\item it it appears $t>2$ times in the walk, it contributes a factor of $\sqrt{\frac{n}{d}}^{t}\cdot \frac{d}{n}\leq  \left( \sqrt{\frac{n}{d}} \right)^{t-2} $; 
%\end{enumerate} 
%
%We are now ready to introduce our edge-distribution scheme. We will first furtherer clarify edges corresponding to $F$ labels,
%
% into whether they appear only once in the walk or not, and we let $F_S$ be the set of legs that correspond to singleton edges. With some abuse of notation, we continue to use the label $F$ to represent legs that correspond to edges that appear at least twice in the walk.

==> factorizing-SMVS.tex <==
\subsection{Factorizing short wedges around $U_\tau\cap V_\tau$ }
A challenge that comes up in counting middle shape is encoding shapes with multiple legs on $U_\tau\cap V_\tau$ as naive encoding would require a factor of $k$ specifying each color-bucket of the destination of each such leg (as vertices across different color-buckets are distinguishable from each other, hence a label in $[k]$ is needed modulo the automorphism machinery thereafter). In this subsection, we show shapes with multiple legs on $U_\tau\cap V_\tau$ can be grouped together and thereby we can avoid the cost of $k$ from counting. For starters, notice we restrict our attention to shapes with each vertex that can be reached from $U_\tau\cap V_\tau$ without passing through $U_\tau\Delta V_\tau$ to have degree at least $2$ via the k-wise symmetry of our Fourier coefficients. In other words, each shape that we factorize has a wedge around $U_\tau\cap V_\tau$ while we do not factorize wedges with only one leg on $U_\tau\cap V_\tau$ (with potentially another leg on $U_\tau\Delta V_\tau$).

	We start with a formal definition of what we wish to factorize out.
	\begin{definition}[Short wedges]
		For a shape $\al$, we call a subgraph $\beta$ a short wedge around $U_\al\cap V_\al$ if each vertex in $V(\beta)$ has two distinct simple paths to $U_\al\cap V_\al$, with each simple path of length at most $k$. 
	\end{definition} 
	Notice that any short wedge around $U_\al\cap V_\al$ yields a better SMVS than $U_\tau$ for $\tau$ a middle shape. Moreover, appealing to the language of our trace norm bounds, we have the following observation,
	\begin{observation}
		Any vertex in $V(\beta)\setminus (U_\al\cap V_\al) $ is ($k$-)doubly constrained by its boundary $U_\al\cap V_\al$.  
	\end{observation}

	\begin{proposition}
	For a fixed graph $G$, and a fixed set of vertices $S\subseteq [n]$, let $c(S):S\rightarrow [k]$ be its corresponding color assignment, let $\mathsf{ext}(S)$ be the set of vertices $k$-doubly-constrained by $U_\tau\cap V_\tau$, there exists a distribution $D_S$ s.t. 
			\[\sum_{E\seq \binom{\mathsf{ext}(S)}{2}} \cval{E}_{c(S)} \cdot \chi_E = \E_{D_S}[x_{S,c(S)}]
			\] 
	\end{proposition}
	\begin{proof}
		
	\end{proof}
	A corollary of such is we have a straightforward magnitude bound for the subshapes supported over the short wedges, and moreover, we know it is non-negative by observing $x_{S,c(S}$ is a $0/1$ indicator variables.
	

==> floating-comp.tex <==

\section{Improved bounds for floating components}
 
 \subsection{Set-up}
  \begin{definition}[Short-cycle parity promise]
 	Given a random graph sample $G$, we call it satisfies cycle parity promise for length-$t$ cycle if \[ 
 	\float_{C_t}\in  \left[\E[\float{C_t}]\pm c_t\sqrt{\Var( \float_{C_t})) } \right]
 	\]
 	We say $G$ satisfies short cycle parity promise if the above holds for any $t\in [3, 0.01\log_d n]$.
 \end{definition}
 \begin{proposition}
 	W.h.p., a random graph sample satisfies short-cycle parity promise.
 \end{proposition}
\begin{corollary}
	Under the promise of short-cycle parity for a random graph $G$, for $C_t$ a floating cycle of length $t$,
	\[ |\float_{C_t}| \leq \sqrt{n}^{t  } \]
\end{corollary}

Our bounds for floating component can be improved by noticing that for any shape $\al$ with non-empty floating cycles, we can decompose the shape into \[ 
\al = \al_{\mathsf{connect}}\cup \al_\float
\]
where $\al_{\mathsf{connect}}$ is the subshape of $\al$ connected to $U_\al\cup V_\al$, and  $\al_\float$ is a shape s.t. $U_\al=V_\al=\emptyset$ with the floating components from $\al$.
\begin{definition}[Floating subshape $\al_\float$]
	Given $\al$ a shape, we define $\al_{\float}$ its corresponding floating shape s.t.\begin{enumerate}
		\item $U_{\al_\float} =V_{\al_\float} =\emptyset$;
		\item $V(\al_\float)$ is the set of floating vertices in $\al$, and $E(\al)$ is the induced subgraph of $\al$ restricted to $V(\al_\float)$.
	\end{enumerate}  
	With some loss of generality, $M_{\al_\float}$ is simply a scalar polynomial of the random graph sample $G$ such that \begin{align*}
		M_{\al_\float}(G)  = \frac{1}{|\aut(\al_{\float})|}\sum_{\substack{\sigma:V(\al_\float)\rightarrow [n] \\\text{injective} }} \prod_{(i,j)\in E(\al_\float)} \chi_{\sigma(i),\sigma(j)} 
	\end{align*}
\end{definition}

 The starting point for our bounds is the following observation, \[
M_{\al} \approx_{\mathsf{int}} M_{\al_{\mathsf{connect}}} \cdot M_{\al_\float}
 \]
  where the approximate inequality ignores intersection terms. Formally, for any $U, V\subseteq [n]$, we have 
 \begin{align*}
 	\int(\al)[U,V] &\coloneqq M_{\al}[U,V] - M_{\al_{\mathsf{connect}}} \cdot M_{\al_\float}[U,V]\\
 	&= \sum_{\substack{\sigma: V(\al)\rightarrow [n]\\\text{injective} \\\sigma(U_\al)=U, \sigma(V)=V_\alpha }}\frac{1}{|\aut(\al)|}\chi_\al - \sum_{\substack{\sigma_{\mathsf{connect}}:V(\al_{\connect})\rightarrow[n]  \\ \text{injective}\\\sigma_\connect(U_{\al_\connect})=U_\al, \sigma_\connect(V_{\al_\connect})=V_\alpha } }\sum_{\substack{\sigma_\float: V(\al_\float)\rightarrow[n]\\ \text{injective} }}\frac{\chi_{\al_\connect}\cdot \chi_{\al_\float}}{|\aut(\al_\connect)|\cdot |\aut(\al_\float)|}
 	\\&=\sum_{\substack{\sigma: V(\al)\rightarrow [n]\\\text{injective} }} \frac{\chi_\alpha}{| \aut(\al)|} -\sum_{\substack{\sigma_\connect: V(\al_\connect)\rightarrow [n]\\ \\ 
 	\substack{\sigma_\float: V(\al_\float)\rightarrow [n]\\ } \\
 	 \sigma_\float\cup \sigma_\connect: \text{injective}\\\sigma(U_{\al_\connect} )=U, \sigma(V_{\al_\connect})=V }} \frac{\chi_{\al_\connect}\cdot \chi_{\al_\float}}{|\aut(\al_\connect)|\cdot |\aut(\al_\float) |} \\
 	 &-\sum_{\substack{\sigma_\connect:V(\al_{\connect})\rightarrow [n],\text{inj.}\\\sigma_{\connect}(U_{\al_\connect})=U, \sigma_{\connect}(V_{\al_\connect})=V
 	 \\ \sigma_{\al_\float}:V(\al_{\connect})\rightarrow [n],\text{inj.}\\ \mathsf{Im}(\sigma_{\connect})\cap \mathsf{Im}(\sigma_{\float})\neq \emptyset } }
 	 \frac{\chi_{\al_\connect}\cdot \chi_{\al_\float}}{|\aut(\al_\connect)|\cdot |\aut(\al_\float)|}\\
 	 &=-\sum_{\substack{\sigma_\connect:V(\al_{\connect})\rightarrow [n],\text{inj.}\\\sigma_{\connect}(U_{\al_\connect})=U, \sigma_{\connect}(V_{\al_\connect})=V
 	 \\ \sigma_{\al_\float}:V(\al_{\connect})\rightarrow [n],\text{inj.}\\ \mathsf{Im}(\sigma_{\connect})\cap \mathsf{Im}(\sigma_{\float})\neq \emptyset } }
 	 \frac{\chi_{\al_\connect}\cdot \chi_{\al_\float}}{|\aut(\al_\connect)|\cdot |\aut(\al_\float)|}  \hspace*{12pt}  (\text{via }\aut(\al) = \aut(\al_\float) \cdot \aut(\al_\connect))
 	   \end{align*}
 \begin{observation}\label{obs: aut-multiplies} For any shape $\al$,\[ 
 \aut(\al) = \aut(\al_\float) \cdot \aut(\al_\connect)
 \]
 \end{observation}
 We now notice $\int(\al)$ can be decomposed into a sequence of (possibly improper) shapes,
 \begin{definition}[Floating intersection shape]
 	Given a shape $\al$, we call $\al_P$ its floating intersection shape if 
 	\begin{enumerate}
 	\item $U_{\al_P} = U_\al$, $V_{\al_P}=V_\al$;
 	\item $\al_P$ can be obtained by merging vertices from $V(\al_\connect)$ and $V(\float)$;
 	\end{enumerate}
 \end{definition}
 Concretely, we have \begin{align*}
 	\int(\al) = \sum_{\al_P} \frac{|\aut(\al_P)|}{|\aut(\al_{\float})|\cdot |\aut(\al_\connect) |} M_{\al_P}
 \end{align*}
 At this point, it suffices for us to bound $\|\int_\al| \leq o(\|M_{\al_\connect}\| \cdot \|M_{\al_\float} \|)$ using our previous norm bounds, which would then allow us to conclude $\|M_\al\| \leq (1+o(1)) \|M_{\al_\connect}\| \cdot \|M_{\al_\float} \| $  by a triangle inequality. However, some intersection term from $\int(\al)$ warrants extra care as it may still contain some floating component (since not every floating component has to intersect with $\al_\connect$ in $\al_P$). 
 
 To handle this issue, we note that we can recursively factorize the remaining floating component such that we only need to apply norm bounds on shapes with no floating component. Formally, we notice any intersection shape would have at least one fewer connected component, and we can then the shapes according to the number of floating components, and then apply the scalar trick on each shape so that we always get to apply tight norm bounds (norm bounds without $\sqrt{2|V(\al)|q_\al}$ factor)) for any intersection shape in a black-box manner.
 \subsection{Intersection term analysis}
 \begin{lemma}
 	For any shape $\al$ (possibly improer) that can be decomposed into disjoint connected components $\al=\al_\connect \cup \al_\float$, where $\al_\connect$ is the subshape of $\al$ connected to $U_\al\cup V_\al$ (including mul-2 edges) and $\al_\float$ is the subshape of the remaining , we have \[ 
 	\|M_\al \| \leq \left(1+o(1)\right) \|M_{\al_\connect} \|\cdot \|M_{\al_\float} \|
 	\] 
 \end{lemma}
 \begin{remark}
 	Despite a double edge may vanish for the purpose of norm bound, they only arise in the intersection and hence we will  analyze that alongside the intersected shape $\al_{P_\connect}$ in the subsequent analysis.
 \end{remark}
 \begin{proof}
 	We prove this by inducting upon the number of floating components of $\al$, and notice this is immediate when $\al$ does not have any floating component. For the induction hypothesis, consider we are factorizing $\al = \al_\connect \cup \al_\float$, and consider $\al_P$ a shape that arises in the intersection term $\int(\al)$. 

	To begin with, we first factorize out the floating component from $\al_P$, and write $\al_P=\al_{P_\connect}\cup \al_{\float}$. We then notice $\al_P$ must have at least one fewer floating component than $\al$, and hence we can apply our induction hypothesis to bound \begin{align*}
		\|M_{\al_P}\| \leq \left(1+o(1)\right)\cdot \|M_{\al_{P_\connect}} \|\cdot \|M_{\al_{P_{\float}}} \|
	\end{align*} 	
	For a given $\al$ and $\al_P$, let $F_{\al_P}$ be the set of floating components that are incident to any intersected vertex in $\al_P$,  
 \end{proof}
 \begin{lemma}
 	Let $\al$ be a connected shape, and $F$ be a floating cycle, and let $\al_P$ be an intersection term arising from the intersection of $\al$ and $F$, then
 \[ 
 \|M_{\al_P}\|\leq \|M_{\al}\| \cdot \|M_F \|
 \]
  \end{lemma}
 \begin{proof}
 	For starters, by applying matrix norm bounds on $M_\al$ and scalar bound for $M_F$ gives us \[
 	RHS = \max_{S:\text{separator for }\al } \sqrt{n}^{V(\al)\setminus V(S)}\cdot \left(\sqrt{\frac{n}{d}}\right)^{E(S)}\cdot \sqrt{n}^{|V(F)|} 
 	 \]
 	 Our proof proceeds by starting with the shape $\al\cup F$ and  merging each pair of intersection between $\al$ and $F$. Notice before any intersection happens, applying matrix norm bounds on $\al\cup F$ without going through scalar bound gives us a bound of \[ 
 	 \max_{S:\text{separator for }\al } \sqrt{n}^{V(\al)\setminus V(S)}\cdot \left(\sqrt{\frac{n}{d}}\right)^{E(S)}\cdot \sqrt{n}^{|V(F)|} \cdot \sqrt{2|V(\al\cup F)|q_{\al\cup F}}
 	 \]
 	 We advise the reader to ignore the $2V(\al)q$ factor as it arises from $F$ being floating in $\al\cup F$ which is no longer true once intersection happens (despite the fact that the intersection may produce new floating components). Before we dig into the analysis, we notice unless each edge of $F$ becomes a double edge in $\al_P$, we can order the intersected vertices from $F$ such that each intersection only produces at most one pair of double edges. And this prompts us to discuss by cases.
 	 \paragraph{Every edge in $F$ becomes a double edge in $\al_P$}
 	 Since each edge in $F$ becomes a double edge, $F$ must be a vertex-induced subgraph in $\al_P$, and for starters, we notice the bound is immediate if no double-edge vanishes, as we would have \[ 
 	 \|M_{\al_P}\| = \|M_\al|\ll \|M_{\al}\|\cdot \|M_F\|
 	 \] 	 
 	 To see the case for potential double-edge vanishing, consider $V_F\subseteq V(\al)$ the set of to-be-intersected vertices in $V(\al)$, and notice they are connected to the SMVS of $\al$ since $\al$ is a connected shape. Let $\psi(\al_P)$ be a linearization of $\al_P$, and $S$ the SMVS for $\al$, by connectivity, we can pick an arbitrary vertex $v_L\in V_F$ that is reachable from $S_L\cap S$ without passing through the intersected and similarly a vertex $v_R\in V_F$ that is reachable from $S_R\cap S$. 
 	 Let $C_P$ be the intersected cycle in $\al$. 
 	 \begin{claim}
 	 	For any linearization $\psi$ of $\al_P$, \[ 
 	 	\max_{\tilde{S}:\text{separator for} \psi(\al_P)}\sqrt{n}^{|V(\al_P)\setminus V(\tilde{S})|} \left(\sqrt{\frac{n}{d}}\right)^{|E(\tilde{S})|}\sqrt{n}^{|I_{\psi(\al_P)}|}\sqrt{2|V(\al_p)|q_{\al_P}}^{|\float\cup \dang|} 	 	\]
 	 \end{claim}
 	 
 	 \begin{enumerate}
 	 	\item $v_L=v_R$: in this case, since $F$ is a short cycle, $F$ is completely contained in $E(S)$, and the vertices and edges in the floating cycle contributes a total factor of $(\sqrt{\frac{n}{d}})^{|E(F)|}$ to $\|M_\al\|$. Notice each iso-connected component is incident to disjoint edges in $E(\al)$, as otherwise we can merge the two iso-connected components into one. Moreover, for each iso-connected component of $c$ isolated vertices, we first notice it is incident to at least $c+2$ edges in $E(S)$. Now consider a traversal of intersected vertices from $v$. 
 	 	
 	 	For each vertex that can be explored by some non-vanishing double edge in $\psi(\al_P)$, notice we can group them into a segment between iso-connected components and $v$. For each connected segment, consider a traversal within the segment, notice for each vertex but the first vertex, the traversal edge contributes $\sqrt{\frac{n}{d}}$ to $\|M_\al\|$ and the vertex contributes a $\sqrt{n}$ through $V(F)$ to the RHS while it contributes a factor of $\sqrt{n}$ to the LHS;
 	 	\item 
 	 	\end{enumerate}
 	 	\end{proof}
 

==> intersection.tex <==
\subsection{Bounding intersection terms}
\label{subsec:intersection-term}
\paragraph{Preliminaries for intersection term}
\begin{definition}[Ribbon composition]
	Given ribbons $R_1, R_2$, we call them \emph{composable} if $V_{R_1}=U_{R_2}$. For ribbons with boundary set indexed by subgraphs, we additionally constrain $E(V_{R_1}) = E(U_{R_2})$. We use $R_1\circ R_2$ to represent the ribbon from the composition of $R_1$ and $R_2$.
\end{definition}
\begin{definition}[Proper composition]
	Given $R_1,R_2$ composable ribbons, we call them a proper composition if there is no surprise intersection beyond the boundary, i.e., $(V(R_1)\setminus V_{R_1})\cap (V(R_2) \setminus U_{R_2})=\emptyset$. 
\end{definition}
\begin{remark}
	For properly composable ribbons $R_1,R_2$, we have $M_{R_1}M_{R_2} = M_{R_1\circ R_2}$.
\end{remark}
\begin{definition}[Improper shape and phantom graph]
	We call a shape improper if it contains multi-vertices (repeated vertices) or multi-edges. The underlying multigraph of an improper shape is also called a \emph{phantom graph}, and we usually use $\tau_P$ to refer to both the improper shape and its underlying multigraph.
\end{definition}
\begin{definition}[Shape composition]
	Given shapes $\al, \beta$, we call them \emph{composable} if $V_\al = U_\beta$. For composable shapes, we write $\zeta = \al\circ \beta$ for $\zeta$ any (possibly improper) shape whose multigraph can be obtained by composing ribbons of shape $\al$ and $\beta$. 
\end{definition}
Unfortunately, it is no longer true that $M_\al M_\beta = M_{\al\circ \beta}$ as ribbon injectivity dose not hold beyond the anticipated boundary, and collision outside the boundary would inevitably produce improper shapes that are the main subject of this section.


\paragraph{Factorizing intersection terms}
We now make concrete our charging strategy for the intersection terms. Recall from our big picture of $LQL^T$ decomposition, intersection can happen whenever shapes from $L, Q, L^T$ intersect with one and another. For a left, middle, right shape $\sigma, \tau, \sigma'$ that intersect to some improper shape $\tau_P$, we follow the recursive factorization framework from planted clique where we factorize the left/right shape from intersection term $\lambda_{\tau_P}M_{\tau_P}$ and attempt to charge to the corresponding diagonal of the new left/right shape.  
%	 With this big picture in mind, we also want to note that in previous works, $\gamma, \gamma'$ are just defined to be any left/right shape; however, this needs to be modified for SMVS case since left shape has one side indexed by vertices, and another indexed by subgraph, while $\gamma$ needs to have both sides indexed by subgraph.

%where $U_\gamma$ is the MVS separating $U_\sigma$ from $V_\sigma\cup \int(\tau_P)$, and $V_{\gamma'}$ is the MVS separating $V_{\sigma'}$ from $U_{\sigma'}\cup \int(\tau_P)$ where $\int(\tau_P)$ is the set of intersected vertices. 
With this big picture in mind, we are ready for more technical definitions.
\begin{definition}[Intersected vertices $\int(\tau_P)$]
	Given a composable pair of $\sigma, \tau,\sigma'$ that intersect to some improper shape $\tau_P$, let $\int(\tau_P)$ be the set of vertices that gets intersected in $\tau_P$, i.e., the vertices that appear with multiplicity greater than $1$ in the associated multigraph of $\tau_P$.
\end{definition}
%we will upgrade $U_\gamma$ from the (dense) MVS to $(U_\gamma, E(U_\gamma)$ being the corresponding SMVS (and ultimately PMVS when combined with the coloring); furthermore, we notice that the dependence of $\gamma$ on $\tau_P$ can be broken once we specify the set of vertices in $U_\gamma$ that get intersected in $\tau_P$, and this motivates our following definition for left/right intersection color-shape. 
		 \begin{definition}[Left-intersection (color-)shape $\gamma$]
	 A (color) shape $\gam$ is a left-intersection color-shape if \begin{enumerate}
	 	\item $\gam$ comes with an an additional label for each vertex in $V(\gam)$ specifying whether this vertex is in \emph{to be intersected}, i.e., whether the vertex is in $\int(\gamma)$
%	 	\item $(U_\gam, \cp_{U_\gam))$ is a positive glyph;
	 	\item $V_\gam.$ is the unique MVS for separating $V_\gam$ and $U_\gam$;
	 	\item $U_\gam $ is a MVS that separates $V_\gam\cup \int(\gam)$ and $U_\gam$;
	 	\item We follow the convention where we put edges in $E(V_\gam)$ to the middle shape $E(U_\tau)$, hence, $E(V_\gamma) = \emptyset$.
	 		 \end{enumerate}
	 		 Consequently, we define the corresponding shape coefficient for $\gam$ to be \[ 
	 		 \lambda_\gamma \coloneqq  \left(\frac{1}{k} \right)^{|V(\gam)|-\frac{|U_\gam|+|V_\gam|}{2} }	 \cdot \edgeco^{|E(\gam)| } \]
	 \end{definition}
	 \begin{remark}
	 	For our application, we will further factorize out the edges in $E(U_\gam)$ as they form the coloring-indicator, hence we actually have $E(U_\gamma)\cup E(V_\gam) = \emptyset$ (and similarly for $\gp$) in our analysis. 
	 \end{remark}
	 Analogously, we define the right-intersection color shape as the following. \begin{definition}[Right-intersection color-shape $\gamma'$]
	 A color-shape	$(\gamma',\cp_{\gam'})$ is a left-intersection color-shape if \begin{enumerate}
	 	\item $\gam'$ comes with an an additional label for each vertex in $V(\gam')$ specifying whether this vertex is in \emph{to be intersected}, i.e., whether the vertex is in $\int(\gamma')$
%	 	\item $V_\gam.$ is the unique MVS for separating $V_\gam$ and $U_\gam$;
	 	\item $V_\gp $ is a MVS that separates $V_\gp\cup \int(\gp)$ and $U_\gp$;
	 	\item We follow the convention where we put edges in $E(U_\gp)$ to the middle shape $E(V_\tau)$, hence, $E(U_\gp) = \emptyset$.	 		 \end{enumerate}
	 		 Consequently, we define the corresponding shape coefficient for $\gp$ to be \[ 
	 		 \lambda_{\gp} =  \left( \frac{1}{k} \right)^{|V(\gp)|-\frac{|U_\gp|+|V_\gp|}{2} }\cdot \edgeco^{|E(\gp)|}
	 		 \]
	 \end{definition}
%	 	Again, for convenience, we will decouple the color-partition and shape from the intersection color shape.
%	 \begin{definition}[Left/right intersection shape and coloring matrix]
%	 	We call a canonical shape $\gamma$ (or $\gam'$) a left/right intersection shape if there exists some $\cp_{\gamma}$ (or $\cp_\gp $) such that  $(\gam,\cp_{U_\gam})$ (or $(\gam', \cp_\gp)  $) is a left/right intersection color shape.
%	 	
%	 	For each left/right intersection shape $\gam$ ($\gam'$), we define its associated left/right coloring matrix as \begin{align*}
%	 		H_\gamma &= \sum_{W(\gam):\text{ canonical}}\sum_{\cp\in W} H_{\gamma,\cp}\\
%	 		H_\gp &= \sum_{W(\gam'):\text{ canonical}} \sum_{\cp\in W} H_{\gp,\cp}
%	 	\end{align*}
%	 	For a fixed color-partition on $U_\gam$ (or $V_\gp)$, we can further partition $H_\gam$ using \begin{align*}
%	 		H_{\gam, \cp_{U_\gam}}  &= \sum_{W(\gam):\text{ canonical}}\sum_{\substack{\cp\in W\\ \cp_{U_\gam}\mapsto \cp }} H_{\gamma,\cp}\\
%	 		H_{\gp,\cp_{V_\gp}} &= \sum_{W(\gam'):\text{ canonical}} \sum_{\substack{\cp\in W\\ \cp_{V_\gp}\mapsto \cp }}H_{\gp,\cp}
%	 	\end{align*}
%	 \end{definition}
%	 
%	 	 	Accompanying the  left/right intersection shape is the corresponding $\Id_{U_\gam}$ shape that would be the PSD mass in our intersection term charging,\begin{definition}[$\Id_{U_\gamma}$-shape]
%		Given a left intersection shape $\gamma$, we define its corresponding identity shape  $\Id_{U_\gam}$ as \begin{enumerate}
%			\item $U_{\Id_{U_\gam}} = V_{\Id_{U_\gam}} = V(\Id_{U_\gam}) \coloneqq U_\gamma$;
%			\item $E(\Id_{U_\gam}) \coloneqq E(U_\gam)$
%		\end{enumerate}
%		Consequently, $\Id_{U_\gamma}$ is a middle shape with coefficient \[
%		 \lambda_{\Id_{U_\gam}} = \edgeco^{|E(U_\gam)|} \]
%	\end{definition}
%	\begin{remark}
%		The definition extends to $\Id_{V_{\gamma'}}$ for a  right-intersection $\gamma'$-shape.
%	\end{remark}
	\begin{definition}[Intersectable tuple $(\gam,\tau,\gam')$]
		We call a composable tuple $(\gam,\tau,\gam')$ intersectable if there exists some intersection pattern $\tau_P$ s.t. any to-be-intersected vertex in $\gamma$ and $\gamma'$ gets intersected in $\tau_P$, i.e.,
	\[ 
	\int(\gamma) \cup \int(\gamma')= \int(\tau_P)
	\] 
	For an intersectable tuple, we define its coefficient \[ 
		\lambda_{\gam\circ\tau\circ\gp} \coloneqq \lambda_\gam\cdot \lambda_\tau\cdot\lambda_\gp =\left(\frac{1}{k}  \right)^{|V(\gam\circ\tau\circ\gp)|-\frac{|U_\gam|+|V_\gp|}{2} }\cdot   \edgeco^{|E(\gam\circ\tau\circ\gp)}
		\]
	\end{definition}
%	\begin{definition}[Coloring matrix for intersection tuple]
%		For an intersection tuple $(\gam,\tau,\gam')$, we define the coloring matrix for the intersection-tuple to be \[ 
%		H_{\gam\circ\tau\circ\gam'} = H_{\gam}\cdot H_{\tau}\cdot H_{\gam'}
%		\]
%		Furthermore, we partition $H_{\gam\circ\tau\circ\gam'}$ according to the color-partition on the boundary,  \[
%		H_{\gam\circ\tau\circ\gam'} = \sum_{\substack{\cp_{U_\gam}\in W(\gam) \\\cp_{V_\gp}\in W(\gam')}} H_{\gam\circ\tau\circ\gp, (\cp_{U_\gam},\cp_{V_\gp})}
%			 \]
%		where we define \[ 
%		H_{\gam\circ\tau\circ\gp, (\cp_{U_\gam},\cp_{V_\gp})} \coloneqq H_{\gam,\cp_{U_\gam}}\cdot H_\tau \cdot H_{\gp, \cp_{V_\gp}}
%		\]
%	\end{definition}
%\begin{definition}[Intersection tuple $(\gam\circ\tau\circ \gam', \tau_P)$]
%	We define intersection tuple as the following, \begin{enumerate}
%		\item $\gam,\gamma'$ are left/right shapes and $\tau$ is a middle shape;
%		\item $\gam,\tau$ are properly composable, and $\tau, \gp$ are properly composable;
%		\item $\tau_P$ indicates valid vertex-pair that are intersected in $\gam,\tau,\gp$, and let $\int(\tau_P)$ be the set of intersected vertices, $\int(\gam) =\int(\tau_P)\cap V(\gam)$ be the set of vertices that get intersected from $\gam$, and analogously $ \int(\gp) =\int(\tau_P)\cap V(\gp)$ those in $\gp$;
%		\item $V_\gam$ is the unique MVS for separating $V_\gam$ and $U_\gam$, and $U_\gam$ is the unique MVS separating $V_\gam\cup \int(\gam)$ and $U_\gam$; 
%		\item $U_\gp$ is the unique MVS for separating $U_\gp$ and $V_\gp$, and $U_\gp$ is the unique MVS separating $U_\gp\cup \int(\gp)$ and $U_\gp$.
%	\end{enumerate}
%\end{definition}

%	 With these definitions in hand, intersection tradeoff in our pursuit now becomes for $(\gamma,\tau,\gamma')$ that intersects to $\tau_P$,\begin{align*}
%	 	\begin{bmatrix}
%	 		\lambda_{\Id_{U_\gam}} M_{\Id_{U_\gam}} & \lambda_{\gam\circ \tau\circ\gam'} M_{\tau_P}\\\\
%	 		\lambda_{\gam\circ \tau\circ\gam'} M_{\tau_P}^T & \lambda_{\Id_{V_{\gam'}}} M_{\Id_{V_{\gam'}}} 
%	 	\end{bmatrix} \succeq 0 
%	 \end{align*} 		 Putting back the coloring matrix, our goal becomes,
%	 \begin{lemma}
%	 For any $\gamma, \gamma'$ left/right intersection shape, $\tau$ a middle shape, and $\calS $ a color partitions for $\gam\circ\tau\circ\gamma'$, i.e., it is a color partition for $U_\gam\cup V_{\gam'}$. For convenience, let $\calS_{U_\gam}$ be the color partition of $\calS$ restricted to $U_\gam$, and similarly for $\calS_{V_{\gam'}}$.
%%	  and $\calS_{U_\tau} \in \cp_{U_\tau}, \calS_{V_\tau}\in \cp_{V_\tau}$ color partitions for $U_\tau, V_\tau$.
%	 \begin{align*}
%	 	\begin{bmatrix}
%	 		\lambda_{\Id_{U_\gam}} M_{\Id_{U_\gam}}\otimes H_{\Id_{U_\gam}, \calS_{U_\gam} } & \lambda_{\gam\circ \tau\circ\gam'} M_{\tau_P}\otimes H_{\gam\circ\tau\circ\gam', \calS } \\\\\\
%	 		\lambda_{\gam\circ \tau\circ\gam'} M_{\tau_P}^T \otimes H^T_{\gam\circ \tau\circ\gam', \calS} & \lambda_{\Id_{V_{\gam'}}} M_{\Id_{V_{\gam'}}} \otimes H_{\Id_{V_{\gam'}},\calS_{V_{\gamma'}}} 
%	 	\end{bmatrix} \succeq 0 
%	 \end{align*}
%	 where we recall that a shape-color matrix for improper shape $\gam\circ\tau \circ \gam'$ with color partition $\calS$ is defined as 
%%	  \begin{align*}
%%	 	H_{\gam\circ\tau\gam', \calS} = H_{\gam,\cp_{U_\gam}}\cdot 
%%	 \end{align*}
%	 \end{lemma}
%	  Recall our shape coefficients are defined to be,\[ 
%	 \lambda_\gam = \left(\frac{1}{\sqrt{k}}\right)^{|U_\gam\Delta V_\gamma|}\left(\eta\sqrt{\frac{d}{n}}\right)^{|E(\gam)\setminus E(V_\gam)| }
%	 \]
%	 and \[ 
%	 \lambda_\tau = \left(\frac{1}{\sqrt{k}} \right)^{|U_\tau \Delta V_\tau|} \left( \eta\sqrt{\frac{d}{n}} \right)^{|E(\tau)| }
%	 \]
\paragraph{Overview of intersection-term charging}
	The charging strategy is largely similar to the 2-step charging strategy for middle-shape charging, despite each step may contain more technical twists.
	 \begin{enumerate}
	 	\item For each intersection term $\gam\circ\tau\circ\gam'$ it can be charged to the appropriate diagonal $U_\gam$ or $V_\gp$ (via \cref{lem:intersection-main}) ;
	 	\item For each diagonal, "not too many" intersection terms are being charged to it so that we can afford a union bound.
	 \end{enumerate}
	 \subsection{Charging a particular intersection shape}
		 \begin{lemma}\label{lem:intersection-main}
	 	For intersection-tuple $(\gam, \tau,\gam')$ that intersect to $\tau_P$, 
	 \[ \lambda_{\gam\circ\tau\circ\gp}\cdot \|\cm_{\tau_P} \|\leq o(1)   \]
	 \end{lemma}	
	 
	 
%	 		 Unpacking the equation gives us \begin{align*}
%	 	LHS&\leq \edgeco^{|E(\tau_P)|}\cdot \|M_{\tau_P}\|\cdot \|H_{\gam\circ\tau\circ\gam',(\cp_{U_\gam},\cp_{V_\gp} )}\|\\
%	 \end{align*}
%	 We will again split into the factors of $n$ and $k$.
%	 
	Since $\tau_P$ is a multigraph that arises from intersection, before we unpack the above equation, we need to first understand what our norm bounds $\|M_{\tau_P}\|$ yield for improper graphs coming from intersections.
	% For starters, let us first recall that our norm bounds for graph matrix for color-shape have essentially three components: 1) the factors of $n$ from usual graph matrix norm bounds; 2) the factors of color-automorphism, or simply shape automorphism when we restrict to the single-color case, and 3) the factor of $k$ as we combine the color choices for a vertex, and the potential edge factor of $k-1$ from color-value of a pure-color edge into graph matrix. 
 % Fortunately, despite our usual norm bounds target (proper) shape that does not have multi-edges (while multi-vertices makes no buzz), it is not too hard to extend the norm bounds for improper shape once we consider linearization of improper shapes. 
	
	\subsubsection{Bounding $\|\cm_{\tau_P}\|$}
\begin{fact}
	For $\chi_e$ a $p$-biased Fourier character, we have \[ 
	\chi_e^k= \E[\chi_e^k] + \E[\chi_e^{k+1}]\cdot \chi_e
	\]
\end{fact}
\begin{definition}[Linearization of $\tau_P$]
	Given a multigraph $\tau_P$, we call $\psi$ a linearization of $\tau_P$ if \begin{enumerate}
		\item Each edge in $\psi$ is a (multi-)edge;
		\item Each multiedge in $\tau_P$ has multiplicity $0$ or $1$ in $\psi$.
	\end{enumerate} 
	\end{definition}
\begin{definition}[Vapor coefficient $\vap$ for mul-$1$ edge]
	Fix $\tau_P$ a multigraph, and $\psi(\tau_P)$ its linearization, for any $e\in \psi(E(\tau_P))$, we define its vapor coefficient to be \[ 
	\vap(e) = \mul_{\tau_P}(e) - 1
	\]  
	For intuition, any edge of multiplicity $2$ in $\tau_P$ that linearizes to a mul-$1$ edge in $\psi$ receives a vapor coefficient of $1$. 
\end{definition}
\begin{definition}[Vapor and phantom coefficient $\theta$ for $\psi(\tau_P)$]
	Fix $\tau_P$ a multigraph, and $\psi(\tau_P)$ its linearization, we define the corresponding vapor coefficient of $\psi$ to be \[ 
	\theta_{\tau_P}(\psi) =\sum_{e\in E(\psi)} \vap(e) 
	\]
	Furthermore, let $\phantom_{\tau_P}(\psi)$ be the number of edges that disappear from $E(\tau_P)$ in the linearization $\psi$. The dependence on $\tau_P$ is dropped whenever it is clear.
\end{definition}
\begin{definition}[Floating stick]
	Given an improper graph $\tau_P$ and its linearization $\psi$, we call a component $C\in \psi$ a \emph{floating stick} if \begin{enumerate}
	\item $C$ is floating;
	\item $V(C) = E_\psi(C) - 1$, i.e., this is path.
	\end{enumerate}
\end{definition}
\begin{definition}[Floating cycle]
	Given an improper graph $\tau_P$ and its linearization $\psi$, we call a component $C\in \psi$ a \emph{floating stick} if \begin{enumerate}
	\item $C$ is floating;
	\item $V(C) \geq  E_\psi(C) $, i.e., this is at least a cycle.
	\end{enumerate}

\end{definition}
We remark that the above floating components are further distinguished as they have different contribution to matrix norm bounds: a floating stick $C$ contributes norm $\sqrt{n}^{V(C)}\exp(-d\cdot (|V(C)|-1) )$ while a floating cycle would contribute norm $\max \left(\sqrt{n}^{V(C)}, (\sqrt{\frac{n}{d}})^{E_\psi(C)} \right) \cdot \left(2|V(\tau_P)|q_{\tau_P} \right) $ depending on whether the floating cycle is part of the separator.  

%\begin{proposition} For an intersectable tuple $(\gamma,\tau,\gam')$ that intersects to $\tau_P$,
%	\[ 
%	\|M_{\tau_P}\| \leq 2^{\vap+ \phantom} \left(\sqrt{\frac{n}{d}} \right)^{\theta(\psi)} \max_{S:\text{separator in } \psi}\left(\sqrt{\frac{n}{d}}\right)^{E_{\psi}(S)}\sqrt{n}^{V(\tau_P)\setminus V(S) }\sqrt{n}^{I_{\psi}}\sqrt{d}^{\dang(\psi)} 
%\]
%\end{proposition}
%\begin{remark}
%	Each phantom/vapor edge comes with an extra $\eta$ factor uncharged that can be used to handle the extra factor $2$ blow-up each edge.
%\end{remark}
%

\begin{proposition}[Norm bounds for improper color-shape from $\gam\circ\tau\circ\gp$ intersection]
	Let $\gam\circ\tau\circ\gp$ be an intersection-tuple that intersect to $\tau_P$, \begin{align*}
		\|\cm_{\tau_P}\| &\leq  \cnorm^{|V(\tau_P) \setminus U_{\tau_P}\cap V_{\tau_P}|} 2^{|E(\tau_P)|} \max_{\substack{(\psi, S)\\ \psi: \text{linearization of $\tau_P$}\\ S:\text{a separator for }\psi }}  \left(\sqrt{\frac{n}{d}} \right)^{\theta(\psi)} \left(\sqrt{\frac{n}{d}}\right)^{E_{\psi}(S)}\sqrt{n}^{V(\tau_P)\setminus V(S) }\sqrt{n}^{I_{\psi}}\\& \cdot  \dang(\psi\setminus S)\cdot \float(\psi) \\& \cdot  (k-1)^{|E(\gam\circ\tau\circ\gp)| }
	\end{align*}
\end{proposition}

\begin{proof}
	We highlight the difference from graph matrix norm bounds for usual color-shape,
	 \textbf{Identifying the linearization:} The linearization $\psi$ is fixed by identifying for each multiedge whether it becomes mul-$0$ or $1$ in $\psi$, hence $ 2^{|E(\tau_P)|}$ is sufficient where $|E(\tau_P)|$ is the number of distinct edges in $\tau_P$;
	
	\textbf{Factors of $k$:} It is not hard to see that the tight case comes from each edge from being a pure-edge for the connected part, as we can either assign a factor of $k-1$ to an edge if it leads to new vertices or it is a pure-edge, giving us a factor of $(k-1)^{|E(\gam\circ\tau\circ\gp)|}$;
	
	\textbf{Factors of $n$:} To bound the factor of $n$, we note that its factor comes from the vapor coefficient via linearization and the norm bound factor for the linearization of $\psi$. Via our linearizartion, each multiplicity of edge that vaporizes gives a factor of $\sqrt{\frac{n}{d}}$, captured by the factor of $\left(\sqrt{\frac{n}{d}}\right)^{\theta(\psi)}$, combining with the norm bound factor for $\psi$ gives us \begin{align*}
		&\sqrt{\frac{n}{d}}^{\theta(\psi)} \cdot \max_{S: \text{separator for }\psi }   \left(\sqrt{\frac{n}{d}}\right)^{E_{\psi}(S)}\sqrt{n}^{V(\tau_P)\setminus V(S) }\sqrt{n}^{I_{\psi}} \\& \cdot  \float(\psi) \cdot \dang(\psi\setminus S)
	\end{align*} 
		
% \jnote{serious changes needed below}		
	
% 	\textbf{Automorphism factor} Recall that the graph matrix by definition also has built-in normalizing factor from automorphism (or color-automorphism as we are working with color-shape), and applying our matrix norm bounds prompts us that we need a normalization of $\frac{1}{\aut(\psi)}$ to off-set the automorphism factor in the norm bounds, while we notice we pick up normalizing constant $\frac{1}{|\aut(\gam)|\cdot |\aut(\tau)|\cdot |\aut(\gp)| }$ from the normalizing factor from graph matrix corresponding to $\gam,\tau,\gp$ respectively. 
% 	\begin{lemma}
% 		For any shape $\psi$ that comes from linearization of intersection-tuple $\gam\circ\tau\circ\gp$, there exists a constant $c_\aut>0$ s.t.  \[ 
% 		\frac{\aut(\tau_P)}{ \aut(\gam) \cdot \aut(\tau)\cdot \cdot \aut(\gp)} \leq c^{|E(\gam\circ\tau\circ\gp)|}
% 		\]	\end{lemma}
% 		\begin{proof} We first observe that given a $\tau_P$ coming from a single level of $\gam\circ\tau\circ\gp$ intersection, each shape $\gam,\tau,\gp$ can be identified using edge-decay; and furthermore, there cannot be too many non-isomorphic shapes on the same number of edges, and this completes the proof.	
% \end{proof}
%	\end{enumerate}
Combining the above gives us the desired norm bound.
\end{proof}
Now that we have identified the quantity of interest for $\|\cm_{\tau_P}\|$, it is time to move on and see why the norm bound factor can be offset by $\lambda_{\gam\circ\tau\circ\gp}$, and hopefully, be left with some gap (at least a constant per edge) for counting. Let's proceed by unpacking the desired equation, \begin{align*}
	\lambda_{\gam\circ\tau\circ\gp} \|\cm_{\tau_P}\| &\leq \left(\frac{1}{k}\right)^{|V(\gam\circ\tau\circ\gp)|-\frac{|U_\gamma|+|V_\gp|}{2} } \cdot  \edgeco^{|E(\gam\circ\tau\circ\gp)|}\cdot 2^{|E(\tau_P)|} \\&\cdot \max_{\substack{(\psi, S)\\ \psi: \text{linearization of $\tau_P$}\\ S:\text{a separator for }\psi }}  \left(\sqrt{\frac{n}{d}} \right)^{\theta(\psi)} \left(\sqrt{\frac{n}{d}}\right)^{E_{\psi}(S)}\sqrt{n}^{V(\tau_P)\setminus V(S) }\sqrt{n}^{I_{\psi}}  \cdot  \float(\psi)\cdot \dang(\psi\setminus S)\\ & \cdot  (k-1)^{|E(\gam\circ\tau\circ\gp)| }\\
	&\leq \left(\frac{1}{\ceta\cdot \sqrt{d}}\right)^{|V(\gam\circ\tau\circ\gp)|- \frac{|U_\gam|+|V_\gp|}{2} }\cdot  \left(\sqrt{\frac{d}{n}} \right)^{|E(\gam\circ\tau\circ\gp)|}\cdot 2^{|E(\tau_P)|} \\&\cdot \max_{\substack{(\psi, S)\\ \psi: \text{linearization of $\tau_P$}\\ S:\text{a separator for }\psi }}  \left(\sqrt{\frac{n}{d}} \right)^{\theta(\psi)} \left(\sqrt{\frac{n}{d}}\right)^{E_{\psi}(S)}\sqrt{n}^{V(\tau_P)\setminus V(S) }\sqrt{n}^{I_{\psi}}\\&  \cdot \float(\psi)\cdot \dang(\psi\setminus S)
\\&\cdot  \left((k-1)\cdot \eta\right)^{|E(\gam\circ\tau\circ\gp)| }
\end{align*}
where we transfer the $\frac{1}{k}$ vertex factor to $\frac{1}{\ceta\sqrt{d}}$ using our hardness assumption.
 
\subsubsection{Controlling the factor of $d$ and $n$ for intersection term}
In this subsection, the quantity of interest would be the factor of $d$ and $n$. Our goal of this section is to show the following lemma,
\begin{lemma}\label{lemma:charging-single-intersection}
For $\tau_P$ that arises from intersection of $\gam\circ\tau\circ\gp$, 
	\begin{align*}
		&\left(\frac{1}{\ceta\cdot \sqrt{d}}\right)^{|V(\gam\circ\tau\circ\gp)|- \frac{|U_\gam|+|V_\gp|}{2} }\cdot  \left(\sqrt{\frac{d}{n}} \right)^{|E(\gam\circ\tau\circ\gp)|}\cdot 2^{|E(\tau_P)|} \cdot \max_{\substack{(\psi, S)\\ \psi: \text{linearization of $\tau_P$}\\ S:\text{a separator for }\psi }}  \left(\sqrt{\frac{n}{d}} \right)^{\theta(\psi)} \ \left(\sqrt{\frac{n}{d}}\right)^{E_{\psi}(S)}\sqrt{n}^{V(\tau_P)\setminus V(S) }\\&\cdot  \sqrt{n}^{I_{\psi}}\cdot  \float(\psi)\cdot \dang(\psi) 
\leq o(1)
	\end{align*} 
\end{lemma}
\paragraph{Proof overview}
The above equation lies at the core of our argument for bounding intersection terms. It would be helpful to unpack and classify the terms from the equation into a couple of components (ordered by their relative magnitude).

To start with, each vertex (outside the separator) contributes a factor of $\sqrt{n}$ to the above equation (ignoring its potential dangling/floating factor captured in a separate argument), it suffices for us to assign a factor of $\sqrt{d}$ for each such vertex, and suppose the vertex is connected to the separator $S$ in $\tau_P$, we can offset its contribution via \[
	\frac{1}{\sqrt{d}}\cdot \sqrt{n} \cdot \sqrt{\frac{d}{n}} \leq 1 
	 \]
	 Similarly, for isolated vertex, we need to assign an extra factor of $\sqrt{d}$ and an extra multiplicity of edges in $E(\gam\circ\tau\circ\gp)$. Besides connectivity in $\tau_P$ that requires some work, the major ingredient for this component is the vertex-intersection-tradeoff that says we have enough $\frac{1}{\sqrt{d}}$ factors for vertices outside the new separator after the intersection, captured by the following lemma,
	\begin{lemma}[Vertex factor for intersection (Intersection trade-off lemma from \cite{JPRTX, potechin2023machinery} )] For $\gam\circ\tau\circ\gp$ that intersects to $\tau_P$,
		\[ 
	 |V(\gam\circ\tau\circ\gp)| - \frac{|U_\gam|+|V_\gp|}{2} \geq |V(\tau_P)\setminus V(S)| + |I_\psi|
	 \]
	 for any linearization $\psi$ and separator $S$ of $\psi$;

	\end{lemma}
	Moreover, we need to assign at least one edge in $E(\gam\circ\tau\circ\gp)$ for each vertex in $V(\tau_P)\setminus V(S)$, and potentially more if they are isolated outlined by the above argument. Additionally, we need to identify extra $\sqrt{\frac{d}{n}}$ factor to handle dangling and floating components. The extra gap here relies upon the $k$-wise symmetry of our coefficients, that we start with $\gam$,$\tau$,$\gp$ that do not have dangling branches in the very beginning; hence, any component that becomes floating/dangling is a result of over-linearization (i.e., multi-edges become mul-$0$). That being said, multi-edges turning mul-$0$ can in general be tricky as they are the reason we pick up extra factors for isolated vertices (and dang/floating factors). Towards this end, we first observe the following,
\begin{proposition}[One phantom edge-mul for one dangling/floating factor]
	It suffices for us to assign one edge-multiplicity to each dangling/floating factor.
\end{proposition}
\begin{proof}
	Observe that we pick up a coefficient $\sqrt{\frac{d}{n}}$ for each edge's phantom multiplicity, and each dangling/floating factor is either $2|V(\psi)|q_\psi$ or $\sqrt{n}\exp(-d)$ (in which case the component is outside the separator). \end{proof}

	At this point, we would like an edge-factor assignment scheme that allows us to 	assign edges (specifically their multiplicities) in $E(\gam\circ\tau\circ\gp)$ such that
	
	\textbf{Edge-factor assignment target: necessary condition}
	\begin{enumerate}
		\item Assign one multiplicity to each multiplicity that vaporizes in $\theta(\psi)$ and separator edges in $E_\psi(S)$;
		\item Assign at least one edge's multiplicity to each non-isolated vertex in $V(\tau_P)\setminus V(S)$;
		\item Assign at least two multiplicities to each isolated vertex;
		\item Assign at at least multiplicity $c>0$ (where $c$ may be fractional if needed) to each floating component or dangling branch to offset the dangling/floating factor.
\end{enumerate}



We note that the following target would also be sufficient, as it strengthens the last condition to each multiplicity being charged to at most one dangling/floating factor.


\begin{mdframed}[frametitle = {Edger-factor assignment target: sufficient condition}]
\begin{enumerate}
	\item Assign one multiplicity to each multiplicity that vaporizes in $\theta(\psi)$ and separator edges in $E_\psi(S)$;
		\item Assign at least one edge's multiplicity to each non-isolated vertex in $V(\tau_P)\setminus V(S)$;
		\item Assign at least two multiplicities to each isolated vertex;
		\item Assign at at least one multiplicity to each floating component or dangling branches to offset the dangling/floating factor.\end{enumerate}	
\end{mdframed}

Before we delve into the argument, we remind the reader that $\phantom(\psi))$ is the multiplicity of edges that vanish from $E(\tau_P)$, i.e., of multiedges that become multiplicity $0$ in $\psi$. And instead of working with $E(\gam\circ\tau\circ\gp)$ that counts multiplicity of edges, it is easier for us to consider the (non multi-)graph  $\psi$ and $\phantom(\psi)$ that allows us to avoid worrying about vapor edges and their multiplicities as well. 
%As each edge needs to be at least mul-$2$ to become phantom (i.e., completely vanish), a straightforward bound we would be working is simply 
\begin{claim}
	Recall $\theta(\psi)$ is the multiplicity of edges that vaporize in the linearization to $\psi$ from $\tau_P$, \[ 
	|E_\psi| +\phantom(\psi) =  |E(\gam\circ\tau\circ\gp)| - |\theta(\psi)| 
	\]
\end{claim}
\begin{lemma}[Edge-assignment] \label{lemma:edge-assignment } For $\gam\circ\tau\circ\gp$ that intersects to $\tau_P$ and let $\psi$ be a linearization of $\tau_P$, s.t. \[ 
|E_\psi|+ \phantom(\psi) \geq |V(\tau_P)\setminus V(S)|+|E_\psi(S)|+|I_\psi| + |\dang_\psi|+|\float_\psi|  \numberthis
\]
where we define \[ 
|\float_\psi|  \coloneqq |\fs_\psi| + |\fc_\psi|  
\]
and remind the reader that $\phantom(\psi)$ counts the multiplicity of edges that completely vanish in $\psi$ from linearization $\tau_P$.
\end{lemma}
% %\paragraph{Proof overview}
% %We give an overview of our edge-assignment scheme. The overall idea proceeds via a BFS from $S$ in $\psi$, and notice \begin{enumerate}
% %	\item For each edge in $E(S)$, it contributes one to LHS via $|E_\psi|$ and one to RHS via $|E_\psi(S)$;
% %	\item For each vertex connected to $S$ in $\psi$, (modulo their potential dangling factor), we can charge each vertex to the edge leading to it in the BFS traversal;
% %	\item For each connected component that is not reachable from $S$, we need to assign an edge in $\phantom$ to effectively initialize a BFS process in the component;
% %	\item Additionally, we need to assign an extra multiplicity in phantom to each isolated vertex;
% %	\item Finally, we will assign phantom multiplicity (potentially partial multiplicity) to each dangling and floating component.
% %\end{enumerate}
% %
% %\subsubsection{Charging the factor of $n$ }	 
% %Since $(U_\gam, E(U_\gam))$ (and analogously $(V_{\gam'^T}, E(V_{\gam'^T}))$ ) are positive glyph by construction, we have  \[ 
% %\lambda_{\Id_{U_\gam}} M_{\Id_{U_\gam}} = \left(\eta\sqrt{\frac{d}{n}}\right)^{|E(U_\gam)|}\left(\sqrt{\frac{n}{d}}\right)^{|E(U_\gam)|} 
% %=\eta^{|E(U_\gam)|} \Id_{U_\gam} 
% %\]
% %and \[ 
% %\lambda_{\Id_{V_\gam'}} M_{\Id_{V_\gam'}} = \left(\eta\sqrt{\frac{d}{n}}\right)^{|E(V_\gam')|}\left(\sqrt{\frac{n}{d}}\right)^{|E(V_\gam')|} 
% %=\eta^{|E(V_\gam')|} \Id_{V_\gam'} 
% %\]
% %
% %
% %Hence, our goal is now reduced to showing \[ 
% %\lambda_{\gam\circ\tau\circ\gam'} \|M_{\tau_P}\| \leq \eta^{\frac{|E(U_\gam)| +|E(V_\gam)|}{2}}
% %\]
% %Unpacking the matrix norm bounds we have,\begin{align*} \label{eq:int-tradeoff}
% %LHS= &\left(\eta\cdot \sqrt{\frac{d}{n}}\right)^{|E(\gamma\circ\tau\circ\gamma'^T)|} \max_{\substack{ \psi: \text{linearization of} \tau_P\\ S:\text{separator for } \psi } } \left(\sqrt{\frac{n}{d}}\right)^{\theta(\psi) }    \sqrt{n}^{V(\tau_P)\setminus V(S)} \left(\sqrt{\frac{n}{d}}\right)^{|E_{\psi}(S)| }\sqrt{n}^{|I(\psi)|}\sqrt{d}^{\dang(\psi, S)}
% %%&\leq \left(\frac{1}{\sqrt{n}}\right)^{|E(\gam\circ\tau\circ\gam')| }\max_{\substack{ \psi: \text{linearization of} \tau_P\\ S:\text{separator for } \psi } } \sqrt{n}^{\theta(\psi)+|V(\tau_P)\setminus V(S)|+|E_\psi(S)|+|I(\psi)|}\cdot \left(\frac{1}{\sqrt{d}}\right)^{\theta(\psi)+|E_\psi(S) | -\dang(\psi, S) }  \numberthis
% %\\&=\left(\frac{1}{\sqrt{n}}\right)^{|E(\gam\circ\tau\circ\gam')| }\max_{\substack{ \psi: \text{linearization of} \tau_P\\ S:\text{separator for } \psi } } \sqrt{n}^{\theta(\psi)+|V(\tau_P)\setminus V(S)|+|E_\psi(S)|+|I(\psi)|} \cdot \sqrt{d}^{\dang(\psi, S) }  \cdot  \eta^{\theta(\psi)+|E_\psi(S) |  }
% %   \end{align*}
% %%   Restricting to the factor of $\eta, d$, and recalling that $\eta \sqrt{d}\ll \frac{1}{c}$ prompts us to show (ignoring the $\frac{1}{c}$ decay) \[ 
% %%   \left(\frac{1}{\sqrt{d}}\right)^{\theta(\tau_P)+|E_{\tau_P}(S)|} \sqrt{d}^{\dang} \leq \left(\frac{1}{\sqrt{d}}\right)^{\frac{|E(U_\gam)|+|E(V_\gam)|}{2} }
% %%   \]
% %   where we recall \[
% %   \theta_{\tau_P}(\psi)=\sum_{e\in E(\psi)}  (\mul_{\tau_P}(e)-1) 
% %   \] 
% %   measures the ''vaporization'' of high-mul edges into mul-1 edges after linearization, and recall we assume $\eta\cdot \sqrt{d} \ll c_\eta $ as our hardness assumption. 
% %\begin{enumerate}
% %   	\item Find a subset of edges  $\exc\subseteq E(\gam\circ\tau\circ\gam')\setminus E(S)$ (in fact, $\exc\subseteq E(U_\gam)\cup E(V_\gp)\setminus E(S) $) s.t. every vertex is still connected to the SMVS $S$ without using these edges in $\tau_P$, the edge coefficient $\edgeco$ of these edges will be transferred to factors in $\eta$ to show we have enough $\eta$ decay on the LHS; 
% %   	\item Each edge-multiplicity that vaporizes, and each edge in $E(S)$ comes with a coefficient of $\eta\cdot\sqrt{\frac{d}{n}}$ and contributes $\sqrt{\frac{n}{d}}$ to the norm bound, leaving a slack of  $\eta$ factor each edge;
% %   	 \item For edges in $E(\gam\circ\tau\circ\gam')\setminus (\exc\cup E(S)) $, each of them appears with coefficient $\eta\cdot \sqrt{\frac{d}{n}}\leq \frac{1}{\sqrt{n}}$ (ignoring the constant factor of decay that leaves a slack for counting), we will use a charging argument to show they handle the factor $\sqrt{n}^{V(\tau_P)\setminus V(S)}\sqrt{n}^{|I(\psi)|}\sqrt{d}^{\dang(\psi,S) }$ 
% %   \end{enumerate} 
% %   Our goal now becomes \begin{align*}
% %   	&\log n\cdot \exc + \theta(\psi)+|E_\psi(S)| \geq \frac{|E(U_\gam)|+|E(V_\gam')|}{2} \numberthis \\
% %   	& |E(\gam\circ\tau\circ\gam')|-\exc-|E(S)|-|V(\tau_P)\setminus V(S)|-|I(\psi)|-\theta(\psi)- c\cdot (\dang\cup \float) \geq 0 \numberthis
% %   \end{align*}
% %   for some constant $c>0$.
% %   \subsubsection{Finding $\exc$}
% %   \jnote{This argument is similar to the middle shape charging for $\tau_c$.}
% %   \begin{claim}
% %   	There is a set of edges $\exc\subseteq (E(U_\gam)\cup E(V_\gp))\setminus E(S)$ we can reserve s.t. each vertex in $\tau_P$ is connected to $S$ without using any of these edges, and moreover,\[ 
% %   	\exc \geq  \lceil \frac{|E(U_\gam)\setminus E(S)|+|E(V_\gp)\setminus E(S)|  }{\log_d n} \rceil 
% %   	\] 
% %   \end{claim}
% %%   We will first classify vertices in $U_\gam$ (and $V_{\gam'^T}$ analogously) as the following,\begin{claim}
% %%   	Each vertex in $U_\gam$ satisfies at least one of the following conditions,\begin{enumerate}
% %%   		\item it is a vertex to-be-intersected;
% %%   		\item it is in $U_\gam\cap V\gam$;
% %%   		\item it has at least $2$ distinct paths to vertices to-be-intersected.
% %%   	\end{enumerate}
% %%   \end{claim}
% %   \begin{definition}[Boundary set $B(\gam)$] 
% %   	Given a left-shape $\gam$, we define its boundary set $B(\gam)\subseteq U_\gamma $ by including each vertex $v\in U_\gam$ into $B(\gam)$ if it satisfies one of the following conditions,
% %   	\begin{enumerate}
% %%   		\item $v$ is to-be-intersected;
% %   		\item $v$ has a path to some to-be-intersected vertex in $V(\gam)\setminus U_\gamma$ without using any edge in $E(U_\gam)$;
% %   		\item $v$ has a path to $V_\gam\setminus U_\gamma $ without passing through any vertex in $U_\gam$.
% %   	\end{enumerate} 
% %   \end{definition}
% %   
% %   \begin{lemma}
% %   	Each vertex in $B(\gam)$ has a path in the phantom graph $\tau_P$ to $V_{\gam'}$ without using any edge in $\left(E(U_\gam)\cup E(V_{\gam'})\right)\setminus \left(E(U_\gam\cap V_\gam)\cup E(U_{\gam'} \cap V_{\gam'})\right)$.   \end{lemma}
% %   	\begin{proof}
% %   		We start by considering $v$ a vertex with a path to some to-be-intersected vertex $v'$ without using any edge in $E(U_\gam)$.
% %   		   	\begin{claim} For $v'$ a to-be-intersected vertex,  it has a $E(U_\gam)\cup E(V_{\gam'^T})$-free path to $V_{\gam'^T}$, or a  $E(U_\gam)\cup E(V_{\gam'^T})$-free path to $U_\gam\cap V_\gam$.
% %   		\end{claim}
% %   		\begin{proof}
% %   		Let $u$ be a vertex that intersects with $v'$. 
% %   		\begin{enumerate}
% %   			\item If $u$ appears in $V(\tau)$, it has a $E(U_\gam)\cup E(V_{\gam'^T})$-free path to $V_\tau$: this is immediate for $u\in V_\tau$. Otherwise,  for $u\in V(\tau)\setminus (U_\tau\cup V_\tau)$, $u$ has a $E(U_\tau)\cup E(V_\tau)$-free path to $V_\tau$ as any vertex in  $V(\tau)\setminus (U_\tau\cup V_\tau)$ is on a path from $U_\tau$ to $V_\tau$.
% %   				
% %   				Given the path to some $u'\in V_\tau$, notice $u'$ has a $E(V_{\gam'^T})$-free path to $V_{\gam'^T}$ as any vertex in $V_\tau= U_{\gam'^T}$ is connected to $V_{\gam'^T}$; this path is not necessarily $E(U_\gam)$-free, however, stopping the path before the first edge in $E(U_\gam)$ gives us a $E(U_\gam)\cup E(V_{\gam'^T})$-free path to some vertex in $U_\gam\cap V_\gam$.
% %   			\item 	If $u$ appears in $V(\gam'^T)$, the claim is again immediate for $u\in V_{\gam'^T}$; for $u\in V(\gam'^T)\setminus (U_{\gam'^T}\cup V_{\gam'^T})$, there is a $E(U_{\gam'^T})\cup E(V_{\gam'^T})$-free path to $V_{\gam'^T}$ by left/right shape structure.
% %   		\end{enumerate}
% %   	   		\end{proof}
% %   		\begin{claim}
% %   			For $v\in U_\gamma$ that has a path to $V_\gamma\setminus U_\gamma$ without passing through any other vertex in $U_\gam$,  it has a $E(U_\gam)\cup E(V_{\gam'^T})$-free path to $V_{\gam'^T}$, or a  $E(U_\gam)\cup E(V_{\gam'^T})$-free path to $U_\gam\cap V_\gam$.
% %   		\end{claim}
% %   		\begin{proof}
% %   			The argument is similar as above. The vertex in $V_\gam=U_\tau$ has a $E(V_{\gam'^T})$-free path to $V_{\gam'^T}$ though it might not be necessarily $E(U_\gam)$-free. However, stopping the path at the first $E(U_\gam)$ edge gives a $E(U_\gam)\cup E(V_{\gam'^T})$-free path to $U_\gam\cap V_\gam$.
% %   		\end{proof}
% %		\begin{claim}
% %			Each connected component of $U_\gam\cap V_\gam$ has a $E(U_\gam)\cup E(V_{\gam'^T})$-free path to $V_{\gam'^T}$. 
% %		\end{claim}
% %		\begin{proof}
% %		Let $C$ be a connected component in $U_\gam\cap V_\gam$. If any vertex in $C$ appears in $V_{\gam'^T}$, the claim is immediate; otherwise, if some vertex $v\in C$ appears in $V_\tau\setminus V_{\gam'^T}$, there is a path in $\gam'$ from this $v$ to $V_{\gam'^T}$ that is $E(V_{\gam'^T})$-free. To ensure the path is also $E(U_\gam')$-free, orient the path from $V_{\gam'^T}$ to $v$, we can stop the path when it reaches some vertex of the component in $U_\gam\cap V_\gamma$. Finally, if some vertex $v$ appears in $U_{\tau}\setminus V_\tau$, the component has a $E(U_\gam)\cup E(V_{\gam'^T})$-free path to $V_\tau$; once at $V_\tau$, consider the path from $V_\tau$ to $V_{\gam'^T}$, by our previous argument, the path is either $E(U_\gam)\cup E(V_{\gam'^T})$-free, or there is a path to some vertex in $U_\gam\cap V_{\tau}$, in which case we can use the argument for $V_\tau\setminus V_{\gam'^T}$.
% %		\end{proof}
% %	This completes our proof to the lemma for $E(U_\gam)\cup E(V_{\gam'^T})$-free connectivity.
% %\end{proof}
% %
% %		\begin{lemma}[Intersection trade-off for factor of $\eta$]
% %   	\[ \log_d n\cdot \exc +\theta(\psi)+|E_\psi(S)|\geq \frac{|E(U_\gam)|+|E(V_{\gam'^T})|}{2}\numberthis \label{eq:int-trade-off-eta}
% %   	\] 
% %   \end{lemma}
% %   \begin{proof}
% %   		\begin{claim}
% %   			Each vertex in $B(\gam)\cup (U_\gam\cap V_\gam)$ is connected to $S$ in $\tau_P$, or some phantom edge that vanishes from the linearization to $\psi$.
% %   		\end{claim}
% %   		\begin{proof}
% %   		Each vertex in $B(\gam)\cup (U_\gam\cap V_\gam)$ has a $E(U_\gam)\cup E(V_{\gam'^T})$-free path to $V_{\gam'^T}$. If this path survives the linearization and appears in $\psi$, it must be blocked by the separator $S$ and hence we can arrive at the vertices $B(\gam)\cup (U_\gam\cap V_\gam)$  via the promised $E(U_\gam)\cup E(V_{\gam'^T})$-free paths from the above lemma. For paths that vanish in the linearization, there must be a phantom edge that vanishes, and the same argument applies.
% %   		\end{proof}
% %%   		
% %%   		Consider the components connected to $S$ in $\tau_P$ and BFS from $S$ in the phantom graph, we can use the paths promised from the previous claims to arrive at vertices in $B(\gam)\cup (U_\gam\cap V_\gam)$ without using any edge in $\left(E(U_\gam)\cup E(V_{\gam'^T})\right)\setminus \left(E(U_\gam\cap V_\gam)\cup E(U_{\gam'^T} \cap V_{\gam'^T})\right)$.
% %   	
% %   	We now show the desired logarithmic trade-off between $\exc$ and $E(U_\gam)\setminus E(S), E(V_{\gam'^T})\setminus E(S)$.
% %		
% %	\begin{claim}
% %		$B(\gam)\cup (U_\gam\cap V_\gam)$ is a left-separator for $\gam$, i.e., $B(\gam)\cup (U_\gam\cap V_\gam)$ separates $U_\gamma$ from $\int(\gam)\cup V_\gam$.
% %	\end{claim}
% %	\begin{proof}
% %	By construction, any path from $V_\gam\setminus U_\gamma$ would be blocked by condition-2 vertex in $B(\gam)$, and any vertex intersected is blocked by $B(\gam)$ by condition-1. 
% %	\end{proof}
% %	Now, if we add the edges (as well as the incidental vertices) of $E(U_\gam)\setminus E(S)$ into $B(\gam)\cup (U_\gam\cap V_\gam)$
% %	, since $(U_\gam, E(U_\gam))$ is the SMVS for $\gam$, we expect a change of $\sqrt{\frac{n}{d}}^{e}\sqrt{n}^{-v}\gg 1$, and noting $e-v=|\exc|$ gives us the desired \[ 
% %	\exc(E(U_\gam)\setminus E(S)) \geq  \frac{|E(U_\gamma)\setminus E(S)|}{\log_d n}
% %	\] 
% %	Repeating the same argument with $\gam'^T$ gives us \[
% %	\exc(E(V_{\gam'^T})\setminus E(S)) \geq  \frac{|E(V_{\gamma'^T})\setminus E(S)|}{\log_d n}
% %	\]
% %	Taking the average gives us \[ 
% %	\exc\geq \frac{|E(U_\gam)\setminus E(S)|+|E(V_{\gam'^T})\setminus E(S)|}{2\log_d n}
% %	\]
% %	Noticing $\theta(\psi)\geq 0$, each edge in $E(S)$ contributes an $1$ to the LHS, and at most an $1$ on the RHS completes our proof for \cref{eq:int-trade-off-eta} .
% %    %   
% %   \end{proof}
% %
% %\subsubsection{Handling log factors}
% % \paragraph{Where do logs come from?}	Each connected component of vertices in $\psi$ a linearization of $\tau_P$ contributes to the norm bound an extra $\log$ factor if the component is not connected in $\psi$ to $U_{\tau_P}\cup V_{\tau_P}$. Similarly, each dangling component in $\psi$ outside the separator also contributes an extra $\log$ factor.
	
% %	\begin{claim}
% %		For each connected component in $\psi$ not reachable from $S$ the separator of $\psi$, we can assigned an edge in $\res \subseteq  E(\gam\circ\tau\circ \gam')$ s.t. each connected component in $\psi$ is reachable from $S$ in $\tau_P$ without using any edge in $\res\cup \exc$.
% %	\end{claim}
% %	\begin{question}
% %		Can one phantom edge vanishing increase the number of components not connected to $S$ by $2$?
% %	\end{question}
% %	\begin{proof}
% %		We give an inductive proof. Starting from $\gam\circ\tau\circ\gam'$ with phantom edges put back, we are going to remove a pair of phantom edges in each iteration $t$, and assign an edge that is either a previously removed-but-uncharged phantom edge, or a newly-removed phantom edge to each new component not connected to any separator of $\psi_t$ after the vanishing of the new phantom edges.
% %		
% %	Let the phantom edges being merged be $(i,j)$ and $(i',j')$ at $\psi_t$. Suppose $i$ collide with $i'$ and $j$ collide with $j'$. Let $C_1$ be the component of vertices connected to $(i,j)$ at $\psi_{t-1}$, and $C_2$ those connected to $(i',j')$. Note $C_1$ and $C_2$ might be the same connected component. Observe that after merging vertices $i$ with $i'$, $j$ and $j'$, and removing the edge $(i,j)$, there can be at most $2$ components connected to $i=i'$ and $j=j'$ in $\psi_t$, and call them $C_i$ and $C_j$.
% %	
% %	We case on whether $C_1$ and $C_2$ are connected to separator of $\psi_{t-1}$ before the merging. The worst case should be when both $C_1$ and $C_2$ are connected to the separator of $\psi_{t-1}$. In this case, assume W.L.O.G. $(i,j)$ comes from $\gam$. Suppose $(i,j)$ is on some path from $U_{\psi_t}$ to $V_{\psi_t}$, and also $(i',j')$, i.e., they are both non-dangling. Assume $i$ has a path to $U_{\psi_t}$ and $j$ has a path to $V_{\gamma}$ and then to $V_{\psi_t}$ without using the edge $(i,j)$. We now case on whether $i'$ has an $(i',j')$-free path to $V_{\psi_t}$. If so, the component connected to $i$ in $\psi_t$ is connected to the separator at $S_i$ since there is an $(i,j)$-free path from $U_{\psi_t}$ to $i$, then to $i'$ and to $V_{\psi_t}$. Otherwise, suppose $j$ in $V(\gam)$ is connected to some vertex $v\in V_\gamma$. Since any vertex in $v\in U_\gam\setminus V_{\gamma}$ has degree at least $2$, there is another path from $U_{\psi_{t}}$ to $j$ without using the vanishing phantom edge $(i,j)$. 
% %	
% %	 This path might already be broken before by some other phantom edge. However, there is at least one vanished-but-uncharged phantom edge as the vanishing edge has multiplicity-$2$ and we only need to use one multiplicity of the phantom edge to reach the component disconnected from the separator at $\psi_{t-1}$. The other multiplicity might be used to pay for a potential $\log$ factor for the component disconnected to the edge, but we can charge the $\log$ factor to the most recently broken path from $U_\gamma$ to $v$ to control the number of $\log$ factors charged to one particular vanished-but-uncharged edge. 
% %	 
% %	 If there are no broken paths from $U_{\tau_P}$ to $u$, we would have found a phantom-free path from $U_{\tau_P}$ to $u$, to $j$, and then to $j'$, finally arriving at $V_{\tau_P}$. Hence, this component is still connected to the separator of $\psi_t$.
% %	 
% %	 Since the phantom edge may be incident to at most $2$ connected components in the phantom graph at $\psi_t$, and one of them is connected to the separator or charged to an. We may use one vanishing phantom edge to connect to the separator in the phantom graph, and use another to charge the $\log$ factor of the other component.
% %	\end{proof}
% %
% %\paragraph{Charging log factors}	
% %		
% %
% %	With this strategy, the quantities we are interested in this subsection are the following parameters, \begin{enumerate}
% %	 	\item $\cc$: the number of connected components not reachable from the separator $S$ after the linearization, each of which requires a $\sqrt{n}$ factor to restart BFS process;
% %	 	\item $I_\psi$: the number of isolated vertices;
% %	 	\item $|\dang_\psi|$: the number of branches that are dangling or floating outside the separator, each of which requires $2|V(\al)|q_\al$ factors;
% %	 	\item $\phantom$: the total multiplicity of edges that \textbf{completely} vanish in the linearization, each of which gives a factor of $\frac{1}{\sqrt{n}}$.
% %	 \end{enumerate}
% %	 The focus in this section is showing \[
% %	 	\phantom - \cc -\iso - \float \geq O(1)\cdot  |\dang|  \numberthis
% %	 	\label{eq: log-branches}
% %	 \]
% %%	 Towards this end, consider the graph $\gam\circ\tau\circ\gam'$ with phantom edges put back, and show \cref{eq: log-branches} inductively in the process of removing potential phantom edges. Let $(i,j)$ be the current phantom edge being processed, and let its other phantom copy be $(i',j')$. 	
% % 	\begin{definition}[log-charged]
% %		We call a (multiplicity of) phantom edge log-charged if it is used to charge $2Vq$ factors from norm bounds instead of $\sqrt{n}$ factors for isolated vertices or restarting BFS in connected component not reachable from the separator. 
% %	\end{definition}
% %	\begin{remark}
% %		The name log-charged is a a ''misnomer'' as $2|V(\al)|q_\al$ factor from norm bounds is not necessarily logarithmic in $n$ as $|V(\al)| \approx n^\delta$ in our setting. However, in the simplest cases, this corresponds to the well-known log factors in norm bounds.   
% %	\end{remark}
	\begin{proof}[Proof to \cref{lemma:edge-assignment }]
	We start by considering $\psi$ the linearized graph (recall $\psi$ may have phantom edges removed) and put phantom edges back along the way. Take $S$ to be the SMVS for $\psi$, we then consider the following recursive process to traverse $\psi$ via edges in $E(\tau_P)$.
	
	 Throughout the process, vertices in the graph $V(\psi)$ can be partitioned as the following,
	\begin{enumerate}
		\item $V_W\subseteq V(\tau_P)$: those reachable from $W$ via edges in $E_\psi$ or already in $W$;
		\item For a connected component $C\subseteq V(\psi)\setminus V_W$ in $E_\psi$ while not yet reachable from $W$, it is either a non-floating component, a floating-stick, or a floating-cyc;
		\item For isolated vertices in $V(\psi)\setminus V_W$, we can group them according to the phantom edges into a collection of iso-connected components.
	\end{enumerate} 
	\begin{mdframed}[frametitle = {$W$-exploration procedure }]
		\begin{enumerate}
		\item Let $W$ be the current set of vertices visited (initialized to be $S$ an arbitrary SMVS of $\psi$);
		\item Explore the vertices (not yet in $W$) while connected to $W$ via edges in $E(\psi)$, i.e., assign the edge to each vertex it leads to;
		\item Process the dangling/floating factor for vertices in $W$, and this may potentially explore component connected to $W$ via phantom edge;
		\item Explore a component connected to $W$ via some phantom edge;
		\item For vertices outside $W$ and not reachable via phantom from $W$, there must be a phantom-edge connecting two different components, process that phantom edge and explore both components;
		\item Repeat this process until all vertices are pushed into $W$.
	\end{enumerate}
	

	\end{mdframed}
	
		
	 For starters, we first notice for the component $C_S$ that is connected to the separator of $\psi$, we have \[
	|E_\psi(C_S)| \geq  |V(C_S)\setminus V(S)| + |E_\psi(S)|
	 \]
	 as each vertex is connected to the separator, and we can charge it to the edge leading to the vertex when we BFS from $S$, and each separator edge in $E_\psi(S)$ contributes an $1$ to both sides. That being said, we may have dangling/floating factors not yet accounted in $C_S$, not to mention there may be components not reachable from $S$ in $\psi$.
	 
	 
	 For the subsequent steps involving dangling/floating factor , we need to repeatedly apply the following proposition which allows us to identify either there is a new phantom edge incident or there is some excess edge not used in the \emph{exploration} process in the component, \begin{proposition}[Degree-at-least-two] \label{prop:at-least-deg-two}
	 In $\tau_P$ where phantom edges are yet to vanish, each vertex in $V(\tau_P)\setminus (U_{\tau_P}\cup V_{\tau_P}) $ have degree at least $2$ (not counting multiplicities).
	 \end{proposition}
	 \begin{proof}
	 Each vertex in $V(\tau_P)\setminus (U_{\tau_P}\cup V_{\tau_P})$ comes from at least one of the following two categories, $V(\gamma)\setminus U_\gam, V(\gp)\setminus V_\gp$ and $V(\tau)\setminus (U_\tau\cup V_\tau)$. Any vertex in the first category has degree at least $2$ in $\gamma$ from $\gamma$ shape property that $V_\gamma$ is the MVS for $\gamma$ (analogously for $\gp)$, and any vertex in $V(\tau)\setminus U_\tau\cup V_\tau$ has degree at least $2$ in $\tau$ by $k$-wise symmetry.
	 \end{proof}

	 
%	 \begin{corollary}
%	 	For any component reached via some phantom edge in the process while currently not in $W$, it is incident to some uncharged phantom edge. 
%	 \end{corollary}
	Let $W$ be the current set, and let $E_\psi(W), \phantom_W(\psi)$ be the multiplicity of edges traversed so far, and $I_\psi, \dang_\psi, \float_\psi$ be the factors processed so far. We maintain the invariant, \[ 
	 |E_\psi(W)|+ \phantom_W(\psi) \geq |V(W)\setminus V(S)|+|E_\psi(S)|+|I_\psi(W)| + |\dang_\psi(W) |+|\float_\psi(W) | \]
	 In the base case, we have $W=S$, and the inequality holds immediately.	As noted above, it is also immediate for $V_W = V(C_S)$. We now start processing potential dangling/floating factors on vertices in $V_W$. Notice in the base case, the only factors involved are dangling factors, and we can restrict our attention to its end-point, and notice it is either incident to an uncharged edge in $E_\psi$, or a phantom edge via Proposition~\ref{prop:at-least-deg-two}. For a phantom edge, we discuss by cases depending on where it leads to, as it may incur new floating factors for which we need to either identify there is either some excess edge in the new component, or a new phantom edge incident to the component.
	 	 \begin{enumerate}
	 	\item The phantom edge leads to another vertex in $W$, and the vertex it leads to may be assigned another dangling/floating factor as well, in which case we pick up at least $2$  (from phantom multiplicities) and $2$ from RHS for $2$ dangling/floating factors;
	 	\item The phantom edge leads to a component $C$ not yet explored, i.e., not in $W$, in which case we pick up at least $2$ phantom multiplicities from the LHS. We assign one multiplicity to the current dangling/floating factor being processed with one remaining phantom multiplicity yet-to-assign . It now remains to assign this multiplicity and identify an excess edge for the floating factor of the new component,
	 	\begin{itemize}
	 		\item If $C$ is a floating-stick, assign the above multiplicity to the vertex in $C$ incident to the current phantom edge, which also puts $C$ into $W$. Moreover, we claim that $V(C)$ must have at least one more degree-$1$ vertex in $\psi$ that is incident to some not yet processed phantom edge by Proposition~\ref{prop:at-least-deg-two} (notice we get extra gap if $C$ has more than $2$ deg-1 vertices);
	 		\item If $C$ is a floating-cycle, it must be outside $S$, while $E_\psi(C)\geq V_\psi(C)$, hence we can use the remaining multiplicity from earlier to assign to the floating factor of $C$, and use the edges in $E_\psi(C)$ to \emph{explore} vertices in $V_\psi(C)$;
	 		\item If $C$ is non-floating, (eg. $V(C)$ intersects with $U_\psi\cup V_\psi$), there is no dangling/floating factor on $C$, and we assign the above multiplicity to the vertex in $C$ incident to the current phantom edge;
	 		\item If $C$ is an iso-connected component, i.e., a connected component in $\tau_P$ that become isolated under $\psi$, since each vertex in $V(C)$ is of degree at least $2$ in $\tau_P$, assign the remaining multiplicity from above to the first vertex in $V(C)$. Note that since it is isolated, it remains for us to find assign this \emph{source} vertex another edge-multiplicity. Putting that aside, we can traverse the iso-connected component, and charge each phantom edge (and its $2$ multiplicities) to the new vertex it explores. Since each vertex has degree at least $2$, there must be an incidental phantom edge, and we can assign one of its multiplicities to the \emph{source} vertex of this component, filling the gap from earlier. The other multiplicity is then reserved to explore the potentially new component.
 	 		 	\end{itemize} 
	 	\end{enumerate}
	 	
	 	For components not yet explored, and they are not connected to the current $W$ via any phantom edge, we claim that there must be a phantom edge that connects two unexplored components. This follows via our intersection-tuple property, that in $\tau_P$, each vertex has a path to $U_\psi$ and a path to $V_\psi$. Hence it is either reachable from the separator in $\psi$, or reachable from some phantom edge. We can then use this two multiplicities to \emph{explore} these two components into $W$, and notice each of them may be floating, while we can follow the above argument and identify a new phantom edge or an excess edge for each floating component. This completes our proof to  Lemma~\ref{lemma:edge-assignment }.	
 \end{proof}

% \clearpage
% \newpage
	 	
% %	 	
% %	 	
% %		For components not explored from the above process, we first consider components connected to $U_{\tau_P}$ or $V_{\tau_P}$, i.e., those not floating. For any such component, it is necessarily incident to a phantom edge by connected truncation, i.e., there must be a path to the other side that gets broken by phantom edges, and any such phantom edge is evidently uncharged from the earlier process; following the path $P$, a $U\rightarrow V$ path from $\tau_P$ while in $\psi$, and consider the the phantom edge along this path; again, we case on where it leads to in $\psi$. For clarity, suppose the current component in examination is connected to $U_{\tau_P}$, \begin{enumerate}
% %	 		\item The phantom edge leads to a component connected to $V_{\tau_P}$, in this case, neither component have floating/dangling factor, and we can restart the BFS in both components as we have at least $2$ multiplicities from the current phantom edge. In other words, we pick up $2$ on both sides of the equation.
% %	 		\item The phantom edge leads to a floating component, analogous to the above, we can use the $2$ multiplicities to restart BFS in both components, however, we now pick up one floating factor for the component the phantom edge leads to. We now claim that we can continue following the $U\rightarrow V$ path we pick to sail in the beginning, and there must be another phantom edge along this path incident to the floating component, and we can now recurse along this path, noticing we now only need to charge a floating factor instead of a BFS restarting factor that we start with.
% %	 		\item The phantom edge leads to an iso-connected component, following the argument for iso-connected component explored from a dangling branch, there is at least one phantom edge incident to the iso-connected component that remains uncharged after charging for the vertices in the iso-connected component; analogously, consider the phantom edge on the path $P$ that leaves the iso-connected component, since we charge each isolated vertex to the edge that leads to it, this phantom edge in question is evidently uncharged, \begin{itemize}
% %	 			\item if the phantom edge leads to a component connected to $V_{\tau_P}$, we can use its two multiplicities to restart BFS in both sides, and there is no dang/floating factor needed;  if we passed through floating component along the way, we can instead use one multiplicity to restart BFS and one multiplicity to charge the floating factor (that gets translated from a BFS restarting factor as we pass through floating component along the way);
% %	 			\item if the excess phantom edge leads to a floating component, we can use the two multiplicities to restart BFS (or one multiplicity to charge dang/floating and one to restart) on both sides (and then follow the argument in Case 2 as we now have translated a BFS restarting factor to dang/floating factor). 
% %	 		\end{itemize} 		
% %	 		For any remaining vertices, we can first contract the isolated vertices into iso-connected components, and therefore, what remains to be charged is a collection of isolated vertices and floating components. We claim they all have path connected to some component already explored, as it have a path to $U_{\tau_P}\cup V_{\tau_P}$ and any component connected (in $\psi$) to $U_{\tau_P}\cup V_{\tau_P}$ is already explored via our recursive exploration procedure by this stage. Now, we can charge the phantom edge (at least $2$ multiplicities) that leads to the isolated vertex/floating component, that is $2$ phantom multiplicities for 	each isolated vertex (for vertex factors), and $1$ for restarting BFS plus $1$ for floating factor if leading to floating components.
% 	%	Let $t$ denote the the iteration in which we process the $t$-th potential-phantom edge.	An edge is potential phantom if it appears with multiplicity at least $2$.  The base case holds by non-dangling truncation for $t=0$. Let $S_t$ be the separator that separates $U_{\tau_P}=U_\gam$ from $V_{\gam'^T}=V_{\tau_P}$ at the $t$-th iteration. We start by asking the question: is $(i,j)$ on an edge-disjoint path from $U_{\tau_{P(t)}}$ to $V_{\tau_{P(t)}}$. And similarly for $(i',j')$. In other words, are these edges dangling? W.L.O.G. we can assume $(i,j) \in E(\gam)$. 
% %	
% %	 Let the component connected to $i$ without using the edge $(i,j)$ before the merge be $C_i$, and define $C_j, C_{i'}, C_{j'}$ analogously. Assume $i$ collides with $i'$ and $j$ collides with $j'$, and notice $C_i$ is connected to $C_{i'}$, and $C_j$ with $C_{j'}$ after the merge regardless of whether the phantom edge vanishes. We now discuss by cases.
% %%
% %
	 
% %	 	 We will show each merge either increases the number of connected components not reachable from the new separator after $(i,j)$ vanishes by $1$, in which case we can use one multiplicity to restart BFS at the newly-added component not reachable from the separator, and another phantom multiplicity to carry logs; or the merge may create two new connected components  not reachable from the separator, in which case, we will identify one more multiplicity of phantom edge that vanishes before iteration $t$ (which may be log-charge before the iteration) \textbf{around} the phantom edge $(i,j)$, in which case we have $3$ multiplicities of phantom edges, and we can use $2$ multiplicities to restart BFS in the $2$ new connected components not reachable from the separator created by the merge, and the other multiplicity to carry log. We additionally show each log-charge edge carries at most $3$ log factors at the end of the charging.
% %	 		
% %	 \begin{enumerate}
% %	 	\item \textbf{$(i,j), (i',j')$ are both non-dangling before the merge}:
% %	 	
% %	 	Without loss of generality, we can assume $(i,j)\in E(\gamma)$. Furthermore, 
% %	 	suppose $(i,j)\in E(\gamma)\setminus E(U_\gamma)$:	
% %	 	 let $j$ be the vertex t hat has an $(i,j)$-free path to $V_\gamma\setminus U_\gamma$ in $\gam$.
% %	 	We case on whether there is a phantom-free (edge-disjoint) and $(i,j)$-free path from $U_{\tau_P}=U_\gamma  $ to $j$ via some vertex in $V_\gamma\setminus U_\gamma$ before the merge of $(i,j)$. Furthermore, we case on whether $j'$ has an $(i',j')$-free path to $V_{\tau_P}$.  
% %	 	\begin{enumerate}
% %	 		\item If both are yes, $C_j\cup C_{j'}$ is connected to the separator as the path from $U_{\tau_P}=U_\gamma  $ to $j$ via some vertex in $V_\gamma\setminus U_\gamma$, then to $j'$ and to $V_{\tau_P}$ is phantom-free after the $(i,j)$-merge at this iteration. Therefore, $\phantom$ increases by $2$, $\cc$ increases by $1$, and $|\dang\cup \float|$ increases by $2$. 
% %	 		\item If $j$ has a phantom-free (edge-disjoint) and $(i,j)$-free path from $U_{\tau_P}=U_\gamma $ while $i'$ (instead of $j'$ in the last case) has an $(i',j')$-free and phantom-free edge-disjoint path to $V_{\tau_P}$, since $(i,j)$ are non-dangling, $i$ has a phantom-free path to $U_{\tau_P}$. In this case, $C_i\cup C_{i'}$ is connected to the separator after the merge since the path from $U_{\tau_P}$ to $i$, to $i'$ and finally to $V_{\tau_P}$ is phantom-free. The effect on the \cref{eq: log-branches} is identical to the last case.
% %	 		\item If $j$ does not have a path from $U_{\tau_P}=U_\gamma $ that is both phantom-free (edge-disjoint) and $(i,j)$-free, the charging is more complicated. By construction of left-shape, $j$ has a path from $U_{\tau_P}=U_\gamma $ that is both phantom-free (edge-disjoint) and $(i,j)$-free, hence that path must already be broken in previous iterations. Consider the $(i,j)$-free path from $j$ to $U_{\gamma}$, and consider the phantom edge closest to $j$, we observe that it has at least one multiplicity that is uncharged or log-charged as we only need one multiplicity to restart BFS in the component potentially disconnected from the separator when that edge vanishes; that being said, the other multiplicity remains uncharged though it might be used to carry one log factors related to itself being a dangling component and another log factor of the disconnected component. Furthermore, observe each multiplicity of phantom edge gets charged at most $3$ dangling factors in this process.
% %%	 		\item If $j$ has a phantom-free (edge-disjoint) and $(i,j)$-free path from $U_{\tau_P}=U_\gamma $ while $i'$ (instead of $j'$ in the last case) has an $(i',j')$-free and phantom-free edge-disjoint path to $V_{\tau_P}$, and $i$ does not have a phantom-free path to $U_{\tau_P}$. We claim that following the path in $\gamma$ from $i$ to $U_\gamma=U_{\tau_P}$, the path must be broken by some phantom edge. Consider the phantom edge closest to $i$ in the backtracking process to $U_{\gamma}$,  
% %	 	\end{enumerate}
% %	 	If $(i,j)\in E(U_\gam)$, the number of connected components can only increase by $1$ after the merge. Since we assume both edges to be non-dangling before the merge, either $i'$ or $j'$ has an $(i',j')$-free path to $V_{\tau_P}$, hence after the merging, either $C_i\cup C_{i'}$ or  $C_j\cup C_{j'}$  still has a phantom-free path to $V_{\tau_P}$. The rest are identical to the first two cases of (1).
% %	 	\item \textbf{If any of $(i,j)$, $(i',j')$ is dangling:}
% %	 	 
% %	 	We case on whether they are connected to the separator before the merge despite dangling. \begin{itemize}
% %	 		\item If they are both connected to the separator, we first observe that each component has one multiplicity of phantom edge assigned to carry their corresponding log factor before the merge.   
% %	 	\end{itemize}
% %
% %\end{enumerate}		
% %\subsubsection{Charging the factor of $n$}
% %	
% %	
% %	\begin{lemma}
% %		\[ |E(\gam\circ\tau\circ\gam')\setminus \exc|-|E(S)|-|V(\tau_P)\setminus V(S)|-|I(\psi)|-\theta(\psi)\geq 0 \numberthis \label{eq:int-trade-off-n} \] 
% %	\end{lemma} 
% %	\begin{proof}
% %	Consider the following charging scheme,
% %		\begin{enumerate}
% %			\item For each edge in $E(S)$ and $\theta(\psi)$: it contributes an $1$ via $|E(\gam\circ\tau\circ\gam'^T)|$ and an $-1$ via $|E(S)|$ or $\theta(\psi)$, giving a balance of $0$;
% %			\item For each vertex in $V_{\tau_P}\setminus S$, we need to assign an edge in $E(\gam\circ\tau\circ\gamma')\setminus\exc$ to it: for vertices inside components connected to $S$, we can consider a BFS from $S$ to traverse the vertices outside the separator and charge each vertex to the edge leading to it. The paths are $\exc$-free by construction of our edge-reservation.
% %			\jnote{the rest is identical to ind-set....i'm curious if non-dangling would buy us more, though that seems unnecessary at the moment}
% %%			\item  For vertices not in the components connected to $S$, since the shapes with non-$0$ Fourier coefficient are all non-dangling, there is a path in $\tau_P$ from $U_\gamma$ to $V_{\gam'^T}$ that vanishes due to phantom edges. Consider the 
% %		\end{enumerate}
% %	\end{proof}
% %	
% %		Consider the components connected to $S$ in $\tau_P$ and BFS from $S$ in the phantom graph, we can use the paths promised from the previous claims to arrive at vertices in $B(\gam)\cup (U_\gam\cap V_\gam)$ without using any edge in $\left(E(U_\gam)\cup E(V_{\gam'^T})\right)\setminus \left(E(U_\gam\cap V_\gam)\cup E(U_{\gam'^T} \cap V_{\gam'^T})\right)$. We now show the desired logarithmic trade-off between $\exc$ and $E(U_\gam)\setminus E(S)$.
% %		
% %	\begin{claim}
% %		$B(\gam)\cup (U_\gam\cap V_\gam)$ is a left-separator for $\gam$, i.e., $B(\gam)\cup (U_\gam\cap V_\gam)$ separates $\int(\gam)\cup U_\gamma$ from $V_\gam$.
% %	\end{claim}
% %	\begin{proof}
% %	By construction, any path from $V_\gam\setminus U_\gamma$ would be blocked by condition-3 vertex in $B(\gam)$, and any vertex intersected is included in $B(\gam)$ by condition-1. 
% %	\end{proof}
% %	Now, if we add the edges (as well as the incidental vertices) of $E(U_\gam)\setminus E(S)$ into $B(\gam)\cup (U_\gam\cap V_\gam)$
% %	, since $(U_\gam, E(U_\gam))$ is the SMVS, we expect a change of $\sqrt{\frac{n}{d}}^{e}\sqrt{n}^{-v}\gg 1$, and noting $e-v=|\exc|$ gives us the desired \[ 
% %	\exc(E(U_\gam)\setminus E(S)) \geq  \frac{|E(U_\gamma)\setminus E(S)|}{\log_d n}
% %	\] 
% %	Repeating the same argument with $\gam'^T$ gives us \[
% %	\exc(E(V_{\gam'^T})\setminus E(S)) \geq  \frac{|E(V_\gamma'^T)\setminus E(S)|}{\log_d n}
% %	\]
% %	Taking the average gives us \[ 
% %	\exc\geq \frac{|E(U_\gam)\setminus E(S)|+|E(V_{\gam'^T}\setminus E(S)|}{2\log_d n}
% %	\]
% %    %   
% %   We first observe in the phantom graph $\tau_P$, each vertex in $B(\gam)$ has a path (potentially of length-$0$) to $V_{\gam'}$ without using any edge in $E(U_\gam)\cup E(V_{\gam'})$. To see this, \begin{enumerate}
% %   	\item For $v\in B(\gam)$ connected to $V_\gam=U_\tau$ without using any edge in $E(U_\gam)$, it has a path in $\tau_P$ to $V_\gam$ as each vertex in $U_\tau$ is connected to $V_\tau$ by middle shape property, and each vertex in $V_\tau$ is connected to $V_{\gam'}$ without using edges in $E(V_{\gam'})$ by left/right shape property. Moreover, the path does not use any edge in $E(U_\gam)$ by construction. 
% %   	\item For $v\in B(\gam)$ that is to-be-intersected,
% %   	\begin{itemize}
% %   		\item  if it intersects with some vertex $v\in V(\tau)$, any vertex in $V(\tau)$ is connected to $V_\tau$ by non-dangling property of the middle shape, and again, by left/right shape property, $V_\tau$ has a path to $V_\gam'$;
% %   		\item if it intersects with some vertex in $V(\gam')\setminus V_\gam'$, it has a path to $V_\gam'$ by left/right shape property; if it intersects with with a vertex in $V_\gam'$, the vertex itself witnesses a path as desired.
% %   	\end{itemize}   
% %   \end{enumerate} 
% %   %   
% %   
% %   \begin{proof}
% % 
% %   	Noticing \[ 
% %   |E(U_\gamma)\cup E(V_\gam)| \geq \frac{|E(U_\gam)|+|E(V_\gam)|}{2}
% %   	\]
% %   	as  each edge in $E(U_\gamma)\cup E(V_\gamma)$ contributes at most an $1$ to the RHS, i.e., when an edge is in the intersection of $E(U_\gamma)\cap E(V_\gamma)$, it suffices for us to show \[ 
% %   \theta(\tau_P) + |E(S)| \geq |E(U_\gam)\cup E(V_\gam)| + \dang
% %   	\]
% %   \end{proof}
% %   To see this, we need the following claim,
% %   \begin{proposition}
% %   For a given shape $\al$, let $S(\al)$ be the corresponding SMVS,
% %   	any wedge around $U_\al$ and $V_\al$ is part of the SMVS, i.e., any edge on the wedge is a separator edge.
% %   \end{proposition}
% %   \begin{proof}
% %   	Assume for the sake of contradiction, that $S$ is the SMVS of $\al$, and there is some vertex $v$ that is on a (short) wedge around $U_\al$ while $v\notin S$, i.e., if  
% %   \end{proof}
% %   
% %   
% %   \begin{proof}[Sketch]
% %   	Each vertex dangling should be charged to an edge that disappears, and it suffices to consider $\frac{|E(U_\gam)|+|E(V_\gam)|}{2}$. For each edge in $E(U_\gam)\cup E(V_\gam)$, it contributes at most $1$ to RHS, and hence it remains to show that it is inside the new SMVS, or it disappears from the linearization. Suppose the edge does not vanish from linearization, we notice it must be on a path from some vertex in $V_\gam$ or even in $V(\tau)$ that leads to an intersected vertex, and we now claim that the upcoming intersection will form a short cycle or wedge-shape walk in $\tau_P$, which would put the edge into the new SMVS. To see this, it suffices to see the vertex being intersected must be connected to either some vertex in $V_\tau$, and we either violate the matching property (by not putting the entire path into SMVS) or we form a short cycle on the same matching path. 
% %   \end{proof}
% %   \subsubsection{Intersection Tradeoff}
% % 	\begin{definition}
% % 		Let $\calM$ be the set of shapes that can appear as the linearization of some $(\gam,\tau,\gam')$ intersection for $\tau\in \calM$ or $\tau\in \midshape$.
% % 	\end{definition}
% % 	\begin{proposition} \label{prop: midshape-connection}
% % 		Given $\tau\in \calM$, any vertex in $U_\tau$ is connected to some vertex in $V_\tau$ and vice versa; any vertex in $V(\tau)\setminus (U_\tau\cup V_\tau)$ is non-dangling.
% % 	\end{proposition}
% % 	We will first restrict our attention to the factor of $n$ in Equation \ref{eq:tradeoff-n}. Noticing each vaporized edge can be charged to an edge with multiplicity $1$ in $E(\gam\circ\tau\circ\gam')$, and let $\phantom$ be the set of edges that vanish under linearization and note that each of them comes with multiplicity at least $2$ in the $E(\gam\circ\tau\gam')$ for vanishing to be possible, we have \[ 
% % 	E(\gamma\circ\tau\circ\gam') \geq E(\psi)+\theta_\psi(\tau_P) + 2\cdot \phantom
% % 	\]
% % 	Rearrange, our goal for the factor of $n$ now becomes
% % 	\begin{lemma}[Intersection-trade-off Lemma] \label{lem:int-trade-off}
% % 		For any intersectable pair $\gam,\tau,\gam'$ for $\tau\in \calM$ that intersects to be $\tau_P$, let $\psi$ be any linearization of $\tau_P$, and $S$ the separator of $\psi$, let $I(\psi)$ be the number of isolated vertices outside $U_{\tau_P}\cup V_{\tau_P}$ under $\psi$,
% % 		\[ 
% % 		E(\psi) + 2\cdot \phantom - E(S) \geq V(\tau_P) - V(S)+I(\psi) +\exc(\psi, S)
% % 		\]
% % 		 where $\exc(\psi,S)\subseteq E(\beta)\setminus E(S) $ is the set of edges in $E(\psi)\setminus E(S)$ that is not on the shortest path from either endpoint to $S$.
		   
% % 		 Moreover, the inequality only holds tight as equality if $I(\psi)=0$.
% % 	\end{lemma}
% % 	\begin{lemma}\label{lem: old-int-tradeoff} [Cite]
% % 		For any linearization $\beta$ of $\tau_P$, and for all separators $S$ of $\beta$, s.t. any isolated vertex in $I(\beta)$ is connected to $S$ in $\tau_P$, \[
% % 		|E(\beta)|+2\cdot \phantom - |E(S)|\geq |V(\tau_P)|+|I_\beta|-|S|
% %  		 \]
% %  		 In particular,
% %  		 \[
% %  		 |E(\beta)|+2\cdot \phantom -|E(S)|-V(\tau_P)-|I_\beta|+|S| = \exc(\beta, S)
% %  		  \]
% % 	\end{lemma}
% % 	\begin{proof}[Proof to Lemma \ref{lem:int-trade-off}]
% % 	 The first part of Lemma \ref{lem:int-trade-off} follows immediately from Lemma \ref{lem: old-int-tradeoff} from previous work, whose proof we defer to the appendix for completeness. And it suffices for us to prove the moreover part which is a strengthening that imposes the condition of equality only when $ I(\psi)$ is empty, and this is made possible via the structure property of our left/right intersection shape, captured by the following proposition,

% % 		\begin{proposition}
% % 			For any linearization $\psi$ of $\tau_P$, any vertex isolated  under $\psi$ has at least $2$ distinct neighbors in $\tau_P$, i.e., it has to be incident to at least $2$ pairs of distinct phantom edges in $\tau_P$.
% % 				\end{proposition}
% % 				\begin{proof}
% % 					Each vertex that can be potentially isolated has to appear in $V(\gam)\setminus U_\gam$ (or respectively $V(\gam')\setminus V_{\gamma'}$).  For vertex $v\in V(\gam)\setminus (U_{\gam}\cup V_\gamma)$, $v$ must have degree at least $2$ in $\gam$ from the non-dangling property. On the other hand, for $v\in V_\gam\setminus U_\gamma$, $v$ also has at least degree-$2$  in $\gamma$ as otherwise let $u$ be the other endpoint of the edge incident to $v$, it either is in $V_\gamma$ in which case removing $v$ increases the SMVS value by $\sqrt{n}(\sqrt{\frac{n}{d}})^{-1}>1$, or we can swap out $v$ by $u$ and obtain a separator of the same SMVS value, violating uniqueness of SMVS for left shape. 
% % 				\end{proof}
% % 			With this proposition in hand, for each component of isolated vertices (isolated in $\psi$) connected by phantom edges in $\tau_P$, since each isolated vertex is adjacent to at least $2$ distinct phantom edges (eg., a wedge of isolated vertices connected by phantom edges to $S$ in $\tau_P$), we can reserve one pair of phantom edge while still preserves the connectivity of the component of isolated vertices to $S$ in the phantom graph, and then applying Lemma \ref{lem: old-int-tradeoff} gives us the desired.		
% % 		\end{proof}
% %	The strengthening condition of equality essentially allows us to transfer the connectivity of vertices using edges in $\tau_P$ to connectivity using edges in $\psi$ where we recall $\psi$ can be any potential linearization of $\tau_P$, unless $\psi$ incurs a loss of factor in $[n]$ from the linearization, which overwhelms the balance of factors in $[d]$ (assuming we can charge the edges where we let go the control of $d$ factor properly). 
% %	\begin{corollary}
% %		Unless there is factor $n$ decay from the linearization of $\psi$, any pair of vertices connected in $\tau_P$ remain connected in $\psi$. 
% %	\end{corollary}
% %	\begin{proof}
% %		We notice only phantom edges vanishing from linearization might affect the connectivity of vertices. Again, ordering the vertices according to their shortest path distance to $S$ and charge the vertex factor to the edge leading to that vertex, if the phantom edges vanish and do not produce isolated vertices, it contributes a $2$ to the LHS while a $1$ on the RHS via $V(\tau_P)$, which is automatically a gap; however, if it produces an isolated vertex, using our global charging argument above, any connected component of isolated vertices produces a gap in $n$ and this proves our corollary.
% %	\end{proof}
% %%	We call a linearization maximal if it does not produce any gap in the factor of $n$.
% %	Starting from this point, we  transfer the excess-edge factor in $n$ to a factor in $d$ for the second part of our analysis,
% %	\begin{lemma}
% %		Fix $\tau\in \calM$ (that is possibly some linearization of intersected shape) with $S\coloneqq  S(\tau)$ being the SMVS for $\tau$, consider $\gamma,\tau,\gamma'$ an intersectable pair that intersect to some $\tau_P$ with linearization $\psi$, and let $\psi$ be a maximal linearization,  let $\widetilde{S}$ be the SMVS for $\tau_P$, \[ 
% %		E(\widetilde{S}) - E(S)+\theta_{\psi}(\tau_P) +\log_d n(\exc (\psi, \widetilde{S})- \exc(\tau, S))  \geq \frac{|E(U_\gam)\setminus E(V_\gamma)| + |E(V_{\gam'})\setminus E(U_{\gam'})| }{2} 
% %		\]
% %	\end{lemma}
% %	\begin{proof}
% %	We now introduce wedge which would be the main object in our analysis here.
% %		\begin{definition}[(Binary) Wedge]
% %		We call $\calW\subseteq E(\psi)$, potentially an edge $(i,j)$, or a path from $(i,j)$ (in which we allow a cycle if $i,j$ collide) a wedge if there is $\calW$-free path from $i$ to $U_\gamma$, and $i$ to $V_{\gamma'}$ without using edges in $\calW$, and there is also a $\calW$-free path from $j$ to $U_\gam$, and $j$ to $V_{\gam'}$. 
% %		\end{definition}
% %		More generally, a wedge can be a subset of connected edges not just with $2$ endpoints.
% %		\begin{definition}[Wedge]
% %			Given a shape $\tau$, We call $\calW \subseteq E(\tau)$ a wedge if each of its degree-$1$ vertex has a $\calW$-free path to $U_\tau$, and to $V_{\tau}$, or every vertex of degree at least $2$ has a path to $U_\tau$ and to $V_{\tau}$.
% %		\end{definition}
% %		\begin{observation}
% %			Let $S$ be the SMVS, then any edge in $E(S)$ is part of a wedge. In particular, this is a wedge with endpoints being $S_L$ and $S_R$, the vertices in $S$ reachable from $U_\al$ and $V_\al$ without passing through $E(S)$.
% %%			Furthermore, we can decompose $E(S)$ into wedges according to 
% %		\end{observation}
% %		\begin{proposition}
% %			Let $\calW$ be a wedge in $E(S)$, unless it vaporizes (as an entire set), it is also a wedge in $\psi$ after intersection.
% %		\end{proposition}
% %		\begin{proof}
% %			This follows by transferring the connectivity in $\tau_P$ and $\psi$. Let $i$ be any deg-1 endpoint of $\calW$, $i$ must have a $\calW$-free path to $U_\tau$ (and then to $U_\gam$), and similarly a $\calW$-free path to $V_\tau$ (and then to $V_{\gam'}$) in $\tau_P$. The similar argument applies to other deg-1 and higher degree endpoints, and by transferal of connectivity, this is a wedge for $\psi$.     
% %		\end{proof}
% %%		The definition of wedge now allows us to formally identify a subset of edges in $\tau$ for excess edges $\exc(\tau, S)$ (and respectively $(\psi, \tilde{S})$. 
% %	Recall that each excess edge that leads to visited vertex when we consider a BFS process from $S$ in $\tau_P$ gives an extra decay, following this definition, we observe that an excess edge is part of some wedge not contained in the SMVS. 	\begin{definition}[Excess wedge]
% %		Given a shape $\tau$, and $S$ its separator with $\exc(\tau,S)$ the corresponding excess vertices, let the excess wedge be the wedge $\text{exc-wedge}=\calW \subseteq E(\tau)\setminus E(S))$ that contains the all the $\exc(\tau,S)$ edges.
% %	\end{definition}		
% %		Each excess wedge can be obtained by BFS on the boundary of $S$ until all the excess edges are visited. And it is immediate from this process that we have a lower bound of the size of the wedge when $S$ is the SMVS, as otherwise the wedge would be merged into SMVS potentially increasing the SMVS value \[ 
% %		|\exwedge |>\frac{|\exc(\tau,S)|}{\log_d n}
% %		\]
% %		Let's now unpack the LHS and describe our charging strategy, \begin{enumerate}
% %			\item For each edge in $E(S)$, unless it vaporizes, 
% %			it is part of a wedge in $\psi$ hence it either contributes to $E(\widetilde{S})$ or contributes to the excess term;
% %			\item For each excess edge, we consider their corresponding excess wedge, which is again a wedge in $\psi$; hence it either contributes at least $\log n$ edges to the LHS via $E(\tilde{S})$, or a factor of $1$ through $\exc(\psi,\tilde{S})$;
% %			\item For each edge in $E(U_\gam)\setminus E(V_\gam)$ (and respectively $E(V_\gam')\setminus E(U_\gam')$), we will show it either vaporizes or forms a wedge.		\end{enumerate}
% %			
% %		 For each edge in $E(U_\gamma)\setminus E(V_\gamma) $, we claim that it either forms a wedge (i.e., connecting 2 vertex disjoint paths from $U_\gamma$ to $V_{\gam'}$, or it forms a cycle around $U_\gamma$ which is again connected to $V_{\gam'}$ in $\psi$), unless it gets vaporized; therefore, for any separator $S$ of $\psi$, the chunk is either included into the $S$ or it witnesses an excess edge that comes with an uncharged $\edgeco$ in $\exc(\psi, S)$. For this idea to go through, we emphasize that it is necessary that both ends of the chunk is connected to $V_{\gam'}$ in $\psi$ as opposed to $\tau_P$. That being said, it suffices for us to consider connectivity in $\tau_P$ as our previous intersection tradeoff ''essentially'' allows us to transfer the connectivity in both graphs. 
% %
% %%		  We will defer the proof of this to the following proposition, but we can see first how this proposition implies the desired inequality. If an edge from $E(U_\gamma)\setminus E(V_\gamma)$ vaporizes, then it contributes at most an $1$ to the RHS, and it also contributes an $1$ to the LHS via the vapor coefficient $\theta_{\alpha}(\tau_P)$.
% %		
% %By Proposition \ref{prop: midshape-connection}, $\gamma$ is a tree rooted at $v_\gamma \cup \{v:v\in \int(\gam)\cup U_\gam\setminus V_\gamma \}$ (where $v_\gam$ is the jumbo vertex that merges $V_\gam$, and $\{v:v\in \int(\gam)\cup U_\gam\setminus V_\gamma \}$ the set of edges between isolated vertices in $U_\gam$ not connected to $V_\gam$) in the auxiliary graph $G[\gam]$ (modulo edges that can be ignored using long-path decay), and we can classify edges of $E(U_\gam)\setminus E(V_\gamma)$ according to the intersected vertex it leads to once we start a BFS from the root $v_\gam$ (and later on $\{v:v\in \int(\gam)\cup U_\gam\setminus V_\gamma \}$). This allows us to decompose the paths from $G[\gam]$ of edges  $E(U_\gamma)\setminus E(V_\gamma)$ into (directed) chunks of edges \[ 
% %	E(U_\gamma)\setminus E(V_\gamma) = \bigcup \{\text{chunk}(i,j)\}_{i,j\in V(\gam)}
% %	\]
% %	Furthermore, notice each consecutive edge on the same path rooted at $V_\gamma$ 
% %	falls into the same chunk as the last edge unless there is a new intersection; hence, for each endpoint of the chunks, we have $i=v_\gamma\cup \int(\gam)$ and $j\in \int(\gam)$ where we recall $\int(\gamma)$ is the set of to-be-intersected vertices. With these notations at hand, we are now ready to prepare a couple of claims about connectivity of vertices in $U_\gamma$.
% %	
% %
% %	\begin{claim}\label{claim: chunk-connectivity}
% %		For each $\text{chunk}(i,j)$, $i$ is connected to $V_\tau$ in $\psi(\tau_P)$ (and hence to $V_{\gam'}$) without passing through the edges in this chunk.
% %	\end{claim}	
% %	\begin{proof} We start by considering edges in $E(U_\gam)\setminus E(V_\gamma)$ connected to $v_\gam$ in $G[\gam]$, and we prove this inductively on $i$. This is immediate when $i=v_\gamma$ as every vertex in $U_\tau=V_\gam$ is connected to $U_{\gam'}=V_\tau$. It now suffices for us to show $j$ is connected to $V_{\gam'}$ without using edges starting from $j$ in $\psi(\tau_P)$, and moreover, the upcoming intersection does not break the connectivity of $i$ to $V_{\gam'}$. 
% %	
% %	 Assuming the edge(s) in $\chunk(i,j)$ are not vaporized, then $j$ the to-be-intersected vertex is also connected to $V_\tau$, as there is a path from $j$ to $i$, and $i$ is connected to $U_\tau$. However, if the edge in $\chunk(i,j)$ is vaporized, we notice it either gets linearized to a mul-1 edge (from the vaporization) in $\psi(\tau_P)$, or it produces a $\sqrt{\frac{d}{n}}$ gap. This is captured in the following claim
% %	\begin{claim}
% %		For $i\in U_\gamma$ connected to $V_\gam'$, and edge $(i,j)$ vanishes in the linearization from intersection, the vaporization can produce at most $1$ isolated vertex; as a result, any multiedge in $U_{\tau_P}$ vaporizes to a mul-1 edge in the maximal linearization.
% %	\end{claim}
% %	\begin{proof}
% %	We discuss by cases. If the vaporization breaks the path from $i$ to $V_\gam'$ (i.e., $j$ is on that path), then $j$ still connected to $V_\gam'$ without using the edge involved in the vaporization. On the other hand, $i$ is still connected to $V_{\gam'}$, and the claim is immediate.
% %
% %	Recall that each isolated vertex in $U_\gam$ does not produce any extra factor in the norm bound and a phantom edge can only vanish if it starts with multiplicity at least $2$, we can charge the isolated vertex's $\sqrt{n}$ factor to the coefficient of $\edgeco$ that comes with one multiplicity of the phantom edge, while the other multiplicity's coefficient leaves uncharged, creating a gap of $\edgeco $. Hence, we conclude in the maximal linearization, each multiedge in $U_\gam$ vaporizes to mul-1 edge.
% %	\end{proof}
% %	Now we return to the main claim showing connectivity of $j$. By our inductive hypothesis, $i$ is connected to $V_\tau$, if the vaporization breaks the path from $i$ to $U_\tau$ and linearizes to a mul-$1$ edge, $j$ is on that particular path and hence still connected to $V_\tau$, and $i$ is still connected using the mul-$1$ edge after vaporization; suppose the vaporization breaks some other path, $j$ is connected to $i$ via the mul-1 edge from vaporization, and again $i$ is connected to $V_{\tau}$ and ultimately $V_{\gam'}$.
% %		
% %	On the other hand, for chunks of edges from each connected component in $E(U_\gamma)\setminus E(V_\gamma)$ not connected to $G[\gam]$, it is possible that $i$ is not $v_\gamma$, nor an intersected vertex explored by previous edges in $E(U_\gamma)\setminus E(V_\gamma)$. However, since the vertex is intersected, its intersection copy (either coming from $V(\tau)\setminus U_\tau$ or $V(\gamma)$) is connected to $V_{\gam'}$), and the previous induction now follows in the new connected component.
% %	\end{proof}
% %	
% %	\begin{proposition}
% %		[Isolated vertex comes with extra $\sqrt{\frac{d}{n}}$ decay] Each connected component (in $\tau_P$) of isolated vertices of size $v$ is incident to at least $2(v+1)$ phantom edges unless the connected component is contained inside $U_\gam$ or $V_{\gam'}$. 
% %		
% %		Let $I(\psi)$ be the set of isolated vertices under the linearization $\psi$,  and let $E(I(\psi))$ be the number (counting multipliicty) of edges in $\tau_P$ that are incident to any isolated vertex, and let $I_\text{boundary}(\psi)\subseteq U_{\tau_P}\cup V_{\tau_P}$ be the set of isolated vertices in $U_{\tau_P}\cup V_{\tau_P}$ that are isolated under $\psi$, then 
% %		\[ 
% %		I(\psi) \leq  2E(I(\psi)) - \min(2,I_{\boundary}(\psi)) 
% %		\]
% %	\[I(\psi) + E(\gam\circ\tau\circ\gam')  \]
% %	\end{proposition}
% %	\begin{proof}
% %		Note that each connected component of isolated vertex is reachable from $U_\tau$ in the phantom graph $\tau_P$, and we now process isolated vertices from their distance to $U_\tau$. For each isolated vertex, there must be at least two phantom edges that vanish from linearization, and we can charge the edges leading to the intersected vertex to isolated vertex it leads to, except when the vertex $v$ being isolated is already in $U_\tau$ that we will handle in the latter part. However, each edge leading to isolated vertex is also an edge in $U_\gam$, and by left-shape property, each edge is on some path to an intersected vertex from $V_\gamma$ to $\int(\gam)\subseteq U_\gamma$; 
% %		
% %		
% %		 To see the $+1$, we case on whether the first intersected vertex being traversed is in $U_\tau\cap U_\gamma$, if not, then we notice the last vertex traversed in the component, must be incident to some vertex non-isolated, or the last vertex being traversed is in $U_\gamma$ since each edge in $E(\gam)$ is on some path to $U_\gam$ from $V_\gam$.  
% %	
% %	\end{proof}
% %	We now introduce the proposition that would be the backbone of our intersection trade-off.
% %
% %	\begin{proposition}
% %		Each edge $e=(i,j)$ in $E(U_\gamma)\setminus E(V_\gam)$ is either vaporized, or forms a wedge/cycle around a path from $U_\gamma$ to $V_\gam'$ in $\psi(\tau_P)$: concretely, there is a path from $j$ to $V_{\gam'}$ that does not use $e$, and there is a path from $i$ to $V_{\gam'}$ that does not use $e$ in $\psi(\tau_P)$.
% %	\end{proposition}  
% %	
% %	\begin{proof}
% %	We continue working with our decomposition of edges in $E(U_\gamma)\setminus E(V_\gam')$ into chunks. For $\chunk(i,j)$, by Claim \ref{claim: chunk-connectivity}, there is a path from $i$ to $V_\tau$ (and to $V_{\gam'}$) without using $\chunk(i,j)$. Let $\int(j)$ be the vertex that intersects with $j$ from $V(\tau)\setminus U_\tau$ or $V(\gam)\setminus U_\tau$.
% %	Since we know $\chunk(i,j)$ does not vaporize in $\psi(\tau_P)$, we can discuss by cases whether $j$ collides with a vertex on any path from $i$ to $V_\tau$. If so, we can consider there is a path from $i$ to $\int(j)$ which is the vertex intersected with $j$ on the path from $i$ to $V_\tau$, in which case the path from $i$ to $\int(j)$, and to $V_{\gam'}$ does not use $\chunk(i,j)$, while $j=\int(j)$ also has a path that does not use $\chunk(i,j)$; on the other hand, $j=\int(j)$ is connected to $V_\gam'$ as $\int(j)$ is either from $V(\tau)$ or $V(\gam')$, both of which connected to $V_{\gam'}$ in $\psi(\tau_P)$, and the proposition follows.  
% %		\end{proof}
% %
% %	\end{proof}

 \subsection{Bounding intersection count}
 Analogous to our charging in the base level for middle shapes, as we have shown each single intersection term can be bounded, we may now complete the proof by bounding the count. That said, we first notice that each intersection term can be specified as the following.

 
%  \begin{lemma}
%  	Let $\exc(\tau_P)$ be the number of excess edges in $\tau_P$ where we recall $\tau_P$ is the graph potentially with multiedges, we can bound the number of  intersection patterns  by \[ 
%  	(c_\int)^{E(\tau_P)} \cdot (2|V(\tau_P)|q_{\tau_P})^{\exc(\tau_P)} 
%  	\]
%  \end{lemma}
%  %Idea: it is not sufficient to simply consider non-equivalent intersection patterns as we may have non-equivalent patterns that correspond to the same intersected shape $\tau_P$ with the same coefficient. The confusion comes in specifying $\dsos$ levels some ''dormant'' vertex if we start from $\tau$ and go outwards to $\gam_k, \gp_k$, but the choice of $\dsos$ levels comes with $-1$ so they can be grouped to get a count of $1$ as opposed to $\dsos$ from the number of choices of picking the levels.

%  Overall idea:
%  \begin{enumerate}	\item The idea is to specify for each edge where which $\dsos$ level it comes from, while only using a constant per edge;
%  	\item The primitive we can use is to keep a counter indicating which $\dsos$ level are we on currently at the vertex, and then for the next edge, we can simply go $+1/0/-1$ indicating whether we change the $\dsos$ level;
%  	\item Unless truly necessary, i.e., we are seeing cycle in $\tau_P$, a label in $2|V(\al)|q$ is not needed in the above argument;
% % %	\item There is a way to traverse non-squeezable intersection tuple s.t. each edge is traversed in adjacent $\dsos$ level.
%  	\end{enumerate}
 \paragraph{Identifying what to bound}
 \begin{definition}[Intersection-pattern]
 	We call a tuple $\left(\gam_t,\dots, \gam_1, \tau, \gp_1, \dots,\gp, P_\int \right)$ an intersection pattern such that  
 	\begin{enumerate}
 		\item $P_\int$ specifies which vertices get intersected and how they are intersected, and let $P_{\int,L,R}$ be $P_\int$ restricted to the first $(L,R)$-levels $\gam_L,\dots,\gam_1,\tau,\gp_1,\dots,\gp_R$.
 		\item For any $\ell,r  \in \N$, $\bigg(\gam_\ell, \left(\gam_{\ell-1},\dots,\gam_1,\tau, \gp_1, \dots, \gp_{r-1}\right), \gam_r\bigg)$ is a intersection-tuple with $P_{\ell, r}$;
 			\item Additionally, call $\depth(P_\int)= l$ the intersection-depth of the corresponding pattern;
		\item For technical reasons, we allow $\gam_i = \gam_{i-1}$ or $\gp_i=\gp_{i-1}$ for $i>1$ to represent the case when there is no \emph{new} left/right intersection. However, both cannot hold at the same time.
  	\end{enumerate}
 	\end{definition}

 \begin{definition}[Intersection shape $\tau_P$]
     We call a shape an intersection shape if it it a shape that can be obtained by ribbon intersections of at most $\dsos$ levels.
 \end{definition}
To bound the count of intersection terms, we first observe that $\tau_P$ when viewed as shape can be counted in the identical way as for middle shape, with the only difference being for a fixed shape, there may be various ways of ribbon interesctions (intersection patterns) that obtain the same underlying multi-graph as a shape. That said, to the number of intersection patterns for a fixed shape, it suffices for us to identify a $\dsos$ label for each edge specifying which level the edge comes from (i.e. the depth of $\gamma_i$ where the edge is from).

As a result, given the final shape $\tau_P$ viewed as a multi-graph with information of where each edge comes from, the intersection pattern is immediately fixed as one may \begin{enumerate}
    \item Draw out each $\gamma_i, \gamma_i'^T$for each $i\in [\dsos]$ and $\tau$ (the base-level) according to the depth-information from each edge;
    \item The vertex intersection, i.e. which vertex colliding with each other, is also fixed as the final shape of $\tau_P$ is also given.
\end{enumerate}

\begin{proposition}\label{prop:int-count}
    Given a shape $\tau_P$, the number of intersection levels can be identified at a cost of \[ 
    c_{int}^{|V(\tau_P)\setminus U_{\tau_P}\cap V_{\tau_P}|}  \cdot \dsos^{|V(\tau_P)|}
    \]
    for some absolute constant $c_{int}$ where we remind the reader that $|V(\tau_P)|$ counts multiplicity of intersected vertices.
\end{proposition}
\begin{proof}
    We apply this bound alongside our norm bound for grouped matrix. In addition to the block-value bound for middle shape, it suffices for us to go through the shape in an extra pass and identify where each edge comes from (i.e., identifying the particular intersection pattern).

   First, identify a level of $[\dsos]$ for each vertex-multiplicity identifying which $\dsos$ level it appears, and this is subsumed by the extra decay factor of $ \frac{1}{\dsos}$ from our coefficient; once all the $\dsos$ levels are identified, we appeal to the following structural left/right-intersection shape property: each $\gamma$-shape is $U$-wedge.
   
   That said, once $\tau_P$ is identified as an edge-set in the trace-method calculation alongside the $[\dsos]$ label for each vertex-multiplicity we are provided now, it suffices for us to apply wedge-bundling idea for each $\gamma_i, \gamma_i^T$ level recursively from outermost level to the base level of $\tau$, and applying \cref{lem: bundling_cost}, this is a single constant per vertex and this completes our bound.
\end{proof}



\subsection{Wrapping up intersection shape bound}
\begin{proof}[Proof to Lemma~\ref{lemma:intmain}]
    This section is in parallel with the summary for middle shape bound. Notice that for a single active-profile $\calP$, apply our graph matrix bound on
\begin{align*}
	\lambda_{\cal_P} \calM_{\calP} \coloneqq  \sum_{\substack{\tau_P: \text{intersection shapes with active profile} \calP  \\ \text{non-trivial, permissible}  \\ E(U_\tau\cap V_\tau)=\emptyset }  } \sum_{\beta:V(\beta)\rightarrow [k]}  \lambda_{\tau_P} \cdot  \cval{E(\tau)}_\beta \cdot  \cm_{\tau_P} \cdot q(\tau) 
	\end{align*}
% where we let $\beta$ be the coloring of any single shape $\tau$, and observe that \begin{align*}
% 	&\sum_{\substack{\tau: \text{middle shapes with active profile} \calP  \\ \text{non-trivial  }  }} \lambda_\tau \sum_{\beta:V(\tau)\rightarrow [k]} \cm_\tau \cval{E(\tau)}_\beta \cdot \\&  = \sum_{\substack{\tau: \text{middle shapes with active profile} \calP  \\ \text{non-trivial, permissible} \\  E(U_\tau\cap V_\tau)=\emptyset  }  } \sum_{\beta:V(\beta)\rightarrow [k]}  \lambda_\tau \cdot  \cval{E(\tau)}_\beta \cdot  \cm_\tau \cdot q(\tau) 
% \end{align*}
Applying our ''grouped'' norm bound on $\lambda_{\calP} \cm_{\calP}$ for active-profile $\calP$  while now $\calP$ is the collection of intersection shapes $\tau_P$ gives us \begin{align*}
	\|\lambda_{\calP} \calM_{\calP}\|&\leq \max_{\tau\in \tau_P(\calP) \text{non-trivial, permissible} } \|  \lambda_{\tau_P}  \cdot \cm_{\tau_P} \cdot q(\tau)  \sum_{\beta:V(\beta)\rightarrow [k]}  \cval{E(\tau)}_\beta \| \\
	&\leq \max_{\tau_P\in \tau_P(\calP) \text{non-trivial, permissible} } \|  \lambda_{\tau_P}  \cdot \cm_{\tau_P}\| \cdot |q(\tau_P)| \cdot  |\sum_{\beta:V(\beta)\rightarrow [k]}  \cval{E(\tau_P)}_\beta | 
\end{align*}

We now mimic our charging strategy for middle shapes , and we note that the factor other than $\dsos$ dependence follows from the charging for a single intersection shape in Lemma~\cref{lemma:charging-single-intersection}, and we make clear the $\dsos$ dependence here as,\begin{enumerate}
    
	\item Assuming $\frac{1}{k} = O(\frac{1}{c_\eta \sqrt{d}\cdot \dsos^4 })$, we first consider the following $\dsos$ dependence that inheir from that of middle shapes.;
	\item Each vertex outside $U_\tau\cup V_\tau$ contributes a single factor of $\dsos$ via the blow-up from hidden-edge indicator, while each comes with a full factor of decay $\frac{1}{\dsos^2}$;
	\item Each vertex in $U_\tau \Delta V_\tau$ does not contribute any $\dsos$ factor from hidden-edge indicator, and each comes with a factor of $\frac{1}{\dsos}$ since each comes with half a vertex coefficient;
	\item By our sparsity bound, $|E(S)|\leq 5|V(S)|$, and moreover, notice since we look at permissible shape, there are no edges inside $E(U_\tau\cap V_\tau)$; and the edges between $U_\tau\cap V_\tau$ and $V(\tau)\setminus (U_\tau\cap V_\tau )$ are at most $2\cdot |V(\tau)\setminus (U_\tau\cap V_\tau )|$, and therefore, we have $|E(S)|\leq 7|V(\tau)\setminus U_\tau\cap V_\tau| \leq c^{|V(\tau)\setminus U_\tau\cap V_\tau|}$ for some constant $c$ subsumed by $c_\eta$ factor of vertex-decay;
    \item The difference in comparing to the middle shape charging is that we incur an overhead to identify intersection patterns, and this is a factor of an extra $\dsos$ for each vertex from Proposition~\ref{prop:int-count};
    \item Recall that we have an $\frac{1}{\dsos}$ excess from charging middle shapes, which can now be used to offset the extra $\dsos$ overhead in Rmemark~\ref{remark:extra-gap-from-middle-shape};
	\item Combining the above gives us a factor of $\left(\frac{1}{\dsos}\right)^{|U_\tau\Delta V_\tau|} = \left(\frac{1}{\dsos}\right)^{|U_{active}(\calP) +|V_{active}(\calP)|   }$. 
\end{enumerate}
	Summing over all active-profiles gives us \begin{align*}
		\|\sum_{\calP} \lambda_{\calP}\calM_{\calP} \| \leq \max_{\calP}{ c(\calP)\cdot  \left(\frac{1}{\dsos}\right)^{|U_{active}(\calP) +|V_{active}(\calP)|   } }  \ll \frac{1}{10}
	\end{align*}
	where we recall that the identification cost of $\calP$ is bounded by $\dsos^{|U_{active}(\calP)| + |V_{active}(\calP)| }$.

 
% %\begin{definition}[Squeezing intersection-pattern]
% %For an intersection pattern $\left(\gam_t,\dots, \gam_1, \tau, \gp_1, \dots,\gp, P_\int \right)$, we call any adjacent left/right shapes $\gam_i, \gam_{i-1}$ (or $\gp_i, \gp_{i-1} $) squeezable, 
% %\begin{enumerate}
% %	\item if there is some edge-component in $\gam_i$ that does not have any intersection with $\gam_{i-1}$ specified by $P_\int$;
% %	
% %\end{enumerate}
% % there is no intersection between $\gam$ and $\gam_{i-1}$ as specified in $P_\int$. In other words, there is a single shape $\gam_{\text{squeeze}}$ that can replace $\gam_i, \gam_{i-1}$ altogether in the given intersection pattern and produces an equivalent $\tau_P$.
% %\end{definition}

%  \begin{proposition}
%  Let $i>1$ be an intersection-depth. In the recursive factorization scheme, any edge-component in $\gam_i$ is connected in $\tau_P$ to some edge-component in $\gam_{i-1}$. \end{proposition} 
%  \begin{proof}
%  	Observe that for any component in $\gam_i$ that does not get intersected with $\gam_{i-1}$, putting the entire component in $\gam_{i-1}$ while adjusting the boundary condition appropriately maintains the left/right shape property and they specify the same collection of ribbons.	
%  \end{proof}

%  \begin{definition}[Minimal intersection-pattern] For a fixed $(\gam_\ell, \dots, \gam_1, \tau,\gp_1, \dots, \gp_r)$ and $P_\int$, we call it a minimal intersection-pattern if for $i>1$, \begin{enumerate}
%  	\item For any edge-component in $\gam_i$, it has an intersection with some edge-component in $\gam_{i-1}$;
%  	\item For any edge-component in $\gp_i$, it has an intersection with some edge-component in $\gp_{i-1}$;
%  \end{enumerate}
%  \end{definition}

% % %\begin{proposition}
% % %For a fixed $\tau_P$, let $P(\tau_P)$ be a minimal intersection-pattern, and 
% % %	 \[ 
% % %	\left| \sum_{P\rightarrow P(\tau_P)} (-1)^{\depth(P)} \cdot \lambda_{\gam_l\circ\dots\circ\gam_1\tau\circ\gp_1\circ\dots\circ\gp_r } \right| \cdot  \|M_{\tau_P}\| 	 
% % %	\leq \lambda_{\tau_P}\cdot \|M_{\tau_P}\|
% % %	\] 
% % %\end{proposition}
% % \begin{comment}
%  \subsubsection{Bounding using portal-crossing}
%  We now proceed to describe our encoding scheme. We first observe that for any minimal-intersection- pattern, we can classify intersections in each $\gam_i$ (respectively $\gp_i$) for $i>1$ into two terms,
%  \begin{definition}[Adjacent intersection/portal]
%  	This corresponds to a vertex in $V(\gam_i)\setminus V_{\gam_i}$ that intersects with some vertex in $V(\gam_{i-1})\setminus U_{\gam_{i-1}}$.
%  \end{definition}
%  \begin{definition}[Free intersection/portal]
%  	This corresponds to an intersected vertex that does not appear in $V(\gam_{i-1})\setminus U_{\gam_{i-1}}$.
%  \end{definition}
%  We encourage the reader to think of each intersection as opening up a portal between $\dsos$ levels to visualize our encoding scheme in the following argument. Let's first consider what kind of encoding primatives we may use if our budget is only a constant per edge.
%  \begin{mdframed}[frametitle = {Portal-crossing primatives }]
%  Goal: draw out the shape of $\tau_P$ from $\gam_\ell, \dots,\gam_1,\tau,\gp, \dots,\gam_r$ specified by $P_\int$, and label each edge (up-to its  multiplcities) a label in $\gam_i$ for $i$ some $\dsos$ level, and identify the vertex status of each vertex. 	\begin{enumerate}
%  		\item $F$: open up an \emph{outgoing} new edge at the current level; and correspondingly $R$ close an \emph{incoming} $F$ edge;
%  		\item $S$, i.e., a surprise visit: open up a new edge leading to a visited vertex;
%  		\item Open an \emph{outgoing} adjacent-portal at the current vertex; and correspondingly, return by closing an \emph{incoming} adjacent-portal;
%  		\item Open an \emph{outgoing} free-portal at the current vertex; and correspondingly, return by closing an \emph{incoming} free-portal;
%  		\item Ground: use a constant to specify the current edge is at $\gam$,$\tau$, or $\gp$.
%  		\item A vertex status for each edge indicating the boundary status of its vertices in the current level;
%  	\end{enumerate}
%  \end{mdframed}
%  \begin{remark}
%  	The reader should be cautious that \emph{no} $\dsos$ factor is needed each time a free-portal is created.
%  \end{remark}
%  It would be useful to think of our argument as maintaining a stack of edges, while we do not necessarily know the $\dsos$ level for each edge when it is pushed into the stack, it would be identified by the time it gets popped out. The root of our encoding exploits the following observations, \begin{enumerate}
%  	\item The decoder, guided by the encoder, is traversing (and at the same time, drawing out) $\tau_P$, and their job is to identify which level each edge comes from;
%  t \item The decoder at the moment does \emph{not} necessarily need to know which $\dsos$ level it is at, however, it may still draw out the edge-component of some corresponding $\gam$ shape (which is known to the decoder), despite not knowing the specific $\dsos$ level; 
%  	\item For each edge-component, guaranteed by minimal-intersection-pattern, has an adjacent portal to the next level, which should be seen as making progress as it helps the decoder move towards ground-$0$ whose $\dsos$-level is specified for free;
%  	\item It is important to ensure that each time the decoder traverses back through an adjacent portal, the current $\dsos$ level is identified, and the decoder can then use this information to assign $\dsos$ labels for edges specified previously before opening the adjacent-portal that just get closed upon, and it may additionally encode new edges at the corresponding level;
%  	\item This process ultimately terminates as we may open up a sequence of adjacent-portals that take us to the \emph{ground}, and the edges of each level can then be decided once be backtrack from the ground-levels;
%  	 	\item Opening up a free-portal does not help with identifying $\dsos$-level for edges specified before the free-portal, and similarly, it does not \emph{directly} help the edges of the destination-level either as the current $\dsos$-level remains unknown; however, it allows us to repeat this argument on the destination component of the free-portal, that we are again in a position where the current level is unknown while it can be decoded relying upon an adjacent-portal.\end{enumerate}

%  \begin{remark}
%  	A vertex may have intersections in various $\dsos$ levels, 
%  \end{remark}

%  \begin{mdframed}[frametitle = {Encoding intersection-tuple via portal-crossing }]
%  	\begin{enumerate}
%  		\item Maintain a stack of various layers which is initialized to empty;
%  		\item At the current stack-layer, the decoder first draws out the corresponding edge-component, and along the way, specify each vertex a label with \emph{FP}, \emph{AP} and potentially another label corresponding to phantom-edge bundle distance (which can be handled by edge-decay);
%  		\item The current depth is potentially unknown;
%  		\item The decoder first trigger edge-bundling process to identify potential multi-edge component of edges appearing in the current level, and this groups the FP/AP labels into components;
%  		\item Open each FP/AP, and move to a new stack-layer;
%  		\item The return to current layer via an AP binds a $\dsos$ level to the edge-component of this layer;
%  		\item Exit the layer via the FP/AP that opens the currents layer, and update the depth-pointer for the destination layer if it is an AP.
%  		\end{enumerate}
%  \end{mdframed}
% % \end{comment}

% % \end{comment}


% \subsection{Intersection count}
% \jnote{the previous approach attempts to use edge-decay alone to assign a $\dsos$ label for each edge in $\tau_P$, while reserving the whole $\aut$ factor to the norm bound. It runs into issue with multi-edges and dormant vertices. I think we can modify it such that imagine we are doing a block-step as in trace-method, and we draw out each $\gam$ with vertices labeled in $[n]$ using wedge-bundling, as well as assign an ordering for each vertex in $V(\gam)$. This allows us to touch upon dormant vertex in $U_{\gam_i}\cap V_{\gam,i} $ without paying any extra decay (regardless of whether that vertex has participated in outer intersections earlier). The key is that if we presume each vertex to be a deg-$0$ vertex in $U_\gam\cap V_\gam$, i.e., each vertex presumes to be dormant, we would only need an edge decay to kick a vertex outside that orbit (which activates the wedge-bundling scheme). Otherwise, if a vertex stays dormant, we need to assign a label in $|dormant(U_\gam\cap V_\gam)|$ which is offset by its corresponding factor in $\aut(\gam)$ }

% \jnote{i have a feeling this idea handles really well with multi-edges as well, not just dormant}
% \\
% \jnote{correction updated Mar. 2023: it works well for multi-edges but unfortunately dormant is a big issue}
% We attempt to give a bound for intersection term in this section. Let's start by making clear of our target. Notice for each intersection term $\tau_P$, we pick up a normalizing constant of \[ 
% \prod_{i} \aut(\gamma_i) \cdot \aut(\tau)\cdot \prod_{i} \aut(\gam'^T_j)
% \]
% To identify an intersection term, alongside its intersection pattern, it suffices for us to specify where each edge comes from, and each vertex's possible boundary status in the corresponding shape. We follow our idea of bounding automorphism factor for sparse matrix norm, i.e., draw out the shape and assign an ordering via automorphism to settle any potential confusion, except we upgrade out goal to not only draw out the shape $\tau_P$ from the current $U_{\tau_P}$ (and $V_{\tau_P}$) boundary, but also to assign a label for each edge and vertex to specify the intersection-level it participates, as well as to assign for each vertex an ordering for each intersection level it participates (i.e. each $\gam, \gp$-level) where \begin{center}
%     We call a vertex $v$ participates in level $\gamma_i$ as long as it appears as a vertex in $V(\gamma_i)$, including when it appears as an isolated vertex in $U_{\gamma_i}\cap V_{\gam_i}$.
% \end{center}

% \begin{proposition}
%     For any $\gamma$ shape with vertices given in $U_\gam$ with labels in $[n]$, in the locally optimal walk, we can draw out $\gamma$ shape with an ordering assigned to each vertex in $V(\gam)$ at a cost of at most \[ 
%     2^{|E(\gam)|} \cdot \aut(\gam)
%     \]
% \end{proposition}

\end{proof}

==> kronecker_factorization.tex <==
\section{Factorization of Middle Shapes via Kronecker Product}
Let $\Lambda_{mid}$ be the middle-shape matrix indexed by set. For concreteness, we consider the following index for the the columns/rows of $\Lambda_{mid}$ which view the index as an order-tuple while we fix the ordering to be the ascending order of the  vertices (hence this is equivalent to the set view as each set of vertices appear only once, i.e., as in one fixed ordering).
\begin{definition}[Matrix index for set]
For any subset $S\subseteq \binom{n}{\leq \dsos}$, let $\vec{S}$ be an order-tuple with vertices in $S$ ordered in the ascending order.
\end{definition}
\begin{remark}
For any set $S$, the map $S\rightarrow \vec{S}$ is a bijection.  
\end{remark}
\begin{observation}
Let $\Lambda_{all}$ be the matrix indexed by all possible order-tuples of size at most $\dsos$ in $[n]$, $\Lambda_{mid}$ is a principle submatrix of $\Lambda_{all}$, in particular, it can be obtained from $\Lambda_{all}$ by removing columns/rows of indices that do not follow the ascending order of vertices.
\end{observation}
It suffices for us to work with $\Lambda_{all}$ that agrees with the desired $\Lambda_{mid}$ on the ''right'' entries (i.e., any entry whose row/col indices when viewed as ordered-tuples agree with the fixed ordering), and show $\Lambda_{all} \succeq 0 $. Moreover, since we are working with middle-shape matrix, we have $U_\al =V_\al $ for any shape $\al$ that appears in $\Lambda_{mid}$, and it suffices for us to further exploit the block-structure of $\Lambda$ and consider each individual block as \[ 
\Lambda_{all} = \sum_{s\leq \dsos} \Lambda_{all,s}
\] 
where $\Lambda_{t}$ is the matrix of $\Lambda_{all}$ restricted to the block with $|U_\al|=|V_\al|= s$.

To show $\Lambda_{all,s} \succeq 0$ and that it agrees with $\Lambda_{set, s}$ on the desired entries, we first give an approximate factorization of $\Lambda_{all, s}$ into a kronecker products, as \[ 
\Lambda_{approx, s} = \otimes_{1\leq i \leq s} \left(Id  + \sum_{\al_i: \text{non-dormant middle-shape}} \lambda_{\al_i} \cdot M_{\al_i}\right)
\]
For starters, we will restrict ourselves to middle shapes that are only consist of parallel paths, and ignore middle shapes that may have multiple $U_\al$ verticees in a single connected component at the moment.
\begin{lemma} Let $\Lambda_{approx, set, s}$ be the principle submatrix of $\Lambda_{approx, s}$ restricted to columns/rows that obey the fixed ordering, and let $\Lambda_{mid, s} $ be the middle shape matrix restricted to $s$ block, and consist of either the trivial shape, or parallel paths.
\[
\Lambda_{approx, set, s} =  \Lambda_{mid, s} + intersection
\]
\end{lemma}
\begin{proof}
We now show that any edge-set either appears exactly once on both sides, or it only appears in the $LHS$ and is due to intersection. On the one hand, for any ribbon edge-set $E(\al)\subseteq \binom{n}{2} $ with shape $\al$, 
we would like to show that it appears on the LHS exactly once, in particular, there is a unique path of the kronecker product to produce $E(\al)\subseteq \binom{n}{2} $
\begin{enumerate}
    \item First for a given edge-set $E(\al)$ of shape $\al$ , order its vertices in $U_\al$ and $V_\al$ in the prescribed ascending order;
    \item Traverse the vertices in $U_\al$ following the fixed order, and for the $i$-th kronecker product term, choose the vertex $U_\al[i]$ and then pick out the corresponding term depending on whether the vertex is incident to any path, and what kind of path, in $E(\al)$, this shows there is some path that gives rise to the same $E(\al)$ without any intersection;
    \item To see the uniqueness, if we didn't follow the kronecker-product path prescribed the above, there must be some kroneck-product step $j$ that we get a mismatch: we either pick a different vertex $v_j \neq U_\al[j]$, or the path being prescriebd is different. However, observe that if we pick a vertex $v_j\neq U_\al[j]$ and suppose that the path gives rise to a column index $S'$  that are the same as $U_\al$ up-to-reordering, we claim that corresponds to a column in $\Lambda_{approx, s}$ that gets removed since it does not obey the fixed ordering. On the other hand, if $v=U_\al[j]$ while we pick out differetn edge-set incident to $v$, the edge-set cannot be equal in the end unless there is intersection, hence the claim.
\end{enumerate}
\end{proof}


==> math_commands.tex <==
% %%%%% NEW MATH DEFINITIONS %%%%%

% % Common
% \def \N {\mathbb{N}}
% \def \R {\mathbb{R}}
% \def \C {\mathbb{C}}
% \def \Q {\mathbb{Q}}
% \def \Z {\mathbb{Z}}
% \def \F {\mathbb{F}}
% \def \E {\mathbb{E}}
% \def \PE {\wt{\mathbb{E}}}
% \def \eps {\epsilon}
% \def \al {\alpha}
% \renewcommand{\Pr}{\mathop{\bf Pr\/}}
% \newcommand{\wt}[1]{\widetilde{#1}}
% \newcommand{\wh}[1]{\widehat{#1}}
% \newcommand{\ol}[1]{\overline{#1}}
% \newcommand{\ul}[1]{\underline{#1}}
% \newcommand{\ot}{\otimes}
% \newcommand{\zo}{\{0,1\}}
% \newcommand{\pmo}{\{\pm1\}}
% \newcommand{\Var}{\mathrm{Var}}
% \newcommand{\Cov}{\mathrm{Cov}}
% \newcommand{\imp}{\Longrightarrow}
% \newcommand{\brac}[1]{\left\langle #1 \right\rangle}
% \newcommand{\KL}{d_{\mathrm{KL}}}
% \newcommand{\TV}{d_{\mathrm{TV}}}
% \def\ceil#1{\lceil #1 \rceil}
% \def\floor#1{\lfloor #1 \rfloor}
%  \def\1{\bm{1}}
% \def \st {\text{s.t.}}
% \newcommand{\TODO}[1]{\textcolor{red}{#1}}
% \newcommand{\calF}{\mathcal{F}}
% % mathsf 
% \newcommand{\SA}{\mathsf{SA}}
% \newcommand{\SOS}{\mathsf{SOS}}

% % complexity classes
% \newcommand{\PTIME}{\mathsf{P}}
% \newcommand{\LOGSPACE}{\mathsf{L}}
% \newcommand{\ZPP}{\mathsf{ZPP}}
% \newcommand{\RP}{\mathsf{RP}}
% \newcommand{\BPP}{\mathsf{BPP}}
% \newcommand{\NP}{\mathsf{NP}}
% \newcommand{\coNP}{\mathsf{coNP}}
% \newcommand{\MA}{\mathsf{MA}}
% \newcommand{\PH}{\mathsf{PH}}
% \newcommand{\TC}{\mathsf{TC}}
% \newcommand{\AC}{\mathsf{AC}}
% \newcommand{\SC}{\mathsf{SC}}
% \newcommand{\SZK}{\mathsf{SZK}}
% \newcommand{\AM}{\mathsf{AM}}
% \newcommand{\IP}{\mathsf{IP}}
% \newcommand{\PSPACE}{\mathsf{PSPACE}}
% \newcommand{\EXP}{\mathsf{EXP}}
% \newcommand{\MIP}{\mathsf{MIP}}
% \newcommand{\NEXP}{\mathsf{NEXP}}
% \newcommand{\BQP}{\mathsf{BQP}}
% \newcommand{\PP}{\mathsf{PP}}
% \newcommand{\SP}{\mathsf{\#P}}

% % Environments
% % \renewenvironment{proof}{{\emph{Proof.}  }}{\hfill$\square$ \vspace{8pt}}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{claim}[theorem]{Claim}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{fact}[theorem]{Fact}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{question}[theorem]{Question}
% \newtheorem{answer}[theorem]{Answer}
% \newtheorem{hypothesis}[theorem]{Hypothesis}
% \newtheorem{exercise}[theorem]{Exercise}
% % \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{notation}[theorem]{Notation}
% \newtheorem{observation}[theorem]{Observation}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{examples}[theorem]{Example}

% % Math terms
% \newcommand{\poly}{\operatorname{poly}}
% \newcommand{\polylog}{\operatorname{polylog}}
% \newcommand{\size}{\textnormal{size}}
% \newcommand{\avg}{\mathop{\textnormal{avg}}}
% \newcommand{\sgn}{\textnormal{sgn}}
% \newcommand{\dist}{\textnormal{dist}}
% \newcommand{\vol}{\textnormal{vol}}
% \newcommand{\spn}{\textnormal{span}}
% \newcommand{\supp}{\textnormal{supp}}
% % \newcommand{\tr}{\operatorname{tr}}
% \newcommand{\codim}{\operatorname{codim}}
% \newcommand{\diag}{\operatorname{diag}}
% \newcommand{\conv}{\operatorname{conv}}


% % Mark sections of captions for referring to divisions of figures
% \newcommand{\figleft}{{\em (Left)}}
% \newcommand{\figcenter}{{\em (Center)}}
% \newcommand{\figright}{{\em (Right)}}
% \newcommand{\figtop}{{\em (Top)}}
% \newcommand{\figbottom}{{\em (Bottom)}}
% \newcommand{\captiona}{{\em (a)}}
% \newcommand{\captionb}{{\em (b)}}
% \newcommand{\captionc}{{\em (c)}}
% \newcommand{\captiond}{{\em (d)}}

% % Highlight a newly defined term
% \newcommand{\newterm}[1]{{\bf #1}}


% % Figure reference, lower-case.
% \def\figref#1{figure~\ref{#1}}
% % Figure reference, capital. For start of sentence
% \def\Figref#1{Figure~\ref{#1}}
% \def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
% \def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% % Section reference, lower-case.
% \def\secref#1{section~\ref{#1}}
% % Section reference, capital.
% \def\Secref#1{Section~\ref{#1}}
% % Reference to two sections.
% \def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% % Reference to three sections.
% \def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% % Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% % Reference to an equation, upper case
% \def\Eqref#1{Equation~\ref{#1}}
% % A raw reference to an equation---avoid using if possible
% \def\plaineqref#1{\ref{#1}}
% % Reference to a chapter, lower-case.
% \def\chapref#1{chapter~\ref{#1}}
% % Reference to an equation, upper case.
% \def\Chapref#1{Chapter~\ref{#1}}
% % Reference to a range of chapters
% \def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% % Reference to an algorithm, lower-case.
% \def\algref#1{algorithm~\ref{#1}}
% % Reference to an algorithm, upper case.
% \def\Algref#1{Algorithm~\ref{#1}}
% \def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
% \def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% % Reference to a part, lower case
% \def\partref#1{part~\ref{#1}}
% % Reference to a part, upper case
% \def\Partref#1{Part~\ref{#1}}
% \def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

% \newcommand{\train}{\mathcal{D}}
% \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}


% % Random variables
% \def\reta{{\textnormal{$\eta$}}}
% \def\ra{{\textnormal{a}}}
% \def\rb{{\textnormal{b}}}
% \def\rc{{\textnormal{c}}}
% \def\rd{{\textnormal{d}}}
% \def\re{{\textnormal{e}}}
% \def\rf{{\textnormal{f}}}
% \def\rg{{\textnormal{g}}}
% \def\rh{{\textnormal{h}}}
% \def\ri{{\textnormal{i}}}
% \def\rj{{\textnormal{j}}}
% \def\rk{{\textnormal{k}}}
% \def\rl{{\textnormal{l}}}
% % rm is already a command, just don't name any random variables m
% \def\rn{{\textnormal{n}}}
% \def\ro{{\textnormal{o}}}
% \def\rp{{\textnormal{p}}}
% \def\rq{{\textnormal{q}}}
% \def\rr{{\textnormal{r}}}
% \def\rs{{\textnormal{s}}}
% \def\rt{{\textnormal{t}}}
% \def\ru{{\textnormal{u}}}
% \def\rv{{\textnormal{v}}}
% \def\rw{{\textnormal{w}}}
% \def\rx{{\textnormal{x}}}
% \def\ry{{\textnormal{y}}}
% \def\rz{{\textnormal{z}}}

% % Random vectors
% \def\rvepsilon{{\mathbf{\epsilon}}}
% \def\rvtheta{{\mathbf{\theta}}}
% \def\rva{{\mathbf{a}}}
% \def\rvb{{\mathbf{b}}}
% \def\rvc{{\mathbf{c}}}
% \def\rvd{{\mathbf{d}}}
% \def\rve{{\mathbf{e}}}
% \def\rvf{{\mathbf{f}}}
% \def\rvg{{\mathbf{g}}}
% \def\rvh{{\mathbf{h}}}
% \def\rvu{{\mathbf{i}}}
% \def\rvj{{\mathbf{j}}}
% \def\rvk{{\mathbf{k}}}
% \def\rvl{{\mathbf{l}}}
% \def\rvm{{\mathbf{m}}}
% \def\rvn{{\mathbf{n}}}
% \def\rvo{{\mathbf{o}}}
% \def\rvp{{\mathbf{p}}}
% \def\rvq{{\mathbf{q}}}
% \def\rvr{{\mathbf{r}}}
% \def\rvs{{\mathbf{s}}}
% \def\rvt{{\mathbf{t}}}
% \def\rvu{{\mathbf{u}}}
% \def\rvv{{\mathbf{v}}}
% \def\rvw{{\mathbf{w}}}
% \def\rvx{{\mathbf{x}}}
% \def\rvy{{\mathbf{y}}}
% \def\rvz{{\mathbf{z}}}

% % Elements of random vectors
% \def\erva{{\textnormal{a}}}
% \def\ervb{{\textnormal{b}}}
% \def\ervc{{\textnormal{c}}}
% \def\ervd{{\textnormal{d}}}
% \def\erve{{\textnormal{e}}}
% \def\ervf{{\textnormal{f}}}
% \def\ervg{{\textnormal{g}}}
% \def\ervh{{\textnormal{h}}}
% \def\ervi{{\textnormal{i}}}
% \def\ervj{{\textnormal{j}}}
% \def\ervk{{\textnormal{k}}}
% \def\ervl{{\textnormal{l}}}
% \def\ervm{{\textnormal{m}}}
% \def\ervn{{\textnormal{n}}}
% \def\ervo{{\textnormal{o}}}
% \def\ervp{{\textnormal{p}}}
% \def\ervq{{\textnormal{q}}}
% \def\ervr{{\textnormal{r}}}
% \def\ervs{{\textnormal{s}}}
% \def\ervt{{\textnormal{t}}}
% \def\ervu{{\textnormal{u}}}
% \def\ervv{{\textnormal{v}}}
% \def\ervw{{\textnormal{w}}}
% \def\ervx{{\textnormal{x}}}
% \def\ervy{{\textnormal{y}}}
% \def\ervz{{\textnormal{z}}}

% % Random matrices
% \def\rmA{{\mathbf{A}}}
% \def\rmB{{\mathbf{B}}}
% \def\rmC{{\mathbf{C}}}
% \def\rmD{{\mathbf{D}}}
% \def\rmE{{\mathbf{E}}}
% \def\rmF{{\mathbf{F}}}
% \def\rmG{{\mathbf{G}}}
% \def\rmH{{\mathbf{H}}}
% \def\rmI{{\mathbf{I}}}
% \def\rmJ{{\mathbf{J}}}
% \def\rmK{{\mathbf{K}}}
% \def\rmL{{\mathbf{L}}}
% \def\rmM{{\mathbf{M}}}
% \def\rmN{{\mathbf{N}}}
% \def\rmO{{\mathbf{O}}}
% \def\rmP{{\mathbf{P}}}
% \def\rmQ{{\mathbf{Q}}}
% \def\rmR{{\mathbf{R}}}
% \def\rmS{{\mathbf{S}}}
% \def\rmT{{\mathbf{T}}}
% \def\rmU{{\mathbf{U}}}
% \def\rmV{{\mathbf{V}}}
% \def\rmW{{\mathbf{W}}}
% \def\rmX{{\mathbf{X}}}
% \def\rmY{{\mathbf{Y}}}
% \def\rmZ{{\mathbf{Z}}}

% % Elements of random matrices
% \def\ermA{{\textnormal{A}}}
% \def\ermB{{\textnormal{B}}}
% \def\ermC{{\textnormal{C}}}
% \def\ermD{{\textnormal{D}}}
% \def\ermE{{\textnormal{E}}}
% \def\ermF{{\textnormal{F}}}
% \def\ermG{{\textnormal{G}}}
% \def\ermH{{\textnormal{H}}}
% \def\ermI{{\textnormal{I}}}
% \def\ermJ{{\textnormal{J}}}
% \def\ermK{{\textnormal{K}}}
% \def\ermL{{\textnormal{L}}}
% \def\ermM{{\textnormal{M}}}
% \def\ermN{{\textnormal{N}}}
% \def\ermO{{\textnormal{O}}}
% \def\ermP{{\textnormal{P}}}
% \def\ermQ{{\textnormal{Q}}}
% \def\ermR{{\textnormal{R}}}
% \def\ermS{{\textnormal{S}}}
% \def\ermT{{\textnormal{T}}}
% \def\ermU{{\textnormal{U}}}
% \def\ermV{{\textnormal{V}}}
% \def\ermW{{\textnormal{W}}}
% \def\ermX{{\textnormal{X}}}
% \def\ermY{{\textnormal{Y}}}
% \def\ermZ{{\textnormal{Z}}}

% % Vectors
% \def\vzero{{\bm{0}}}
% \def\vone{{\bm{1}}}
% \def\vmu{{\bm{\mu}}}
% \def\vtheta{{\bm{\theta}}}
% \def\va{{\bm{a}}}
% \def\vb{{\bm{b}}}
% \def\vc{{\bm{c}}}
% \def\vd{{\bm{d}}}
% \def\ve{{\bm{e}}}
% \def\vf{{\bm{f}}}
% \def\vg{{\bm{g}}}
% \def\vh{{\bm{h}}}
% \def\vi{{\bm{i}}}
% \def\vj{{\bm{j}}}
% \def\vk{{\bm{k}}}
% \def\vl{{\bm{l}}}
% \def\vm{{\bm{m}}}
% \def\vn{{\bm{n}}}
% \def\vo{{\bm{o}}}
% \def\vp{{\bm{p}}}
% \def\vq{{\bm{q}}}
% \def\vr{{\bm{r}}}
% \def\vs{{\bm{s}}}
% \def\vt{{\bm{t}}}
% \def\vu{{\bm{u}}}
% \def\vv{{\bm{v}}}
% \def\vw{{\bm{w}}}
% \def\vx{{\bm{x}}}
% \def\vy{{\bm{y}}}
% \def\vz{{\bm{z}}}
% \def\valpha{{\bm{\alpha}}}
% \def\vbeta{{\bm{\beta}}}

% % Elements of vectors
% \def\evalpha{{\alpha}}
% \def\evbeta{{\beta}}
% \def\evepsilon{{\epsilon}}
% \def\evlambda{{\lambda}}
% \def\evomega{{\omega}}
% \def\evmu{{\mu}}
% \def\evpsi{{\psi}}
% \def\evsigma{{\sigma}}
% \def\evtheta{{\theta}}
% \def\eva{{a}}
% \def\evb{{b}}
% \def\evc{{c}}
% \def\evd{{d}}
% \def\eve{{e}}
% \def\evf{{f}}
% \def\evg{{g}}
% \def\evh{{h}}
% \def\evi{{i}}
% \def\evj{{j}}
% \def\evk{{k}}
% \def\evl{{l}}
% \def\evm{{m}}
% \def\evn{{n}}
% \def\evo{{o}}
% \def\evp{{p}}
% \def\evq{{q}}
% \def\evr{{r}}
% \def\evs{{s}}
% \def\evt{{t}}
% \def\evu{{u}}
% \def\evv{{v}}
% \def\evw{{w}}
% \def\evx{{x}}
% \def\evy{{y}}
% \def\evz{{z}}

% % Matrix
% \def\mA{{\bm{A}}}
% \def\mB{{\bm{B}}}
% \def\mC{{\bm{C}}}
% \def\mD{{\bm{D}}}
% \def\mE{{\bm{E}}}
% \def\mF{{\bm{F}}}
% \def\mG{{\bm{G}}}
% \def\mH{{\bm{H}}}
% \def\mI{{\bm{I}}}
% \def\mJ{{\bm{J}}}
% \def\mK{{\bm{K}}}
% \def\mL{{\bm{L}}}
% \def\mM{{\bm{M}}}
% \def\mN{{\bm{N}}}
% \def\mO{{\bm{O}}}
% \def\mP{{\bm{P}}}
% \def\mQ{{\bm{Q}}}
% \def\mR{{\bm{R}}}
% \def\mS{{\bm{S}}}
% \def\mT{{\bm{T}}}
% \def\mU{{\bm{U}}}
% \def\mV{{\bm{V}}}
% \def\mW{{\bm{W}}}
% \def\mX{{\bm{X}}}
% \def\mY{{\bm{Y}}}
% \def\mZ{{\bm{Z}}}
% \def\mBeta{{\bm{\beta}}}
% \def\mPhi{{\bm{\Phi}}}
% \def\mLambda{{\bm{\Lambda}}}
% \def\mSigma{{\bm{\Sigma}}}

% % Tensor
% \DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
% \SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
% \newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
% \def\tA{{\tens{A}}}
% \def\tB{{\tens{B}}}
% \def\tC{{\tens{C}}}
% \def\tD{{\tens{D}}}
% \def\tE{{\tens{E}}}
% \def\tF{{\tens{F}}}
% \def\tG{{\tens{G}}}
% \def\tH{{\tens{H}}}
% \def\tI{{\tens{I}}}
% \def\tJ{{\tens{J}}}
% \def\tK{{\tens{K}}}
% \def\tL{{\tens{L}}}
% \def\tM{{\tens{M}}}
% \def\tN{{\tens{N}}}
% \def\tO{{\tens{O}}}
% \def\tP{{\tens{P}}}
% \def\tQ{{\tens{Q}}}
% \def\tR{{\tens{R}}}
% \def\tS{{\tens{S}}}
% \def\tT{{\tens{T}}}
% \def\tU{{\tens{U}}}
% \def\tV{{\tens{V}}}
% \def\tW{{\tens{W}}}
% \def\tX{{\tens{X}}}
% \def\tY{{\tens{Y}}}
% \def\tZ{{\tens{Z}}}


% % Graph
% \def\gA{{\mathcal{A}}}
% \def\gB{{\mathcal{B}}}
% \def\gC{{\mathcal{C}}}
% \def\gD{{\mathcal{D}}}
% \def\gE{{\mathcal{E}}}
% \def\gF{{\mathcal{F}}}
% \def\gG{{\mathcal{G}}}
% \def\gH{{\mathcal{H}}}
% \def\gI{{\mathcal{I}}}
% \def\gJ{{\mathcal{J}}}
% \def\gK{{\mathcal{K}}}
% \def\gL{{\mathcal{L}}}
% \def\gM{{\mathcal{M}}}
% \def\gN{{\mathcal{N}}}
% \def\gO{{\mathcal{O}}}
% \def\gP{{\mathcal{P}}}
% \def\gQ{{\mathcal{Q}}}
% \def\gR{{\mathcal{R}}}
% \def\gS{{\mathcal{S}}}
% \def\gT{{\mathcal{T}}}
% \def\gU{{\mathcal{U}}}
% \def\gV{{\mathcal{V}}}
% \def\gW{{\mathcal{W}}}
% \def\gX{{\mathcal{X}}}
% \def\gY{{\mathcal{Y}}}
% \def\gZ{{\mathcal{Z}}}

% % Sets
% \def\sA{{\mathcal{A}}}
% \def\sB{{\mathcal{B}}}
% \def\sC{{\mathcal{C}}}
% \def\sD{{\mathcal{D}}}
% \def\sE{{\mathcal{E}}}
% \def\sF{{\mathcal{F}}}
% \def\sG{{\mathcal{G}}}
% \def\sH{{\mathcal{H}}}
% \def\sI{{\mathcal{I}}}
% \def\sJ{{\mathcal{J}}}
% \def\sK{{\mathcal{K}}}
% \def\sL{{\mathcal{L}}}
% \def\sM{{\mathcal{M}}}
% \def\sN{{\mathcal{N}}}
% \def\sO{{\mathcal{O}}}
% \def\sP{{\mathcal{P}}}
% \def\sQ{{\mathcal{Q}}}
% \def\sR{{\mathcal{R}}}
% \def\sS{{\mathcal{S}}}
% \def\sT{{\mathcal{T}}}
% \def\sU{{\mathcal{U}}}
% \def\sV{{\mathcal{V}}}
% \def\sW{{\mathcal{W}}}
% \def\sX{{\mathcal{X}}}
% \def\sY{{\mathcal{Y}}}
% \def\sZ{{\mathcal{Z}}}

% % Entries of a matrix
% \def\emLambda{{\Lambda}}
% \def\emA{{A}}
% \def\emB{{B}}
% \def\emC{{C}}
% \def\emD{{D}}
% \def\emE{{E}}
% \def\emF{{F}}
% \def\emG{{G}}
% \def\emH{{H}}
% \def\emI{{I}}
% \def\emJ{{J}}
% \def\emK{{K}}
% \def\emL{{L}}
% \def\emM{{M}}
% \def\emN{{N}}
% \def\emO{{O}}
% \def\emP{{P}}
% \def\emQ{{Q}}
% \def\emR{{R}}
% \def\emS{{S}}
% \def\emT{{T}}
% \def\emU{{U}}
% \def\emV{{V}}
% \def\emW{{W}}
% \def\emX{{X}}
% \def\emY{{Y}}
% \def\emZ{{Z}}
% \def\emSigma{{\Sigma}}

% % entries of a tensor
% % Same font as tensor, without \bm wrapper
% \newcommand{\etens}[1]{\mathsfit{#1}}
% \def\etLambda{{\etens{\Lambda}}}
% \def\etA{{\etens{A}}}
% \def\etB{{\etens{B}}}
% \def\etC{{\etens{C}}}
% \def\etD{{\etens{D}}}
% \def\etE{{\etens{E}}}
% \def\etF{{\etens{F}}}
% \def\etG{{\etens{G}}}
% \def\etH{{\etens{H}}}
% \def\etI{{\etens{I}}}
% \def\etJ{{\etens{J}}}
% \def\etK{{\etens{K}}}
% \def\etL{{\etens{L}}}
% \def\etM{{\etens{M}}}
% \def\etN{{\etens{N}}}
% \def\etO{{\etens{O}}}
% \def\etP{{\etens{P}}}
% \def\etQ{{\etens{Q}}}
% \def\etR{{\etens{R}}}
% \def\etS{{\etens{S}}}
% \def\etT{{\etens{T}}}
% \def\etU{{\etens{U}}}
% \def\etV{{\etens{V}}}
% \def\etW{{\etens{W}}}
% \def\etX{{\etens{X}}}
% \def\etY{{\etens{Y}}}
% \def\etZ{{\etens{Z}}}

% % The true underlying data generating distribution
% \newcommand{\pdata}{p_{\rm{data}}}
% % The empirical distribution defined by the training set
% \newcommand{\ptrain}{\hat{p}_{\rm{data}}}
% \newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% % The model distribution
% \newcommand{\pmodel}{p_{\rm{model}}}
% \newcommand{\Pmodel}{P_{\rm{model}}}
% \newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% % Stochastic autoencoder distributions
% \newcommand{\pencode}{p_{\rm{encoder}}}
% \newcommand{\pdecode}{p_{\rm{decoder}}}
% \newcommand{\precons}{p_{\rm{reconstruct}}}

% \newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\Ls}{\mathcal{L}}
% \newcommand{\emp}{\tilde{p}}
% \newcommand{\lr}{\alpha}
% \newcommand{\reg}{\lambda}
% \newcommand{\rect}{\mathrm{rectifier}}
% \newcommand{\softmax}{\mathrm{softmax}}
% \newcommand{\sigmoid}{\sigma}
% \newcommand{\softplus}{\zeta}
% \newcommand{\standarderror}{\mathrm{SE}}
% \newcommand{\cl}{\text{cl}}
% % \newcommand{\1}[1]{\mathds{1}\left[#1\right]}


% % Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% % But then they seem to use $L^2$ for vectors throughout the site, and so does
% % wikipedia.
% \newcommand{\normlzero}{L^0}
% \newcommand{\normlone}{L^1}
% \newcommand{\normltwo}{L^2}
% \newcommand{\normlp}{L^p}
% \newcommand{\normmax}{L^\infty}

% \newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \DeclareMathOperator{\sign}{sign}
% % \DeclareMathOperator{\Tr}{Tr}
% \let\ab\allowbreak

% \newcommand{\seq}{\subseteq}



==> maximal-value-labeling.tex <==

\section{Block value and maximal-value labeling}
\label{sec: maxval-labeling}
%\begin{proposition}
%	Consider the length-$q$ walk as consist of $q$ blocks of $\al\circ\al^T$, given the edge labeling of each block $B_1,...,B_q$, notice the final trace is given by \begin{align*}
%		\Tr\bigg((M_{\al} M_{\al^T})^q\bigg) = \sum_{\text{shape-walk path} P}n^{|\comb(P)|}\cdot \E_G[\edgeval(P)\cdot \cycle \cdot \bdd  ]
%	\end{align*}
%	
%	
%	there are at most $\vtxcost_q$ many terms of expected value $\edgeval_q$, where 
%	\[ \vtxcost_q = \prod_{i=1}^q \vtxcost(B_i) \]
%	and \[ 
%	\edgeval_q= \prod_{i=1}^q \edgeval(B_i)
%	\]
%\end{proposition}
In this section, we show that the block value is determined by vertex separator. On the one hand, this identifies the dominant term of the trace being governed by the SMVS; on the other hand, the structure lemma also provides us with a primitive to identify the gap from our trace-walk that offers slack for encoding auxiliary data.

 Towards this end, we start by constructing a vertex separator out of any locally-optimal labeling, and then relate the value of the labeling to the desired norm bound. However, before we proceed to construct a vertex separator, we need to understand the structure of a locally optimal labeling.
 
 \subsection{Set-up for structure lemmas}
 Before we dig into the core of our structure lemmas, we first make some (re-)definitions of our vertex-factors. In the previous section, we should an $R$ edge to represent the second-time an edge appears, and crucially, we show that the vertex reached by an $R$-edge (unless dangling) is \emph{fixed}. On the other hand, it would be convenient for us to consider $R$ leg as the last appearance of an edge appearance due to potential assymmetries of the shape, and we note that for any edge, we can assume exchange its potential vertex factors for the second time and last time appearance. 
 
 In the following section, we will now think of $F/H/R$ corresponding to the first/middle/last appearance of an edge, which also motivates the following assignment scheme for edge-value depending on edge-labels,
	\paragraph{Edge-value assignment scheme}
	\begin{mdframed}
	\begin{enumerate}
		\item $F$: each corresponds to some edge appearing for the first time,
		\begin{itemize}
			\item $F_\single$: the corresponding edge does not lead to visited vertices, while it is going to appear only once in the walk, and it gets assigned a factor $\sqrt{\frac{d}{n}}\cdot \frac{d}{n}\cdot \singdecay $;
			\item $F$: the corresponding edge leads to a new vertex, and it appears at least twice throughout the entire walk. This gets assigned a factor of $1$;
		\end{itemize} 
		\item $H$: each corresponds to middle appearance of some high-mul edge, and each contributes a factor of $\sqrt{\frac{n}{d}}$.
		\item $R$: each corresponds to some edge appearing for the last time, and we assign a factor of  $1$.
	\end{enumerate}
	\end{mdframed}

 
 
 %\begin{claim}
%	For a fixed labeling $\calL$ for $\al$ when we traverse from $U_\al$ to $V_\al$, any vertex that is arrived along some $F$ edge contributes a factor of at most $\sqrt{n}$ to the block value $\vtxcost\cdot \edgeval$.
%\end{claim}
%\begin{proof}
%	For starters, the block value $\vtxcost\cdot \edgeval(\calL)$ can be bounded in two ways, either via a traversal from $U_\al$ to $V_\al$, or via a traversal from $V_\al$ to $U_\al$, and it suffices for us to bound it by \[\sqrt{\vtxcost_{U\rightarrow V}(\calL) \cdot \vtxcost_{V\rightarrow U}(\calL^\top) } \cdot \edgeval \]
%	where we observe that edgeval comes from $H$ edges and does not depend on the direction of traversal.
%	
%	Let $v \in V(\al)\setminus U_\al$ be a vertex that is arrived along some non-signleton $F$ edge using the labeling $\calL$ when we traverse from $U_\al$ to $V_\al$, we pick up at most a vertex factor of $n$ for this vertex; however, once we traverse from $V_\al$ to $U_\al$ along the same path (but in the reverse direction), the vertex $v$ is either fixed from the last block (if it is in $V_\al$), or the corresponding $F$ leg now becomes an $R$ leg and the vertex factor is fixed,  hence we pick up an average of $\sqrt{n}$. 
%	
%	For vertices arrived along singleton $F$ edge, the claim is immediate as in either direction, we pick up a vertex cost of $n$ for the corresponding vertex while there is at least one leg coming with singleton decay, giving us $n\cdot \sqrt{\frac{d}{n}}\cdot \singdecay \ll \sqrt{n} $.
%\end{proof}
\subsection{Structure lemma for locally optimal labelings}
\begin{lemma}[Structure lemma]
% For any locally optimal labeling from $U_\al$ to $V_\al$, there is no unnecessary turn on any simple path from $U_\al  $ to $V_\al $, i.e., any simple path from $U_\al $ to $V_\al$ is of the structure $R\rightarrow H\rightarrow F$, where we allow each edge-label set to be empty, i.e., a path of all $R$ or of all $F$ edges can be considered to be of the above structures; analogously, for any locally optimal labeling from $V_\al$ to $U_\al$, there is no unnecessary turn on any simple path from $V_\al$ to $U_\al$.

For any locally optimal labeling from $U_\al$, there is no unnecessary turn on any simple path originating from $U_\al$. In other words,  any simple path that starts from $U_\al $  is of the structure $R\rightarrow H\rightarrow F$, where we allow each edge-label set to be empty, i.e., a path of all $R$ or of all $F$ edges can be considered to be of the above structures; analogously, for any locally optimal labeling from $V_\al$, there is no unnecessary turn on any simple path from $V_\al$ to $U_\al$.


%	Analogously, we can apply this argument when we traverse from $V_\al$ to $U_\al$.	
\end{lemma}
%
%
% \begin{lemma}[Structure lemma for dangling branch]
%For any locally optimal labeling from $U_\al$ to $V_\al$, the simple path from $U_\al$ to any dangling branch has no unnecessary turn; analogously, for any locally optimal labeling from $V_\al$ to $U_\al$, the simple path from $V_\al$ to any dangling branch has no unnecessary turn. In other words, any of the above path is of the structure $R\rightarrow H\rightarrow F$.
% \end{lemma}
 \begin{lemma}[Structure lemma for floating component]
 For any locally optimal labeling, for any floating component and any fixed landing vertex $v$, any simple path from $v$ has no turn, i.e., they are either all $F/R$ or $H$.
 \end{lemma}
% \begin{lemma}[''Strengthened'' structure lemma for floating component]
% 	For any locally optimal labeling $\calL$, and $C$ a floating component s.t. any vertex in $V(C)$ has degree at least $1$, and $C$ is viable in a typical random graph sample, let $\calL_C$ be the restriction of $\calL$ into floating component $C$,  \[ 
% 	\vtxcost\cdot\edgeval(\calL_C) \leq c^{|E(C)|} \cdot \sqrt{n}^{|V(C)|}\cdot \min \left(\sqrt{d}^{|V(C)|} \right) 
% 	\]
% \end{lemma}
% \begin{proof}
% 	This is subsumed by 
% \end{proof}
\begin{proof}
We prove the above structure lemmas altogether. Note that any path not of the above structure contains a surprise visit in the current block, and hence its value can be locally improved. It also suffices for us to assume each $F$ edge explores a \emph{new} vertex (and the edge is promised to appear again, i.e., non-singleton), as otherwise we pick up at least one factor of singleton decay and we can locally improve the block-value via a promise to use the edge again, or $O(1)$ factors of $2|V(\al)|q_\al$ via our forced-return bound. 

 W.L.O.G., suppose we are traversing from $U_\al$ to $V_\al$ and let $\calL$ be a labeling for this direction. We first note that we can identify such \emph{bad} edge by considering the following process,\begin{enumerate}
 	\item BFS from $U_\al$;
 	\item Identify the first $R$ or $H$ edge preceded by an $F$ edge in this process, and let the vertex that splits out such edge, i.e. the vertex reached by the prior $F$ edge, be $v$; 
 \end{enumerate}
 
 
% Take any simple path from $U_\al$ to $V_\al$, if it is not of the structure above, following this path, there is some $F$ edge that appears in the path followed some $H$ or $R$ edge, and we claim that such an $F$ edge is a surprise visit and can be locally improved. If there are multiple $F$ edges, we can pick the first such edge traversed along the path. Let the vertex reached by the $F$ edge be $v$, and the starting point of this vertex in $U_\al$ be $a$.

There may be multiple paths from $U_\al$ to $v$, while we know that each such path must be all $F$ until they arrive at $v$ in $\calL$. We now consider an alternative labeling $\calL'$ obtained by flipping edges on the path from $ U_\al$ to $v$ from $F$ to $R$. For each vertex on the path $a_i\in U_\al$ to $v$ (except $a_i$ and $v$), it contributes at most a $\sqrt{n}$ vertex factor to the norm bound under $\calL$ once we average over both traversal directions in $\calL$: a vertex reached using an $F$ edge in the $U\rightarrow V$ direction receives a factor $n$, while in the other direction $V\rightarrow U$ it is either fixed (via in the boundary $V$) or arrived along an $R$ edge which is also fixed.  Moreover, notice each such vertex still contributes a $\sqrt{n}$ to the norm bound under $\calL'$ via the same argument. 	
 	
 	For each vertex $a_i \in U_\al$, notice it does not contribute any vertex factor in neither traversal direction of $\calL$. However, it picks up a value of $n$ when we traverse $\calL'^\top $ from $V_\al$ to $U_\al$ as it is arrived using an $F$ edge, and in average it contributes a vertex factor of $\sqrt{n}$ under $\calL$.
 	
 		For vertex $v$, let $f(v)$ be its vertex factor when we traverse in $\calL^T$ from $V_\al$ to $U_\al$. Notice we can pick the encoding such that $v$ is encoded via the same edge when traverse in $V\rightarrow U$ direction in both $\calL$ and $\calL'$, and therefore it contributes the same vertex factor in the reverse direction under $\calL'$. However, notice $v$ is a surprise visit as it is incident to some $H/R$ edge, a vertex cost of $\csurp$ factors of $2|V(\al)|q_\al$ is sufficient where the $\csurp = O(1)$ takes into account the overhead of our unforced-return-bound due to surprise visit. Combining the above, the vertex $v$ contributes a factor of $\sqrt{(2|V(\al)q_\al)^c_s\cdot f(v) }$ in $\calL$ while it contributes a vertex factor of $\sqrt{f(v)}$ under $\calL'$, giving a change of $\frac{1}{\sqrt{2|V(\al)|q}}$.
 	
Finally, notice the vertex factors not on any path from $U_\al$ to $v$ remain unaffected, and the edge-value is unchanged when we move from $\calL$ to $\calL'$, and combining the above changes for the vertex factors along the path gives us a gap of \[ 
 	\frac{\vtxcost\cdot \edgeval(\calL')}{\vtxcost\cdot \edgeval(\calL)} \geq \frac{\sqrt{n}}{\sqrt{2|V(\al)|q}} \gg 1
 	\]
 provided $2|V(\al)|q\ll n$.
 
 The above argument as stated shows that along any simple path from $U_\al$, there is no $F$ edge before any $R/H$ edge in a locally optimal labeling while this does not preclude a path of the structure $R\rightarrow H\rightarrow R$. To rule out these paths, notice we can apply the above argument on the reverse labeling $\calL^T$, in which an $R\rightarrow H\rightarrow R$ path becomes $F\rightarrow H\rightarrow F$ that can be locally improved, and this completes the proof to our structure lemma for non-dangling components.
 
 For floating components, the idea is essentially identical while we can further observe that for each floating component, we have freedom to pick a vertex to encode with a label in $2|V(\al)|q$ to effectively \emph{land} into the component and start the encoding process there. Therefore, if the component contains a mix of $F$ and $R/H$ edges, we can essentially land at a vertex, and pick a direction to traverse the component such that some $F$ edge is traversed before the $R/H$ edge, rendering us a surprise visit that can again be locally improved.
% 
% For dangling components, the above lemma can be strengthened such that each edge in the component must receive the same label, since we have the freedom of picking the \emph{landing} vertex for each component if it is incident to some $R/H$ edge. Hence, if the component contains some $F$ edge, we can always locally improve the value by avoiding surprise visit if we switch any non-$F$ edge in the labeling to $F$. Similarly, we can apply the argument to show any component containing $R$ edge must also be all $R$ by considering its reverse labeling. 
 \end{proof}
% 
% \begin{lemma}[Strengthened structure lemma for floating component]
% 	For any locally optimal labeling, if the component is tree-like, edges in any floating component are either all $F$ or all $R$; moreover, any edge that is part of a short cycle is an $H$ edge. 
% 	 \jnote{not sure if we would want this...not necessary for our applicaton}
% \end{lemma}
% \begin{proof}
% The idea is essentially identical with the argument we just see, with an exception that for each floating component, we have freedom to pick a vertex to encode with a label in $2|V(\al)|q$ to effectively ''land'' into the component and start the encoding process there. Moreover, the choice for each connected component can be agreed upon before the encoding-decoding process, and the labeling follows the direction of the BFS traversal outwards from the landing vertex. 
%  
% Applying the previous argument on any outwards traversal from the landing vertex, note that any path that has an unnecessary turn is again a surprise visit and be locally improved using the previous argument, hence we can already conclude each simple path from the landing vertex follows the structure of $R\rightarrow H\rightarrow F$. However, this can be further strengthened.
% 
%  For tree-like component, we claim that the edges are either all $F$ or all $R$. Suppose not, notice in either direction, there is a vertex that can be identified using a factor $2|V(\al)|q$, with each other vertex contributing at most a factor of $\sqrt{n}$. However, if we flip all edges into all $F$ or all $R$, each vertex contributes a factor of $\sqrt{n}$, and moreover, there is one landing vertex that contributes an additional $\sqrt{2|V(\al)|q}$ factor. 
% \end{proof}
 
 %
% Let $b$ be the vertex incident to both $e_1$ and $e_2$, and let $a$ be the vertex incident to the last non-$F$ edge on the path from $U_\al$ to $b$. Consider the path from $a$ to $b$, notice we pick up a gain of at least $\frac{n}{2|V(\al)|q}$ in the SMVS value if we flip all the edges between $a$ and $b$ on the path to be $R$, as 
% \begin{enumerate}
%	\item For each vertex on the path between $a$ and $b$, it contributes at most  a vertex factor of $\sqrt{n}$ once we take average of the vertex cost for $\calL$ and $\calL^\top$ when we traverse from the other direction; %	  \[ 
%%	\frac{\sqrt{\frac{n}{d}}\cdot \frac{1}{\singdecay} }{n\cdot \frac{d}{n} \cdot \sqrt{\frac{n}{d}}\cdot \singdecay} >1	\]
%\[ 
%\frac{n\cdot \frac{1}{\sqrt{n}}}{\sqrt{n}}=1
%\]
%	\item For vertex $b$, it is incident to a non-$F$ edge in the current block, hence it gets a factor of at most $2|V(\al)|q $ in the vertex cost at the original labeling, and flipping the last edge from $F$ to $R$ gives a change of \[
%	 \frac{n\cdot\frac{1}{\sqrt{n}} }{2|V(\al)|q} > \1	 	 \]
%	 provided $|V(\al)|\ll n^{1/4} $.
%\end{enumerate}

%
%
%if it contains an excess turn, we can find two points $a\neq b\in V(\al) $ that are both incident to edges of $F,R$ labels on the path. W.L.O.G., let $a$ be the first vertex that witnesses a turn and $b$ the second, let $e_1$ be the path from $U_\al$ into $a$, $e_2$ the path between $a$ and $b$, and $e_3$ the path from $b$ to $V_\al$ or the next turn vertex on the path, now we discuss by cases:\begin{itemize}
%	\item  $e_1=F, e_2=R, e_3=F$: by local injectivity, $e_2=R$ restricts the vertex cost of encoding $a$ to be at most $2q|V(\al)|$, and hence, we can either flip all the edges in $e_1$ to $R$ to locally improve the value of edge, for all the vertices between $U_\al$ and $a$, we may lose a vertex factor of at most $n$, however, it can be charged to the edge factor we pick up, giving a change of \[
%	\frac{\sqrt{\frac{n}{d}}\cdot \frac{1}{\singdecay} }{n\cdot \frac{d}{n} \cdot \sqrt{\frac{n}{d}}\cdot \singdecay} >1	 \] Charging each vertex to the edge  leading to it from $U_\al$ on the simple path, we have an extra factor from the last edge incident to $a$ and this gives us a gain of \[\sqrt{\frac{n}{d}}/\left(2|V(\al)|q \cdot \sqrt{\frac{d}{n}}\cdot \singdecay\right) >\frac{n}{2|V(\al)|q}
% \] 
%	\item $e_1=R, e_2=F, e_3=R$: similarly, the value can be locally improved by either flipping $e_3$ to $F$ to avoid a surprise visit at $b$.
%\end{itemize}  
%\begin{lemma}
%	For any vertex $v$ in block $\al$ that has multiple simple paths from $U_\al$,  each of this path is of the structure $R\rightarrow H$ in any locally optimal labeling. Similarly, for any vertex $v$ that has multiple paths to $V_\al$, consider a BFS from $v$, each of this path is of the structure $H\rightarrow F$ in any locally optimal labeling.
%\end{lemma}
%\begin{proof}
%	It suffices for us to show the first half of the lemma. 
%\end{proof}
% From the structure lemma above, we notice any simple path from $U_\al$ to $V_\al$ is either all $F$ or all $R$ until some point, and then the label would be flipped thereafter. Let $S$ be the endpoints of $H$ edges in the optimal labeling (that uses the fewest $H$ labels), we notice that the above structure theorem of the labeling can also be extended to the following,
%\begin{lemma}
%	Any simple path from $U_\al$ to $V_\al$ is of the structure $R\rightarrow H\rightarrow F$. 
%\end{lemma}
%\begin{proof}
%[Proof required]
%\end{proof}
%\begin{claim}
%	Consider any optimal labeling $\calL$ of length-2 block, W.L.O.G., we can assume $\calL$ is symmetric w.r.t. $V_\al$, i.e., any edge that receives label $F$ (or $R$) in one copy would receive label $R$ (or $F$) in the other copy, and any edge that receives $H$ would receive $H$ in both copies.
%\end{claim}
\subsection{Bounding the block value for a locally optimal labeling}
Given $\calL$ any locally optimal labeling on $\al$ (or $\al^T$), we show in this section that it corresponds to a vertex separator. Let's start by building a separator from a locally optimal labeling.
\begin{mdframed}[frametitle = {Building a separator}]
\begin{enumerate}
	\item We include any vertex incident to an $H$ edge in $\calL$ into $S_\al$;
	\item Any vertex that is a turn vertex, i.e., it gets encoded into the cut along an $R$ edge and it is incident to some  $F$ edge;
	\item We include any vertex that is in $U_\al\cap V_\al$ into $S_\al$.
	\item Additionally, for any path from $U_\al$ to $V_\al$  that does not go through any included vertex, the path must be either all $R$ or all $F$ by our structure lemma, and we include the vertex from $V_\al$ into $S_\al$ if the path is all $R$, or the vertex from $U_\al$ into $S_\al$ if the path is all $F$.
\end{enumerate}	
\end{mdframed}



With a separator built at hand, we are ready to bound the corresponding block value for a given separator constructed from $\calL$. Let $S_L$ be the boundary of $S$ that can be reached from $U_\al$ without passing through any other vertex in $S$, and let $S_R$ be the boundary os $S$ that can be reached from $V_\al$ without passing through any other vertex in $S$. 



\subsubsection{Factors of $\sqrt{n}$}\label{sec:factors-of-root-n}
We start by bounding the vertex factors coming from $F/R$ edges in this subsesction.
\begin{claim}
	For a fixed labeling $\calL$ for $\al$, any non-dangling vertex that is arrived along some $F$ edge in either $\calL$ or $\calL^T$ contributes a factor of at most $\sqrt{n}$ to the block value $\vtxcost\cdot \edgeval$.
	Furthermore, for dangling vertices, they contribute an additional dangling factor $\dang(\al\setminus S)$.
	For floating vertices, they contribute an additional floating factor $\float(\al)$.
	\end{claim}
\begin{proof}
	For starters, the block value $\vtxcost\cdot \edgeval(\calL)$ can be bounded in two ways, either via a traversal from $U_\al$ to $V_\al$, or via a traversal from $V_\al$ to $U_\al$, and it suffices for us to bound it by \[\sqrt{\vtxcost_{U\rightarrow V}(\calL) \cdot \vtxcost_{V\rightarrow U}(\calL^\top) } \cdot \edgeval \]
	where we observe that edgeval comes from $H$ edges and does not depend on the direction of traversal.
	
	Let $v \in V(\al)\setminus U_\al$ be a vertex that is arrived along some non-signleton $F$ edge using the labeling $\calL$ when we traverse from $U_\al$ to $V_\al$, we pick up at most a vertex factor of $n$ for this vertex; however, once we traverse from $V_\al$ to $U_\al$ along the same path (but in the reverse direction), the vertex $v$ is either fixed from the last block (if it is in $V_\al$), or the corresponding $F$ leg now becomes an $R$ leg and the vertex factor is ''fixed'' (up to dangling factor). Combining with Prop.~\ref{prop: pur-invariant} , we have ,
	\begin{enumerate}
		\item For non-dangling vertices, the return leg is fixed and we do not pick up any vertex factor, hence on average, we pick up a factor of $\sqrt{n}$;
		\item For dangling branches, each branch contributes at most one factor of $2|V(\al)|q_\al$ for identifying the furtherest point on the each branch reachable via $R\cup H$ edges, and it suffices for us to assign a factor of $2|V(\al)|q_\al$ for each branch and set $\dang(\al) = \left(2|V(\al)|q_\al\right)^{|\branch(\al)|}$.
%		\item For each floating component, one of its vertices incident to a return leg in the component picks up an extra vertex factor of at most $2|V(\al)|q$, which is captured by the factor $\float(\al)$, hence in average we pick up $\sqrt{n\cdot 2|V(\al)|q}$.
	\end{enumerate}
%	
%	
%	For dangling vertices, we pick up an average of $\sqrt{n} \cdot  \dang(\al\setminus S)[v]$  where $\dang(\al\setminus S)[v]$ is the dangling factor assigned for vertex $v$ (upper bounded by $\sqrt{d}$).
%	
%	For each floating component, notice in addition to the factor in dangling vertex, an extra label in $2|V(\al)|q$ is needed when it appears again after the first time. Taking the average gives us a factor of $\sqrt{2|V(\al)q}$ for each connected component, and we assign this factor into $\float(\al)$.
	
	For vertices arrived along a singleton $F_\single$ edge in non-floating components, the claim is immediate since we can assign each vertex to an edge that leads to it: in either direction, we pick up a vertex cost of $n$ for the corresponding vertex while there is at least one leg (with factor assigned to this vertex) coming with singleton decay, giving us $n\cdot \sqrt{\frac{d}{n}}\cdot \singdecay \ll \sqrt{n} $. 
	
	\begin{claim}
		It suffices for us to assign a factor of $\sqrt{n}\exp(-d)$ for each floating component, i.e., $\float(\al) \leq \left(\sqrt{n}\exp(-d)\right)^{|\float(\al)|}$ where we recall $|\float(\al)|$ is the number of floating components. 
	\end{claim}
	\begin{proof}	Via our structure lemma, the edges in a floating component is either all $F$, $R$, or $H$:
	\begin{enumerate}
		\item \textbf{Singleton floating component}  We first consider $F$-component, where some extra care is warranted as singleton edges may now be troublesome. The previous argument for handling singleton edges crucially replies upon being able to assign each vertex to an edge that comes with singleton decay. However, this is no longer true for floating component, especially tree-like floating component: for example, consider an edge floating around in $\al$: should the edge be a singleton edge in the walk, it can contribute \[
	n^2 \cdot \sqrt{\frac{d}{n}}\cdot \singdecay \approx n^{1.5} \exp(-d) \gg \sqrt{n^2}\cdot (2|V(\al)|q_\al)	 \]
	where we recall $\sqrt{n^2}\cdot (2|V(\al)|q_\al)	$ is the cost we would expect if there is no conditioning. That being said, we may have one $\sqrt{n}$ blow-up, giving a bound of \[ 
	\sqrt{n}^{|V(C_i)|}\cdot \underbrace{\sqrt{n}\cdot \singdecay^{V(C_i)-1} }_{\float(C_i)}	\]	
	for each floating component $C_i$ where we can capture the potential blow-up by the corresponding floating factor.
	
	\begin{remark}
		A natural question is whether the $\sqrt{n}$ blow-up from conditioning is tight. We remark that it is possible as it comes down to bounding $\E[\chi_e \cdot 1_\calF ]$ where we recall $\calF$ is the conditioning on bounded-degree, and we can ignore the conditioning on $2$-cycle for this part. \begin{align*}
			\E[\chi_e \cdot 1_\calF ] &= \Pr\left[1_\calF \cap \left(\chi_e=\sqrt{\frac{1-p}{p}} \right)\right] \cdot \sqrt{\frac{1-p}{p}} + \Pr\left[1_\calF \cap \left(\chi_e=-\sqrt{\frac{p}{1-p}} \right)\right] \cdot (-\sqrt{\frac{p}{1-p}})\\
			&=\Pr\left[1_\calF|\chi_e=\sqrt{\frac{1-p}{p}}\right]\sqrt{\frac{1-p}{p}}\cdot p - \Pr\left[1_\calF|\chi_e=-\sqrt{\frac{p}{1-p}}\right] \cdot \sqrt{\frac{p}{1-p}}\cdot (1-p)\\
			& = (\sqrt{(1-p)p}) \left( \Pr\left[1_\calF|\chi_e=\sqrt{\frac{1-p}{p}}\right] - \Pr\left[1_\calF|\chi_e=-\sqrt{\frac{p}{1-p}}\right]\right)
			\end{align*}
			To bound the difference in the probability, we note that this is equivalent to resampling all the edges but $e$, what's the probability that at least one of the two endpoints of $e$ hit degree $10d-1$ (suppose we truncate at degree $10d$), and an $\exp(-d)$ bound here is the best we can hope for, which would give a bound of $\E[\chi_e\cdot 1_\calF] \approx \sqrt{\frac{d}{n}} \cdot \exp(-d)$ . Notice we need an extra $\frac{1}{\sqrt{n}}$ decay to offset the blow-up for a singleton $F$ component.
	\end{remark}
		\item \textbf{Non-singleton floating component} The argument is identical to the non-floating case except for the first vertex in the component (when being traversed the second-time or later), giving us a bound of \[ 
		\sqrt{n}^{V|(C_i)|}\cdot \dang(C_i) \cdot \underbrace{2|V(\al)|q_\al}_{\float(C_i)}
		\] 
		\end{enumerate}
		Combing the above, for each floating component, it suffices for us to take \[ 
		\float(C_i) \leq \max(\sqrt{n}\cdot (\singdecay)^{V(C_i)-1}, 2|V(\al)|q_\al) \leq \sqrt{n}\cdot \exp(-d)
		\]
		\end{proof}
 Applying the above claim on $\calL$ when we traverse from $U_\al$ to $V_\al$, and on $\calL'$ when we traverse from $V_\al$ to $U_\al$, any vertex that is arrived along an $F$ edge is outside the separator by our structure lemma, hence each vertex outside the separator contributes at most a factor $\sqrt{n}$ (modulo their corresponding dangling factors discussed above).
 \end{proof}
 
 \begin{corollary}
 	Any non-isolated vertex outside  $S$ contributes a vertex factor of $\sqrt{n}$ (modulo their corresponding floating and dangling factors).
 \end{corollary}
 \begin{proof}
 	This follows by observing that any vertex outside the separator is either \begin{enumerate}
 		\item if a vertex is connected to some path between $U$ and $V$, then it can be reached using $F$ edge in either $\calL$ or $\calL^T$ and contributes a $\sqrt{n}$ factor as above;
 		\item for vertices not connected to any path between $U_\al$ and $V_\al$, it may be a vertex that is in either $U_\al\setminus V_\al$ or in $V_\al\setminus U_\al$ while not connected to any path between $U$ to $V$, and they contribute $n$ in one direction and is again fixed in another direction;
 		\item Floating vertices have its factor captured by the floating component for the blow-up, that it gives a factor $n$ in one direction and a $2|V(\al)|q_\al$ factor in the other.
 	\end{enumerate}
 \end{proof}
 
 
%\subsubsection{Floating components don't like a re-visit}
%
%From the discussion in the above subsection, dangling vertices and floating components contribute an extra factor when they are visited the second-time and forwards. In particular, each floating component (even contained in the SMVS) requires an extra $2|V(\al)|q_\al$ label when it is being visited the second time or onwards. A peculiar question at this point is whether each floating component contributes an extra factor of $\sqrt{2|V(\al)q_\al}$ or a factor of $2|V(\al)|q_\al$ to the final norm bound?  Specifically, can we rule out a floating component being visited more than twice (beyond necessity to avoid singleton decay)? If so, a $2|V(\al)|q_\al$ is only required when a floating component is visited the second time, and averaging with the first visit gives us a $\sqrt{2|V(\al)|q_\al}$ contribution to the final bound. 
%
%	For convenience, we restrict our attention to component with no dangling branch, i.e., degree-$1$ vertex, or a path of those.  We case on whether the component contains more than $1$ cycle. Let $C$ be a floating component.
%\paragraph{Monocycle component}
%In this case, we have $|E(C)|\leq |V(C)|$, and we first observe that via structure lemma, all edges must be either all $F$, all $R$ or all $H$ as any mix of edge-status results in surprise visit for a floating component. It suffices for us to observe that in this case, the component must be either all $F$ or all $R$ to obtain maximal-value as an all $H$ labeling may contribute a value of at most \[ 
%2|V(\al)|q_\al \cdot \sqrt{\frac{n}{d} }^{|E(C)|} 
%\] 
%while taking 
%
%
%\begin{claim}[$R$-edge-value bound]\label{claim: R-edge-val-bound}
%	The edge-value coming from $R$ edges is at most $\sqrt{n}^{|L(U_\al\setminus S_L , S_L)|}$.
%\end{claim}
%\begin{remark}
%	Note this is a strengthened bound than assigning each $R$ edge a $\sqrt{n}$ factor. This is useful for avoiding a blow-up in the labeling value due to $R$ cycle.
%\end{remark}
%\begin{proof}
%	Consider a BFS from $S_L$ to traverse the vertices in $L(U_\al\setminus S_L , S_L)$, and note that the claim is immediate if there is no edge leading to visited vertices, as each edge comes with a value at most $\sqrt{n}$, and we can charge each edge to the vertex it leads to. However, by design of our edge-value assignment scheme, each excess $R$ edge corresponds to some excess $F$ edge (which only gets assigned a factor $1$), hence they do not contribute extra edge-value. 
%\end{proof}
%\begin{claim}
%	Each vertex reachable from $S$ via an $F$ edge comes with a most a vertex cost of $n$, and it suffices for us to assume each $F$ edge is non-singleton.
%\end{claim}
%\begin{proof}
%	For any singleton $F$ edge, it comes with an edge value of $\sqrt{\frac{n}{d}}\cdot \frac{d}{n}\cdot \singdecay \leq \sqrt{\frac{d}{n}}\cdot \exp(-d)  $, while flipping it to an non-singleton edge gives us an $\exp(d)$ improvement (as non-singleton $F$ edge comes with a value of $\frac{1}{\sqrt{n}}$.
%	\end{proof}



	

\subsubsection{Bounding the block value for any separator}
	Let's now try to bound the block value $\edgeval(\calL)\cdot \vtxcost(\calL)$ for any locally optimal $\calL$, let $S$ be the corresponding separator,
  \begin{enumerate}
  	\item Each vertex outside $S$ contributes a factor of $\sqrt{n}$;
	\item Each vertex in $S$ that is not doubly constrained in the encoding process is arrived along an $H$ edge, and hence requires at most a $\sqrt{d}$ vertex factor if non-dangling, and a factor of $d$ if dangling;
	\item Each edge receiving an $H$ label is in $E(S)$ and contributes a value of at most $\sqrt{\frac{n}{d}}$;
	\item For dangling branches, we pick up an additional dangling factor $\dang(\al)$, that is an additional $2|V(\al)|q_\al$ for each dangling branch;
	\item For floating components, an extra label in $2|V(\al)|q$ for each component is sufficient for each component.
\end{enumerate} 

For intuition, we recommend the reader to ignore factors from excess $F$ edges, and dangling vertices. However as stated, the above bound is not easy to apply as it is not immediately clear what vertex factors are needed for encoding vertices inside $S$; fortunately, this can be simplified once we restrict our attention to a class of separators, \emph{irreducible} separators, without any loss in the SMVS value.
 
 We now unpack the factors from the above in a more illustrative manner, and show that it suffices for us to assume each vertex in $S$ is doubly constrained by $S_L$, and moreover, there is no dangling vertex inside $S$.
%\begin{observation}[$\sqrt{n}$ for each vertex outside $S$, and an extra $\sqrt{d}$ if dangling]
%	Charging the edge-value of the $R$ edge leading to that vertex in the BFS process from $S_L$ if the vertex is in $L(U_\al\setminus S_L, S_L)$, or the edge value of the non-excess $F$ edge that leads to the vertex in the BFS from $S$, and the vertex cost, each (non-dangling) vertex in $V(\al)\setminus S$ contributes a value of $\sqrt{n}$. Each vertex dangling picks up an extra $\sqrt{d}$ factor and contribute a total of $\sqrt{nd}$.
%\end{observation}
%\begin{observation}[$\sqrt{\frac{n}{d}}$ for each separator edge] Each edge inside the separator receives an $H$ label, and contributes a value of $\sqrt{\frac{n}{d}}$.
%\end{observation}
\subsubsection{Pruning superfluous $H$ edges}\label{sec:pruning-superfluous-H}

\begin{definition}[Irreducible SMVS]
	We call a separator $S$ an irreducible SMVS for a shape $\al$ if for any vertex $v\in S$ of degree $1$ in $E(S)$,  \begin{enumerate}
		\item There are two edge-disjoint paths $P_U, P_V$ from $v$ to $U_\al$ and $v$ to $V_\al$
		\item Both paths do not pass through any other vertex in $S$
	\end{enumerate}
\end{definition}

\begin{claim}
	For each locally optimal $\calL$ labeling that produces separator vertices in $S(\calL)$ not doubly constrained by $S_L(\calL)$, there is a labeling $\calL'$ with at least the same SMVS value while each vertex in $S(\calL')$ is doubly constrained by $S_L(\calL')$. Moreover, there is no dangling vertex in $S(\calL')$.
\end{claim}
\begin{proof} We start by considering non-dangling vertices in $S$.
	We first notice for any vertex in $S_L$ of degree $1$ in $S$, unless it is incident to an $F$ edge, we can pop it out of the separator and obtain the same value by turning the incident $H$ edge into an $R$ edge: the $H$ edge contributes at most a $\sqrt{d}$ vertex factor to indicate the destination of the edge and it contributes a factor of $\sqrt{\frac{n}{d}}$ through the edge-value, while we obtain the same value by picking the $\sqrt{n}$ value from the vertex being outside the separator. 
	
	Let $\calL'$ be the labeling obtained by applying the above procedure on $\calL$, and let $S = S(\calL')$ be its corresponding separator. Consider a BFS from $S_L$ to traverse vertices in $S\setminus S_L$, and note that each vertex in the separator not doubly constrained by $S_L$ has only one simple path to $S_L$, and it is not on any path from $S_L$ to a cycle. In other words, given $S_L$, each non-doubly constrained vertex forms a tree rooted at $S_L$. For each branch, starting from the leaf vertex, notice each vertex (if non-dangling) contributes to the block value via the edge that leads to that vertex from $S_L$ a factor of $\sqrt{\frac{n}{d}}$ and a vertex factor $\sqrt{d}$ for indicating the destination of the $H$ edge, giving a total of $\sqrt{\frac{n}{d}}\cdot \sqrt{d}=\sqrt{n}$. However, the same value can be attained by flipping the $H$ edge to an $F$ edge and pop this vertex out of the separator. 
	
	For each dangling vertex, the pop-out procedure is rather identical except we now need to take into account the dangling factor. Suppose it is indicated using a label in $d$, it contributes a value of $\sqrt{\frac{n}{d}}\cdot d=\sqrt{nd}$ while we can again pop the vertex out of the separator and obtain a value of $\sqrt{nd}$ with the extra $\sqrt{d}$ coming from the dangling factor $\dang$; analogously, we can generalzie this argument for long dangling branch inside the separator, we can again use the idea in Proposition~\ref{prop:long-high-mul-path}, and obtain a $\sqrt{2|V(\al)|q}$ bound as we would have 
%		For each dangling branch, notice each edge comes with a value of $\sqrt{\frac{n}{d}}^{\branch(i)}$, while each time a label in $2|V(\al)|q$ or a sequence of labels in $d$ is needed, giving us a total of 
\begin{align*}
		\sqrt{\frac{n}{d}}^{\branch(i)}\min(2|V(\al)|q, d^{\branch(i)}) &\leq 
	\sqrt{n}^{\branch(i)} \min(\frac{2|V(\al)q}{\sqrt{d}^{\branch(i)} }, \sqrt{d}^{\branch(i)}) \\&\leq \sqrt{n}^{\branch(i)}\min(\sqrt{2|V(\al)|q} ,\sqrt{d}^{\branch(i)})
	\end{align*}
	Note that this is the same value we would pick up from vertex factors if we pop out the entire dangling branch, and this completes our proof to the claim.
%	Recall that the factors of $\sqrt{n}^{\branch(i)}$ is already taken into account by the vertex factors of $\sqrt{n}$ for each vertex outside the separator, hence, each block's dangling blow-up is still at most $\min(\sqrt{2|V(\al)|q} ,\sqrt{d}^{\branch(i)})$ for each branch. Combining the argument for all dangling branches gives us the desired proposition.
%
%	
\end{proof}
%
%Wrapping up, the above claim allows us to assume each vertex in $S$ being doubly-constrained by $S_L$; analogously, applying this argument on $\calL^T$ allows us to assume $S\setminus S_R$ being doubly constrained by $S_R$. 
% \begin{align*}
%	\val(\calL)= \vtxcost(\calL)\cdot \edgeval(\calL) \leq \max_{S:\text{separator}}\sqrt{n}^{|V(\al)\setminus S|}\cdot \left(\sqrt{\frac{n}{d}}\right)^{|E(S)|}\cdot \sqrt{d}^{\dang}\cdot  \sqrt{d}^{|\exc(F)|}
%\end{align*}
%
%\subsubsection{Is there floating component inside $S$?}
%\begin{claim}
%	Let $S$ be the separator, $S\cap \float_\al = \emptyset$.
%\end{claim}
%\begin{proof}
%	Let $C$ be a floating component, and consider $C\cap S$. Pick an arbitrary vertex in $C\cap S$ to be the landing vertex for the corresponding floating component, for which we use a label in $2|V(\al)|q$. Notice the above pruning argument applies and we can assume any vertex in $C\cap S$ is doubly-constrained by any other vertex in $C\cap S$. Moreover, for each landing vertex, there is at most one nearby short-cycle, hence there is no extra encoding needed for identifying the vertices in $C\cap S$ beyond the landing vertex, giving us a block value of $ 
%	2|V(\al)|q\cdot  \sqrt{\frac{n}{d}}^{|E(C\cap S)| }
%	$.
%	
%	However, consider the separator obtained by popping out $C\cap S$, we pick up a value of $
%	\sqrt{n}^{|V(C\cap S)| }\cdot \sqrt{2|V(\al)|q}
%	$
%	where we note that any vertex doubly-constrained by the landing vertex of $C\cap S$ is also fixed (up to cyclic rotation) and there is no encoding factor needed beyond the landing factor. Ignoring the $\sqrt{2|V(\al)|q}$ gap, notice the separator value with $C\cap S$ is dominating unless $|E(C\cap S)|- |V(C\cap S)| \geq \frac{|E(C\cap S)|}{\log_d n}$.
%\end{proof}
%

\subsubsection{Not too many excess edges outside $S$}\label{sec:not-too-many-exc}
We remind the reader that $\sqrt{d}^{|\exc(F)|}$ is an artifact of our encoding since we encode a potential direction for future unforced return that may be incurred due to the excess edge, however, we point out that this is not too terrible a cost to pay as in any optimal labeling, there cannot be too many $\exc(F)$ edges, and we can handle the blow-up via edge-decay in the optimal labeling. \begin{proposition}
	Let $\calL$ be a locally optimal labeling, and $\exc(F)$ be the number of $F$ edges that lead to visited vertices when we consider a BFS from $S$,  \[ 
	\exc(F)< \lceil \frac{|F\setminus \exc(F)|}{\log_d n}\rceil
	\]
\end{proposition}
\begin{proof}
This follows from the optimality of SMVS, consider the new separator formed by including all vertices reached by $F$ edges, which gives us a change of $
\sqrt{n}^{-|F\setminus \exc(F)| } \cdot \sqrt{\frac{n}{d}}^{|F|}<1
$.
\end{proof}

	
\subsubsection{Wrapping up block value bound}
We are now ready to wrap up our bound for the block value.
\begin{proposition}
	For any irreducible locally optimal labeling $\calL$, let $S$ be its corresponding separator, \[		\vtxcost(\calL)\cdot \edgeval(\calL) \leq  (1+\eps)^{E(\al)}\cdot \sqrt{n}^{|V(\al)\setminus S|}\cdot \left(\sqrt{\frac{n}{d}}\right)^{|E(S)|}\cdot \dang(\al\setminus S)\cdot \float(\al )\cdot \sqrt{n}^{\mathsf{iso}(\al)}
	\]
	with \[ 
	\dang(\al\setminus S) \leq \prod_{b_i\in \branch(\al\setminus S)}\min \left(\sqrt{d}^{|b_i|}, 2|V(\al)|q_\al\right)
	\]
	and 
	\[
	\float(\al) = \left(2|V(\al)|q_\al \right)^{|\float_\al| }
	 \]
	 where $|\float_\al|$ is defined to be the number of floating components in $\al$, and $\iso$ the number of isolated vertices.
\end{proposition}
\begin{proof}
Recalling the factors accounted from above, 
	\begin{enumerate}
  	\item Each vertex outside $S$ contributes a factor of $\sqrt{n}$  (via \cref{sec:factors-of-root-n});
	\item Each vertex in $S$ is doubly constrained by the boundary of $S$ (via \cref{sec:pruning-superfluous-H});
	\item Each edge receiving an $H$ label is in $E(S)$ and contributes a value of at most $\sqrt{\frac{n}{d}}$;
	\item For dangling vertices, we pick up an additional dangling factor $\dang(\al\setminus S)$; each floating component comes with an extra $2|V(\al)|q_\alpha$ factor captured by $\float(\al)$;	\item  Each excess $F$ edge that leads to visited vertices incur an extra cost of $d$ for the potential unforced return it may induce, however, this is subsumed by edge decay (via \cref{sec:not-too-many-exc}).
	\end{enumerate} 

\end{proof}


\paragraph{Bounding the number of maximal value labelings}
To complete our norm bound, it remains for us to bound the number of maximal value labeling, and a naive bound would be $3^{E(\al)}$ by specifying the edge label for each edge, while we notice this can be improved to $3^{|V(\al)\setminus (\iso_\al\cup  U_\al\cap V_\al)|}$ as it suffices for us to indicate whether each vertex is inside the separator, and whether it is reached using an $H$ edge. Moreover, each vertex in $U_\al\cup V_\al$ is by definition inside the separator while vertex in $\iso_\al$ is bound to be outside the separator (otherwise giving a $2|V(\al)q/n$ gap from the maximal value). 

 The following corollary is then immediate once we maximize over any block labelings, \begin{corollary} 
For any $\eps>0$, any shape $\al$,we can bound its block value by\begin{align*}
	B_q(\al)&\coloneqq   \cdot 3^{|V(\al)\setminus (\iso_\al\cup  U_\al\cap V_\al)|} \cdot   \max_{\calL} \vtxcost(\calL)\cdot \edgeval(\calL) \\&\leq 3^{|V(\al)\setminus (\iso_\al\cup  U_\al\cap V_\al)|} \max_{S:\text{separator}}\cdot \sqrt{n}^{|V(\al)\setminus S|}\cdot \left(\sqrt{\frac{n}{d}}\right)^{|E(S)|} \cdot \dang(\al\setminus S)\cdot \float(\al)\cdot \sqrt{n}^{\iso_\al}
\end{align*}
\end{corollary}

\begin{lemma}\label{lem:shape-walk-val}
Given edge labeling on $t$-blocks $B_1,\dots, B_t$ for some $t\leq q_\al $, let $\vtxcost_t, \edgeval_t$ denote the vertex-cost and edge-value at the end of the $t$-th block,  \[ 
\vtxcost_{q} \cdot \edgeval_{q} \leq \sqrt{n}^{|U_\al|+|V_\al|}\cdot  B_q(\al)^{2q}
\]  
%Moreover, if there are $s$ singleton edges in the first $t$ blocks, the above bound can be improved to \[ 
%\vtxcost_{t} \cdot \edgeval_{t} \leq n^{|U_\al|}\left(\max_{S:\text{separator}}  \sqrt{n}^{2(|V(\al)|-|S|)}\left(\frac{n}{d}\right)^{|E(S)| }\right)^{t} (\singdecay)^s
%\]
\end{lemma}
\begin{proof}
	To see the above bound, first considering traversing from the direction of $U_\al\rightarrow V_\al$. And note that we can bound $\vtxcost_q\cdot \edgeval_q\leq n^{|U_\al|}\cdot B_q(\al)^{2q}$ by induction. Traversing the other way gives us $\vtxcost_q\cdot \edgeval_q \leq n^{|V_\al|} \cdot B_q(\al)^{2q}$. Taking the average then yields the desired bound.
		

%		 Taking the $\frac{1}{2q}$-th root gives us the desired upper bound of \[ 
%	 \max_{\calL:\text{labeling}} (\vtxcost(\calL)\cdot \edgeval(\calL))^{2q}\leq \max_{S:\text{separator}}\left(\sqrt{\frac{n}{d}}\right)^{|E(S)|}\cdot \sqrt{d}^{\dang}\cdot (2|V(\al)|q)^{\float }
%	 \]
%	 provided $n^{\frac{|U_\alpha|}{2q}}<1+o(1)$, which would suffice if we take $q=\Theta(|U_\al|\log^2 n)$. By symmetry, we can also apply this argument on $\al^T$, which would require us to have $n^{\frac{|V_\al|}{2q}|}<1+o(1)$, and hence we can take the average by setting $q=\Theta(\sqrt{|U_\al|\cdot |V_\al| }\log^2n )$.
\end{proof}


This completes our discussion for order-tuple indexed graph matrix. That being said, we work with a slightly more challenging setting in which our matrix is indexed by set, and this shall be our topic for the upcoming section.

%%

%\subsection{Wrapping up}
%We now show our main theorem from the above lemmas. For any $\eps>0$ and $q\in \N$, \begin{align*}
%	\Pr[\|M_\al\|> B_q(\al)+\epsilon ] &\leq \Pr[\Tr \left(M_\al M_\al^T \right)^q> (B_q(\al)+\epsilon)^{2q} ] \\
%	&\leq \frac{\E\left[\Tr\left(M_\al M_\al^T)^q\right)\right] }{(B_q(\al)+\eps)^{2q}}\\
%	&\leq \frac{n^{|U_\alpha|}B_q(\al)^{2q} }{(B_q(\al)+\eps)^{2q} }  &\text{(by main lemma )}\\
%	&\leq 
%\end{align*}


==> middle_shape.tex <==

	\section{Middle shape $Q_0$ is PSD }
	We recall the main lemma of our section,
%	\begin{lemma}[Middle shape $Q_0$ is PSD]\label{lem: midshape-psd}
%		\[ \sum_{\tau \in \midshape} \lambda_{\tau} M_{\tau}\otimes H_\tau \succeq 0   \]
%	\end{lemma}
%\midshapepsd*	
Concretely, as unpacked in the last section, our goal would be to show for any color-shape $(\psi, \beta)$ pair in which $\psi$ is a diagonal shape, $\beta$ a coloring of $\psi$, and any glyph $\Glyph$ of color shape $(\psi,\beta)$ that is PSD, \begin{align*} 
 &\Bigg(\lambda_{\psi}\cval{E(\psi)}_{\beta}\cdot M_{(\Glyph,\beta)} + \sum_{\substack {(\psi',\beta')\\ \Glyph': \text{that has a charging path  to } \Glyph } } \lambda_{\psi'}\cval{E(\psi')}_{\beta'}\cdot M_{(\Glyph',\beta')}\\&+ \sum_{\substack{(\tau,\beta')\in \midshape \\ (\tau,\beta') \text{ has a charging path to } \Glyph }} \lambda_{\tau}\cval{E(\tau)}_{\beta'} M_{(\tau,\beta')} \Bigg) \succeq 0
\end{align*}
Recall that $\Glyph$ of color shape $(\psi,\beta )$ is a PSD glyph only if it is a maximal glyph s.t. $\yes(\Glyph) = E(\psi)$, we have \begin{align*} 
\lambda_{\psi}\cval{E(\psi)}_\beta \cdot M_{(\Glyph,\beta)} &= \left(\eta\cdot \sqrt{\frac{d}{n}}\right)^{E(\psi)} \cdot \left(\frac{1}{\sqrt{k}} \right)^{|U_\psi\Delta V_\psi |} \cdot \cval{(E(\psi)}_\beta\cdot \left(\sqrt{\frac{n}{d}}\right)^{E(\psi)} \cdot \Id_{(\Glyph,\beta)}\\
&=\eta^{E(\psi)} \cdot \Id_{(\Glyph,\beta)}
\end{align*}

	
 \subsection{Structure of middle shape}		
%	 				 For starters, we first consider the case in which $\tau$ has no edges interior in $U_\tau$ and $V_\tau$, $E(U_\tau)=E(V_\tau)=\emptyset $ and $U_\tau\cap V_\tau=\emptyset$. Consider the graph $P(\al)$ formed by vertices $U_\al\cup V_\al$, for each pair of vertices $u\neq v\in U_\al\cup V_\al$, we connect an edge between $(u,v)$ if there is a ''simple'' path (that does not use any edge more than once) of length at most $\frac{\log_d n}{2}$ from $u$ to $v$ in $\al$. Notice by construction, $u,v$ can be both from $U_\al$ or $V_\al$, however, it can be ruled out by the following claim,
	 	It turns out crucial to understand the graph structure that arises in our middle shape. And we will show in this section that they are essentially a matching between vertices in $U_\tau \Delta V_\tau$, with each matching edge $(u,v)$ a long path in $\tau$ between $u\in U_\tau\setminus V_\tau, v\in V_\tau\setminus U_\tau$.	 Towards this end, we first ignore the vertices in $U_\tau\cap V_\tau$ and edges in $E(U_\tau) \cup E(V_\tau)$, and form a graph $P(\tau)$ on vertices $U_\tau\Delta V_\tau$, and connect an edge between any pair of vertices if there is a simple path in $\tau$ of length at most $0.4\log_d n$. We first observe the graph is bipartite.
		 \begin{claim}
		 	For any non-trivial middle shape $\tau$, the graph $P(\tau)$ is bipartite on the vertices $U_\tau\Delta V_\tau$ , with bipartition given by $U_\tau\setminus V_\tau $ and $V_\tau\setminus U_\tau$. When $U_\tau\cap V_\tau \neq \emptyset$, the intersected vertices fall into both partitions.
		 \end{claim}
		 \begin{proof}
		 Suppose there is an edge from $u$ to $v$ in $P(\tau)$ for both $u,v\in U_\tau$, there is a path of length at most $t\leq \frac{\log_d n}{2}$ from $u$ to $v$ in $\tau$. However, if we include every vertex on the path into the SMVS, we have a change of \[
		 \sqrt{n}^{-t}\sqrt{\frac{n}{d}}^{t+1}\gg 1
		  \]
		  given $t\leq \frac{\log_d n}{2}$, which violates our assumption that $U_\tau$ is the SMVS.
		 \end{proof}
		 A similar argument reveals that the bipartite graph is a matching,
		 \begin{claim}\label{claim: middle-shape-matching}
		 	The bipartite graph $P(\tau)$ is a matching.
		 \end{claim}
		 \begin{proof}
		 Suppose there is some vertex $u\in U_\tau$ with $2$ neighbors $v_1,v_2\in V_\tau$, consider the path SMVS formed by including $V_\tau \cup \{u\}$  as well as any vertex on the path in $\tau$, let $t_1, t_2$ be the number of vertices the simple paths pass through before hitting $v_1$ and $v_2$, we have a change of \[
		 \sqrt{n}^{-(t_1+t_2+1)}\sqrt{\frac{n}{d}}^{t_1+t_2+2}=\sqrt{n}\cdot \left(\frac{1}{\sqrt{d}}\right)^{t_1+t_2+2}\gg 1
		  \] 
		  Again, we have a contradiction to the maximality of the SMVS we start with.
		 \end{proof}
%		 Fix an arbitrary order to traverse edges of $\tau$ by the non-backtracking paths from $U_\tau$ to $V_\tau$. Let $e$ be the number of edges in $E(\tau)$ that leads to visited vertices in $V(\tau)\setminus (U_\tau\cup V_\tau)$, and let $r$ be the number of edges in $E(\tau)$ that leads to vertices in $V_\tau\setminus U_\tau$.
		 By contracting each ''not-too-long'' path in $\tau$ from $U_\tau\setminus V_\tau$ to $V_\tau \setminus U_\tau$, it is possible some edges between vertices in $V(\tau)\setminus (U_\tau\cup V_\tau)$ are ignored. However, those edges can also be controlled.
		 \begin{claim}
		 	Let $\exc(P,\tau)$ be the set of edges in $E(\tau)\setminus (E(U_\tau)\cup E(V_\tau)) $ that is not on any simple path between $U_\tau\setminus V_\tau$ and $V_\tau\setminus U_\tau$ in the paths corresponding to the matching edges of $P$, there is a  
		 \end{claim}
		 \begin{corollary} The excess edges in $E(\al)$ can be handled by edge decay,
		 	 \[
		 	e\ll \frac{|E(\al)\setminus( E(U_\al)\cup E(V_\al))|}{\log_d n}
		 	 \]
		 \end{corollary}
\subsection{Charging diagram for middle shapes}
	Our charging strategy for middle shape is encapsulated in the following diagram,\\\\ 
\begin{center}
 \begin{tikzpicture}[->,shorten >=1pt,auto,node distance=4cm,
                thick,main node/.style={circle,draw,font=\Large\bfseries}]
  \node[main node] (1) {$U_\tau= V_\tau$};
  \node[main node] (2) [left of=1] {$U_\tau\neq V_\tau$};
  \path
  (2) edge node [above] {$\phi$} (1)
      (1) edge [loop above] node {\text{Glyph casing on } $\lambda_{\tau,\beta}$ and $E(U_\tau)$} (1);
\end{tikzpicture}
\end{center}


\subsection{From off-diagonal to diagonal shapes}


This subsection corresponds to the first arrow in our charging strategy. 
%Fix $\psi$ to be a diagonal shape $U_\psi = V_\psi$, and let $\tau$ be any non-trivial middle shape s.t. $\phi(\tau) = \psi$, i.e. $U_\tau = U_\psi$ or $V_\tau= V_\psi$, and $E(\tau)\setminus E(U_\tau\cap V_\tau)\neq \emptyset$. For technical reasons, instead of working with shapes and a coloring matrix, we will instantiate the colors on the boundaries, specifically, we will work with color-shape $(\psi,\beta)$ and $(\tau, \beta')$  s.t. $U_\psi =U_\tau, \beta_{U_\psi} = \beta'_{U_\tau}=S\subseteq [k] $ or $V_\psi = V_\tau, \beta_{V_\psi} = \beta'_{V_\tau}=T\subseteq [k] $.   
%

As a first step, let $\widetilde{\tau}$ be a non-trivial (color) middle shape s.t. $U_{\widetilde{\tau}}\neq V_{\widetilde{\tau}}$ or there is some middle vertex in $V(\tilde{\tau})$, we first factor out edges inside $U_{\widetilde{\tau}}\cap V_{\widetilde{\tau}}$ (and their corresponding coefficients), and let $\tau$ be the shape $\widetilde{\tau}$ with edges inside $U_{\widetilde{\tau}}\cap V_{\widetilde{\tau}}$ removed. Our strategy for these shapes would be to argue once the edges in $E(U_\tau\cap V_\tau)$ are factored out, we can crudely charge these terms to the trivial shape $\trivial(U_\tau)$ and $\trivial(V_\tau)$, whose definitions are recalled in the following,
\begin{definition}[Trivial shape]
	For any shape $\tau$, we define the trivial shape $\trivial(U_\tau)$ to be the shape with\[
	U_{\trivial(U_\tau)}=V_{\trivial(U_\tau)}=U_\tau\], and\[ E(\trivial(U_\tau))=\emptyset 
	 \] The definition extends for $V_\tau$ naturally.
\end{definition} 
%\begin{claim}
%	\begin{align*}
%		\begin{bmatrix}
%			\lambda_{U_\tau} M_{\Id_{U_\tau}}\otimes H[S,S], &\lambda_{\tau}M_\tau\otimes H[S,T]\\
%			\lambda_{\tau}M_\tau^T\otimse H[S,T}^T, & \lambda_{V_\tau} M_{\Id_{V_\tau}} \otimes H[T,T]
%		\end{bmatrix}
%	\end{align*}
%\end{claim}
%%
%\begin{claim}
%	\begin{align*}
%		\begin{bmatrix}
%&\lambda_{\Id_{U_{W(\tau)}}}M_{(\Id_{U_{W(\tau)}},\beta(U_\tau))} , &\lambda_{W(\tau), \beta} M_{\tau,\beta}\\\\
%&\lambda_{W(\tau)}M_{\tau, \beta}^T, &\lambda_{\Id_{V_{W(\tau)}}}M_{(\Id_{V_{W(\tau)}},\beta(V_\tau))}
%		\end{bmatrix} 		 \succeq 0 
%	\end{align*}
%\end{claim}
%\begin{proof}
%Noticing \[ 
%\lambda_{\Id_{U_{W(\tau)}}} = \lambda_{\Id_{V_{W(\tau)}}} = 1
%\]
%and 
%let $S=\beta(U_\tau)\subseteq [k], T=\beta(V_\tau)\subseteq [k]$, we have \[
%M_{(\Id_{U_{W(\tau)}},\beta(U_\tau))} = M_{\Id_{U_{W(\tau)}}} \otimes  
% \]
Recall that our strategy would be to show 
  	\begin{align*}
 		\begin{bmatrix}
 			&\left|\lambda_{\Id_{U_\tau}} M_{\Id_{U_\tau}} \otimes H_{\Id_{U_\tau}}\right|, &\lambda_\tau M_\tau \otimes H_\tau\\
 			\\
 			& \lambda_{\tau}M_\tau^T\otimes H_\tau^T, &\left|\lambda_{\Id_{V_\tau}} M_{\Id_{V_\tau}}\otimes H_{\Id_{V_\tau}}\right|
 		\end{bmatrix}\succeq 0
 	\end{align*}
Notice for middle shape $\tau$, the above can be greatly simplified as  \[ 
 \lambda_{\trivial(U_\tau)} =   \lambda_{\trivial_{V_\tau}} = 1  \]
 and \[ 
  M_{\trivial_{U_\tau}}  = M_{\trivial_{V_\tau}} = \Id_{\trivial(\tau)}
 \]
 where $\trivial(\tau)$ is well-defined since $|U_\tau|=|V_\tau|$ for a middle shape $\tau$, and $ H_{\Id_{U_\tau}}$ is simply an identity matrix of dimension $k^{|U_\tau|}\times k^{|U_\tau|}$. Hence, it suffices for us to show
\begin{lemma}
	\[ 
\|\lambda_{\tau} M_\tau\otimes H_\tau\| =\left(\frac{1}{\sqrt{k}}\right)^{|U_\tau\Delta V_\tau |} \left(\eta\sqrt{\frac{d}{n}}\right)^{|E(\tau)|} B(M_\tau)\cdot \|H_\tau\| \leq o(1)
\]
where $B(M_\tau)$ is our proxy to the matrix norm bound.
\end{lemma}
\begin{proof}

To unpack the above inequality and motivate our upcoming section, we notice \[ 
LHS = \left(\frac{1}{\sqrt{k}}\right)^{|U_\tau\Delta V_\tau|}\left(\eta\cdot\sqrt{\frac{d}{n}} \right)^{|E(W(\tau))|}B(M_{\tau})\cdot\| H_{\tau}\|\cdot \slack \ll 1
\]
To upper bound the LHS, we will split the terms into two groups, and bound

 \[
 \left(\frac{1}{\sqrt{k}}\right)^{|U_\tau\Delta V_\tau|} \|H_\tau\| \cdot \slack_1 <k^{|E(U_\tau)\Delta E(V_\tau)|}
\]
and \[ 
\left(\eta\cdot\sqrt{\frac{d}{n}} \right)^{|E(\tau)|}\cdot B(M_{\tau})\cdot \slack_2 < \left(\sqrt{\frac{d}{n}}\right)^{|E(U_\tau)\Delta E(V_\tau)|}
\]
%To unpack a little bit,
%	 our strategy for this section is standard in previous works, which is to pull out the ''trivial'' shapes, $\tau_\text{trivial}$ s.t. $E(\tau) = \emptyset, U_\tau=V_\tau$. This corresponds to the diagonal of the moment matrix, and as it appears with positive coefficient $(\frac{1}{\sqrt{k}})^{|U_\tau\Delta V_\tau |} = 1$, and $H_\tau$ is essentially an identity matrix on the (square) block with non-zero entries at $k^{|U_\tau|}\times k^{|V_\tau|}$.	 \[ 
%	\sum_{\tau\in \midshape, \text{trivial}} \lambda_\tau M_\tau \otimes H_\tau =\Id
%	 \]
%	  We will be using it as our PSD mass and charge other shapes to it. Concretely, our goal is to show \[
%	\left\| \sum_{\substack{\tau\in \midshape \\ U_\tau\cap V_\tau =\emptyset\\ E(U_\tau)=E(V_\tau)=\emptyset }} \lambda_\tau M_\tau \otimes H_\tau \right\| \leq o(1)
%	 \]
%	 which would imply \[ 
%	 \sum_{\tau\in \midshape, {\text{trivial}}} \lambda_\tau M_\tau \otimes H_\tau +  \sum_{\substack{\tau\in \midshape\\ U_\tau\cap V_\tau =\emptyset\\ E(U_\tau)=E(V_\tau)=\emptyset } } \lambda_\tau M_\tau \otimes H_\tau \succeq (1-o(1)) \Id
%	 \]
%In our new language, the strategy here is simply setting \[ 
%\phi(\lambda, \tau) = (\lambda_{\Id_{U_\tau}}, \Id_{U_\tau}, \text{slack}) 
%\]
%and we will then verify in the remaining subsection the conditions for the charging function, in particular, its first condition.
		 \subsubsection{Factors of $k$}
		In this section, we will show for each non-trivial middle shape $\tau$, the factor in $k$ can be controlled; concretely, we want to show
		\begin{lemma}\label{lemma: mid-shape-k}
			For any non-trivial middle shape $\tau$ with no internal edges in $E(U_\tau\cap V_\tau)$,
			\[ 
			(\frac{1}{\sqrt{k}})^{|U_\tau\Delta V_\tau|}\|H_\tau\| \leq 2^{|V(\tau)\setminus U_\tau|}\cdot k^{|E(U_\tau)\Delta E(V_\tau)|}
			\]
%			 \[
%		(\frac{1}{k})^{\frac{|U_\tau \Delta V_\tau|}{2}} H_{W(\tau)}[S,T] \leq 2^{|V(\tau)\setminus U_\tau|}
%		 \]
		\end{lemma} 		 We are now ready to bound the factor of $k$. Let $S,T \subseteq [k]^{|U_\tau|}$ denote the coloring to each boundary, by a row sum bound, 
		 \begin{align*}
		 	\max_{S} \sum_{T}\left|H_\tau[S,T]\right| 		 	&\leq \max_{S\subseteq [k]^{U_\al}} \sum_{T\subseteq [k]^{V_\al}} \left| \sum_{\substack{\beta: V(\al)\setminus (U_\al\cup V_\al)\rightarrow [k] \\ \text{coloring vertices outside the boundary }} }  \beta(\al) \cdot \left(\frac{1}{k}\right)^{|V(\al)\setminus (U_\al\cup V_\al)| } \right|\\
		 	&\leq \max_{S\subseteq [k]^{U_\al}}\sum_{\substack{\beta: V(\al)\setminus (U_\al)\rightarrow [k] \\ \text{coloring all vertices except } U_\alpha} }  \left|\beta(\al) \cdot \left(\frac{1}{k}\right)^{|V(\al)\setminus (U_\al\cup V_\al)| }   \right|\\
%		 	&\leq \max_{S\subseteq [k]^{U_\al}} \sum_{T\subseteq [k]^{V_\al}} \left| \sum_{\substack{\beta: V(\al)\setminus (U_\al\cup V_\al)\rightarrow [k] \\ \text{coloring vertices outside }  \right|
&\leq 2^{|V(\al)\setminus U_\tau|}\cdot k^{e}k^{r} k^{|E(U_\tau)\Delta E(V_\tau)|}
		 \end{align*}
		 where $r$ is the number of edges incident to $V_\tau$, and $e$ the number of excess edges in $V(\tau)$. To see this, we appeal to the following scheme in bounding the sum over colorings of the middle vertices: for each (non-floating) component connected to some vertex $u$ in $U_\alpha$, \begin{itemize}
		\item Fix an ordering to traverse the edges in the connected component from $u$;
		\item For each edge, use a label in $[2]$ to decide whether the destination vertex has the same color as the origin unless it leads to a visited vertex;
		\item If the edge leads to a new vertex not in $V_\al$, we either pick up a value of $k-1$ from the edge, or we pick up $k-1$ choices of the color; either way, we can charge it to the vertex decay of $\frac{1}{k}$ from the vertex factor of the new vertex;  
		\item For each edge leading to visited vertex, we bound its value by $k$.
	\end{itemize}
%	For each floating component, the encoding is largely identical as we can pick a vertex in the floating component arbitrarily and encode as above except till the last step we no longer have the vertex decay from the starting vertex of $\frac{1}{k}$ in the connected component (as the first vertex no longer has its color fixed).
		 Combining the the norm bound with the vertex coefficient, we have \begin{align*}
		 	\left(\frac{1}{k}\right)^{\frac{|U_\al\Delta V_\al| }{2}}\|H_\al\|&\leq \left(\frac{1}{k}\right)^{\frac{|U_\al\Delta V_\al| }{2}} 2^{|V(\al)\setminus (U_\tau \setminus V_\tau )|}\cdot k^{e}k^{r}
		 	\\&\leq k^e 2^{|V(\al)\setminus (U_\tau \setminus V_\tau)| }
		 \end{align*}
		 where the second inequality follows from $r= \frac{|U_\tau\Delta V_\tau|}{2} $ as the graph is a matching (modulo excess edges).
		
\subsubsection{Factors of $n$}
In this section, we are interested in bounding the factor of $n$, 
\begin{lemma} For any non-trivial middle shape $\tau$ s.t. $E(U_\tau\cap V_\tau)=\emptyset$, 	 \[ 
\left(\eta\cdot\sqrt{\frac{d}{n}} \right)^{|E(\tau)|}\cdot B(M_{\tau})\cdot \slack_2 < \left(\sqrt{\frac{d}{n}}\right)^{\frac{|E(U_\tau)\Delta E(V_\tau)|}{2}}
\]
\end{lemma}
\begin{proof}
We first unpack our matrix norm bounds for middle shape $\tau$, \begin{align*}
	B(M_\tau) = c^{E(\tau)} \max_{S:\text{separator}} \sqrt{n}^{V(\tau)\setminus V(S)} \left(\sqrt{\frac{n}{d}}\right)^{E(S)}
\end{align*}

It suffices for us to consider first the edge case when $E(U_\tau))\Delta E(V_\tau)=\emptyset$. By construction, $(U_\tau, E(U_\tau))$ and $(V_\tau, E(V_\tau))$ are both SMVS for $\tau$, and it suffices for us to fix $S=U_\tau$ as the maximizer for the norm bound. 
	For each vertex outside the separator, it must be connected to $S$, as there cannot be any vertex floating in the middle shape, and as long as it is connected to $S$, we can charge its norm bound factor to the edge connecting to it from $S$ as \[
	\sqrt{n}\cdot \sqrt{\frac{d}{n}}\cdot \eta = \frac{1}{c} <1	 \]
	
	To see the bound for $E(U_\tau)\Delta E(V_\tau) \neq \emptyset$, since we fix $S=U_\tau$ by assumption, each edge in $E(V_\tau)\setminus E(U_\tau)$ does not contribute $\sqrt{\frac{n}{d}}$ to the norm bound as a separator edge while it comes with a $(\eta \sqrt{\frac{d}{n}})$ in the coefficient that would be uncharged,  hence we have \[ 
	\left(\eta\cdot \sqrt{\frac{d}{n}}\right)^{E(\tau)} \cdot B(M_\tau) \leq c^{E(\tau)} (\frac{1}{c_0})^{|V(\tau)\setminus U_\tau|}\eta^{|E(U_\tau)}\left(\sqrt{\frac{d}{n}}  \right)^{\frac{|E(U_\tau)\Delta E(V_\tau) |}{2} }
	\]
\end{proof}
	%		\subsection{Handling interior edges $E(U_\tau)\Delta E(V_\al)$}
%	We will continue to assume $U_\tau \cap V_\tau = \emptyset$ while relax our first assumption that there is no interior edge on both sides. Notice if $(U_\tau, E(U_\tau))$ and $(V_\tau, E(V_\tau))$ are both SMVS, then $|E(U_\tau)|=|E(V_\tau)|$. However, only half of the edges may contribute a factor of $\sqrt{\frac{n}{d}}$ to the norm bound, while all of them may contribute a factor of $k$ to the labeling value in $\|H_\al\|$, as well as a coefficient of $\eta\cdot \sqrt{\frac{d}{n}}$, giving a total of \[ 
%	\left(\sqrt{\frac{n}{d}}\right)^{\frac{|E(U_\al)|+|E(V_\al)|}{2}}\cdot \left(\eta\cdot\sqrt{\frac{d}{n}}\right)^{|E(U_\al)|+|E(V_\al)|}\cdot k^{|E(U_\al)|+|E(V_\al)|} \ll \left(k^2\cdot \sqrt{\frac{d}{n}}\right)^{|E(U_\al)|}
%	\] 
	
%	\subsection{Handling intersection $U_\tau \cap V_\tau$ and $E(U_\tau)\cap E(V_\tau) $}
%	Unfortunately, the previous strategy falls short in handling vertices and edges in the intersection of $U_\tau$ and $V_\tau$. To see this, we notice that each vertex in the intersection no longer comes with $\frac{1}{\sqrt{k}}$ vertex decay, while each edge would still come with a factor $k$ blow-up, leading to a blow up in $k$ when compared to the trivial middle shape. To get around with this issue, we notice each set of intersected edge, is either bringing extra PSD mass (if all edges are actually present in the graph), or some edge is amiss in the random graph sample (which results in a rapid dropping of the norm) and renders it possible to charge to the usual trivial middle shape.
%
%For any non-trivial shape $\tau$ with non-empty interior edges, we start by restricting our attention to $\tau$ with only interior edges, and we will then combine our argument with that of last section to handle $\tau$ with both interior and exterior edges. In this subsection, instead of working with shapes, as we will be ultimately interested in whether certain edge appears in our random graph sample, we will work with ribbons (i.e., shape with vertices labeled in $[n]$), and specifically we will work with color-ribbons as the potentially minus sign from the shape-coloring matrix requires an extra argument to be addressed. 
%
%For starters, we start with $\tau$ s.t. $U_\tau = V_\tau$ but with non-empty interior edges, which correspond the entries that appear in the diagonal of our moment matrix. Let $R$ be a ribbon of shape $\tau$, and $\beta$ a coloring of $U_R\cup V_R$,  \begin{align*}
%	\lambda_{\tau} (M_\tau \otimes H_{\tau})[(U_R, \beta_U), (V_R, \beta_V)] &= \left(\frac{1}{\sqrt{k}}\right)^{|U_\tau \Delta V_\tau|}\cdot \cval{E(\tau)}_{\beta} \left(\eta\sqrt{\frac{d}{n}}\right)^{|E(\tau)|} \cdot \chi_{E(R)}(G) \\
%	&=\cval{E(V_\tau\cap U_\tau)}_\beta \cdot \left(\eta\sqrt{\frac{d}{n}}\right)^{|E(U_R\cap V_R)| }	\cdot \chi_{E(R)}(G)
%	\end{align*}
% \begin{observation}
% 	Let $s\coloneqq |\{e\in E_\tau(U_R\cap V_R): \chi_e(G)=\sqrt{\frac{n}{d}}\} | $ be the number of edges in $E_\tau(U_R\cap V_R)$ that are present in the random graph sample $G$, and let $\crosscol(\beta)\coloneqq |\{e=\{i,j\} \in E_\tau(U_\tau\cap V_\tau): \beta(i)\neq \beta(j)  \} | $ be the number of edges that have endpoints of different color, ,   then \[ 
% 	\lambda_{\tau} (M_\tau \otimes H_{\tau})[(U_R, \beta_U), (V_R, \beta_V)] = (-1)^{|E(\tau)|-s} (-1)^t k^{|E_\tau(U_R\cap V_R)|-t }\cdot  \eta^{|E(U_R\cap V_R)|} \left(\sqrt{\frac{d}{n}}\right)^{|E(\tau)|-2s }
% 	\]
% \end{observation}
%As revealed by the above observation, our charging strategy now needs to depend on the parity of $\eta$ and $t$. \begin{enumerate}
%	\item Notice each missing edge in the random graph sample comes with a decay of $\frac{d}{n}$, we have a large slack for those to charge to the trivial identity and hence we will ignore the sign change coming from missing edges; for the rest of our argument, it suffices to consider $s=|E(U_\tau\cap V_\tau)| $.
%	\item For $\eta>0 $ and even $t$, or $\eta<0$ and odd $t$ the above quantity is positive and provides us with the PSD mass;
%	\item Hence, it remains for us to give a charging argument for even $t$ when $\eta>0$, and odd $t$ for $\eta<0$.
%\end{enumerate}
\subsubsection{Wrapping up}
We are now ready to combine our individual bounds for $k$ and $n$ together. \begin{align*}
	\|\lambda_{\tau}M_\tau\otimes H_\tau\| &= \left(\frac{1}{\sqrt{k}}\right)^{|U_\tau\Delta V_\tau |} \left(\eta\sqrt{\frac{d}{n}}\right)^{|E(\tau)|} B(M_\tau)\cdot \|H_\tau\|\\
	&\leq \left((\frac{1}{\sqrt{k}})^{|U_\tau\Delta V_\tau|}\|H_\tau\| \right)\left(\left(\eta\sqrt{\frac{d}{n}}\right)^{|E(\tau)|} B(M_\tau)  \right) \\&\leq 2^{|V(\tau)\setminus U_\tau|}\cdot k^{|E(U_\tau)\Delta E(V_\tau)|} \cdot c^{E(\tau)} (\frac{1}{c_0})^{|V(\tau)\setminus U_\tau|}\eta^{|E(U_\tau)}\left(\sqrt{\frac{d}{n}}  \right)^{\frac{|E(U_\tau)\Delta E(V_\tau) |}{2} }
	\\& \leq o(1)
\end{align*}
provided $c_0>2c$.
\begin{corollary}
	For any non-trivial middle shape $\tau$ s.t. $E(U_\tau\cap V_\tau)=\emptyset$, we can set 
	\begin{align*}
		\phi(\tau) = (\lambda_{\trivial(\tau)}, \trivial(\tau), o(1))
	\end{align*}
	\jnote{the o(1) slack to be plugged in later for counting }
\end{corollary}
\end{proof}
\subsection{Charging diagonal shapes: color-partition and glyph casing}
In this subsection, we restrict our attention to diagonal shapes $\tau$ with no middle vertices $U_\tau=V_\tau=V(\tau)$,  while $E(\tau)$ is potentially non-empty. Notice in the previous section, our analysis goes through without considering the colorings of $U_\tau\cup V_\tau$. However, since we consider diagonal shapes with potential internal edges now, the coloring on the boundaries are going to be important as they determine the corresponding edge coefficient, in particular, they determine whether certain shape on the diagonal comes with positive or negative sign! Hence, we will instantiate color assignment on $U_\tau\cup V_\tau$ from this point, and we here introduce the color-partition,
\begin{definition}[Colro-partition $\cp$]
For a fixed shape $\tau$, for any coloring $\beta: U_\tau\cup V_\tau \rightarrow [k] $ of the boundary vertices $U_\tau\cup V_\tau$, we associate it with a color partition $\calS\in \cp_\tau $ s.t. for any $\beta_1, \beta_2 \in \calS$, there is a permutation $\sigma\in P[k]$ s.t. \[ 
\sigma(\beta_1(v)) = \beta_2(v)
\]
for any $v\in U_\tau\cup V_\tau$ and we let $\cp_\tau$ denote the collection of color-partition for $\tau$.
\end{definition}
For each color partition, we can also define the corresponding shape-coloring matrix for color-partition,\begin{definition}[Shape-coloring matrix for color-partition] 
	Given a shape $\tau$ and $\calS\in \cp_\tau$, we define its corresponding edge-coloring matrix $H_{\tau,\calS}$ as \begin{align*}
		H_{\tau,\calS}[A,B ] = \sum_{\substack{\beta: \text{coloring $V(\tau$)}\\ A\cup B \mapsto \beta \text{ boundary consistent} }} \cval{E(\tau)}_\beta 	\end{align*}
\end{definition}


It should be noted that for $\beta_1,\beta_2\in \calS$ for $S\in \cp_\tau $, each edge in $E(U_\tau\cup V_\tau)$ receive the same pure/cross color relation, where an edge is a pure-color edge if it is between endpoints of the same color, and cross-color otherwise. This allows us to associate each color-partition $\calS$ with $\pure(\calS)$ and $\crosscol(\calS)$,
\begin{definition}[$\pure, \crosscol$ for a color partition]
	For a color-partition $\calS\in \cp_\tau $, let $\pure_\tau(\calS)$ be the number of edges in $E(U_\tau\cup V_\tau)$ whose endpoints receive the same color in $\cp(\tau)$, and $\crosscol_\tau(\calS)$ be the number of those whose endpoints receive different colors. The dependence on $\tau$ is usually ignored.
\end{definition} 

\begin{remark}
	For a diagonal shape $\tau$, and $\calS$ a color-partition, $H_{\tau,\calS}$ is a diagonal matrix of dimension $k^{|U_\tau|}\times k^{|V_\tau|}$, with non-zero entry at $H_{\tau,\calS}[\beta,\beta] = \cval{E(\tau)}_\beta = (k-1)^{\pure(\calS)}\cdot (-1)^{\crosscol(\calS)}$ for $\beta\in \calS$.  
\end{remark}

 To motivate our charging strategy for diagonal shapes, we recall the quantity of interest for a fixed color ribbon $(R,\beta)$ of shape $\tau$, and color partition $\beta\in \calS$ is  given by \[
 \lambda_\tau M_\tau \otimes H_{\tau,\calS} 
  \] 
  with non-zero entry  on the diagonal \begin{align*} &\lambda_\tau M_\tau \otimes H_{\tau,\calS} \left[(U_R,\beta_{U_R}), (V_R, \beta_{V_R}) \right]\\ &=\sum_{\substack{\beta: \text{coloring $V(\tau$)}\\ A\cup B \mapsto \beta \text{ boundary consistent} }}  \left(\frac{1}{\sqrt{k}}\right)^{|U_\tau\Delta V_\tau|} \left(\frac{1}{k} 	\right)^{|V(\tau)\setminus (U_\tau\cup V_\tau)| } \cval{E(\tau)}_\beta\cdot \edgeco^{E(\tau)} \cdot \chi_{E(R)}(G)\\
  &= (k-1)^{\pure(\calS)}\cdot (-1)^{\crosscol(\calS)} \cdot \eta^{E(\tau)} \left(\sqrt{\frac{d}{n}}\right)^{E(\tau)} \cdot \chi_{E(R)}(G)
  \end{align*}
where the second equality follows from $\tau$ a diagonal shape with no vertex outside $U_\tau\cup V_\tau$ and $U_\tau=V_\tau$.
 It is easy to notice that $\chi_{E(R)}(G)$, the instantiation of the random graph sample, is crucial here. Consider an edge $e\in \chi_{E(R)}(G)$, if the edge appears in the random graph sample, it would contribute a $\sqrt{\frac{n}{d}}$ (which would exactly cancel out with edge coefficient modulo the $\eta$ slack); however, it would contribute a $-\sqrt{\frac{d}{n}}$ otherwise, which if combined with the corresponding edge coefficient, would give us a double decay in the magnitude of $\sqrt{\frac{d}{n}}$, rendering a gap to apply magnitude bounds to the ribbon with the absent edge removed. This motivates us to work with a finer partition of shapes, glyphs, which indeed take into account the instantiation of the edges here. To give an overall picture, our strategy for handling diagonal shapes is summarized as 
\begin{enumerate}
	\item Notice each missing edge in the random graph sample comes with a decay of $\frac{d}{n}$, we have a large slack for those to charge to the trivial identity and hence we will ignore the sign change coming from missing edges;	\item For $\eta>0 $ and even $\crosscol(\calS) $, or $\eta<0$ and odd $\crosscol(\calS)$ the above quantity is positive and provides us with the precious PSD mass;
	\item Hence, it remains for us to give a charging argument for even $\crosscol(\calS) $ when $\eta>0$, and odd $\crosscol(\calS) $ for $\eta<0$.
\end{enumerate}
\subsubsection{Diagonal charging for non-maximal $\text{Yes}(\calQ)$}
Consider $\Glyph=(\tau, \calQ, \calS)$ a (color)-glyph with $\text{Yes}(\calQ) \neq E(\tau)$ and $\calS$ a color-partition for $\tau$. Let $e\in E(\tau)$ be an edge absent in $\calQ$, and let $\Glyph_{-e} =\left(\tau\setminus\{e\}, \text{Yes}(\calQ), S\right)$, 
  \[ 
\phi( \lambda_\tau, \Glyph) = (\lambda_{\tau\setminus\{e\}}, \Glyph = \left(\tau\setminus\{e\}, \text{Yes}(\calQ), S\right), \frac{d}{n})
\]
It suffices for us to verify that \begin{align*}
%	\begin{bmatrix}
%	&|\lambda_{\tau\setminus \{e\}} \cdot M_{\Glyph_{-e}} \otimes H_{\tau\setminus\{e\}, \calS} |, &\lambda_\tau }
%	 \end{bmatrix}
 \left| \lambda_{\tau\setminus{e}} M_{\Glyph_{-e}}\otimes H_{\tau\setminus\{e\} ,\calS}  \right| \succeq  \slack\cdot \lambda_\tau \cdot M_\Glyph\otimes H_{\tau,\calS}
 \end{align*}
 To see this, notice for any non-maximal glyph $\Glyph$ with $e\in E(\tau)$ missing in the random graph sample, we have \begin{align*}
 \left|\lambda_{\tau} M_{\Glyph} \otimes H_{\tau,\calS}\right| &= \left|\left(\eta\cdot \sqrt{\frac{d}{n}}\right)^{E(\tau)} M_{\Glyph}\otimes H_{\tau,\calS}\right| \\
 &=\left|(-\sqrt{\frac{d}{n}})\cdot \left(\eta\cdot \sqrt{\frac{d}{n}}\right)^{E(\tau)} M_{\Glyph-\{e\}} \otimes (\cval{e}_{\calS}\cdot H_{\tau\setminus \{e\} , \calS})\right|\\
 &\leq (k\cdot \frac{d}{n}) \cdot \left| \lambda_{\tau\setminus \{e\}} M_{\Glyph-\{e\}} \otimes H_{\tau\setminus\{e\},\calS} \right|
  \end{align*}
 For the rest of our argument, it suffices to consider maximal glyphs, i.e. those with the set of edges present in the random graph sample $\text{Yes}(\calQ)=E(\tau) $.
\subsubsection{Diagonal charging for $\eta>0$}
 For $\eta>0$, we case on the parity of $\crosscol(\calS)$. For even $\crosscol(\calS)$, the glyph can be used as the PSD mass,
 \begin{claim}
 		For $\tau$ a diagonal shape, if  $|\crosscol(calS)|$ is even and $\eta>0$, then for any maximal glyph $\Glyph$ of shape $\tau$, \[ 
 		\lambda_{\tau} M_\Glyph \otimes H_{\tau, \calS}   \succeq 0
 	 		\]
 	 	In particular, we have \begin{align*}
 	 		\lambda_{\tau} M_\Glyph \otimes H_{\tau, \calS} 	 		&=\eta^{E(\tau)} (k-1)^{\pure(\calS)}\cdot\Id_{\trivial(\Glyph)}\otimes H_{\trivial(\tau), \calS}
 	 	\end{align*}
 	\end{claim}
 	\begin{proof}
 		It suffices to observe that \[ 
 		(k-1)^{\pure(\calS)}(-1)^{\crosscol(\calS)} H_{\trivial(\tau),\calS} = H_{\trivial(\tau),\calS}
 		\]
 		and for a maximal glyph $\Glyph$ of a diagonal shape $\tau$ with $U_\tau=V_\tau=V(\tau)$,\[ 
 		\edgeco^{E(\tau)}M_{\Glyph} = \eta^{E(\tau)}\cdot \Id_{\trivial(\Glyph)}
 		\]
 	\end{proof}
On the other hand, if $|\crosscol(\calS)|$ is odd, we can arbitrarily remove a cross-color edge and charge to the corresponding glyph with that particular edge removed. 
 \begin{claim}
 	If $|\crosscol(\tau,S)|$ is odd and $\eta>0$, for any maximal glyph $\Glyph=(\tau,\calQ)$, let $e\in E(\tau)$ be a cross-color edge picked arbitrarily, then we can set \[ 
 	\phi(\Glyph) = \left(\lambda_{\tau\setminus\{e\}}, \Glyph' = (\tau\setminus \{e\}, \yes(\calQ') = \yes(\calQ), \calS, \eta\right) 
 	\] 
 	In particular, we have \begin{align*}
 		\lambda_{\tau\setminus \{e\} } M_{\phi(\Glyph)} \otimes H_{\tau\setminus\{e\}, \calS} \succeq \slack\cdot \lambda_{\tau} M_{\Glyph} \otimes H_{\tau,\cal{S}} 
 	\end{align*}
 	with $\slack= \frac{1}{2\eta}$.
 \end{claim}
 \begin{proof} Fix shape $\tau$, and its maximal glyph $\Glyph$, $\calS$ a color partition of $\tau$, and let $e$ be a cross-color edge.
 	Notice both matrices are diagonal, and supported over the same entries $(R,\beta)$ for $R$ a $\Glyph$-ribbon and $\beta\in \calS$, hence it suffices for us to compare each non-zero entry on the diagonal. For the RHS, we have \begin{align*}
 		\lambda_{\tau}M_{\Glyph}\otimes H_{\tau,S}[(R,\beta),(R,\beta)] &= \edgeco^{E(\tau)}(k-1)^{\pure(\calS)}(-1)^{\crosscol(\calS)}\cdot \chi_{E(R)}(G) \\
 		&= (-1)\cdot \eta^{E(\tau)}(k-1)^{\pure(\calS)}
 	\end{align*}
 	while for the LHS we have \begin{align*}
 		\lambda_{\tau\setminus \{e\} }M_{\phi(\Glyph)}\otimes H_{\tau\setminus\{e\} ,\calS}[(R,\beta),(R,\beta)] &= \edgeco^{E(\tau)-1}(k-1)^{\pure(\calS)}(-1)^{\crosscol_{\tau\setminus\{e\} } (\calS)}\cdot \chi_{E(R)\setminus\{e\} }(G) \\
 		&= \eta^{E(\tau)-1}(k-1)^{\pure(\calS)}
 	\end{align*}
 	Hence, rearrange, we have \begin{align*}
 		\lambda_{\tau\setminus\{e\}}M_{\phi(\Glyph)}\otimes H_{\tau\setminus\{e\} ,
 		\calS} + \slack\cdot \lambda_{\tau}M_{\Glyph}\otimes H_{\tau,\calS}     &\succeq (1 - \slack\cdot \eta )\cdot\eta^{E(\tau)-1}\Id_{\trivial(\Glyph) } \otimes H_{\tau,\calS} \\
 		&\succeq 0
 			\end{align*}
 			for any $0<\slack< \frac{1}{\eta}$.
 \end{proof}
 
 
\subsubsection{Diagonal charging for $\eta<0$}
For $\eta<0$, given a maximal glyph $\Glyph$ of shape $\tau$, and $\calS$ a color partition of $\tau$,
recall that our quantity of interest $\lambda_\tau M_\Glyph\otimes H_{\tau,\calS} $ is a diagonal matrix with entries\begin{align*} \lambda_\tau M_\Glyph \otimes H_{\tau,\calS} \left[(R,\beta), (R, \beta) \right]&= (k-1)^{\pure(\calS)}\cdot (-1)^{\crosscol(\calS)} \cdot \eta^{E(\tau)} \left(\sqrt{\frac{d}{n}}\right)^{E(\tau)} \cdot \chi_{E(R)}(G)\\
&=(k-1)^{\pure(\calS)}(-1)^{E(\tau)+\crosscol(\calS)}|\eta|^{E(\tau)} \hspace*{12pt} \text{(since $\Glyph$ is maximal)}
  \end{align*}
  for $R$ a $\Glyph$-ribbon, and $\beta\in \calS$. 
Again, we case on the parity of $|E(\tau)| + |\crosscol(\tau, S)|$.
\begin{itemize}
	\item if $|E(\tau)| + |\crosscol(\tau, S)|$ is even, this is a PSD shape;
	\item otherwise, let $e$ be an edge between the same color in $S$, and set \[ 
	\phi(\lambda_{\tau},\Glyph) = (\lambda_{\tau\setminus\{e\}}, \Glyph=(\tau\setminus\{e\}, \text{Yes}(\calQ), S), \frac{\eta}{k-1})
\]
\end{itemize}
For $|E(\tau)| + |\crosscol(\tau, S)|$ even, we have the usual PSD mass.
\begin{claim}
	For $\tau$ a diagonal shape, if$ |E(\tau)| + |\crosscol_\tau(\calS)|$ is even and $\eta<0$, then for any maximal glyph of shape $\tau$,\[ 
	\lambda_{\tau}M_\Glyph\otimes H_{\tau,\calS}\succeq 0
	\]
	In particular,
	\begin{align*}
		\lambda_{\tau}M_\Glyph\otimes H_{\tau,\calS} =(k-1)^{\pure(\calS)} \eta^{E(\tau)}\Id_{\trivial(\Glyph)}\otimes H_{\trivial(\tau),\calS}
			\end{align*}
\end{claim}
However, for $|E(\tau)|+|\crosscol(\tau,\calS)|$ odd, some more work is needed as we now might have a blow-up in a negative direction of magnitude $(k-1)$ from pure-color value, for example, when $|E(\tau)|=1$ and the particular edge is pure-color under $\calS$. To handle this, we need to exploit the relation between $\eta$ and $k$ in the $\eta<0$ regime. Recall that we set our average in-degree to be\[ 
\din =d(1+(k-1)\eta)\geq 0
\]
\begin{fact}
	For $\eta<0$, we have $\eta>-\frac{1}{k-1}$, and hence $|\eta\cdot k|\leq  1$. For simplicity, we will restrict our attention to the regime where $|\eta\cdot k|<\frac{1}{c_\eta}$ for some absolute constant $c_\eta>0$ measures our gap to the boundary.
\end{fact}
Our charging here would be a two-step process. In the first step, we first ask whether there is any edge that is cross-color under $\calS$, and if so, we can apply the argument from the above section with a gap of $\frac{1}{2\eta}$. In the second step, we handle the case where there is no cross-color edge, i.e. $|E(\tau)| = |\pure(\calS)| $ is odd.
\begin{claim}
For $\tau$ a diagonal shape, and $\eta<0$, and $|E(\tau)|=|\pure(\calS)| $ is odd, for any maximal glyph $\Glyph$ with color partition $\calS\in \cp_\tau$, let $e$ be a pure-color edge under $\calS$, we can set \[ 
\phi(\tau) = \left(\lambda_{\tau\setminus\{e\}}, \Glyph'=(\tau\setminus\{e\}, \yes(\Glyph), \calS), \frac{1}{c_\eta}\right) 
\]
In particular, 
\begin{align*}
	\lambda_{\tau\setminus \{e\}} M_{\phi(\Glyph)}\otimes H_{\tau\setminus\{e\}, \calS} \succeq \slack \cdot \lambda_{\tau} M_{\Glyph}\otimes H_{\tau,\calS}
\end{align*}
for $\slack = \frac{1}{c_\eta}$.
\end{claim}
\begin{proof}
	Again, we start by fixing a diagonal shape $\tau$, its maximal glyph $\Glyph$ and $\calS\in \cp_\tau$ a color partition. Let $e$ be a pure-color edge under $\calQ$, we notice both matrices are diagonal and supported over the same entries $(R,\beta)$ for $R$ a $\Glyph$-ribbon and $\beta\in \calS$, and it remains to compare each non-zero entry on the diagonal. For the RHS, \begin{align*}
		\lambda_{\tau}M_{\Glyph} \otimes H_{\tau,\calS}[(R,\beta),(R,\beta)] &= \edgeco^{E(\tau)}(k-1)^{\pure(\calS)}\cdot \chi_{E(R)}(G)
		\\&=\eta^{E(\tau)}(k-1)^{\pure(\calS)}
	\end{align*} 
	 For LHS, we have \begin{align*}
	 	\lambda_{\tau\setminus\{e\}}M_{\phi(\Glyph)}\otimes H_{\tau\setminus\{e\} ,\calS} &= \edgeco^{E(\tau)-1}(k-1)^{\pure_\tau(\calS) - 1}\chi_{E(R)\setminus\{e\}}(G)\\
	 	&=\eta^{E(\tau)-1}(k-1)^{\pure_{\tau}(\calS)-1}
	 \end{align*}
	 Rearranging gives us 
	 \begin{align*}
	 	\lambda_{\tau\setminus\{e\}}M_{\phi(\Glyph)}\otimes H_{\tau\setminus\{e\},\calS} + \lambda_{\tau}M_{\Glyph}\otimes H_{\tau,\calS}& \succeq (1-\slack\cdot\eta\cdot k)\eta^{E(\tau)-1}\Id_{\trivial(\Glyph)}\otimes H_{\tau,\calS} \\&\succeq 0  
	 \end{align*}
	 provided $|\slack|< \frac{1}{k\cdot\eta} $
\end{proof}

%
%\begin{lemma} 
%For any non-trivial middle shape $\tau$,	 let $R_\tau$ be a ribbon of shape $\tau$, with $S=U_R\cap V_R \subseteq [n]$, let $\beta_S$ be a coloring of $S$,  let $t=|E_\tau(U_\tau \cap V_\tau)|$ be the number of interior edges, and let $s\coloneqq |\{e\in E_\tau(U_R\cap V_R): \chi_e(G)=\sqrt{\frac{n}{d}}\} | $ be the number of edges in $E_\tau(U_R\cap V_R)$ that are present in the random graph sample $G$, then\end{lemma}
	\subsection{Counting non-trivial middle shapes}
	\begin{proof}[Sketch:]
		want a bound of $c^{|E(\al)|}$.
	\end{proof}


==> norm_bound.tex <==
%\input{main-thm}
%\input{preliminaries}
%%\input{new-prelim}
%\input{blockwalk_overview}
%\input{edgeval}
%\input{maximal-value-labeling}
%%\input{return-factor}
%%\input{automorphsm-factor}
%\input{autfactor-augmented-ribbon}

%\input{sparse_trace_method/main-thm}
%\input{sparse_trace_method/preliminaries}
%\input{sparse_trace_method/blockwalk_overview}
\input{sparse_trace_method/edgeval}
\input{sparse_trace_method/maximal_val_labeling_redistributed_factor.tex}
%\input{return-factor}
%\input{automorphsm-factor}
\input{sparse_trace_method/autfactor-augmented-ribbon}
%\input{improved-dependence-for-intersection}
\input{sparse_trace_method/application}


==> order-return.tex <==
\subsection{(Non-dangling) Second-use return is forced} \label{sec:return-cost}
%For each vertex, consider the following quantity 
%\begin{proposition}
%	 Let $\calL$ be a maximal-value labeling, for any vertex $v\in V(\al)$ and any $H_v$ an $H$ component in $\calL$, \[ 
% \branch(H_v) \leq \dang(H_v) + 1
%\]
%\end{proposition}

In this subsection, we identify the cost of identifying a vertex arrived using some $R$ edge, i.e., edge that appears the second-time. On a high-level, the vertex-choice for the destination of such edge is fixed: for example, when we are traversing a tree from some root, each vertex only has $1$ edge that goes towards the root. That said, things might get slightly more complicated when the walk is no longer tree-like. Intuitively, any confusion for determining the vertex reached by an $R$ edge can be settled with a cost of $O(d)$ using degree bound, however, this would render us a trivial bound of $\sqrt{nd}$ analogous to row-sum bound. 

To get around with this, we note that any such confusion can be charged with a gap in the previous walk, which offers us a gap to encode auxiliary data for settling such confusion. Concretely, we relate the potential confuseion in determining destination of a return edge via \emph{surprise visit} \footnote{The argument in this section also relies upon another quantity \emph{missed-immediately-return} which can be seen as a proxy to surprise visits} , i.e., edges leading to visited vertices in the walk which correspond to some gap in our walk.

\begin{definition}[Potential-unforced-return factor $\pur$]
	At time $t$ (before the corresponding edge being processed), for each vertex $v$, let $\pur_t(v)$ be defined as the following,\begin{enumerate}
		\item Each return leg closed from $v$ contributes an $1$ to $\pur_t(v)$;
		\item Each unclosed $F$ edge currently incident to $v$ contributes an $1$;
		\item An extra $-1$ as we can maintain a counter for each vertex such that there is always one potential return-leg presumed to be forced.	\end{enumerate}
		Let $H_{v,t}$ be the component reachable using subsequent $H$ edges from $v$ at time $t$, and define \[ 
		\pur_t(H_v) \coloneqq \sum_{i\in H_{v,t}} \pur_t(i)
		\] 
\end{definition}
\begin{remark}
	The definition of $\pur_t(v)$ does not require $v$ to be on the boundary at time $t$ (similarly for $H_{v,t}$), while we are only interested at the desired invariant when it appears on the boundary.  
\end{remark}
%%\begin{definition}[Anchor vertex]
%	We call a vertex $v$ an anchor vertex if it opens up multiple $F$ edges at some single time-stamp in the walk.
%\end{definition}
\begin{definition}[Surprise visit counter] For a time-stamp $t$, for each vertex $v$ and $H_{v,t}$ defined above, let $s_t(v)$ be the number of surprise visits arriving at $v$ revealed by time $t$; we analogously define $s_t(H_v) = \sum_{i\in H_v} s_t(i)$.
\end{definition}
\subsection{Starting from the basic: a forced-return argument for $1$-in-$1$-out}

\begin{proposition}\label{prop: pur-invariant}
	Throughout the walk in which any vertex opens up at most $1$ edge each time it appears on the boundary,  we maintain the invariant \[ 
	\pur_t(H_{v,t}) \leq 2\cdot s_t(H_{v,t}) 
	\]
	for $H_{v,t}$ the $H$-component reachable from the current boundary vertex $v$.
	
%	In general, for a walk with no dangling vertex while a vertex (or an $H$ component) may open up more than $1$ $F$ edge at the boundary, we maintain the invariant \[ 
%	\pur_t(H_{v,t}) \leq 2\cdot s_t(H_{v,t}) + \mir_t(H_{v,t})
%	\]
\end{proposition}
\paragraph{Overview: unforced-return ignoring $H$ edges }
For starters, we observe for a single vertex $v$, if there is no $H$ edge being used throughout the walk and each vertex opens up at most $1$ edge on the boundary, \begin{enumerate}
%	\item Since each vertex opens up at most $1$ $F$ edge on the boundary, $\mir$ is $0$ throughout;
	\item When $v$ is first revealed, as base case, the return from $v$ must be using the edge that explores $v$, and we have $\pur(v)=0$;
	\item Each departure from $v$ may add $1$ potential-unforced-return edge as it adds an unclosed incidental $F$ edge to $v$, and departure from $v$ using $R$ edge does not change the $\pur$ factor at $v$;	\item However, the subsequent arrival may close an $F$ edge that is previously contributing as an unclosed $F$ edge incident to $v$ (though not necessarily the $F$ edge opened by the last departure), and hence $\pur(v)$ does not change from the last time when $v$ is at the boundary if arriving via an $R$ edge;
%\item In general, if it opens up $b_v>1$ many $F$ edges the last time on the boundary, notice each of the newly open legs that remains open while we arrive at vertex $v$ again (regardless of the arrival followed by $H$ or $R$ edge) is a missed immediate-return leg; 	%	\item  In general, if it opens up $b(v)$ $F$ edges that are not immediately closed in the last departure, and the subsequent arrival closes an open $F$ edge (to avoid surprise visit), we pick up a change of at most $b(v)-1$ for $\pur(v)$ (where this is an upper bound as multiple $F$ edges may get closed simultaneously in the arrival as well);

%
	\item The arrival, if using a new $F$ edge, is a surprise visit arriving at $v$ and contributes an $1$ to $s_t$ and an $1$ to $\pur$ on LHS;  the bound holds if we assign an increment of $2$ via the one single surprise visit.
	\end{enumerate}
	
	\paragraph{Incorporating $H$ edges}
	To extend our above argument for using $H$ edges, we give an argument based on $H$-component which may evolve over time. We first appeal to the following two claims building upon the prior observation that arriving at a vertex via an $R$ edge does not increase its $\pur$ factor compared to when it last appears on the boundary (for the case only a single edge may be opened up), \begin{claim}[Calling an $R$ edge does not change $\pur$ on vertices already in the current $H$-comp]
		Let $v$ be the current boundary at time $t$, let $H_{v,t}$ be the $H$-component of the boundary at time $t$, and an $R$ edge is called from $H_{v,t}$ (concretely from $v$) \[ 
		\sum_{i\in H_{v,t}} \pur_{t+1}(i) \leq \sum_{i\in H_{v,t}} \pur_t(i)
		\]  
		In other words, despite $H_{v,t}$ is not necessarily the same as $H_{v,t+1}$ since calling an $R$ edge may expand the current $H$ component, it does not increase $\pur$ factor restricted to the vertices in the current $H$ component.
	\end{claim}
	\begin{proof}
		To see the upper bound, observe that calling an $R$ edge from an $H$ component, restricted to the vertices already in the $H$ component prior to the closing of this $R$ edge, we simply have an edge contributing as an unclosed $F$ edge shifted to a closed return leg called from the component. The inequality follows when we close an $R$ edge between vertices already in the same $H$ component.
	\end{proof}
		\begin{claim}[Getting merged into an $H$ component via an $R$ edge does not change $\pur$ on the annexed vertices]
		Let $v$ be the boundary at time $t$, and let $t'$ be the subsequent time-mark such that $H_{v,t}$ is $H$-connected to the boundary (at $t'$) again and an $R$ edge is used at this step, i.e., $H_{v,t}\subseteq H_{u,t'}$, the $H_{v,t}$ component gets merged into a $H$ component via an $R$ edge at the current step for $u$ the boundary vertex at $t'$ followed by an $R$ edge \[ 
		\sum_{i\in H_{v,t}} \pur_{t'}(i) = \sum_{i\in H_{v,t}} \pur_t(i)
		\]
%		In general, if $H_{v,t}$ opens up $b(H_{v,t})> 1$ not-immediately-closed $F$ edges when it appears at the boundary last time, we have \[ 
%		\sum_{i\in H_{v,t}} \pur_{t'}(i) = \sum_{i\in H_{v,t}} \pur_t(i) + b(H_{v,t}) 
%		\]
	\end{claim}
	\begin{proof}
		Since we depart from $H_{v,t}$ at time $t$ via an $F$ edge, we have $\pur_{t_m}(H_{v,t}) = \pur_{t}(H_{v,t_m})+1$ for any $t<t_m<  t'$; however, since we arrive back at a vertex in $H_{v,t}$ at time $t'$ by closing an $R$ edge, we have $\sum_{j\in H_{v,t}} \pur_{t'}(j)  = \sum_{j\in H_{v,t}}\pur_{t'-1}(j)-1 = \sum_{j\in H_{v,t}}\pur_{t}(j)$, giving us the desired.
	\end{proof}
	
	We now proceed to prove the main proposition.
	\begin{proof}[Proof to  Proposition~\ref{prop: pur-invariant}]
	Suppose this is true throughout the walk so far, and we are currently at $H_{v,t}$, and move to $u$ from $v$ at time $t$, we need to show the above for $H_{u,t+1}$. By construction, it suffices for us to consider whether this is an $F/R$ edge.  Notice this is immediate if $v$ is a new vertex, as $H_{u,t+1} = \{u\}$, and there is no potential-unforced-return from $u$ at this time. Otherwise, if the $v\rightarrow u$ leg opens up a new surprise visit,
		\begin{enumerate}
		\item If $u\in H_{v,t}$, the new $F$ edge that gets open may contribute an $1$ to both $\pur_{t+1}(v)$ and $\pur_{t+1}(u)$ while $\pur$ factor of other vertices in $H_{v,t}$ does not get changed. That said, we pick up a gain of $2$ on the LHS, while the surprise visit also now contributes to $s_{t+1}(H_{v,t+1})$, giving an increment of $2$ on the RHS as well;	
		\item If $u\notin H_{v,t}$, let $t_u$ be the last time vertex $u$ appears at a boundary $H$ component, and call this component $H_{u,t_u}$, in addition to the factors contributing to $\pur_{t_u}(H_{u,t})$, the departure at time $t_u$  opens up $1$ $F$ edge from $H_{u,t_u}$. Plus the new surprise visit that we just open up, we have \begin{align*}
		\pur_{t+1}(H_{u,t+1}) &= \pur_{t_u}(H_{u,t_u}) +  2 \\&
		\leq 2\cdot s_{t_u}(H_{u,t_u}) +  2\\&=	 2\cdot s_{t+1}(H_{u,t}) 	
		\end{align*}
		where we observe that $s_{t+1}(H_{u,t}) = s_{t_u}(H_{u,t_u}) + 1$ as we just pick up a new surprise visit, and $H_{u,t_u} = H_{u,t}$ as a set of vertices.
		
%
%		and our arrival at $H_{u,t}$ via the surprise visit at time $t$ again contributes a gain of $2$ to the $RHS$ i.e., $\pur_{t+1}(H_{u,t}) = \pur_{t_u}(H_{u,t})+ b(H_{u,t_u})$, while we pick up a change of $2$ on the RHS as above.  
\end{enumerate}
		If $v\rightarrow u$ is an $R$ leg that closes some $F$ edge, let $t_u$ be defined as earlier,
		 \begin{enumerate}
		 	\item  $u\notin H_{v,t}$: This yields a merge of $H$ components, and we can partition $H_{u,t+1}$ into vertices $H$-reachable either via $u$ or $v$ at time $t$,  \begin{align*}
				\pur_{t+1}(H_{u,t+1})& = \sum_{i\in H_{v,t}} \pur_{t+1}(i) + \sum_{j\in H_{u,t}} \pur_{t+1}(j)
			\end{align*}
		By our claim that calling $R$ edge does not increase $\pur$ on the vertices in the current $H$ component, \begin{align*}
			 \sum_{i\in H_{v,t}} \pur_{t+1}(i)  \leq  \sum_{i\in H_{v,t}}\pur_t(i) =\pur_t(H_{v,t})\leq  2\cdot s_t(H_{v,t}) 
		\end{align*}
		Since $u\notin H_{v,t}$, for component $H_{u,t} = H_{u,t_u}$, it gets annexed into a new $H$-comp via an $F$ departure and a $R$ return, \[
		\sum_{j\in H_{u,t}}\pur_{t+1}(j) = \sum_{j\in H_{u,t}} \pur_{t_u}(j) = \pur_{t_{u}}(H_{u,t_u}) \leq 2\cdot s_{t_u}(H_{u,t_u}) 		 \] 
%		 If multiple $F$ edges get open up, among which $b(H_{v,t})$ are not immediately-return, we have \begin{align*}
%		 	\sum_{i\in H_{v,t}} \pur_{t'}(i) = \sum_{i\in H_{v,t}} \pur_t(i) + b(H_{v,t}) &\leq 2\cdot s_{t_u}(H_{u,t_u}) + \mir_{t_u}(H_{u,t_u})  +b(H_{v,t}) \\&= 2\cdot s_{t_u}(H_{u,t_u}) + \mir_{t+1}(H_{u,t_u}) 
%		 \end{align*}
%		 where we observe any edge in $b(H_{v,t})$ is a newly gained not-immediately-return leg. 
Combining the above yields 
\begin{align*}
		 	\pur_{t+1}(H_{u,t+1}) &\leq 2\cdot s_{t+1}(H_{v,t}) + 2\cdot s_{t+1}(H_{u,t_u})  = 2\cdot s_{t+1}(H_{u,t+1})  
		 \end{align*}
		 as $H_{v,t}$ and $H_{u,t_u}$ form a partition for $H_{u,t+1}$ for $u\notin H_{v,t}$, and the surprise visits inherit over time.
		 \item $u\in H_{v,t}$: This is a return within an $H$-component, and we have \[
		 \pur_{t+1}(H_{u,t}) \leq  \pur_{t}(H_{v,t})
		  \]
		  since calling a return leg within the same $H$ component does not increase $\pur$ factor (in fact, a decrease by $1$ as the corresponding $F$ edge contributes a factor $1$ to both endpoints in the $H$ component, while after being closed, it only contributes as a closed $R$ edge to one endpoint).
		  \end{enumerate}
	\end{proof}
	
\subsection{Upgrading towards $1$-in-many-out: branching}
\paragraph{Branching} The above argument crucially relies upon that each vertex can only encode at most $1$ edge when it is on the boundary each time, however, this is not true in the general setting for graph matrix, and particularly why rough matrix norm bounds depend crucially on \enquote{minimum vertex separator} of the underlying graph. That said, we note that the argument can be extended in a lightweight manner to the general case when the matrix is indexed by order-tuple, i.e., there is no permutation-jump involved in the walk.


For concreteness, we call a vertex an \emph{anchor} vertex if it encodes multiple (out-going) edges on the boundary at a single time in the walk. The crux of the argument observes that we can further constrain each such vertex to have each of its $F$ edge opens up in the branching to be closed before the vertex appears again on the boundary, as otherwise there is a gap from surprise visit that we can identify locally in the constraint graph, and this is captured by the counter $\mir$ to be defined momentarily.

\paragraph{Return bound for tuple-indexed walk}
Let's start with some definitions in this setting, and fix the traversal direction from $U_\al$ to $V_\al$.
\begin{definition}[Anchor vertex]
For a vertex $v$ in the shape $\al$ (or $\al^T$) and an edge-labeling $\calL$, we call it an \emph{anchor} vertex if it pushes out more than $1$ non-dangling edge, i.e., an edge on a simple path from $v$ to the next boundary.  \end{definition}
 \begin{definition}[Mirror copy]
 	For any vertex $v$ in $\al$ (or in $\al^T$), we let $\sigma(v) \in V(\al^T)$ or (in $V(\al)$) be the counterpart of $v$ obtained by shape-transpose. 
 \end{definition}
%For starters, we observe that the linearized constraint graph can decomposed as having $U_\al =V_\al$ vertex disjoint paths from $U_1$ to $V_q$ attaching path-segments between anchor vertex and its mirror copy. 

\begin{definition}[Missed-immediate-return factor counter $\mir$]
	For a vertex $v$ that opens up multiple $F$ edges from the boundary, let $\mir_t(v)$ be the number of $F$ edges it opens up as an anchor vertex so far in the walk that are not immediately closed when $v$ appears on the boundary again. Analogously, we define $\mir_t(H_{v,t})$ for the corresponding $H$-component.
\end{definition}
\begin{remark}
	For adjacency matrix or line graph, $\mir_t(v) = 0$ throughout the walk as each vertex may open up at most $1$ $F$ edge when at boundary.\end{remark}



For starters, consider the linearized constraint graph obtained by forgoing the trace-walk condition $U_1 = V_q$ (as an equality of order-tuples), and this is a graph of $q$ blocks of $\al$ and $\al^T$. We observe that the constraint graph can be encoded via the following process, and use this process to identify the charging of potential-surprised-visit with $\mir$ factor. For the following discussion, fix the traversal direction from $U_1$ to $V_q$.

\begin{mdframed}[frametitle = {Decomposing (linearized) constraint graph into path-segments}]
\begin{enumerate}
	\item We start with at most $U_\al=V_\al$ \emph{directed} vertex-disjoint paths from $U_1$ to $V_q$;
	\item Attach  \emph{directed} path-segments from an anchor vertex to its mirror copy in the subsequent block; 
	\item Attach path-segments between anchor vertices in the same block;
	\item Attach \emph{directed}(dangling) path-segment from an anchor vertex to a dangling vertex in the same block.
\end{enumerate}
\end{mdframed}


\begin{proposition}
	For each block, process the anchor-vertices pair according to their distance in increasing order in $\al\circ\al^T$. For each starting anchor vertex being processed, each path-segment crossing the boundary starting with $F$ edges is either immediately backtracking, or we can assign a surprise visit from the path segment (or its adjacent one) to the starting anchor vertex for its corresponding $\mir$ factor. Moreover, each surprise visit is assigned to at most $2$ $\mir$ factors.
\end{proposition}
\begin{proof}
		 We first observe that for any path-segment that departs from the starting anchor vertex with $F$ edge may only return to the anchor vertex (with label in $[n]$) within the path-segment at the corresponding mirror copy location (aka. the ending anchor vertex) if the starting anchor vertex (labeled in $[n]$) ever appears again the in the path segment. This follows from the injectiivty assumption: the starting anchor vertex may only appear in the current block, and unless there is a surprise visit in the segment, the path returning to the starting anchor vertex lands the starting anchor vertex (its label in $[n]$) at the ending anchor vertex location in the constraint graph. That said, for any anchor vertex that gets returned too early, aka. prior to the corresponding mirror copy location, the branch that returns to the current vertex gets assigned a surprise visit and each other path-segment that opens up new $F$ branches departing from the anchor vertex also gets assigned a surprise visit.		  
		 
		 	 Next, we observe that the return to the starting anchor vertex at its mirror location is mandatory for any segment starting with $F$. Suppose the current path-segment does not return, the starting anchor-vertex picks up $1$ $\mir$ factor from the path-segment. Suppose there is no surprise visit in the current segment (i.e., the $\mir$ factor from the segment is uncharged yet), we claim that this must be the first processed path-segment between the current pair of starting and ending vertices, as otherwise the current path-segment has to arrive at some known vertex at the mirror-copy location which gives a surprise visit to assign to the corresponding $\mir$ factor. However, notice for any anchor vertex with path-segment added to its mirror copy in its subsequent block, there are at least two edge-disjoint paths (given by distinct path segments) to its mirror copy. For concreteness, call the second path-segment processed the adjacent of the first segment. Notice these two path segments are disconnected in the graph sample once the starting anchor vertex is removed, while these two paths need to merge eventually at the mirror copy location. By assumption, the mirror copy is not the starting anchor vertex, hence there must be a surprise visit in the second path-segment and we can charge it to the $\mir$ factor of both the first and second path-segments. 
	 
	Furthermore, to see that a factor of $2$ is sufficient, notice each subsequent path-segment between the current pair of starting and ending anchor vertex either comes with a surprise visit or it is an immediate backtracking segment itself that does not contribute $\mir$ factor to the starting anchor vertex. This completes the proof to our proposition. 
	\end{proof}
	
%		
%\subsubsection{Forced return for walks with permutation-jump}
%In this section, we show ''return-being-forced'' without using injectivity assumption, as permutation-jump may now produce anchor vertices that branch out while each path-segment does not immeidately rejoin (or at all in the whole walk!) in the subsequent block. 
%
%For starters, we maintain an anchor vertex for each active path-segment (i.e., path with vertices in the current boundary) that identifies as the first vertex in the current path-segment without unclosed $F$ edge opened up by the current path-segment. The anchor vertex (and its extension, anchor component) will now serve as a joint connecting various path-segments.
%
%\begin{definition}[$R$-branch invasion]
%We call an $R$ leg a branch invasion at an anchor vertex (and component) if the corresponding $F$ edge is not opened-up by the current branch. 
%\end{definition}
%
%\begin{definition}[Active $F$-path]
%At any step in the walk, for any anchor component, call its path to any vertex in the current boundary an active $F$-path if the path departs from the anchor component via an $F$ edge.
%\end{definition}
%\begin{proposition}
%	For any path-segment, the active $F$-path from the anchor component is eventually closed in a reverse direction, unless there is a surprise visit in, or arriving at the active $F$-path.
%\end{proposition}
%
%\begin{proposition}
%	Swapping $R$ and $H$ label for path-segment invasion.
%\end{proposition}
%
%	\begin{proposition} Let $P_\al$ be a trace walk for shape $\al$,
%We can assign $\pur(P_\al) \coloneqq \sum_{H_{v,q}: \text{H-component at time }q} \pur(H_{v,q})$ factors to surprise visit such that \begin{enumerate}
%	\item each surprise visit is only charged $O(1)$ $\pur$ factors;
%	\item all but $\frac{|U_\al|+|V_\al|}{2} $ many (non-dangling) $\pur$ factors are assigned to some surprise visit.
%\end{enumerate} each surprise visit is only charged to $O(1)$ $\pur$ factors.
%\end{proposition}
%
%\begin{proof}
% For each $H$-component $H_v$, consider the final time $t$ it appears on the boundary in the walk, notice $\pur_t(H_v)$ by construction is an upper bound for the number of unforced-returns called from vertices in $H_v$ throughout the walk. We first see each surprise visit is not being assigned to too many $\pur$ factors. By Proposition~\ref{prop: pur-invariant}, there are two components of $\pur$ factors, (past) surprise visit and (future) missed-immediate-return. Before we start, observe the assignment for past surprise visits is immediate.
% 
% We now consider the assignment for $\mir$ factors. Call a vertex in the constraint graph an \emph{anchor vertex} if it splits out multiple $F$ edges when on the boundary, and we can restrict our attention to anchor vertex (as non-anchor vertex in the constraint graph does not contribute to $\mir$ factor). For starters, consider the linearized constraint graph obtained by forgoing the trace-walk condition $U_1 = V_q$ (as a set equality), and this is a graph of $q$ blocks of $\al$ with $\al^T$ glued with potentially non-trivial permutation jump. We observe the constraint graph can be encoded via the following process, and use this process to identify charging of potential-surprised-visit with $\mir$ factor. For the following discussion, fix the traversal direction from $U_1$ to $V_q$.
%
%\begin{mdframed}[frametitle = { Assigning $\mir$ factor to future surprise visit}]
%\begin{enumerate}
%	\item Attaching a segment: we can attach a (directed) path-segment between a start-vertex and an end-vertex such that the end-vertex is a vertex on an encoded path-segment unless it is a free vertex that is dangling vertex or in $V_q$;
%	\item For each path-segment that arrives at non-free end-point while starting with $F$ edges, we track whether the first edge on the path is closed when arriving at the end-point of the path-segment;
%	\item  If not,  there is at least one surprise visit on the path and we can assign it to the starting vertex as a $\mir$ factor.
%\end{enumerate}
%\end{mdframed}
%   We now observe that a vertex may only be an ''anchor'' vertex if it is the starting point of some path-segment, and each path-segment contributes at most one $\mir$ factor to the final $\pur$ factor via the potential $F$ edge it opens up at the starting vertex. It suffices for us to assign path-segments, and each path-segment that arrives at non-free end-point either dose not contribute to any $\mir$ factor, or contributes at least $1$ surprise visit.
%   
%   For each path segment, we claim that there is either a surprise visit that we can assign to along this segment, or the $F$ edge that opens up the segment is closed in a ''forced'' way, i.e., it does not contribute to any unforced return.
%   
%    To see that not too many $\mir$ factors are not accounted for, notice it must correspond to some free-path-segment, which is at most the number of dangling branches in the constraint graph with $|V_\al|$. Repeating this argument from the other direction gives us the $\frac{|U_\al|+|V_\al|}{2}$ bound.
% \end{proof}
% 
% 


%Branch-chasing
%
%
%
%Below is the branch-chasing argument
%\subsubsection{Branch-chasing using $R$ is free}
%\paragraph{Troubles for immediate-return based argument}
%To recap our prior argument, we essentially give a special treatment for \enquote{branching} vertices, i.e., those in the constraint graph that may encode multiple edges across the boundary, and we claim that for any such vertex, each $F$ edge that gets opened up when departing from this vertex must be immediately closed before this vertex appears again in the boundary: in particular, the branching vertex needs to match in its mirror-copy location unless there is a surprise visit that offers a gap for charging potential unforced return due to the vertex opening up multiple $F$ edges simultaneously in a single-shot. 
%
%However, this heuristic falls apart when we combine with permutation jump, as we no longer have injectivity assumption across the boundary: in particular, mirror copy is no longer well-defined. That said, we can consider a branching vertex that opens up simultaneously multiple $F$ branches, and one of them returns sooner than others, causing a potential confusion when calling an $R$ edge at the anchor vertex, that it may refer to any of the $F$ edges leading to the alive $F$ branch (and the $F$ edge leading to the anchor vertex before any of the $F$ branches get opened up). 
%
%
%\paragraph{Branch-chasing graph}
%We start by considering an auxiliary graph constructed as the following. It should be cautious that \emph{boundary} in the following section typically refers to the boundary of the walk unless otherwise specified. Notice each vertex on the boundary gives us a tiny constant decay via their edges. However, the core of our argument relies upon coloring the edges such that red edge is the only possible confusion, and furthermore, maintaining the invariant each vertex is not incident to \emph{too many red edges}.
% 
%\begin{mdframed}[frametitle = {Constructing and maintaining the branch-chasing graph}]
%\begin{enumerate}
%	\item This is a directed graph with each vertex receiving a label in $[n]$, moreover, we can color the edges into \emph{red} and \emph{black}, such that we are interested in the desired invariant each vertex is incident to only one out-going red edge unless there are further surprised visits assigned to this vertex;
%	\item Observe that there is no confusion if there the incident red-edge is \emph{unique};
%% 	\item In this graph, we are primarily interested in unclosed $F$ edges and vertices that split out multiple $F$ edges at a single time in the boundary;
%	\item We start with an empty graph and build the graph as the walk proceeds;
%	\item For each $F$ edge, we open up a \emph{directed black} edge from the original vertex to the vertex it arrives;
%	\item If the $F$ edge that gets opened up is a surprise visit, i.e., it leads to a previously explored vertex, we flip all the \emph{black} unclosed $F$ edges that have a directed path in the branch-chasing graph to the surprise destination to \emph{red}. 
%\end{enumerate}
%\end{mdframed}
%With this graph in hand, we first see how it may help us in deciding $R$ edges that arise in the chasing process when there are multitple walkers.
%\begin{observation}
%	 	If there is no dangling branch, any black edge is on a directed path to the current boundary of the walk, i.e., the boundary of the branch-chasing graph is equivalent to the walk boundary.
%\end{observation}
%\begin{corollary}
%	Each chase using black edge is fixed.
%\end{corollary}
%\begin{proof}
%	Despite each vertex may be incident to multiple black edges, notice the subgraph cut across by any black edge is a rooted tree, in particular, with some \emph{active} walker in the current boundary. We then consider the following process, at each (block) step in the walk,  it suffices for us to go through the vertices on the current boundary and query
%	\begin{enumerate}
%		\item whether it is an \enquote{branching} vertex looking for $R$ chase;
%		\item whether it is a vertex assigned to \enquote{beacon guidance} for $R$ chase;
%	\end{enumerate}
%	For each step, for each walker at some branching vertex looking for $R$ chase, the encoder can assign the  boundary vertex on the path promised by the out-going $R$ edge as the following,
%	\begin{enumerate}
%		\item For vertex $v$ looking for beacon-guidance, consider the subtree reached by the desired outgoing edge, assign beacon guidance for any branching vertex with $R$ chase query contained in the subtree;
%		\item Assign an arbitrary vertex in its subtree reached by the desired out-going edge not assigned for beacon-guidance to $v$. 	\end{enumerate}
%	
%	 To decode, since the branch-chasing graph (restricted to black edges) is a directed tree (forest), there exists some query node whose (out-going) subtree is query-node free; by out encoding, there is also promised to be at least one guidance node in that subtree, assign the outgoing edge pointing to the (potentially multiple) guidance beacon to the query-node. Remove their colors (temporarily), and repeat this process.
%\end{proof}
%\begin{remark}
%	It should be pointed out that we only aim to identify the edge-set used by $R$ chase from this process, as any further confusion is then resolved using edge-decay and automorphism factor.
%\end{remark}
%
%We now proceed to handle the potential confusion caused by surprise visit in the branch-chasing graph, i.e., red edges. Throughout the process, a surprise visit may turn black edges into red edges, and call this path the corresponding flip path of the surprise visit. 
%\begin{proposition}
%Consider the path of edges that have their colors flip, the \emph{flip path} passes through at most $2$ vertices that are incident to \emph{out-going} red edge before the current flip.
%\end{proposition}
%\begin{proof}
%	Without loss of generality, suppose the surprise visit proceeds from $a\rightarrow b$, we observe that any edge that gets flipped by this surprise visit. Let $u_a$ be the closest vertex on the flipped path to $a$ that is already incident to some out-going red edge before the current flip, and suppose there is some other vertex $v_a$ that also has a black path to $a$ before the current flip. We observe that it needs to pass through $u_a$ as the subgraph restricted to black edges is a directed tree. However, consider the supposedly black path from $v_a$ to $u_a$, we claim that it must be already be red before the current flip as $u_a$ has an out-going red-edge, which by construction, requires the $v_a$ to $u_a$ path to be flipped to red. Therefore, there can be at most $1$ vertex incident to  \emph{out-going} red edge before the current flip that has a flip-path to $a$; apply the above argument to the flip-path leading to $b$ then gives us the desired bound.
%\end{proof}
%\begin{corollary}
%	Assigning each surprise visit to two of the vertices its flipped path pass through that may be incident to more than $1$ out-going red edge captured by the factor $\red$,  we can maintain the following invariant for each vertex \[ 
%	\text{out-going red edges incident to $v$} \leq 1 + w_t(v)
%	\]
%	where $w_t(v)$ accounts the number of surprise visits assigned to vertex $v$ for creating new excess red edge originating from $v$.
%\end{corollary}
%
%% \begin{comment}
%% 
%% 	 \begin{mdframed}[frametitle = {Constructing and maintaining the branch-chasing graph}]
%%\begin{enumerate}
%%	\item This is a directed graph with each vertex receiving a label in $[n]$, moreover, we can color the vertices in the current boundary of the \emph{walk} using red and blue such that each blue vertex represents a vertex currently in the boundary serving as a beacon guidance, and a red vertex is an branching vertex currently in the boundary with possible $R$ chase query. One vertex may receive two colors at the same time.
%%	\item We start with an empty graph and build the graph as the walk proceeds;
%%	\item Push a vertex into the branch-chasing graph if it appears in the walk as some \emph{branching} vertex that splits out multiple edges simultaneously at the boundary (fix traversal direction from $U$ to $V$ w.l.o.g.);
%%	\item For each walker the \emph{branching} vertex splits out using $F$ edge (i.e., edge splits out from the branching vertex), add a vertex for the corresponding walker, and a directed edge from the branching vertex to the walker, which also receives a label in $[n]$; for each walker that departs using $H$ edges, maintain a vertex recording the current walker's location while no edge is added;
%%	\item For any walker on the boundary, update its current label in $[n]$ in its corresponding location at each step; if a walker vertex receives the same label in $[n]$ as a vertex that has a directed edge to itself, this corresponds to a return via closing the $F$ segment it used to depart from the last anchor vertex, remove the directed edge in-between, and collapse the two vertices;
%%	\item For any \emph{branching} vertex not currently on the boundary, if it has only one out-going directed edge, remove the vertex and merge its two incident directed edges into one (if one-in-one-out) with the same direction;
%%	\item If any vertex on the boundary witnesses a surprise visit, update the current vertex's label, remove the directed edge going into the current head of arm and if the new vertex is on any path between current anchor vertices (or current head of arm), make it a \emph{branching} vertex if not already, and replace the one directed edge that represents the active path passing through the surprise visit destination by two directed edges (passing through the new branching vertex).
%%\end{enumerate}
%%\end{mdframed}
%%
%%\begin{proposition}
%%	The branch-chasing graph is a tree (acyclic viewed as an undirected graph) throughout the walk, and each vertex in the branch-chasing graph receives a unique label in $[n]$.\end{proposition}
%%\begin{proof}
%%	Any surprise visit gets removed when it appears on the boundary.
%%\end{proof}
%%\begin{proposition}[Boundary equivalency] \label{prop:peaceful-merging}
%%	Throughout the walk, any $0$ out-degree vertex of the branch-chasing graph is in the walk boundary. In other words, any out-going edge from a branching vertex in the graph is on a directed path to the boundary. Moreover, a surprise visit may remove at most $1$ directed-edge in the branch-chase graph.
%%\end{proposition}
%%\begin{proof}
%%	We prove this by induction, and consider how the latest move may affect $v$ the boundary vertex of the branch-chasing graph.  By induction hypothesis $v$ is also at the boundary of the walk, and consider (potentially multiple) walkers from $v$, and process them sequentially (in arbitrary order). If there are multiple walkers currently at $v$, process them in order. 
%%	
%%	 If the current walker at $v$ moves to a new vertex using non-surprise $F/H$ edge, the walker has its label updated to the current destination in $[n]$, and potentially adding a directed edge (if $v$ has walkers-to-be processed or have other out-going edges in the branch-chase graph), while the current walker and $v$ (if remaining in the graph) both maintain the walk boundary status, and the potential out-going $F$ edge we add from $v$ points outwards to the boundary.
%%	 
%%%	  For a walker using surprise visit, let $p(v)$ be the parent of $v$ in the directed tree before this move, and we case on whether $v$ is currently a branching vertex in the branch-chasing graph, i.e., whether it has other walkers to be processed or out-going edges. If so, the surprise visit split out by the current arm removes the directed edge from $v$ to the current walker, while any other out-going edge from $v$ remains unaffected by this move, and hence still has a directed path to the current walk boundary. If $v$ does not have any more walker or out-going edges, observe that $v$ gets removed (ignored in the branch-chasing graph) after the surprise visit, while the invariant holds true for $p(v)$ as we create a new directed edge from $p(v)$ to the destination of the current head-of-arm, and other out-going edge from $p(v)$ remains unaffected.
%%	  
%%	  
%%	  For a walker using surprise visit, we first consider the out-going edges it may affect that are already present in the branch-chasing graph before the surprise visit. Let $p(v)$ be the parent of $v$ in the directed tree before this move: 
%%	  \begin{enumerate}
%%	  	\item The edge in the branch-chasing graph $p(v)\rightarrow v$ may be affected, but notice either $v$ gets removed from the branch-chasing graph after this surprise visit, or $v$ has other walkers or other out-going edge towards the current boundary, in which case the edge $p(v)\rightarrow v$ remains as pointing outwards to the boundary, and this is the only directed edge in the branch-chasing graph the walker can remove;
%%	  		  	\item Let the walker's surprise destination be $u$. Recall that if $u$ is currently passed through by some path-segment represented by some directed edge $a\rightarrow b$ in the branch-chasing graph, we divide the path-segment into two directed segments $a\rightarrow u \rightarrow b$. Notice the edge $a\rightarrow u$ is pointing outwards to the boundary as $u$ is on the boundary, and $u\rightarrow b $ is also pointing to the boundary by the invariant hypothesis on $a$ a \emph{branching vertex} in the branch-chasing graph;
%%	  	\item $v$ may remain in the branch-chasing graph as a \emph{branching vertex} after the surprise visit and any of its other out-going edges do not get affected by the current walker.
%%	  \end{enumerate} 
%%	  
%%	 \end{proof}
%%	 
%%\begin{corollary}
%%We can assign each surprise visit to at most $1$ directed edge in the branch-chasing graph such that for each vertex in the branch-chasing graph, each of its out-going directed-edge that gets removed without being closed from the reverse-direction is assigned $1$ factor of surprise visit. \end{corollary}	 
%%In other words, each return is either forced (via $1$-in-$1$-out argument) or can be assigned $1$ factor of surprise visit.
%%
%%	 
%%\begin{proposition}
%%	Each $R$ chase of a block (step) can be decoded as an edge-set for free, i.e., at a cost $O(2^{|U_\al|})$ (and $O(2^{|V_\al|}) $ for $\al^T$ block) where we call a step from an anchor vertex an $R$ chase if it uses an out-going $F$ edge from the branching vertex in the branch-chasing graph.
%%\end{proposition}
%%\begin{proof}
%%	At each (block) step in the walk, each out-going $F$ edge is on a path leading to some vertex in the walk boundary, it suffices for us to go through the vertices on the current boundary and query
%%	\begin{enumerate}
%%		\item whether it is an \enquote{branching} vertex looking for $R$ chase;
%%		\item whether it is a vertex assigned to \enquote{beacon guidance} for $R$ chase;
%%	\end{enumerate}
%%	For each step, for each anchor vertex looking for $R$ chase, the encoder can assign the  boundary vertex on the path promised by the out-going $R$ edge as the following,
%%	\begin{enumerate}
%%		\item For vertex $v$ looking for beacon-guidance, consider the subtree reached by the desired outgoing edge, assign beacon guidance for any branching vertex with $R$ chase query contained in the subtree;
%%		\item Assign an arbitrary vertex in its subtree reached by the desired out-going edge not assigned for beacon-guidance to $v$ (guaranteed by ~Proposition \ref{prop:peaceful-merging} ). 	\end{enumerate}
%%	
%%	 To decode, since the branch-chasing graph is a directed tree (forest), there exists some query node whose (out-going) subtree is query-node free; by encoding, there is also promised to be at least one guidance node in that subtree, assign the outgoing edge pointing to the (potentially multiple) guidance beacon to the query-node. Remove their colors (temporarily), and repeat this process.
%%	\end{proof}
%%
%% \end{comment}

\subsubsection{Return is still ''forced'' with dangling branches}
% We now put the above arguments together, concretely, we combine the argument for $1$-in-$1$-out and $R$-chase being free argument for walks with permutation-jump. We start by taking into account our prior observation of $R$-chase being free into $\pur$ factor, the potential function that controls the number of potential-unforced-returns throughout the walk. 
Before we dig into our final bound, we first see how having dangling edges may affect our forced return bound. Notice that having dangling edges indeed brings $\pur$ factor that does not get assigned to any surprise visit, however, our goal in this section is to show that beyond the ''anticpated'' $\pur$ factors, dangling edges do not contribute further confusion.

\paragraph{Attaching dangling branches and dangling factor assignment}
It should be pointed out that the return for each dangling branch is not necessarily fixed, and our goal here is to show each dangling branch, regardless of how many vertices the single branch may pass through, only incurs $1$ factor of potential-unforced-return.

 Let's start by recalling dangling branches (in a shape) can be encoded in the following manner: we can recursively attach a dangling branch to some identified vertex in the shape. And this begets our dangling factor assignment scheme:in each block-step, we assign each dangling factor to the vertex it attaches to, and update the $\pur$ function for each vertex on the newly attached segment via the $1$-in-$1$-out argument. At this point, it should be clear that the $\pur$ factor is associated with the number of dangling branches as opposed to dangling vertices. To formalize this intuition, we introduce \emph{attachment} edge, as this is the edge part of a dangling branch that comes with extra $\pur$ factor in our argument. Notice not all the edges in a dangling branch come with extra $\pur$ factor, and this is crucial for us in obtaining a norm bound with extra factor only depending on the number of dangling branches as opposed to the number of dangling vertices.
 
\begin{definition}[Attachment edge]
    Given a shape and a block-step walk of the corresponding shape, for each dangling branch, call the edge an attachment edge of the corresponding branch if its origin vertex is identified using $R/H$ edge while it spits out an $F$ edge as part of the dangling branch.
\end{definition}
 \begin{observation}
          For any dangling branch, at any block-step of the walk, there is at most one attachment edge unless there is a surprise visit locally along the branch. 
 \end{observation}
 We now introduce an edge-coloring scheme to take into account dangling branch's effects on $\pur$. For each dangling branch that gets encoded, we will color its $F$ edges as the following scheme,
 \begin{mdframed}[frametitle = {Coloring scheme for dangling branches}]
 \begin{enumerate}
     \item Following the encoding order that we start from some non-dangling vertex or landing vertex if floating and encode the edges along the dangling branch;
     \item We restrict our attention to $F$ edges along the dangling branch, and
     \item color each attachment edge \emph{yellow};
     \item color each non-attachment edge \emph{green} if it is not a surprise visit.
 \end{enumerate}
\end{mdframed} 
\begin{remark}
   An out-going green edge is an edge opened as part of dangling branched while it does not get assigned any dangling factor.
\end{remark}
\begin{definition}[Green edge assigment $\green(v)$]
	For any vertex $v$ at time $t$, we define the green edge counter as the number of surprise visits assigned to $v$ by time $t$.\end{definition}
For each $H$ component connected to $v$ at time $t$, we define \[ 
\green_t(H_{v,t}) = \sum_{v\in H_{v,t}} \green_t(v)  \,.
\]
%\begin{claim}
%For any $H$ component $H_v$ at time $t$, let $s_{\dang,t}(H_{v,t})$ be the number of surprise visits arriving at $v$ by time $t$ that is part of any dangling branch, we have \[ 
%\green_t(H_{v,t}) \leq s_{\dang,t}(H_{v,t} )
%\]
%\end{claim}
%\begin{proof}
%	The number of out-going green edges from $v$ may only change when $v$ pushes out non-attachment edge as part of some non-dangling branch, and unless this happens when $v$ is first encountered, in which case we have $0$ on the LHS and $1$ on the RHS, any increment on the LHS comes after a surprise visit arriving at $v$  
%\end{proof}
%

\begin{claim}
	Throughout the walk, for any vertex $v$ at time $t$, we maintain the invariant \[
	\# \text{out-going green edges from $v$ by time $t$} \leq  \green_t(v) + 1 	 \]
\end{claim}
%\begin{claim}
%%	For any dangling branch segment that passes through a sequence of vertices $\{v_i\}$, and suppose that for any vertex $v_i$ on the segment, we have $\green(v_i)=0$ before the segment is processed, we can assign surprise visits from the dangling segment such that $\green(v_i)=0$ continues to hold after the dangling segment is processed.
%%\end{claim}
\begin{proof}
	We prove this by induction on dangling branches. Notice this is true in the base case when each vertex first appears.We now process this by each dangling segment.  For starters, observe that this is also immediate if there is no surprise visit in the branch segment: let $v_0$ be the last ''seen'' vertex passed through by the dangling branch before the current block, that said, $v_0$ pushes out a yellow edge, and thus its invariant on $\green(v_0)$ continues to hold. For any vertex that is visited in the segment after $v_0$, since there is no surprise visit, each such vertex is new and the invariant holds immediately. 
	
	In the case there is some surprise visit, we can process the vertex in order of their distance to the attachment vertex of the current branch from shortest to farthest: for any vertex $v_i$ that pushes out a green $F$ edge while not its first green edge, let $e_i$ be the last $F$ edge before $v_i$ pushes out the $F$ edge in the dangling segment, and we note that $e_i$ is well-defined as otherwise this would be the first $F$ edge pushed out by the dangling branch, and hence be colored ''yellow''. Since $e_i$ is well-defined, we can further observe that this is a surprise visit and we assign it to $v_i$. 
\end{proof}

\subsection{Ultimate return bound}
We now put the above arguments together, concretely, we combine the argument for $1$-in-$1$-out and $R$-chase being free argument for walks with permutation-jump. Towards that end, we need to modify the definition of $\pur$ factor to take into account our prior observation that return is still forced if it is an $R$ chase,
\begin{definition}[Time $t$] We can associate each edge a particular time-mark. That said, we use time $t$ to represent the moment before the edge at the corresponding time-mark is used.	
\end{definition}
\begin{definition}[Upgraded $\pur$ factor] At time $t$ (before the edge of time $t$ is used), for each vertex $v$, let $\pur_t(v)$ be the counter for the following,\begin{enumerate}
		\item Each return leg closed from $v$ by time $t$ contributes an $1$ to $\pur_t(v)$;
		\item Each unclosed $F$ edge (that is not colored ''green'') currently incident to $v$, that also does not come with any immediate-return guarantee, contributes an $1$;
		\item An $-1$ as we can maintain a counter for each vertex such that there is always one potential return-leg presumed to be forced;
%		\item An extra $-1 \cdot 1_{v \text{ has seen outgoing red edge by } t} $ as we can maintain a counter for each vertex such that there is always one outgoing red edge presumed to be forced, and this is only needed when $v$ has outgoing red edge; 
		\item Each out-going green edge contributes an $1$;
		\item Each vertex contributes an $-1$ if it opens up any out-going green edge.
		\end{enumerate}
		Let $H_{v,t}$ be the component reachable using subsequent $H$ edges from $v$ at time $t$, and define \[ 
		\pur_t(H_v) \coloneqq \sum_{i\in H_{v,t}} \pur_t(i)
		\] 	
\end{definition}
\jnote{an attempt to reproduce and simplify the bound}
\begin{lemma}[Ultimate $\pur$ bound] Throughout the walk, we maintain the variant \[ 
\pur_t(H_{v,t}) \leq 2 s_t(H_{v,t})  + \mir_t(H_{v,t})+ \dang_t(H_{v,t}) + \green_t(H_{v,t}) 
\]
for $H_{v,t}$ the $H$-component reachable from the boundary vertex $v$ at the end of time $t$ (after the edge at time $t$ is used).
\end{lemma}
\begin{proof}
	Suppose the current edge being processed goes from $y$ to $v$, let $t$ be the last time mark $v$ appears in an $H$-component at the boundary, and let the corresponding component be $H_{v,t}$. Let $t'$ be the current time-mark, and we are to show the invariant for $H_{v,t'+1}$. For convenience, we introduce the shorthand \[ \Delta_{t_1, t_2}\circ f(a) \coloneqq f_{t_1}(a) -f_{t_2}(a)
		\]
		for our counter function $f \in \{s,\dang,\green\}$ and $t_1\geq  t_2$, and $a$ any vertex, or set of vertices.
 
	
	
	Following our prior observation, it suffices to consider $v,u$ to be in disjoint $H$-components before the edge $(u,v)$. And it suffices for us to show the following, \[ 
	\Delta_{t'+1, t} \circ \pur ( H_{v,t} )\leq  2\Delta_{t'+1, t}\circ H_{v,t}  + \Delta_{t+1, t}\circ \mir(H_{v,t}) +\Delta_{t+1, t}\circ \dang(H_{v,t})  + \Delta_{t+1,t} \circ \green( H_{v,t})
	\] 
	where we observe that each edge that contributes to $\pur_{t'+1}(H_{v,t})$ while not to $ \pur_t(H_{v,t})$ admits the following classification:\begin{enumerate}
		\item Notice this may be the edge used at time $t'$ if it is an $F$ edge, or an edge opened up in the last departure from $H_{v,t}$;
		\item We fist focus on edges opened up in the previous departure, for each such edge, depending on whether the edge opened up as part of some dangling branch, if this is a yellow edge (attachment edge), it is captured by $\Delta_{t+1, t}\circ \dang(H_{v,t})$;
		\item if this is a green edge, suppose it is opened up from vertex $v_t \in H_{v,t}$, we case on whether this is the first green edge opened up from $v_t$, if so, we have \[ 
		-1 \cdot 1_{v_t \text{has opened-up out-going green edge at time t+1}} - (-1)\cdot 1_{v_t \text{has opened-up out-going green edge at time t}}  + 1 = -1 +1 =0
		\]
		where the $+1$ comes from the particular green edge in inspection, and we observe \[ -1 \cdot 1_{v_t \text{has opened-up out-going green edge at time t}} = 0\,;\]
		\item if this is not the first green edge opened up from the source vertex, this is offset by the $ -1$ from the surprise visit in the dangling branch attached at the block of $t$ assigned to $v_t$;
		\item if this is not opened up as part of dangling branch, we case on whether the last departure from $H_{v,t}$ opens up multiple $F$ edges: if so each such	 edge either receives the immediate-return guarantee (in which case does not contribute to the $\pur$ factor), or it is offset by the corresponding factor from $\mir$;
		\item Otherwise, the last departure from $H_{v,t}$ may create one unclosed $F$ edge, and it is either offset by the arrival at $v$ again using $R$ edge at time $t'$, or this is a surprise visit and it suffices for us to offset the gain by assigning the surprise visit a factor $2$ on the RHS; 		\item Finally, inspecting the edges being used at time $t'$, note that W.L.O.G., we can assume there is at most one $F$ edge, as any subsequent ones are considered as surprise visits. Casing on whether this is an $F$ edge, if so, this is either a surprise visit in which case we pick up an increment of $1$ from RHS for each such edge from that gain of surprise visits, or $v$ is a new vertex and the hypothesis holds trivially for $H_{v,t'+1}$.
		\end{enumerate}
\end{proof}




%\begin{lemma}[Ultimate forced-return bound] Throughout the walk, we maintain the invariant \[
%\pur_t(H_{v,t}) \leq  s_t(H_{v,t})  + \mir_t(H_{v,t})+ \dang_t(H_{v,t}) +\green_t(H_{v,t})  \]
% for $H_{v,t}$ the $H$-component reachable from the boundary vertex $v$ at the end of time $t$ (after the edge at time $t$ is used),  where \begin{enumerate}
% 	\item 
%  $s_t$ is the surprise visit counter that counts the number of surprise visits arriving at $H_{v,t}$;
%   \item $\dang_t$ is the counter that counts the number of dangling branches attached to $H_{v,t}$, i.e., yellow edges;
% \end{enumerate}
%\end{lemma}
%\begin{proof}
%For clarity, in the case a vertex splits out multiple walkers at the block-step boundary at time $t$, we can process them in an arbitrary order, and notice each $F$ edge splits out does not affect the desired invariant at time $t$ since each such edge that appears in the branch-chasing graph with a walker on the boundary via local injectivity of graph matrix.
%
%% Suppose this is true for vertex $v$ when it last appears in an $H$-connected component on the boundary at time $t$, and we arrive at $v$ again at time $t'$ from $u$ using a leg $u\rightarrow v$ , we are to show the invariant at the end of current time-mark $t'$. We consider how $v$'s incidental $F$ edges may change from $t$ to the end of $t'$. Notice there may be multiple edges in the current step lead to $v$ at time $t'$, however, we can process the walkers in order and therefore assume in each time-mark only one edge is being used.
% 
% Suppose the current edge being used goes from $u$ to $v$, let time $t$ be the last time mark $v$ appears in the $H$ component at the boundary (before the edge at time $t$ gets used), and call the component $H_{v,t}$. We start by partitioning the unclosed $F$ edges incident to $H_{v,t}$ at time $t$ according to whether they contribute to $\pur_t(v)$, i.e. whether they appear as a directed edge going out from some vertex in $ H_{v,t}$ in the branch-chasing graph at time $t$. Let those that contribute (i.e. unprotected) be in $O_{t}(v)$ and the others (i.e. protected edges) be in $B_{t}(v)$.  Notice the last departure from $H_{v,t}$ (not necessarily from vertex $v$) at time $t$ may create one edge that is either in $B$ or in $O$ at time $t+1$. Our argument relies upon keeping track of how $B$ and $O$ may change between these two time-marks, and we now case on the status of the leg $u\rightarrow v$ at the current time-mark $t'$ (after the edge at $t'$ is used),
% \begin{comment}
%  \begin{enumerate}
% 	\item if the walker arrives via an $R$ edge, this edge does not contribute to any gain of $\pur_{t'}(H_{v,t})$ over $\pur_{t}(H_{v,t})$: 
%	 at time $t<t_m<t'$, there are two cases while either we close an edge that we use to depart from $H_{v,t}$, or the edge that we open at time $t$ remains open while we close a previously open edge $F$ at the return and therefore this edge is no longer contributing to the vertices in 
%		 any such leg alone does not contribute to any gain of $\pur_{t'}(H_{v,t})$ over $\pur_t(H_{v,t})$;
%	\item if the walker arrives via an $F$ edge, any such edge is a surprise visit and contributes to both the gain of  of $\pur_{t'}(H_{v,t})$ over $\pur_t(H_{v,t})$ and the gain of $s_{t'}(H_{v,t})$ over $s_t(H_{v,t})$; moreover, if the arriving walker also departs $H_{v,t}$ using $F$ edges at time $t$, i.e. it breaks an edge on branch-chase graph at the same time, and we pick up another factor of $1$ from $w_{t'}(H_{v,t})$;
%	\item there may be new non-surpirse $F$ edges (not part of dangling branches) open up from $v$ at time $t$ that now act as an incident $F$ edge to $v$, however, notice each such edge appears in the branch-chasing graph at time $t+1$ (i.e., right after edge in $t$ are encoded), and hence they either remain as an $F$ edge that points to the boundary on branch-chase graph, or they get removed while each removal assigns vertex $v$ a factor of surprise visit via a gain in $w_{t'}(H_{v,t})$ over $w_{t}(H_{v,t})$;
%	\item there may be surprise $F$ edges (not part of dangling branches) open up from $v$ at time $t$, though they never appear in the branch-chasing graph, while they contribute to the gain of  $w_{t'}(H_{v,t'})$ over $w_{t}(H_{v,t'})$ as a factor of hardwire surprise visits originating from this component; 
%	\item similarly for $F$ edges open before time $t$ that do not contribute to $\pur_t(H_{v,t})$ at time $t$  as they are part of the branch-chasing graph pointing to the boundary, that they either remain as an $F$ edge that points to the boundary on branch-chase graph, or they get removed while each removal assigns vertex $v$ a factor of surprise visit via a gain in $w(H_{v,t})$;
%	\item for new $F$ edges opened up at time $t$ by attaching dangling branches to $H_{v,t}$, they may now appear as unclosed $F$ edges that contribute to the gain of $\pur_{t'}(H_{v,t'})$, however, they also contribute to the gain of $\dang_{t'}(H_{v,t'})$ over $\dang_{t}(H_{v,t})$.
%\end{enumerate}
%\end{comment}
%
%\begin{enumerate}
%	\item Again, by construction, it suffices for us to consider the edge used at time $t'$ be $u\rightarrow v$ as either $F$ or $R$, since $H$ edge is automatically captured when we consider $H$-components;
%	\item If the walker arrives via an $R$ leg, and assume $v,u$ not in the same $H$ component before this leg as the other case is immediate via prior argument that calling an $R$ edge within the same component cannot increase $\pur$ factor. Therefore, it suffices for us to assume $u$ and $v$ being in disjoint $H$ components at time $t'-1$, i.e., before the use of the leg $u\rightarrow v$, and we can further restrict our attention to $H_{v,t'-1}$ as \[ 
%	\pur_{t'+1}\left(H_{v,t'}\right) = \pur_{t'+1}(H_{u,t'}) + \pur_{t'+1}(H_{v,t'}) \leq \pur_{t'}(H_{u,t'}) + \pur_{t'+1}(H_{v,t'})
%	\]
%	since calling an $R$ edge from an $H$-component cannot increase the $\pur$ factor on the original vertices, i.e. \[ 
%	\pur_{t'+1}(H_{u,t'})\leq \pur_{t'}(H_{u,t'}) 
%	\]
%	\item  Let $E_t$ be the edge that gets opened up at time $t$ when departing from $H_{v,t}$;
%	\item Consider the edges that may now contribute to $\pur_{t'}(H_{t,v})$ while not accounted for at time $t$, let this set of edges be $\Delta_{t'-t}(H_{v,t})$: they are either the edge $E_t$ if it is opened as a dangling edge, or an edge that shifts from $B_{t}$ to $O_{t'}$ (as well as potentially non-dangling $E_t$ that shifts from black to red), i.e., they are protected on the branch-chase graph at some time between $t$ and $t'-1$ as \emph{black} edges,  while no longer so at $t'$ since they are now \emph{red} edges; 	
%	\item For the edges that shift from black to red within the time interval $[t,t']$, we process them in an arbitrary order of their out-vertex in $a\in H_{v,t}$, and for each vertex's first edge being processed, we additionally case on whether the out-vertex $a$ has out-going red edge at time $t$: if not, the first edge flips $1_{a \text{ ever has outgoing red edge}}$ and this offsets the gain to the LHS; otherwise, any such edge assigns $a$ a factor of surprise visit via a gain in $w_{t'}(a)$ over $w_{t}(a)$, yielding  \begin{align*}
%	& |\Delta_{t'-t}(a) | \leq -1 \cdot \left( 1_{a \text{ has seen out-going red edge by } t' } - 1_{a \text{ has seen out-going red edge by } t } \right) + \left(w_{t'}(a) - w_{t}(a)\right)	
%%	&= -1 \cdot \left( 1_{a \text{ has seen out-going red edge by } t' } - 1_{a \text{ has seen out-going red edge by } t } \right) + \left(w_{t'}(a) - w_{t}(a)\right)	
%	\end{align*}
%	where we further observe $w_t(a) = w_{t+1}(a)$ as otherwise 
%	\item Furthermore, let $E_t$ be the edge that gets opened up at time $t$ when departing from $H_{v,t}$, notice the above bound can be improved to reserve the factor of $E_t$ should it shift to red from black, as we are only considering edges already revealed at time $t$, hence, introducing $w_t^{\setminus E_t}$ the short-hand that restricts the $w$ function to edge-recipient other than $E_t$, we can improve the above bound to \begin{align*}
%	&\text{number of revealed black out-going edges from $a$ shifted to red from $t$ to $t'$ } \\&\leq -1 \cdot \left( 1_{a \text{ has seen out-going red edge by } t' } - 1_{a \text{ has seen out-going red edge by } t } \right) + \left(w^{\setminus E_t}_{t'}(a) - w_{t}(a)\right)	
%	\end{align*}
%				\item As stated $E_t$ may contribute a gain of factor $1$ on the LHS via a gain in $\pur_{t'+1}(H_{v,t})$ if $E_t$ is not closed in the current arrival at $v$. Assuming not, we need to case on the status of the $E_t$ at time $t'$;
%		\item If the $R$ edge that gets closed contributed to $\pur_t(H_{v,t})$, i.e., $u\rightarrow v \in O_t(v)$,  (e.g. the edge is a surprise visit or a red out-going edge), this edge witnesses a drop of $1$ in $\pur_{t'+1}(v)$ over $\pur_t(v)$. On the other hand, the edge that gets open up at the departure from $v$ at time $t$ may now remain open at time $t'$ as an edge in $O$, contributing a $1$ to the $\pur$ factor. Combining the above, the $\pur_t(v)$ factor does not increase and we can additionally shift the color of $E_t$ from black to red without incurring any cost;
%	\item If the $R$ edge did not contribute to  $\pur_t(v)$, this is an $R$-chase, i.e., it is a \emph{black} edge incident to $v$ protected at time $t$, and it gets closed at time $t'$, and we need to case on the status of $E_t$, the edge that gets opened up at time $t$.
%%	\item If $E_t$ was opened up as a black edge, it either remains protected as a black edge or a sole red edge, hence does not contributing a gain to $\pur_{t'}(v)$, or it turns red while its gain is now offset by the gain in $w_{t'}(v)$ over $w_t(v)$ where we recall $w$ is the function that assigns surprise visits to vertices incident to excess red edges;
%	\item If $E_t$ was opened up as dangling edge, and moreover, as a dangling attachment edge, we pick up a gain in $\dang_{t'}(H_{v,t})$ over $\dang_t(H_{v,t})$ that can offset the gain from edge. Otherwise, $E_t$ is a  a green edge, i.e., part of some dangling branch while not an attachment edge, $E_t$ is then captured by the factor of $\green_t(v)$: it is either forced as the sole green edge, or it gets assigned surprise visit factors via the function $\green_t(v)$, letting $E_t$'s out-going vertex be $a$, we have \begin{align*}
%&1_{E_t \text{ is opened as a dangling edge} } \\& \leq \left(\underbrace{\dang_{t'}(a) - \dang_{t}(a)}_{\text{dangling attachment} } \right) + \bigg(-1\cdot 1_{E_t \text{ is the first out-going green edge from } a} + \left(\green_{t'}(a)- \green_t(a)\right) \bigg) 		
%	\end{align*} 
%%		\item  In this case, we conider whether  $E_t$ is a black edge at time $t'$: it either remains protected or it gets assigned a factor via a gain of surprise visit in $w_{t'}(H_{v,t'-1})$ over $w_t(H_{v,t})$ which offsets the gain of $1$ on the LHS from $E_t$;
%%	\item Notice the arguments are identical to the $1$-in-$1$-out if the edge that gets closed is not protected in time $t$, and we have $|O_t(v)| = |O_{t'}(v)|$ though they may differ as sets;	
%%\item Vertices in $H_{v,t}$ incident to green edges while not so anymore at time $t'$ may contribute a gain of factor $1$ in that gain of $\pur_{t'}(H_{v,t})$ over $\pur_t(H_{v,t})$, while noticing each such vertex gets assigned a drop of at least one green edge that ceases to contribute to  
%\item From the above, for the $H$-component restricted to vertices $H$-connected to $v$ at time $t'$, suppose an $R$ edge is used, (and noticing $H_{v,t'} = H_{v,t}$)
%	\begin{align*}
%		&\pur_{t'+1}(H_{v,t'}) - \pur_{t}(H_{v,t'}) \leq  \pur_{t'}(H_{v,t'}) - \pur_{t}(H_{v,t'})\\&\leq |\Delta_{t'-t}(H_{v,t})| +1_{E_t \text{ is opened up as a dangling edge}} \\&\leq \sum_{a \in H_{v,t} } -1 \cdot \left( 1_{a \text{ has seen out-going red edge by } t' } - 1_{a \text{ has seen out-going red edge by } t } \right) + \left(w_{t'}(a) - w_{t+1}(a)\right) \\
%		&+ \underbrace{\dang_{t'}(H_{v,t}) - \dang_{t}(H_{v,t})}_{\text{dangling attachment for } E_t} + \bigg(-1\cdot 1_{E_t \text{ is the first out-going green edge from } a} + \left(\green_{t'}(a)- \green_t(a)\right) \bigg) 	  \\
%		&\leq \sum_{a \in H_{v,t}} (w_{t'}(a) - w_t(a)) + (\dang_{t'}(a) - \dang_t(a)) + (\green_{t'}(a) - \green_t(a))
%		\\&= \sum_{a \in H_{v,t}} \Delta_{t'-t}\circ w(a) + \Delta_{t'-t}\circ \dang(a) + \Delta_{t'-t} \circ \green(a)
%				\end{align*}
%		where we introduce the short hands \[ 
%		\Delta_{t_1- t_2}\circ f(v) \coloneqq f_{t_1}(a) -f_{t_2}(a)
%		\]
%		for $f \in \{s,w,\dang,\green\}$ and $t_1> t_2$.
%%		Furthermore, recall we are considering the annexation of $H$-components (i.e. $v,u$ not $H$-connected at time $t'$) , combining with the factor of $H$-component restricted to $u$ at time $t'$ yields, \begin{align*}
%%			&\pur_{t'+1}(H_{v,t'+1}) = \pur_{t'+1}(H_{u,t'}) + \pur_{t'+1}(H_{v,t'})\\ &\leq \pur_{t'+1}(H_{u,t'})+  
%%		\end{align*} 
%	\ Combining with the component connected to $u$ at time $t'$ gives, (assuming $u,v$ again not in the same $H$-component at time $t'$) \begin{align*}
%		&\pur_{t'+1}(H_{v,t}) = \pur_{t'+1}(H_{u,t'}) + \pur_{t'+1}(H_{v,t'})\\
%		&\leq \pur_{t'}(H_{u,t'}) + \pur_{t}(H_{v,t'})  + \left(\pur_{t'+1}(H_{v,t}) - \pur_{t}(H_{v,t})\right) \\
%		&\leq s_{t'}(H_{u,t'}) + w_{t'}(H_{u,t'}) + \green_{t'}(H_{u,t'}) + s_{t}(H_{v,t}) + w_{t}(H_{u,t}) + \green_{t}(H_{u,t'}) \\
%		&+ s_{t'+1}(H_{v,t'})-s_{t}(H_{v,t'}) +\sum_{a \in H_{v,t}} \left(\Delta_{(t'+1)-t} \circ w(a) + \Delta_{(t'+1)-t}\circ \dang (a)  + 	\Delta_{(t'+1)-t}\circ \green(a) \right) \\
%		&\leq s_{t'+1}(H_{v,t'}) +  w_{t'+1}(H_{v,t'+1}) +  \dang_{t'+1}(H_{v,t'+1}) +  \green_{t'+1}(H_{v,t'+1})
%		 \end{align*}
%	where we use the property that the counter functions $\{s,w,\green, \dang \}$ is non-decreasing over time and factorizes over connected components. 
%	\item On the other hand, if the leg $u\rightarrow v$ is an $F$ edge, again assuming $u,v$ not being in the same $H$-component at time $t'$ and the other case is analogous, restricted to the $H_{v,t'}$, we have 
%	\begin{align*}
%		&\pur_{t'+1}(H_{v,t'}) - \pur_{t}(H_{v,t}) \leq |\Delta_{(t'+1) - t'}(H_{v,t})| + |\Delta_{t'-t}(H_{v,t})|   + 1_{E_t \text{is opened up as a dangling edge}} \\
%		&\leq |\Delta_{(t'+1) - t'}(H_{v,t})| + \sum_{a \in H_{v,t}}  \Delta_{t'-t}\circ w(a) + \Delta_{t'-t}\circ \dang(a) + \Delta_{t'-t} \circ \green(a)
%	\end{align*}
%	where we notice the factors restricted to last two terms are identical to the previous calculation when $R$ edge is used, and we can focus on the first term $|\Delta_{(t'+1) - t'}(H_{v,t})|$. Notice this set of edges are either the surprise visit we just opened up at time $t'$, or the edges that switch from black to red due to the current surprise visit (eg. potentially the edge $E_t$ that remains black at time $t'$ while now becoming red), and \begin{align*}
%		|\Delta_{(t'+1) - t'}(H_{v,t})| &\leq s_{t'+1}(H_{v,t'})-s_{t'}(H_{v,t'}) + \sum_{a\in H_{v,t'}} |\Delta_{(t'+1)-t'}(a)|
%			\end{align*}
%			Combining the above yields \begin{align*}
%		\pur_{t'+1}(H_{v,t'}) - \pur_{t}(H_{v,t}) 		\leq &s_{t'+1}(H_{v,t'})-s_{t}(H_{v,t'}) \\ +&\sum_{a \in H_{v,t}}  \Delta_{(t'+1)-t}\circ w(a) + \Delta_{(t'+1)-t}\circ \dang(a) + \Delta_{(t'+1)-t} \circ \green(a)
%			\end{align*}
%		Combining with the invariant for $H_{v,t}$ at time $t$ yields, \begin{align*}
%		\pur_{t'+1}(H_{v,t'+1}) &= \pur_{t'+1}(H_{v,t'}) \leq \pur_{t}(H_{v,t})	+ s_{t'+1}(H_{v,t'})-s_{t}(H_{v,t'}) \\ +&\sum_{a \in H_{v,t}}  \Delta_{(t'+1)-t}\circ w(a) + \Delta_{(t'+1)-t}\circ \dang(a) + \Delta_{(t'+1)-t} \circ \green(a)\\
%		&\leq s_{t'+1}(H_{v,t'+1}) + w_{t'+1}(H_{v,t'+1}) +  \dang_{t'+1}(H_{v,t'+1}) +  \green_{t'+1}(H_{v,t'+1})
%		\end{align*}
%
%%		%	\item if the walker arrives via an $F$ edge, any such edge is a surprise visit and contributes to both the gain of  of $\pur_{t'}(H_{v,t})$ over $\pur_t(H_{v,t})$ and the gain of $s_{t'}(H_{v,t})$ over $s_t(H_{v,t})$; moreover, if the arriving walker also departs $H_{v,t}$ using $F$ edges at time $t$, i.e. it breaks an edge on branch-chas
%\end{enumerate}
%\end{proof}

\paragraph{Putting things together for the final unforced return bound throughout the walk}
It suffices for us to consider each $H$-connected component when they last appear in the walk. Let $\{H_i,t_i\}$ be a sequence of $H$-connected components at the end of the walk, and time $t_i$ their last appearance time-mark, for a shape-walk $W$, we have \begin{align*}
	\pur(W) &\leq \sum_{H_i, t_i} \pur_{t_i}(H_{t_i})\\
	&\leq 2s_{t_i}(H_{i}) + \mir_{t_i}(H_i)+ \dang_{t_i}(H_{i}) +\green_{t_i}(H_i) \\
	&\leq 4\cdot s(W)+  \dang(W)
\end{align*} 
where we observe that each surprise visit may contribute a $2$ to the final bound via $s$ counter, and  a factor of $1$ via $\mir$ counter, a factor of $1$ via $\green$, and each $\dang$ attachment contributes a $1$ via $\dang$.

\begin{corollary}
Each surprise visit can cause at most $4$ unforced returns, i.e., it can be assigned to incur an extra vertex cost of at most $(2|V(\al)|q_\al)^{4}$ as each such confusion can be settled via a label in $2|V(\al)|q_\al$.
\end{corollary}
%\paragraph{Putting together unforced-return bound for set-indexed walk}

==> proof_strategy.tex <==
\section{Proof Overview}
\subsection{$LQL^T$ Decomposition}
Recall that our goal is to show \[\Lambda = \sum_{\al \in \mathcal{S}} \lambda_{\al} M_\al \otimes H_\al \succeq 0   \]
Towards this goal, we will decompose each shape $\al$ into $\sigma\circ\tau\circ \sigma'^T$, for $\sigma, \sigma'^T \in \leftshape $ some left shape, and $\tau\in \midshape$ some middle shape, which corresponds to writing the matrix (modulo intersection terms) 
\[M_\al \approx M_\sigma  M_\tau M_{\sigma'^T} \]
Analogously, we will also factorize the coefficients of $\lambda_\al$, and with the decomposition in hand, we can simply write \[
\Lambda \approx (\sum_{\sigma\in \leftshape} \lambda_{\sigma} M_\sigma \otimes H_{\sigma} ) (\sum_{\tau\in \midshape}  \lambda_{\tau} M_\tau\otimes H_{\tau} ) (\sum_{\sigma'^T\in \leftshape} \lambda_{\sigma'^T} M_{\sigma'^T} \otimes H_{\sigma'^T} )  = LQL^T
 \]
 Our goal now reduces to showing $Q\succeq 0$, and this would allow us to restrict our attention to the middle shapes. Unfortunately, the above is an over-simplification as the equality only holds in an approximate sense, in which we hide out terms arising from ribbon intersection that warrants some extra care.
 
 Consider ribbons of shape $\sigma, \tau, \sigma'$ intersect into some shape $\zeta$  we follow the usual strategy of recursive factorization and factor out $\gamma, \gamma'$ s.t. $\gamma$ is the leftmost SMVS separating $U_\sigma$ and $V_\sigma \cup \int(P)$, and $\gamma'$ the rightmost SMVS separating $V_{\sigma'^T}$ and $U_{\sigma'^T} \cup \int(P)$, i.e., we decompose \[ 
 M_{\zeta} \approx M_{(\sigma-\gamma)} M_{\tau_P} M_{(\sigma'^T-\gamma'^T)}
 \]
 to further handle the intersection terms. The recursive factorization will create more intersection terms, however, the key is to notice the leftmost/rightmost SMVS will move closer towards $U_\sigma$ and $V_{\sigma'^T}$ after each intersection, and hence this process would terminate. Another technical detail that we ignore so far is the truncation error, and we deter this to the later section. To summarize the above, our decomposition strategy can be captured by \begin{align*}
 	\Lambda &= L(Q_0-Q_1+Q_2+\dots+Q_\dsos)L^T \\
 	&=(\sum_{\sigma\in \leftshape } \lambda_{\sigma}M_\sigma\otimes H_\sigma)(\sum_{\tau\in \midshape} \lambda_{\tau} M_\tau\otimes H_\tau + \sum_{\tau_P\in \int} \lambda_{\tau_P}M_{\tau_P}\otimes H_{\tau_P}) (\sum_{\sigma'\in \leftshape} \lambda_{\sigma'^T} M_{\sigma'^T}\otimes H_{\sigma'^T} ) + \text{Truncation} 
 \end{align*} 
\subsection{Recursive charging made explicit}
The idea of charging is prevalent in previous works on SoS lower bounds, especially among those that utilize the recursive factorization machinery. In this work, we will make the charging idea explicit via the charging function \[
\phi: (\lambda_{\alpha},\alpha  ) \rightarrow (\lambda_\beta,\beta,  \slack(\al\rightarrow\beta)) 
 \]
 For intuition, $\phi$ should be viewed as a function that sends shape $\alpha$ to shape $\beta$, meaning we will charge shape $\al$ to $\beta$. As in our application, shape always appear with certain coefficient which would be crucial for us to charge across different shapes, hence we introduce the extra parameters $\lambda_\al, \lambda_\beta$  as the coefficient for shape $\al, \beta$; additionally, we introduce $\slack(\alpha\rightarrow \beta)$ to measure the slack that incurs during the charging (which would be needed for counting). 
 
 For technical reasons, we will impose some constraints on the tuples of shape/ribbons $(\al, \beta)$, as for example to avoid cyclic charging in the process; but in the end, our goal would be to control the quantity $\slack(\al\rightarrow\beta)$ which essentially measures the cost of ''charging'' shape $\lambda_\al M_\alpha$ to $\lambda_\beta M_\beta $. The idea of $\phi$ is implicit in many previous works, as shown in the following.  
 \paragraph{Planted Clique in $\phi$ language}
 For starters, we will restrict our attention to charging middle shape first.
  The main idea has been to charge any non-trivial middle shape $\tau$ to the trivial shape of the corresponding block, which corresponds to the identity matrix (after factoring out the clique indicator function) that offers the ultimate PSD mass. In this language, the previous strategy for planted clique  can be essentially cast as\[ 
 \phi(\lambda_\tau, \tau)  = \left(\lambda_{\Id_{U_{\tau}}}, \Id_{U_\tau}, \left(\frac{1}{n^\epsilon}\right)^{|V(\tau)\setminus (U_\tau\cup V_\tau)|} \right)
 \]
 with the slack  given by vertex decay.
 
 This leads to a question of whether we need to restrict the range of $\phi$ to the trivial shape. As we will see in the middle shape with  non-empty interior edges, we will in fact exploit extra PSD mass from non-trivial shapes on the diagonal. However, a natural follow-up question here might be whether the shape in the range has to be on the diagonal (i.e. $U_\al=V_\al$). Though those shapes would be factually our sole PSD mass in the charging process, we will allow $\phi$ to map to non-diagonal shapes, as long as the shapes is being  mapped to another in a lower order for some ordering of the shape that we will define.
 
 \subsection{Shape/ribbon ordering, and PSD shape/ribbon}
 Let $\mathcal{S}$ be the set of shapes, we define an ordering relation $\mathcal{O}$ on the $\mathcal{S}$ as the following.
 \begin{definition}
 	Given a shape $\al$ and $\beta$, we say $\al <_{\mathcal{O}} \beta $  if \begin{itemize}
 	\item  $U_\al = V_\al = U_\beta$ or $U_\al=V_\al= V_\beta$, and $E(\al)\subsetneq E(\beta)$.
    \item $U_\al = U_\beta= V_\al = V_\beta$, and $E(U_\al\cap V_\al)\subsetneq E(U_\beta\cap V_\beta) $
 \end{itemize}
 \begin{remark}
 	The first relation captures the cases in which we charge non-trivial middle shape to the corresponding trivial shape by taking $E(\al)=\emptyset$.
 \end{remark}
 \end{definition}
 \begin{definition}[PSD (color)-shape]
 	For any $\tau\in \midshape$, we call it a PSD (color)-shape if \[
 	\lambda_{\tau} M_\tau \otimes H_\tau \succeq 0
 	 \]
 	 For example, any trivial middle shape s.t. $U_\tau=V_\tau, E(\tau)=\emptyset$ is a PSD shape.
 \end{definition}
 \begin{definition}[PSD (color)-ribbon]
 For any color-ribbon $\calR = (R,\beta) $ with color $\beta$, we call it a PSD (color)-ribbon if \[ 
 \lambda_{R} (M_R\otimes H_{R,\beta}) \succeq 0
 \] 
 i.e.,
 \[ 
 \lambda_{R}\cdot M_R[U_R,V_R]\cdot H_R[\beta_{U_R}, \beta_{V_R}] \geq 0
 \]
 For example, it is immediately true that any ribbon of the trivial shape is a PSD ribbon. However, there could be ribbon that is not necessarily true as a PSD shape while it could still be a PSD ribbon. This corresponds to the case where $U_\tau=V_\tau$ with non-empty interior edges.
 \end{definition}
 Since we recursively charge across the shape/ribbons, we would need to take into account the coefficient increase coming from terms of higher order being charged to lower order terms, and we take into account of those via the $F$ function.
 \begin{definition}[Charge-collecting function $F$]
 For a fixed shape $\alpha$, we define \[ 
 F(\al) = \sum_{\beta: \phi(\beta) =\al } \frac{\lambda_\beta+ F(\beta)}{\slack(\beta\rightarrow \alpha )}
 \]
  \end{definition} 
 With the ordering relation in mind, we are ready to answer the question of what shape/glyph can be charged to what, and define a charging function as the following,
 
 
\begin{definition}[Charging function]
	We call a pair of functions \[\{\phi_1(\lambda_R, R) \rightarrow (\lambda_{\phi_1(R))}, \phi(R), \slack(R\rightarrow \phi(R)),\phi_2(\lambda_R, R) \rightarrow (\lambda_{\phi_1(R))}, \phi(R), \slack(R\rightarrow \phi(R)) \}\] a charging function if for $i=\{1,2\}$ \begin{itemize}
		\item $\phi_i$ maps (color) shape/glyph to (color) shape/glyph;
		\item for any glyph/shape $R$, either $\phi_i(R)< R$, or
 		\item $\phi_i(R)= R$ and $R$ is a PSD (color) shape/glyph.
	\end{itemize}
	Moreover, if $R$ is a diagonal glyph/shape,\[ 
	\phi_1(\lambda_R, R) = \phi_2(\lambda_R,R)
	\]
	Otherwise, we follow the convention such that \begin{itemize}
		\item $U_{\phi_1(R)} = V_{\phi_1(R)} = U_R $, and $U_{\phi_2(R)} = V_{\phi_2(R)} = V_R $ 
	\end{itemize}
	For our own sanity, we will constrain the target shape/glyph $\phi(R)$ to be a diagonal (color) shape/glyph s.t. $U_R=V_R$ and $\beta_{U_R}=\beta_{V_R}$ if colored.  Additionally, for $\phi_1(R), \phi_2$ both PSD glyph, we require
\begin{align*}
	\begin{bmatrix}
		&\lambda_{\phi_1(R)} M_{\phi_1(R)}, &\lambda_R M_R\\\\
		&\lambda_R M_R^T, &\lambda_{\phi_2(R)}M_{\phi_2(R)}
	\end{bmatrix}\succeq 0
\end{align*} 
if $R$ is off-diagonal, or 
\begin{align*}
		\lambda_{\phi_1(R)}M_{\phi_1(R)} + \lambda_R M_R \succeq 0 
			\end{align*} 
if $R$ is diagonal.
For $\phi_1(R), \phi_2(R)$ non-PSD, we require
 
 
\begin{align*}
	\begin{bmatrix}
		&\left|\lambda_{\phi_1(R)} M_{\phi_1(R)}\right|, &\lambda_R M_R\\\\
		&\lambda_R M_R^T, &\left|\lambda_{\phi_2(R)}M_{\phi_2(R)}\right|
	\end{bmatrix}\succeq 0
\end{align*} 
if $R$ is off-diagonal, or 
\begin{align*}
		\left|\lambda_{\phi_1(R)}M_{\phi_1(R)}\right| + \lambda_R M_R \succeq 0 
			\end{align*} 
if $R$ is diagonal.

\end{definition}
 
  \subsection{From a charging function $\phi$ for middle shapes to PSDness of $Q_0$}
 \begin{restatable}{lemma}{midshapepsd}
  	Given a charging function $\phi$ for middle shapes $\tau$, \[ 
 	 \sum_{\tau:\in \midshape} \lambda_{\tau} M_\tau\otimes H_\tau \succeq 0
 	\]
 \end{restatable}
 \begin{definition}[Diagonal shapes $\mathcal{D}$]\label{lem: midshape-psd}
 	Let $\calD\subseteq \midshape $ be the set of diagonal shapes with no middle vertices, i.e., for $\psi\in \calD$, $U_\psi=V_\psi=V(\psi)$. With some abuse of notation, we also let 	$\calD(\tau)$ denote the diagonal middle shape obtained by the intersection of $U_\tau\cap V_\tau$, i.e., $U_{\calD(\tau)} = V_{\calD(\tau)} = V(\calD(\tau))$ and $E(\calD(\tau)) = E(U_\tau\cap V_\tau)$.  
 \end{definition}
% \begin{definition}[Off-diagonal middle shapes $\mathcal{W}$] Let $\calW$ be the set of off-diagonal middle shapes, s.t. for $\omega\in \calW \subseteq \midshape$, we have $|U_\omega |=|V_\omega|$ and $U_\omega \cap V_\omega = \emptyset$. With some abuse of notation, we also let 	$W(\tau)$ denote the middle shape obtained by the symmetric difference of $U_\tau\Delta V_\tau$, i.e., $U_{W(\tau)} = U_\tau\setminus V_\tau, V_{W(\tau)} = V_{\tau} \setminus U_\tau, V(W(\tau))= V(\tau)\setminus (U_\tau\cap V_\tau) $, and  $E(W(\tau)) = E(U_\tau\cap V_\tau)$.  
% \end{definition}
% \begin{proposition}
% 	Any middle shape $\tau \in \midshape$ can be (uniquely) decomposed into $\tau =\psi \circ \omega $ for some $\psi \in \calD, \omega\in \calW$.
% \end{proposition}
 \begin{proof}
 	It'd be easier to work with color-ribbons directly.\begin{align*}
 		&\sum_{\tau\in \midshape} \lambda_{\tau} M_\tau \otimes H_\tau \\&= \sum_{\tau \in \midshape }\sum_{R:\text{ Ribbon of shape } \tau} \sum_{\beta: V(R)\rightarrow [k]} \lambda_{\tau}\cdot \cval{E(R)}_{\beta}\cdot M_{(R,\beta)}\\
 		&=\sum_{\psi\in \calD}\sum_{\substack{\tau\in \midshape\\ \calD(\tau)=\psi}}\sum_{R:\text{ Ribbon of shape } \tau} \sum_{\beta: V(R)\rightarrow [k]} \lambda_{\tau}\cdot \cval{E(R)}_{\beta}\cdot M_{(R,\beta)}\\ 	
 		&=\sum_{\psi\in\calD}\sum_{\beta: V(\psi)\rightarrow [k]} \Bigg(\sum_{\substack{\Glyph: \text{of color-shape }(\psi,\beta)\\ \text{PSD glyph}} } \lambda_{\psi} \cval{E(\psi)}_{\beta}\cdot M_{(\Glyph,\beta)}+\\&	   \sum_{\substack{\Glyph: \text{of color-shape }(\psi,\beta)\\ \text{non-PSD glyph}} } \lambda_{\psi} \cval{E(\psi)}_{\beta}\cdot M_{(\Glyph ,\beta)}+
 		\sum_{\substack{\tau\in \midshape\\\calD(\tau)=\psi\\ \tau\neq \psi}}
 		\sum_{\substack{\widehat{\beta}: V(\tau)\rightarrow [k]\\ \beta\mapsto \widehat{\beta}\\\text{ subject to boundary coloring} }}\lambda_{\tau} \cval{E(\tau)}_{\beta}\cdot M_{(\tau ,\beta)}\Bigg)\\	
 		 &=\sum_{(\psi,\beta)}\sum_{\substack{\Glyph: \text{of color-shape }(\psi,\beta)\\ \text{PSD glyph}} } \Bigg(\lambda_{\psi}\cval{E(\psi)}_{\beta}\cdot M_{(\Glyph,\beta)} + \sum_{\substack {(\psi',\beta')\\ \Glyph': \text{that has a charging path  to } \Glyph } } \lambda_{\psi'}\cval{E(\psi')}_{\beta'}\cdot M_{(\Glyph',\beta')}\\
 		 &+ \sum_{\substack{(\tau,\beta')\in \midshape \\ (\tau,\beta') \text{ has a charging path to } \Glyph }} \lambda_{\tau}\cval{E(\tau)}_{\beta'} M_{(\tau,\beta')} \Bigg)
 		\\& \succeq 0
 		 \end{align*}
 \end{proof}
 
% \begin{proof}
% \begin{align*}
%\sum_{\tau:\in \midshape} \lambda_{\tau} H_\tau\otimes H_\tau &\succeq \sum_{\text{PSD ribbon}(R,\beta) \in \midshape} \left(\lambda_{R} -\sum_{T:\phi(T)=R} \frac{|\lambda_T|+ |F(T)|}{\slack(T\rightarrow R)}\right) M_R\otimes H_R   \\
%&\succeq 0
% \end{align*}	 
% \end{proof}

==> set_up.tex <==
%\newcommand{\1}[1]{\mathds{1}\left[#1\right]}
%\input{math_commands.tex}
%\newcommand{\val}{\text{val}}
%\newcommand{\calP}{\mathcal{P}}
%\newcommand{\calH}{\mathcal{H}}
%\newcommand{\calG}{\mathcal{G}}
%\newcommand{\calB}{\mathcal{B}}
%\newcommand{\calL}{\mathcal{L}}
%\newcommand{\calE}{\mathcal{E}}
%\newcommand{\calO}{\mathcal{O}}
%\newcommand{\calW}{\mathcal{W}}
%\newcommand{\mul}{\text{mul}}
%\newcommand{\ind}[1]{1_{{#1}}}
%\newcommand{\cycle}{\ind{\calE}}
%\newcommand{\bdd}{\ind{\calF}}
%\newcommand{\depth}{\mathsf{depth}}
\section{Problem Set-up}
 We consider the algorithmic task of distinguishing Stochastic Block Model and  the null distribution being $G_{n,d/n}$.
%\subsection{Independent Set}
%	For independent set of $G\sim G_{n,d/n}$, we want to show an SoS value of $\frac{n}{c\sqrt{d}}$ where the $\poly(\dsos)$ decay is avoided; we will consider the following planted distribution $D_{\text{IndSset}}$: 
%		\begin{itemize}
%			\item  Sample a random graph $G\sim G_{n,d/n}$;
%			\item  For each $i\in [n]$, set $x_i=1$ w.p. $\frac{d}{n}$ u.a.r.;
%			\item Remove edges with both endpoints inside the independent set.
%		\end{itemize}
The planted distribution, $D_{\text{SBM}}$ for any $d,k=O(1)$, is formualted as the following\begin{itemize}
	\item  Sample a color in $[k]$ uniformly at random for each vertex;
			\item For each pair of vertices $i,j\in \binom{n}{2}$, we sample an edge with probability $\frac{\din}{n}$ if $i,j$ have the same color, and with probability $ \frac{\dout}{n}$ otherwise.
\end{itemize}
The parameters we will be interested in will be, \begin{enumerate}
	\item $d$: average degree;
	\item $k$: the number of colors;
	\item $\eta$: SNR
	\item $\din = d(1+(k-1)\eta)$;
	\item $\dout = d(1-\eta)$.
\end{enumerate}
The gap we should be shooting for SBM would be $d\eta^2\ll \frac{1}{c}$ where $c\geq 2$ is some absolute constant independent of $k, d$. Information-theoretically, detection is possible whenever \[
d\eta^2>\Theta(\frac{\log k}{k})
 \]
 
 Setting $\eta = -\frac{1}{k-1}$ gives us a planted distribution for $k$-coloring. Combining the hardness assumption for $d\cdot \eta^2\leq \frac{1}{c}$ prompts us to set $k > c\cdot \sqrt{d}$. 

%\jnote{Let's throw away all the statistics from short exact cycles, so we dont need aks to parity promise...the idea was to say a given random graph sample has all the cycles parity within constant std....but that in the end is only constant probability (and its crucial that we are not able to tolerate any log slack there in the charging)...the idea now is to drop all those short cycle statistics, and use the slack from local statistics constraint where we have log slack}
%


==> sparse_trace_method/automorphsm-factor.tex <==
\section{Handling automorphism factor}
\label{sect: permutation-jump}


\paragraph{Walk for set-indexed graphical matrix} Analogous to the trace of ordered-tuple indexed graphical matrix  $M_{\al,\calO}$ being written as a sum over walks in the complete graph (with additional injectivity condition), the trace for set-indexed graphical matrix can also be decomposed into a sum over walks, except we additionally allow permutation-jump in the boundary.

\begin{definition}[Left/right permutation-jump]
	Given a shape $\al$, we call a permutation of $U_\al$ (and similarly $V_\al$) a left (right) permutation jump. 
\end{definition}
\begin{observation}
	Each walk in the trace for $M_{\al}$ the set-indexed graphical matrix can be described by a sequence of locally injective maps along with permutation jumps on the boundaries. For instance, for block $\al_t$ in the shape walk, in addition to specifying the vertices of $V(\al_t)$ in $[n]$, we also need to specify how vertices from $U_{\al_{t-1}^T}$ maps to vertices in $U_{\al_t}$. The mapping can be described using a permutation of $U_\al$. 
\end{observation}
\begin{definition}[Automorphism $\aut(\al)$] For a shape $\al$, $\aut(\al)$ is the group of bijections from $V(\al)$ to itself such that $U_\al$, $V_\al$ are fixed as sets, and the map is a multigraph automorphism on $E(\al)$. We use $|\aut(\al)|$ to represent the number of such bijections.
\end{definition}
A naive bound for the trace of shaped-walk would be to take a factor of $\sqrt{|U_\al|!|V_\al|!}$ per step,  however, this turns out to be way too pessimistic and introduces a blow-up polynomial in the size of $\al$. To get away with this issue, we want to bound \[ 
B_{\text{set}}(\al)\leq \left((1+o(1))^{V(\al)}\cdot |\aut(\al)|\right) \cdot B_{\text{order-tuple}}(\al)
\]
Our strategy can be encapsulated by the following, for each block $\al$, we want to show \[ 
\text{choice of permutation jump} \times \text{shape-walk factor} \leq \aut(\al) \cdot \text{maximal-labeling value}
\]
For starters, we will assume $\al$ to not have  any dangling vertices/edges. At the beginning of the block, a question we need to answer is \begin{center}
	Can we obtain the maximal value in this block after we take a (non-trivial) permutation jump on the boundary?
\end{center}
From the structure lemma, we can instead ask the question for left/right permutation jump at the boundary of the separator from the last block. Recall in the maximal vale-labeling walk, any (non-dangling) vertex that is not reachable without going through $S$ in the last block are reached along an $F$ edge, and it is moreover, expected to return immediately when the separator is ''fixed'' (i.e. ''all-F/R labeling does not obtain maximal value). For notational convenience, throughout this section, we will study the permutation jump at $V_{\al_{i}}$ for $\al$ at block $B_i$ for some $i\in [2V(\al)q]$. Let $\calL_{i}$ be the labeling for the current block, and $\calL_{i+1}$ be the labeling for the upcoming block. Recall that the boundaries between these two blocks $V_{\al_{i}}$ and $V_{\al_{i+1}}^T$ only agree as a set, it suffices for us to fix an ordering for $V_\al$ and let $P$ be a permutation in $V_\al$. Our goal is to show unless there is a gap in the labeling-vale either from the adjacent block $B_i$ or $B_{i+1}$, the choice of $P$ is limited.
%
%
%\subsection{Preliminaries for Aut factor}
%\begin{proposition}
%	Let $RS$ be the rightmost separator (with minimal high-mul edges) for $\al$, for any vertex $v\in RS\setminus V_\alpha$, for any maximal value labeling (equivalently any SMVS) , $v$ is either incident to at least one separator edge with an $F$ path to $V_\al$,  or it has multiple $F$ paths to $V_\al$.
%\end{proposition}
%\begin{proof}
%	Suppose not, $v$ must only have one path to $V_\al$  with no separator edge, in which case, let $u$ be the next vertex on the path from $v$ to $V_\al$, we notice we can replace $v$ by $u$ into the $RS$, flip the $F$ edge between $v$ and $u$ into an $R$ edge, and obtain a separator of the same value, which violates the assumption of $RS$ being the rightmost separator.
%\end{proof}
%
%For two adjacent blocks $\al$ and $\al^T$ from $B_i, B_{i+1}$, let $\aut_i$ be the subgraph restricted to those between $S$ and $V_\al$ in  $\al$ block, and those between $V_{\al^T}$ and $S^T$ in $\al^T$ block. See below for the formal definition.
%\begin{definition}[Perm-jump graph $\aut_i$]
%For a given separator $S$, $\aut_S$ is a graph formed by two subgraph $L(\aut_S),R(\aut_S)$ with  4 distinct sets of vertices  $S, V_\al, V_\al^T, S^T \in V(\aut_S)$ and 2 distinct sets of edges $E_\al\cup E_\al^T$ and $M_\aut$  s.t. \begin{enumerate}
%	\item $L(\aut_S)$ has two distinct set of vertices $S, V_\al\subseteq V(\al)$;
%	\item $L(\aut_S)$ is the subgraph obtained by vertices and edges that can be reached from $V_\al$ without passing through $RS$ in $\al$;
%	\item $R(\aut_S)$ has two distinct set of vertices $S^T, V_\al^T \subseteq V(\al)^T$;
%	\item $R(\aut_S)$ is the subgraph obtained by vertices and edges that can be reached from $V_\al^T$ without passing through $S^T$ in $\al^T$;
%	\item There is an ordering for vertices in $V_\al$ and in $V_\al^T$;
%	\item The two set of vertices $V_\al$ and $V_\al^T$ is connected by a set of permutation edges $M_\aut$ with $i\in V_\al$ connected to $j\in V_\al^T $ via some edge $(i,j)\in M_\aut$ if $i$ is mapped to $j$ in the permutation jump.
%\end{enumerate}	
%\end{definition}
%\begin{remark}
%	Recall $RS$ is the rightmost SMVS for $\al$, by assumption, $RS$ appears as a subgraph in $L(\aut_i)$ (and analogously $RS^T$ in $\al^T$); however, it is not necessary that $RS=S$.\end{remark}
%
%
%\begin{proposition}[The separator is ''essentially'' fixed]
%If both blocks obtain maximal block value, the edge-labels restricted to $R_i$ is a mirror copy, i.e., up to automorphism of the graph $R_i$,
%\begin{enumerate}
%	\item Any edge that receives an $F$ label in $\al$ receives an $R$ label in $\al^T$;
%	\item Any edge in $E(S)$ that receives an $H$ label in  $\al$ also receives an $H$ label in $\al^T$;
%	\item Any superfluous $H$ edge that appears on any path from $RS$ to $V_\al$ is a high-mul mirror walk.
%	 \end{enumerate} 
%\end{proposition}
%
%
%\begin{claim}
%In the maximal-value labeling, for any vertex $v\in RS$, any path from $V_\al^T$ to $v^T$ must be is an $R\rightarrow H$ path; moreover, if there are multiple all-$H$ path from $V_\al^T$ to $v^T$ is a high-mul mirror walk. 
% \end{claim}
%\begin{proof}
%	The first part of the claim follows from the structure lemma. Any $F$ edge before $v^T$ would result either in surprise visit (in the case when $v$ has multiple paths to $V_\al$) or misses an $H$ edge in the separator (when $v\in S_R$ is incident to a separator edge). The second part follows from local $2$-cycle freeness.
%\end{proof}
%
%\begin{claim}
%	Any separator edge in $RS$ that does not receive $H$ label in $\al$ also does not receive $H$ label in $\al^T$. Moreover, they have to receive $F$ and $R$ label respectively.
%\end{claim}
%
%\begin{definition}[Rightmost separator with fixed edges]
%Given an SMVS $S$ for a shape $\al$, we cal $S'$ a separator the rightmost separator with fixed edges for $S$ if:
%\begin{enumerate}
%	\item $E(S) = E(S')$: they have the same set of separator edges;
%	\item $S'$ is to the right of $S$: there is some vertex $v\in S'\in S$ that is on some path from $u\in S\setminus S'$ to $V_\al$.
%	\item $S$ and $S'$ have the same SMVS value.
%\end{enumerate}
%\end{definition}
%\begin{remark}
%	If the prescribed separator $S$ does not contain any edge, its rightmost separator with fixed edges is simply the rightmost SMVS of the shape.
%\end{remark}
%
%\begin{claim}
%	Consider the subgraph restricted to the boundary $B_S$, the set of vertices in $S$ that have a path to $V_\al$ without passing through any other vertex in $S$, 
%\end{claim}
%
%\begin{claim}
%	Any path from $S$ to $RS$ in $\al$ is an $F$-path, and similarly, the path is all $R$ in $\al^T$
%\end{claim}
%\jnote{This is shaky...i know...}

%

%
%
%\begin{proof}
%We start by showing the first part. Consider $v\in RS\setminus V_\alpha$, we case on the path from $v$ to $V_\al$ in block $\al$. Suppose $v$ is not incident to any separator edge, since $v$ is in $RS\setminus V_\al$, it has multiple paths to $V_\al$, W.L.O.G., suppose $v$ has 2 paths leading to some $a,b\in V_\al$. Suppose the paths leading to $a, b$ are both arrived along $F$ edges, we note that each path must be a mirror copy in $\al^T$. It suffices for us to flip superfluous $H$ edges in $\al$ to $F$ as they do not affect our argument. First, we notice each path to $a,b$ must be all $F$ in $\al$ given they start with $F$ edges and our structure lemma. Consider the path between $a^T, b^T$ and $v^T$ in $\al^T$, by our structure lemma, they must be $R\rightarrow H\rightarrow F$. However, since $a,b$ are arrived from the last block along $F$ edge, unless there is a surprise visit which causes a drop in the last block's walk-value, there is no $H$ option at either vertex. Finally, observe that each path using $F$ edges on the path from $a^T, b^T$ to $v^T$ either come with surprise visit or excess $F$ edge, whose value can be improved if we flip the entire path to $R$ edges. Similarly, for the case when $v\in RS\setminus V_\alpha$ is incident to a separator edge, and there is some $F$-path from $v$ to $a\in V_\alpha$: we note the path from $a^T$ to $v^T$ is either all $R$, or all $F$ arriving at $v^T$ which renders an inferior walk since the separator edge in $E(\al^T)$ incident to $v^T$ is either non-H or there is a surprise visit in the $F$ path leading to $v^T$.
%
%\begin{remark}
%	This argument is oblivious of the perm-jump between $V_\al$ and $V_\al^T$ as it only relies upon $a^T,b^T$ being explored via $H$ or $F$ edge.
%\end{remark}
%
%\end{proof}
%%
%
%
%To get some intuition, we start by investigating permutation jumps within the same connected component.
%
%\subsection{Jumps within the same connected component} Fix a labeling for $B_i$ and $B_{i+1}$. Let $S_i$ be the separator for $B_{i}$ and $S_{i+1}$ the separator for $B_{i+1}$, each built from the corresponding labeling. It suffices for us to assume $S_i$ and $S_{i+1}$ are both SMVS for $\al$, as otherwise, there is already a drop in the block value. 
%%\begin{definition}[$L(\al)$ and $R(\al)$]
%%	Let $S_i$ be a separator for the last block $B_i$ with labeling $\calL_i$, and $S_{i+1}$ be a separator the upcoming block $B_{i+1}$ with labeling $\calL_{i+1}$, we define $L(\al)$ to be subgraph that can be reached from $S_i$ using only $F$ edges (including $H$ edges inside $S_i$), and $R(\al)$ be the subgraph that can be reached from $S_{i+1}$ using only $R$ edges (including $H$ edges inside $S_{i+1}$). 
%%\end{definition}
%
%
%\begin{proposition}
%If the walk obtains maximal-label value in both blocks, any edge that receives a $F$ label in $L(\al)$ must receive an $R$ label in $R(\al)$, up to automorphism of $L(\al)$ (and $R(\al)$ analogously).
%\end{proposition}
%\begin{proof}
%	This is a corollary of our structure lemma. Nope.
%\end{proof}
%


==> sparse_trace_method/floating-comp.tex <==

\section{Improved bounds for floating components}
 
 \subsection{Set-up}
  \begin{definition}[Short-cycle parity promise]
 	Given a random graph sample $G$, we call it satisfies cycle parity promise for length-$t$ cycle if \[ 
 	\float_{C_t}\in  \left[\E[\float{C_t}]\pm c_t\sqrt{\Var( \float_{C_t})) } \right]
 	\]
 	We say $G$ satisfies short cycle parity promise if the above holds for any $t\in [3, 0.01\log_d n]$.
 \end{definition}
 \begin{proposition}
 	W.h.p., a random graph sample satisfies short-cycle parity promise.
 \end{proposition}
\begin{corollary}
	Under the promise of short-cycle parity for a random graph $G$, for $C_t$ a floating cycle of length $t$,
	\[ |\float_{C_t}| \leq \sqrt{n}^{t  } \]
\end{corollary}

Our bounds for floating component can be improved by noticing that for any shape $\al$ with non-empty floating cycles, we can decompose the shape into \[ 
\al = \al_{\mathsf{connect}}\cup \al_\float
\]
where $\al_{\mathsf{connect}}$ is the subshape of $\al$ connected to $U_\al\cup V_\al$, and  $\al_\float$ is a shape s.t. $U_\al=V_\al=\emptyset$ with the floating components from $\al$.
\begin{definition}[Floating subshape $\al_\float$]
	Given $\al$ a shape, we define $\al_{\float}$ its corresponding floating shape s.t.\begin{enumerate}
		\item $U_{\al_\float} =V_{\al_\float} =\emptyset$;
		\item $V(\al_\float)$ is the set of floating vertices in $\al$, and $E(\al)$ is the induced subgraph of $\al$ restricted to $V(\al_\float)$.
	\end{enumerate}  
	With some loss of generality, $M_{\al_\float}$ is simply a scalar polynomial of the random graph sample $G$ such that \begin{align*}
		M_{\al_\float}(G)  = \frac{1}{|\aut(\al_{\float})|}\sum_{\substack{\sigma:V(\al_\float)\rightarrow [n] \\\text{injective} }} \prod_{(i,j)\in E(\al_\float)} \chi_{\sigma(i),\sigma(j)} 
	\end{align*}
\end{definition}

 The starting point for our bounds is the following observation, \[
M_{\al} \approx_{\mathsf{int}} M_{\al_{\mathsf{connect}}} \cdot M_{\al_\float}
 \]
  where the approximate inequality ignores intersection terms. Formally, for any $U, V\subseteq [n]$, we have 
 \begin{align*}
 	\int(\al)[U,V] &\coloneqq M_{\al}[U,V] - M_{\al_{\mathsf{connect}}} \cdot M_{\al_\float}[U,V]\\
 	&= \sum_{\substack{\sigma: V(\al)\rightarrow [n]\\\text{injective} \\\sigma(U_\al)=U, \sigma(V)=V_\alpha }}\frac{1}{|\aut(\al)|}\chi_\al - \sum_{\substack{\sigma_{\mathsf{connect}}:V(\al_{\connect})\rightarrow[n]  \\ \text{injective}\\\sigma_\connect(U_{\al_\connect})=U_\al, \sigma_\connect(V_{\al_\connect})=V_\alpha } }\sum_{\substack{\sigma_\float: V(\al_\float)\rightarrow[n]\\ \text{injective} }}\frac{\chi_{\al_\connect}\cdot \chi_{\al_\float}}{|\aut(\al_\connect)|\cdot |\aut(\al_\float)|}
 	\\&=\sum_{\substack{\sigma: V(\al)\rightarrow [n]\\\text{injective} }} \frac{\chi_\alpha}{| \aut(\al)|} -\sum_{\substack{\sigma_\connect: V(\al_\connect)\rightarrow [n]\\ \\ 
 	\substack{\sigma_\float: V(\al_\float)\rightarrow [n]\\ } \\
 	 \sigma_\float\cup \sigma_\connect: \text{injective}\\\sigma(U_{\al_\connect} )=U, \sigma(V_{\al_\connect})=V }} \frac{\chi_{\al_\connect}\cdot \chi_{\al_\float}}{|\aut(\al_\connect)|\cdot |\aut(\al_\float) |} \\
 	 &-\sum_{\substack{\sigma_\connect:V(\al_{\connect})\rightarrow [n],\text{inj.}\\\sigma_{\connect}(U_{\al_\connect})=U, \sigma_{\connect}(V_{\al_\connect})=V
 	 \\ \sigma_{\al_\float}:V(\al_{\connect})\rightarrow [n],\text{inj.}\\ \mathsf{Im}(\sigma_{\connect})\cap \mathsf{Im}(\sigma_{\float})\neq \emptyset } }
 	 \frac{\chi_{\al_\connect}\cdot \chi_{\al_\float}}{|\aut(\al_\connect)|\cdot |\aut(\al_\float)|}\\
 	 &=-\sum_{\substack{\sigma_\connect:V(\al_{\connect})\rightarrow [n],\text{inj.}\\\sigma_{\connect}(U_{\al_\connect})=U, \sigma_{\connect}(V_{\al_\connect})=V
 	 \\ \sigma_{\al_\float}:V(\al_{\connect})\rightarrow [n],\text{inj.}\\ \mathsf{Im}(\sigma_{\connect})\cap \mathsf{Im}(\sigma_{\float})\neq \emptyset } }
 	 \frac{\chi_{\al_\connect}\cdot \chi_{\al_\float}}{|\aut(\al_\connect)|\cdot |\aut(\al_\float)|}  \hspace*{12pt}  (\text{via }\aut(\al) = \aut(\al_\float) \cdot \aut(\al_\connect))
 	   \end{align*}
 \begin{observation}\label{obs: aut-multiplies} For any shape $\al$,\[ 
 \aut(\al) = \aut(\al_\float) \cdot \aut(\al_\connect)
 \]
 \end{observation}
 We now notice $\int(\al)$ can be decomposed into a sequence of (possibly improper) shapes,
 \begin{definition}[Floating intersection shape]
 	Given a shape $\al$, we call $\al_P$ its floating intersection shape if 
 	\begin{enumerate}
 	\item $U_{\al_P} = U_\al$, $V_{\al_P}=V_\al$;
 	\item $\al_P$ can be obtained by merging vertices from $V(\al_\connect)$ and $V(\float)$;
 	\end{enumerate}
 \end{definition}
 Concretely, we have \begin{align*}
 	\int(\al) = \sum_{\al_P} \frac{|\aut(\al_P)|}{|\aut(\al_{\float})|\cdot |\aut(\al_\connect) |} M_{\al_P}
 \end{align*}
 At this point, it suffices for us to bound $\|\int_\al| \leq o(\|M_{\al_\connect}\| \cdot \|M_{\al_\float} \|)$ using our previous norm bounds, which would then allow us to conclude $\|M_\al\| \leq (1+o(1)) \|M_{\al_\connect}\| \cdot \|M_{\al_\float} \| $  by a triangle inequality. However, some intersection term from $\int(\al)$ warrants extra care as it may still contain some floating component (since not every floating component has to intersect with $\al_\connect$ in $\al_P$). 
 
 To handle this issue, we note that we can recursively factorize the remaining floating component such that we only need to apply norm bounds on shapes with no floating component. Formally, we notice any intersection shape would have at least one fewer connected component, and we can then the shapes according to the number of floating components, and then apply the scalar trick on each shape so that we always get to apply tight norm bounds (norm bounds without $\sqrt{2|V(\al)|q_\al}$ factor)) for any intersection shape in a black-box manner.
 \subsection{Intersection term analysis}
 \begin{lemma}
 	For any shape $\al$ (possibly improer) that can be decomposed into disjoint connected components $\al=\al_\connect \cup \al_\float$, where $\al_\connect$ is the subshape of $\al$ connected to $U_\al\cup V_\al$ (including mul-2 edges) and $\al_\float$ is the subshape of the remaining , we have \[ 
 	\|M_\al \| \leq \left(1+o(1)\right) \|M_{\al_\connect} \|\cdot \|M_{\al_\float} \|
 	\] 
 \end{lemma}
 \begin{remark}
 	Despite a double edge may vanish for the purpose of norm bound, they only arise in the intersection and hence we will  analyze that alongside the intersected shape $\al_{P_\connect}$ in the subsequent analysis.
 \end{remark}
 \begin{proof}
 	We prove this by inducting upon the number of floating components of $\al$, and notice this is immediate when $\al$ does not have any floating component. For the induction hypothesis, consider we are factorizing $\al = \al_\connect \cup \al_\float$, and consider $\al_P$ a shape that arises in the intersection term $\int(\al)$. 

	To begin with, we first factorize out the floating component from $\al_P$, and write $\al_P=\al_{P_\connect}\cup \al_{\float}$. We then notice $\al_P$ must have at least one fewer floating component than $\al$, and hence we can apply our induction hypothesis to bound \begin{align*}
		\|M_{\al_P}\| \leq \left(1+o(1)\right)\cdot \|M_{\al_{P_\connect}} \|\cdot \|M_{\al_{P_{\float}}} \|
	\end{align*} 	
	For a given $\al$ and $\al_P$, let $F_{\al_P}$ be the set of floating components that are incident to any intersected vertex in $\al_P$,  
 \end{proof}
 \begin{lemma}
 	Let $\al$ be a connected shape, and $F$ be a floating cycle, and let $\al_P$ be an intersection term arising from the intersection of $\al$ and $F$, then
 \[ 
 \|M_{\al_P}\|\leq \|M_{\al}\| \cdot \|M_F \|
 \]
  \end{lemma}
 \begin{proof}
 	For starters, by applying matrix norm bounds on $M_\al$ and scalar bound for $M_F$ gives us \[
 	RHS = \max_{S:\text{separator for }\al } \sqrt{n}^{V(\al)\setminus V(S)}\cdot \left(\sqrt{\frac{n}{d}}\right)^{E(S)}\cdot \sqrt{n}^{|V(F)|} 
 	 \]
 	 Our proof proceeds by starting with the shape $\al\cup F$ and  merging each pair of intersection between $\al$ and $F$. Notice before any intersection happens, applying matrix norm bounds on $\al\cup F$ without going through scalar bound gives us a bound of \[ 
 	 \max_{S:\text{separator for }\al } \sqrt{n}^{V(\al)\setminus V(S)}\cdot \left(\sqrt{\frac{n}{d}}\right)^{E(S)}\cdot \sqrt{n}^{|V(F)|} \cdot \sqrt{2|V(\al\cup F)|q_{\al\cup F}}
 	 \]
 	 We advise the reader to ignore the $2V(\al)q$ factor as it arises from $F$ being floating in $\al\cup F$ which is no longer true once intersection happens (despite the fact that the intersection may produce new floating components). Before we dig into the analysis, we notice unless each edge of $F$ becomes a double edge in $\al_P$, we can order the intersected vertices from $F$ such that each intersection only produces at most one pair of double edges. And this prompts us to discuss by cases.
 	 \paragraph{Every edge in $F$ becomes a double edge in $\al_P$}
 	 Since each edge in $F$ becomes a double edge, $F$ must be a vertex-induced subgraph in $\al_P$, and for starters, we notice the bound is immediate if no double-edge vanishes, as we would have \[ 
 	 \|M_{\al_P}\| = \|M_\al|\ll \|M_{\al}\|\cdot \|M_F\|
 	 \] 	 
 	 To see the case for potential double-edge vanishing, consider $V_F\subseteq V(\al)$ the set of to-be-intersected vertices in $V(\al)$, and notice they are connected to the SMVS of $\al$ since $\al$ is a connected shape. Let $\psi(\al_P)$ be a linearization of $\al_P$, and $S$ the SMVS for $\al$, by connectivity, we can pick an arbitrary vertex $v_L\in V_F$ that is reachable from $S_L\cap S$ without passing through the intersected and similarly a vertex $v_R\in V_F$ that is reachable from $S_R\cap S$. 
 	 Let $C_P$ be the intersected cycle in $\al$. 
 	 \begin{claim}
 	 	For any linearization $\psi$ of $\al_P$, \[ 
 	 	\max_{\tilde{S}:\text{separator for} \psi(\al_P)}\sqrt{n}^{|V(\al_P)\setminus V(\tilde{S})|} \left(\sqrt{\frac{n}{d}}\right)^{|E(\tilde{S})|}\sqrt{n}^{|I_{\psi(\al_P)}|}\sqrt{2|V(\al_p)|q_{\al_P}}^{|\float\cup \dang|} 	 	\]
 	 \end{claim}
 	 
 	 \begin{enumerate}
 	 	\item $v_L=v_R$: in this case, since $F$ is a short cycle, $F$ is completely contained in $E(S)$, and the vertices and edges in the floating cycle contributes a total factor of $(\sqrt{\frac{n}{d}})^{|E(F)|}$ to $\|M_\al\|$. Notice each iso-connected component is incident to disjoint edges in $E(\al)$, as otherwise we can merge the two iso-connected components into one. Moreover, for each iso-connected component of $c$ isolated vertices, we first notice it is incident to at least $c+2$ edges in $E(S)$. Now consider a traversal of intersected vertices from $v$. 
 	 	
 	 	For each vertex that can be explored by some non-vanishing double edge in $\psi(\al_P)$, notice we can group them into a segment between iso-connected components and $v$. For each connected segment, consider a traversal within the segment, notice for each vertex but the first vertex, the traversal edge contributes $\sqrt{\frac{n}{d}}$ to $\|M_\al\|$ and the vertex contributes a $\sqrt{n}$ through $V(F)$ to the RHS while it contributes a factor of $\sqrt{n}$ to the LHS;
 	 	\item 
 	 	\end{enumerate}
 	 	\end{proof}
 

==> sparse_trace_method/floating-conditioning.tex <==
\section{Floating conditioning}
In this section, we show the factors for floating cycles can be strengthened if we apply an extra conditioning that the cycle parity of the random graph sample is nicely concentrated.\jnote{second thought...isn't this just a constant probability event since we are not tolerating any polylog slack here?}

==> sparse_trace_method/funny-cloud.tex <==


\begin{section}{Set-up}
We restrict our attention to the normalized adjacency matrix of $G\sim G_{n,d/n}$ for $d$ some large constant, where $G_{i,j}=\frac{n}{d}$ with probability $d/n$, and $-\sqrt{\frac{d}{n}}$ otherwise. Our goal is to show under the removal of the high-degree vertices, $\|G\|\leq O(\sqrt{n})$ w.h.p.

We now proceed to define the terminologies that would be helpful for our closed-walk counting for the trace method.
\begin{subsection}{Defining the Cloud graph}

\begin{definition}
We consider a length-$k$ walk being consist of $k$ legs. Different legs may be mapped to the same edge. (In other words, an edge is a leg without time-stamp.)
\end{definition}

\begin{definition}
An edge is high-mul in a walk if it is used more than $2$ times.
\end{definition}

\begin{definition} (Cloud)
Each cloud corresponds a vertex on the walk that is either incident to some high-mul edge, or incident to $>2$ different edges.
\end{definition}

\begin{definition} (Cloud Vertex)
Each cloud contains $a_i$ many cloud vertices where $a_i$ is the number of legs vertex $i$ is incident to on the walk.
\end{definition}

\begin{definition}(Cloud Leg) A cloud leg is an edge between two cloud vertices, and it corresponds to a leg along a high-mul edge in the walk.
\end{definition}

\begin{definition}(Cloud Edge) A set of cloud legs between the same pair of clouds is called a cloud edge, which corresponds to a high-mul edge in the walk. Furthermore, we call such a pair of cloud a pair of cloud neighbors.
\end{definition}

\begin{definition}(Ordinary Vertex) An ordinary vertex is a vertex that gets visited in the walk but it does not correspond to any cloud.

\end{definition}

\begin{definition}(Innovative Leg) We call a leg innovative if it leads to a new ordinary vertex.

\end{definition}

\begin{definition}(Non-innovative/Surprise leg) We call a leg non-innovative if it leads to a vertex already visited in the walk, and the leg is not along a high-mul edge.

\end{definition}

\begin{definition}($\triangle$-Vertex/Hike) A $\triangle$-vertex is consist of a sequence of ordinary vertices. It is associated with a $\triangle$-hike that represents a journey from some cloud $i$ that takes visits a sequence of ordinary vertices, and then backtracks to the same cloud $i$.
\end{definition}

\begin{definition}($\square$-Vertex/Hike) A $\square$-vertex is consist of a (potentially empty) sequence of ordinary vertices. It is associated with a $\square$-hike that represents a journey from some cloud $i$ that takes visits a sequence of ordinary vertices and ultimately  reaches a cloud $j\neq i$. (Surprise visit)
\end{definition}
\jnote{not every $\square$-leg corresponds to a surprise leg}
\begin{proposition}
For any $\square$-vertex $s$, there exists unique $\square$-vertex $t\neq s$ s.t. $t$-hike visits the same sequence of ordinary vertices as those of $s$-hike. 
\end{proposition}
\begin{proof}
This follows from the assumption that any edge along the $\square$-hike will appear exactly twice in the walk.
\end{proof}

\begin{proposition}
Each cloud vertex takes one of the three possible status, it is either:
\begin{itemize}
    \item connected to a cloud vertex (on a different cloud) via a cloud leg;
    \item or connected to a $\triangle$-vertex;
    \item or connected to a $\square$-vertex.
\end{itemize}
\end{proposition}

\end{subsection}

\begin{subsection}{Encoding}
\begin{enumerate}
    \item We identify the starting vertex which takes a label in $[n]$, and identify whether it is on a cloud;
    \item We repeat the above procedure for every new vertex visited until we hit a cloud vertex;
    \item At a cloud vertex, \begin{enumerate}
        \item (if this is on a new cloud) Identify all its cloud neighbors (at most $\tau$ of them that take labels in $[m]$);
        \item and we identify a leg out of the current cloud by identifying the status of a cloud vertex:
        \begin{enumerate}
            \item if it's connected to a cloud vertex via a cloud edge, we identify the cloud neighbor, and move along that cloud edge;
            \item if it's connected to a $\triangle$-vertex, we identify all the new ordinary vertices visited at this $\triangle$-hike, and return to (3);
            \item if it's connected to a new $\square$-vertex, we record a number for the square vertex, and identify all the the new ordinary vertices visited along this hike until we hit a destination cloud vertex, on which we return to (3) depending on whether this vertex is a new cloud or not;
            \item if it's connected to an explored $\square$-vertex, we identify the number corresponding to the $\square$-vertex, and move along the $\square$-hike to a previously identified cloud destination, and return to (3).
        \end{enumerate}
        
    \end{enumerate}
\end{enumerate}
Let's now fix $m$ to be the number of clouds, and $M=\sum_{i\in[m]} a_i$ the number of cloud vertices, and fix $(a_1,...,a_m)$ s.t. $a_i\geq 3$ for any $i\in [m]$, and with abuse of notation, we are going to denote the number of $\square$-vertices by $\square$, and similarly for $\triangle$. Furthermore, we fix the number of distinct high-mul edges to be $t$, and the total number of legs along high-mul edges to be $T=\sum_{i\in [t]} e_i$. We will also fix $\tau=2d$. Let $\gamma$ be the number innovative legs.
\end{subsection}
\begin{subsection}{Hopefully Useful Trade-offs}
\begin{proposition}
$2\gamma + \square + T =k $
\end{proposition}
\begin{proof}
Recall that $\gamma$ is the number of innovative legs leading to a new ordinary vertex, and $T$ is the number of legs that are along high-mul edges, and we consider a length-$k$ walk where every edge appears at least twice. We note that a leg is either a high-mul leg, a  surprise-leg, an innovative leg or a backtracking of some innovative leg. And each $\square$-vertex corresponds to a surprise-leg.
\end{proof}
\begin{proposition}
$2T+2\square+2\triangle =M=\sum_{i} a_i \geq 3m$
\end{proposition}
\begin{proof}
Each high-mul leg, $\triangle$-hike and $\square$-hike contributes $2$ end-points on the cloud-graph.
\end{proof}
\begin{proposition}
By definition of our random matrix, we have $E[(G_{i,j})^r]\leq \left(\sqrt{\frac{n}{d}}\right)^{r-2} $ for $r>2$.
\end{proposition}
\end{subsection}
We return to the counting now. For a fixed $m, M, (a_1,...,a_m), \square, T, t$ \begin{align*}
    count(m,M,(a_1,...,a_m),\square, T,t)\cdot val(\cdot) &\leq n^{\gamma}\cdot (m^\tau)^m \cdot (\tau+2)^M\cdot (\square)^\square\cdot n^m \cdot (\sqrt{n/d})^{T-2t}\\
    &\leq  m^{\tau \cdot m}\cdot (\tau+2)^M\cdot (\square)^{2\square} \cdot n^{m+\gamma +T/2-t}\cdot (1/d)^{T/2-t}
\end{align*}
where we use $(m^\tau)^m$ to record the neighbors of each cloud, and $(\tau+2)^M$ to record the status of each cloud vertex (whether they are connected to some cloud neighbor that takes label in $[\tau]$, or they are $\square/\triangle$); for each $\square$-vertex, we record its $\square$ number for its endpoint on the cloud, this gives the $\square^{2\square}$; and for each innovative leg we use on $\triangle$-hike, we record its label in $[n]$, giving $n^\gamma$; for each cloud vertex, we identify its label in $[n]$, and finally the value of such walk is given by the last term.

Combining Proposition 1.15 and 1.16, and plug it into the above would give us a bound of \begin{align*}
    m^{\tau \cdot m}\cdot (\tau+2)^M\cdot (\square)^{2\square} \cdot n^{k/2+m-\square/2-t}\cdot (1/d)^{T/2-t}
\end{align*}
\begin{claim}
For any $m, \square, t$ we consider, \[m-\square/2-t\leq 1\]
\end{claim}
\begin{proof}
Recall that $m$ is the number of clouds, and $t$ is the number of distinct cloud edges, we first observe that the cloud graph must be connected since we are counting closed walk. Furthermore, we can start a DFS on the cloud graph, viewing each cloud edge or $\square$-hike an edge, except at the root, for each cloud we visit, by definition it must be reached via a cloud edge, or a $\square$-hike; we will charge the cloud edge to this cloud then, and since a $\square$-hike appear in pairs, we will also charge the two $\square$ vertices corresponding to that particular $\square$-hike to that cloud, and hence we only incur a possible excess at the root.
\end{proof}
\jnote{
A sanity check that we have at least the right order up-to polylog order...which is supposed to be free i guess..}
\end{section}

==> sparse_trace_method/improved-dependence-for-intersection.tex <==
\section{Improved Dependence for $E(U_\al\cap V_\al)\neq \emptyset$}
In this section, we improve the dependence of our norm bounds for edges in $E(U_\al\cap V_\al)$. A priori, each edge in $E(U_\al\cap V_\al)$ contributes a factor of $\cnorm\cdot \sqrt{\frac{n}{d}}^{E(S)}$ assuming the edge in  $E(U_\al\cap V_\al)$ appears in the random graph sample, as otherwise we would pick up a factor of $\sqrt{\frac{d}{n}}$. As usual, we restrict our attention to the tight case when edges in $E(U_\al\cap V_\al)$ are actually present, and our goal now is to remove the dependence of $\cnorm$. Note that this improvement, though marginal, is necessary for our applications to SoS lower bounds where edges in $E(U_\al\cap V_\al)$ do not come with any decay as they effectively do not participate in the charging. 





==> sparse_trace_method/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

% Common
\def \N {\mathbb{N}}
\def \R {\mathbb{R}}
\def \C {\mathbb{C}}
\def \Q {\mathbb{Q}}
\def \Z {\mathbb{Z}}
\def \F {\mathbb{F}}
\def \E {\mathbb{E}}
\def \PE {\wt{\mathbb{E}}}
\def \eps {\epsilon}
\def \al {\alpha}
\renewcommand{\Pr}{\mathop{\bf Pr\/}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\ot}{\otimes}
\newcommand{\zo}{\{0,1\}}
\newcommand{\pmo}{\{\pm1\}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\imp}{\Longrightarrow}
\newcommand{\brac}[1]{\left\langle #1 \right\rangle}
\newcommand{\KL}{d_{\mathrm{KL}}}
\newcommand{\TV}{d_{\mathrm{TV}}}
\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
 \def\1{\bm{1}}
\def \st {\text{s.t.}}
\newcommand{\TODO}[1]{\textcolor{red}{#1}}
\newcommand{\calF}{\mathcal{F}}
% mathsf 
\newcommand{\SA}{\mathsf{SA}}
\newcommand{\SOS}{\mathsf{SOS}}

% complexity classes
\newcommand{\PTIME}{\mathsf{P}}
\newcommand{\LOGSPACE}{\mathsf{L}}
\newcommand{\ZPP}{\mathsf{ZPP}}
\newcommand{\RP}{\mathsf{RP}}
\newcommand{\BPP}{\mathsf{BPP}}
\newcommand{\NP}{\mathsf{NP}}
\newcommand{\coNP}{\mathsf{coNP}}
\newcommand{\MA}{\mathsf{MA}}
\newcommand{\PH}{\mathsf{PH}}
\newcommand{\TC}{\mathsf{TC}}
\newcommand{\AC}{\mathsf{AC}}
\newcommand{\SC}{\mathsf{SC}}
\newcommand{\SZK}{\mathsf{SZK}}
\newcommand{\AM}{\mathsf{AM}}
\newcommand{\IP}{\mathsf{IP}}
\newcommand{\PSPACE}{\mathsf{PSPACE}}
\newcommand{\EXP}{\mathsf{EXP}}
\newcommand{\MIP}{\mathsf{MIP}}
\newcommand{\NEXP}{\mathsf{NEXP}}
\newcommand{\BQP}{\mathsf{BQP}}
\newcommand{\PP}{\mathsf{PP}}
\newcommand{\SP}{\mathsf{\#P}}

% Environments
% \renewenvironment{proof}{{\emph{Proof.}  }}{\hfill$\square$ \vspace{8pt}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{question}[theorem]{Question}
\newtheorem{answer}[theorem]{Answer}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem{exercise}[theorem]{Exercise}
% \theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{example}[theorem]{Example}
\newtheorem{examples}[theorem]{Example}

% Math terms
\newcommand{\poly}{\operatorname{poly}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\size}{\textnormal{size}}
\newcommand{\avg}{\mathop{\textnormal{avg}}}
\newcommand{\sgn}{\textnormal{sgn}}
\newcommand{\dist}{\textnormal{dist}}
\newcommand{\vol}{\textnormal{vol}}
\newcommand{\spn}{\textnormal{span}}
\newcommand{\supp}{\textnormal{supp}}
% \newcommand{\tr}{\operatorname{tr}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\conv}{\operatorname{conv}}


% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\valpha{{\bm{\alpha}}}
\def\vbeta{{\bm{\beta}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathcal{A}}}
\def\sB{{\mathcal{B}}}
\def\sC{{\mathcal{C}}}
\def\sD{{\mathcal{D}}}
\def\sE{{\mathcal{E}}}
\def\sF{{\mathcal{F}}}
\def\sG{{\mathcal{G}}}
\def\sH{{\mathcal{H}}}
\def\sI{{\mathcal{I}}}
\def\sJ{{\mathcal{J}}}
\def\sK{{\mathcal{K}}}
\def\sL{{\mathcal{L}}}
\def\sM{{\mathcal{M}}}
\def\sN{{\mathcal{N}}}
\def\sO{{\mathcal{O}}}
\def\sP{{\mathcal{P}}}
\def\sQ{{\mathcal{Q}}}
\def\sR{{\mathcal{R}}}
\def\sS{{\mathcal{S}}}
\def\sT{{\mathcal{T}}}
\def\sU{{\mathcal{U}}}
\def\sV{{\mathcal{V}}}
\def\sW{{\mathcal{W}}}
\def\sX{{\mathcal{X}}}
\def\sY{{\mathcal{Y}}}
\def\sZ{{\mathcal{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\Ls}{\mathcal{L}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\cl}{\text{cl}}
% \newcommand{\1}[1]{\mathds{1}\left[#1\right]}


% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak




==> sparse_trace_method/maximal-value-labeling.tex <==

\section{Block value and maximal-value labeling}
\label{sec: maxval-labeling}
%\begin{proposition}
%	Consider the length-$q$ walk as consist of $q$ blocks of $\al\circ\al^T$, given the edge labeling of each block $B_1,...,B_q$, notice the final trace is given by \begin{align*}
%		\Tr\bigg((M_{\al} M_{\al^T})^q\bigg) = \sum_{\text{shape-walk path} P}n^{|\comb(P)|}\cdot \E_G[\edgeval(P)\cdot \cycle \cdot \bdd  ]
%	\end{align*}
%	
%	
%	there are at most $\vtxcost_q$ many terms of expected value $\edgeval_q$, where 
%	\[ \vtxcost_q = \prod_{i=1}^q \vtxcost(B_i) \]
%	and \[ 
%	\edgeval_q= \prod_{i=1}^q \edgeval(B_i)
%	\]
%\end{proposition}
In this section, we show that the block value is determined by vertex separator. On the one hand, this identifies the dominant term of the trace being governed by the SMVS; on the other hand, the structure lemma also provides us with a primitive to identify the gap from our trace-walk that offers slack for encoding auxiliary data.

 Towards this end, we start by constructing a vertex separator out of any locally-optimal labeling, and then relate the value of the labeling to the desired norm bound. However, before we proceed to construct a vertex separator, we need to understand the structure of a locally optimal labeling.
 
 \subsection{Set-up for structure lemmas}
 Before we dig into the core of our structure lemmas, we first make some (re-)definitions of our vertex-factors. In the previous section, we should an $R$ edge to represent the second-time an edge appears, and crucially, we show that the vertex reached by an $R$-edge (unless dangling) is \emph{fixed}. On the other hand, it would be convenient for us to consider $R$ leg as the last appearance of an edge appearance due to potential assymmetries of the shape, and we note that for any edge, we can assume exchange its potential vertex factors for the second time and last time appearance. 
 
 In the following section, we will now think of $F/H/R$ corresponding to the first/middle/last appearance of an edge, which also motivates the following assignment scheme for edge-value depending on edge-labels,
	\paragraph{Edge-value assignment scheme}
	\begin{mdframed}
	\begin{enumerate}
		\item $F$: each corresponds to some edge appearing for the first time,
		\begin{itemize}
			\item $F_\single$: the corresponding edge does not lead to visited vertices, while it is going to appear only once in the walk, and it gets assigned a factor $\sqrt{\frac{d}{n}}\cdot \frac{d}{n}\cdot \singdecay $;
			\item $F$: the corresponding edge leads to a new vertex, and it appears at least twice throughout the entire walk. This gets assigned a factor of $1$;
		\end{itemize} 
		\item $H$: each corresponds to middle appearance of some high-mul edge, and each contributes a factor of $\sqrt{\frac{n}{d}}$.
		\item $R$: each corresponds to some edge appearing for the last time, and we assign a factor of  $1$.
	\end{enumerate}
	\end{mdframed}

 
 
 %\begin{claim}
%	For a fixed labeling $\calL$ for $\al$ when we traverse from $U_\al$ to $V_\al$, any vertex that is arrived along some $F$ edge contributes a factor of at most $\sqrt{n}$ to the block value $\vtxcost\cdot \edgeval$.
%\end{claim}
%\begin{proof}
%	For starters, the block value $\vtxcost\cdot \edgeval(\calL)$ can be bounded in two ways, either via a traversal from $U_\al$ to $V_\al$, or via a traversal from $V_\al$ to $U_\al$, and it suffices for us to bound it by \[\sqrt{\vtxcost_{U\rightarrow V}(\calL) \cdot \vtxcost_{V\rightarrow U}(\calL^\top) } \cdot \edgeval \]
%	where we observe that edgeval comes from $H$ edges and does not depend on the direction of traversal.
%	
%	Let $v \in V(\al)\setminus U_\al$ be a vertex that is arrived along some non-signleton $F$ edge using the labeling $\calL$ when we traverse from $U_\al$ to $V_\al$, we pick up at most a vertex factor of $n$ for this vertex; however, once we traverse from $V_\al$ to $U_\al$ along the same path (but in the reverse direction), the vertex $v$ is either fixed from the last block (if it is in $V_\al$), or the corresponding $F$ leg now becomes an $R$ leg and the vertex factor is fixed,  hence we pick up an average of $\sqrt{n}$. 
%	
%	For vertices arrived along singleton $F$ edge, the claim is immediate as in either direction, we pick up a vertex cost of $n$ for the corresponding vertex while there is at least one leg coming with singleton decay, giving us $n\cdot \sqrt{\frac{d}{n}}\cdot \singdecay \ll \sqrt{n} $.
%\end{proof}
\subsection{Structure lemma for locally optimal labelings}
\begin{lemma}[Structure lemma]
% For any locally optimal labeling from $U_\al$ to $V_\al$, there is no unnecessary turn on any simple path from $U_\al  $ to $V_\al $, i.e., any simple path from $U_\al $ to $V_\al$ is of the structure $R\rightarrow H\rightarrow F$, where we allow each edge-label set to be empty, i.e., a path of all $R$ or of all $F$ edges can be considered to be of the above structures; analogously, for any locally optimal labeling from $V_\al$ to $U_\al$, there is no unnecessary turn on any simple path from $V_\al$ to $U_\al$.

For any locally optimal labeling from $U_\al$, there is no unnecessary turn on any simple path originating from $U_\al$. In other words,  any simple path that starts from $U_\al $  is of the structure $R\rightarrow H\rightarrow F$, where we allow each edge-label set to be empty, i.e., a path of all $R$ or of all $F$ edges can be considered to be of the above structures; analogously, for any locally optimal labeling from $V_\al$, there is no unnecessary turn on any simple path from $V_\al$ to $U_\al$.


%	Analogously, we can apply this argument when we traverse from $V_\al$ to $U_\al$.	
\end{lemma}
%
%
% \begin{lemma}[Structure lemma for dangling branch]
%For any locally optimal labeling from $U_\al$ to $V_\al$, the simple path from $U_\al$ to any dangling branch has no unnecessary turn; analogously, for any locally optimal labeling from $V_\al$ to $U_\al$, the simple path from $V_\al$ to any dangling branch has no unnecessary turn. In other words, any of the above path is of the structure $R\rightarrow H\rightarrow F$.
% \end{lemma}
 \begin{lemma}[Structure lemma for floating component]
 For any locally optimal labeling, for any floating component and any fixed landing vertex $v$, any simple path from $v$ has no turn, i.e., they are either all $F/R$ or $H$.
 \end{lemma}
% \begin{lemma}[''Strengthened'' structure lemma for floating component]
% 	For any locally optimal labeling $\calL$, and $C$ a floating component s.t. any vertex in $V(C)$ has degree at least $1$, and $C$ is viable in a typical random graph sample, let $\calL_C$ be the restriction of $\calL$ into floating component $C$,  \[ 
% 	\vtxcost\cdot\edgeval(\calL_C) \leq c^{|E(C)|} \cdot \sqrt{n}^{|V(C)|}\cdot \min \left(\sqrt{d}^{|V(C)|} \right) 
% 	\]
% \end{lemma}
% \begin{proof}
% 	This is subsumed by 
% \end{proof}
\begin{proof}
We prove the above structure lemmas altogether. Note that any path not of the above structure contains a surprise visit in the current block, and hence its value can be locally improved. It also suffices for us to assume each $F$ edge explores a \emph{new} vertex (and the edge is promised to appear again, i.e., non-singleton), as otherwise we pick up at least one factor of singleton decay and we can locally improve the block-value via a promise to use the edge again, or $O(1)$ factors of $2|V(\al)|q_\al$ via our forced-return bound. 

 W.L.O.G., suppose we are traversing from $U_\al$ to $V_\al$ and let $\calL$ be a labeling for this direction. We first note that we can identify such \emph{bad} edge by considering the following process,\begin{enumerate}
 	\item BFS from $U_\al$;
 	\item Identify the first $R$ or $H$ edge preceded by an $F$ edge in this process, and let the vertex that splits out such edge, i.e. the vertex reached by the prior $F$ edge, be $v$; 
 \end{enumerate}
 
 
% Take any simple path from $U_\al$ to $V_\al$, if it is not of the structure above, following this path, there is some $F$ edge that appears in the path followed some $H$ or $R$ edge, and we claim that such an $F$ edge is a surprise visit and can be locally improved. If there are multiple $F$ edges, we can pick the first such edge traversed along the path. Let the vertex reached by the $F$ edge be $v$, and the starting point of this vertex in $U_\al$ be $a$.

There may be multiple paths from $U_\al$ to $v$, while we know that each such path must be all $F$ until they arrive at $v$ in $\calL$. We now consider an alternative labeling $\calL'$ obtained by flipping edges on the path from $ U_\al$ to $v$ from $F$ to $R$. For each vertex on the path $a_i\in U_\al$ to $v$ (except $a_i$ and $v$), it contributes at most a $\sqrt{n}$ vertex factor to the norm bound under $\calL$ once we average over both traversal directions in $\calL$: a vertex reached using an $F$ edge in the $U\rightarrow V$ direction receives a factor $n$, while in the other direction $V\rightarrow U$ it is either fixed (via in the boundary $V$) or arrived along an $R$ edge which is also fixed.  Moreover, notice each such vertex still contributes a $\sqrt{n}$ to the norm bound under $\calL'$ via the same argument. 	
 	
 	For each vertex $a_i \in U_\al$, notice it does not contribute any vertex factor in neither traversal direction of $\calL$. However, it picks up a value of $n$ when we traverse $\calL'^\top $ from $V_\al$ to $U_\al$ as it is arrived using an $F$ edge, and in average it contributes a vertex factor of $\sqrt{n}$ under $\calL$.
 	
 		For vertex $v$, let $f(v)$ be its vertex factor when we traverse in $\calL^T$ from $V_\al$ to $U_\al$. Notice we can pick the encoding such that $v$ is encoded via the same edge when traverse in $V\rightarrow U$ direction in both $\calL$ and $\calL'$, and therefore it contributes the same vertex factor in the reverse direction under $\calL'$. However, notice $v$ is a surprise visit as it is incident to some $H/R$ edge, a vertex cost of $\csurp$ factors of $2|V(\al)|q_\al$ is sufficient where the $\csurp = O(1)$ takes into account the overhead of our unforced-return-bound due to surprise visit. Combining the above, the vertex $v$ contributes a factor of $\sqrt{(2|V(\al)q_\al)^c_s\cdot f(v) }$ in $\calL$ while it contributes a vertex factor of $\sqrt{f(v)}$ under $\calL'$, giving a change of $\frac{1}{\sqrt{2|V(\al)|q}}$.
 	
Finally, notice the vertex factors not on any path from $U_\al$ to $v$ remain unaffected, and the edge-value is unchanged when we move from $\calL$ to $\calL'$, and combining the above changes for the vertex factors along the path gives us a gap of \[ 
 	\frac{\vtxcost\cdot \edgeval(\calL')}{\vtxcost\cdot \edgeval(\calL)} \geq \frac{\sqrt{n}}{\sqrt{2|V(\al)|q}} \gg 1
 	\]
 provided $2|V(\al)|q\ll n$.
 
 The above argument as stated shows that along any simple path from $U_\al$, there is no $F$ edge before any $R/H$ edge in a locally optimal labeling while this does not preclude a path of the structure $R\rightarrow H\rightarrow R$. To rule out these paths, notice we can apply the above argument on the reverse labeling $\calL^T$, in which an $R\rightarrow H\rightarrow R$ path becomes $F\rightarrow H\rightarrow F$ that can be locally improved, and this completes the proof to our structure lemma for non-dangling components.
 
 For floating components, the idea is essentially identical while we can further observe that for each floating component, we have freedom to pick a vertex to encode with a label in $2|V(\al)|q$ to effectively \emph{land} into the component and start the encoding process there. Therefore, if the component contains a mix of $F$ and $R/H$ edges, we can essentially land at a vertex, and pick a direction to traverse the component such that some $F$ edge is traversed before the $R/H$ edge, rendering us a surprise visit that can again be locally improved.
% 
% For dangling components, the above lemma can be strengthened such that each edge in the component must receive the same label, since we have the freedom of picking the \emph{landing} vertex for each component if it is incident to some $R/H$ edge. Hence, if the component contains some $F$ edge, we can always locally improve the value by avoiding surprise visit if we switch any non-$F$ edge in the labeling to $F$. Similarly, we can apply the argument to show any component containing $R$ edge must also be all $R$ by considering its reverse labeling. 
 \end{proof}
% 
% \begin{lemma}[Strengthened structure lemma for floating component]
% 	For any locally optimal labeling, if the component is tree-like, edges in any floating component are either all $F$ or all $R$; moreover, any edge that is part of a short cycle is an $H$ edge. 
% 	 \jnote{not sure if we would want this...not necessary for our applicaton}
% \end{lemma}
% \begin{proof}
% The idea is essentially identical with the argument we just see, with an exception that for each floating component, we have freedom to pick a vertex to encode with a label in $2|V(\al)|q$ to effectively ''land'' into the component and start the encoding process there. Moreover, the choice for each connected component can be agreed upon before the encoding-decoding process, and the labeling follows the direction of the BFS traversal outwards from the landing vertex. 
%  
% Applying the previous argument on any outwards traversal from the landing vertex, note that any path that has an unnecessary turn is again a surprise visit and be locally improved using the previous argument, hence we can already conclude each simple path from the landing vertex follows the structure of $R\rightarrow H\rightarrow F$. However, this can be further strengthened.
% 
%  For tree-like component, we claim that the edges are either all $F$ or all $R$. Suppose not, notice in either direction, there is a vertex that can be identified using a factor $2|V(\al)|q$, with each other vertex contributing at most a factor of $\sqrt{n}$. However, if we flip all edges into all $F$ or all $R$, each vertex contributes a factor of $\sqrt{n}$, and moreover, there is one landing vertex that contributes an additional $\sqrt{2|V(\al)|q}$ factor. 
% \end{proof}
 
 %
% Let $b$ be the vertex incident to both $e_1$ and $e_2$, and let $a$ be the vertex incident to the last non-$F$ edge on the path from $U_\al$ to $b$. Consider the path from $a$ to $b$, notice we pick up a gain of at least $\frac{n}{2|V(\al)|q}$ in the SMVS value if we flip all the edges between $a$ and $b$ on the path to be $R$, as 
% \begin{enumerate}
%	\item For each vertex on the path between $a$ and $b$, it contributes at most  a vertex factor of $\sqrt{n}$ once we take average of the vertex cost for $\calL$ and $\calL^\top$ when we traverse from the other direction; %	  \[ 
%%	\frac{\sqrt{\frac{n}{d}}\cdot \frac{1}{\singdecay} }{n\cdot \frac{d}{n} \cdot \sqrt{\frac{n}{d}}\cdot \singdecay} >1	\]
%\[ 
%\frac{n\cdot \frac{1}{\sqrt{n}}}{\sqrt{n}}=1
%\]
%	\item For vertex $b$, it is incident to a non-$F$ edge in the current block, hence it gets a factor of at most $2|V(\al)|q $ in the vertex cost at the original labeling, and flipping the last edge from $F$ to $R$ gives a change of \[
%	 \frac{n\cdot\frac{1}{\sqrt{n}} }{2|V(\al)|q} > \1	 	 \]
%	 provided $|V(\al)|\ll n^{1/4} $.
%\end{enumerate}

%
%
%if it contains an excess turn, we can find two points $a\neq b\in V(\al) $ that are both incident to edges of $F,R$ labels on the path. W.L.O.G., let $a$ be the first vertex that witnesses a turn and $b$ the second, let $e_1$ be the path from $U_\al$ into $a$, $e_2$ the path between $a$ and $b$, and $e_3$ the path from $b$ to $V_\al$ or the next turn vertex on the path, now we discuss by cases:\begin{itemize}
%	\item  $e_1=F, e_2=R, e_3=F$: by local injectivity, $e_2=R$ restricts the vertex cost of encoding $a$ to be at most $2q|V(\al)|$, and hence, we can either flip all the edges in $e_1$ to $R$ to locally improve the value of edge, for all the vertices between $U_\al$ and $a$, we may lose a vertex factor of at most $n$, however, it can be charged to the edge factor we pick up, giving a change of \[
%	\frac{\sqrt{\frac{n}{d}}\cdot \frac{1}{\singdecay} }{n\cdot \frac{d}{n} \cdot \sqrt{\frac{n}{d}}\cdot \singdecay} >1	 \] Charging each vertex to the edge  leading to it from $U_\al$ on the simple path, we have an extra factor from the last edge incident to $a$ and this gives us a gain of \[\sqrt{\frac{n}{d}}/\left(2|V(\al)|q \cdot \sqrt{\frac{d}{n}}\cdot \singdecay\right) >\frac{n}{2|V(\al)|q}
% \] 
%	\item $e_1=R, e_2=F, e_3=R$: similarly, the value can be locally improved by either flipping $e_3$ to $F$ to avoid a surprise visit at $b$.
%\end{itemize}  
%\begin{lemma}
%	For any vertex $v$ in block $\al$ that has multiple simple paths from $U_\al$,  each of this path is of the structure $R\rightarrow H$ in any locally optimal labeling. Similarly, for any vertex $v$ that has multiple paths to $V_\al$, consider a BFS from $v$, each of this path is of the structure $H\rightarrow F$ in any locally optimal labeling.
%\end{lemma}
%\begin{proof}
%	It suffices for us to show the first half of the lemma. 
%\end{proof}
% From the structure lemma above, we notice any simple path from $U_\al$ to $V_\al$ is either all $F$ or all $R$ until some point, and then the label would be flipped thereafter. Let $S$ be the endpoints of $H$ edges in the optimal labeling (that uses the fewest $H$ labels), we notice that the above structure theorem of the labeling can also be extended to the following,
%\begin{lemma}
%	Any simple path from $U_\al$ to $V_\al$ is of the structure $R\rightarrow H\rightarrow F$. 
%\end{lemma}
%\begin{proof}
%[Proof required]
%\end{proof}
%\begin{claim}
%	Consider any optimal labeling $\calL$ of length-2 block, W.L.O.G., we can assume $\calL$ is symmetric w.r.t. $V_\al$, i.e., any edge that receives label $F$ (or $R$) in one copy would receive label $R$ (or $F$) in the other copy, and any edge that receives $H$ would receive $H$ in both copies.
%\end{claim}
\subsection{Bounding the block value for a locally optimal labeling}
Given $\calL$ any locally optimal labeling on $\al$ (or $\al^T$), we show in this section that it corresponds to a vertex separator. Let's start by building a separator from a locally optimal labeling.
\begin{mdframed}[frametitle = {Building a separator}]
\begin{enumerate}
	\item We include any vertex incident to an $H$ edge in $\calL$ into $S_\al$;
	\item Any vertex that is a turn vertex, i.e., it gets encoded into the cut along an $R$ edge and it is incident to some  $F$ edge;
	\item We include any vertex that is in $U_\al\cap V_\al$ into $S_\al$.
	\item Additionally, for any path from $U_\al$ to $V_\al$  that does not go through any included vertex, the path must be either all $R$ or all $F$ by our structure lemma, and we include the vertex from $V_\al$ into $S_\al$ if the path is all $R$, or the vertex from $U_\al$ into $S_\al$ if the path is all $F$.
\end{enumerate}	
\end{mdframed}



With a separator built at hand, we are ready to bound the corresponding block value for a given separator constructed from $\calL$. Let $S_L$ be the boundary of $S$ that can be reached from $U_\al$ without passing through any other vertex in $S$, and let $S_R$ be the boundary os $S$ that can be reached from $V_\al$ without passing through any other vertex in $S$. 



\subsubsection{Factors of $\sqrt{n}$}\label{sec:factors-of-root-n}
We start by bounding the vertex factors coming from $F/R$ edges in this subsesction.
\begin{claim}
	For a fixed labeling $\calL$ for $\al$, any non-dangling vertex that is arrived along some $F$ edge in either $\calL$ or $\calL^T$ contributes a factor of at most $\sqrt{n}$ to the block value $\vtxcost\cdot \edgeval$.
	Furthermore, for dangling vertices, they contribute an additional dangling factor $\dang(\al\setminus S)$.
	For floating vertices, they contribute an additional floating factor $\float(\al)$.
	\end{claim}
\begin{proof}
	For starters, the block value $\vtxcost\cdot \edgeval(\calL)$ can be bounded in two ways, either via a traversal from $U_\al$ to $V_\al$, or via a traversal from $V_\al$ to $U_\al$, and it suffices for us to bound it by \[\sqrt{\vtxcost_{U\rightarrow V}(\calL) \cdot \vtxcost_{V\rightarrow U}(\calL^\top) } \cdot \edgeval \]
	where we observe that edgeval comes from $H$ edges and does not depend on the direction of traversal.
	
	Let $v \in V(\al)\setminus U_\al$ be a vertex that is arrived along some non-signleton $F$ edge using the labeling $\calL$ when we traverse from $U_\al$ to $V_\al$, we pick up at most a vertex factor of $n$ for this vertex; however, once we traverse from $V_\al$ to $U_\al$ along the same path (but in the reverse direction), the vertex $v$ is either fixed from the last block (if it is in $V_\al$), or the corresponding $F$ leg now becomes an $R$ leg and the vertex factor is ''fixed'' (up to dangling factor). Combining with Prop.~\ref{prop: pur-invariant} , we have ,
	\begin{enumerate}
		\item For non-dangling vertices, the return leg is fixed and we do not pick up any vertex factor, hence on average, we pick up a factor of $\sqrt{n}$;
		\item For dangling branches, each branch contributes at most one factor of $2|V(\al)|q_\al$ for identifying the furtherest point on the each branch reachable via $R\cup H$ edges, and it suffices for us to assign a factor of $2|V(\al)|q_\al$ for each branch and set $\dang(\al) = \left(2|V(\al)|q_\al\right)^{|\branch(\al)|}$.
%		\item For each floating component, one of its vertices incident to a return leg in the component picks up an extra vertex factor of at most $2|V(\al)|q$, which is captured by the factor $\float(\al)$, hence in average we pick up $\sqrt{n\cdot 2|V(\al)|q}$.
	\end{enumerate}
%	
%	
%	For dangling vertices, we pick up an average of $\sqrt{n} \cdot  \dang(\al\setminus S)[v]$  where $\dang(\al\setminus S)[v]$ is the dangling factor assigned for vertex $v$ (upper bounded by $\sqrt{d}$).
%	
%	For each floating component, notice in addition to the factor in dangling vertex, an extra label in $2|V(\al)|q$ is needed when it appears again after the first time. Taking the average gives us a factor of $\sqrt{2|V(\al)q}$ for each connected component, and we assign this factor into $\float(\al)$.
	
	For vertices arrived along a singleton $F_\single$ edge in non-floating components, the claim is immediate since we can assign each vertex to an edge that leads to it: in either direction, we pick up a vertex cost of $n$ for the corresponding vertex while there is at least one leg (with factor assigned to this vertex) coming with singleton decay, giving us $n\cdot \sqrt{\frac{d}{n}}\cdot \singdecay \ll \sqrt{n} $. 
	
	\begin{claim}
		It suffices for us to assign a factor of $\sqrt{n}\exp(-d)$ for each floating component, i.e., $\float(\al) \leq \left(\sqrt{n}\exp(-d)\right)^{|\float(\al)|}$ where we recall $|\float(\al)|$ is the number of floating components. 
	\end{claim}
	\begin{proof}	Via our structure lemma, the edges in a floating component is either all $F$, $R$, or $H$:
	\begin{enumerate}
		\item \textbf{Singleton floating component}  We first consider $F$-component, where some extra care is warranted as singleton edges may now be troublesome. The previous argument for handling singleton edges crucially replies upon being able to assign each vertex to an edge that comes with singleton decay. However, this is no longer true for floating component, especially tree-like floating component: for example, consider an edge floating around in $\al$: should the edge be a singleton edge in the walk, it can contribute \[
	n^2 \cdot \sqrt{\frac{d}{n}}\cdot \singdecay \approx n^{1.5} \exp(-d) \gg \sqrt{n^2}\cdot (2|V(\al)|q_\al)	 \]
	where we recall $\sqrt{n^2}\cdot (2|V(\al)|q_\al)	$ is the cost we would expect if there is no conditioning. That being said, we may have one $\sqrt{n}$ blow-up, giving a bound of \[ 
	\sqrt{n}^{|V(C_i)|}\cdot \underbrace{\sqrt{n}\cdot \singdecay^{V(C_i)-1} }_{\float(C_i)}	\]	
	for each floating component $C_i$ where we can capture the potential blow-up by the corresponding floating factor.
	
	\begin{remark}
		A natural question is whether the $\sqrt{n}$ blow-up from conditioning is tight. We remark that it is possible as it comes down to bounding $\E[\chi_e \cdot 1_\calF ]$ where we recall $\calF$ is the conditioning on bounded-degree, and we can ignore the conditioning on $2$-cycle for this part. \begin{align*}
			\E[\chi_e \cdot 1_\calF ] &= \Pr\left[1_\calF \cap \left(\chi_e=\sqrt{\frac{1-p}{p}} \right)\right] \cdot \sqrt{\frac{1-p}{p}} + \Pr\left[1_\calF \cap \left(\chi_e=-\sqrt{\frac{p}{1-p}} \right)\right] \cdot (-\sqrt{\frac{p}{1-p}})\\
			&=\Pr\left[1_\calF|\chi_e=\sqrt{\frac{1-p}{p}}\right]\sqrt{\frac{1-p}{p}}\cdot p - \Pr\left[1_\calF|\chi_e=-\sqrt{\frac{p}{1-p}}\right] \cdot \sqrt{\frac{p}{1-p}}\cdot (1-p)\\
			& = (\sqrt{(1-p)p}) \left( \Pr\left[1_\calF|\chi_e=\sqrt{\frac{1-p}{p}}\right] - \Pr\left[1_\calF|\chi_e=-\sqrt{\frac{p}{1-p}}\right]\right)
			\end{align*}
			To bound the difference in the probability, we note that this is equivalent to resampling all the edges but $e$, what's the probability that at least one of the two endpoints of $e$ hit degree $10d-1$ (suppose we truncate at degree $10d$), and an $\exp(-d)$ bound here is the best we can hope for, which would give a bound of $\E[\chi_e\cdot 1_\calF] \approx \sqrt{\frac{d}{n}} \cdot \exp(-d)$ . Notice we need an extra $\frac{1}{\sqrt{n}}$ decay to offset the blow-up for a singleton $F$ component.
	\end{remark}
		\item \textbf{Non-singleton floating component} The argument is identical to the non-floating case except for the first vertex in the component (when being traversed the second-time or later), giving us a bound of \[ 
		\sqrt{n}^{V|(C_i)|}\cdot \dang(C_i) \cdot \underbrace{2|V(\al)|q_\al}_{\float(C_i)}
		\] 
		\end{enumerate}
		Combing the above, for each floating component, it suffices for us to take \[ 
		\float(C_i) \leq \max(\sqrt{n}\cdot (\singdecay)^{V(C_i)-1}, 2|V(\al)|q_\al) \leq \sqrt{n}\cdot \exp(-d)
		\]
		\end{proof}
 Applying the above claim on $\calL$ when we traverse from $U_\al$ to $V_\al$, and on $\calL'$ when we traverse from $V_\al$ to $U_\al$, any vertex that is arrived along an $F$ edge is outside the separator by our structure lemma, hence each vertex outside the separator contributes at most a factor $\sqrt{n}$ (modulo their corresponding dangling factors discussed above).
 \end{proof}
 
 \begin{corollary}
 	Any non-isolated vertex outside  $S$ contributes a vertex factor of $\sqrt{n}$ (modulo their corresponding floating and dangling factors).
 \end{corollary}
 \begin{proof}
 	This follows by observing that any vertex outside the separator is either \begin{enumerate}
 		\item if a vertex is connected to some path between $U$ and $V$, then it can be reached using $F$ edge in either $\calL$ or $\calL^T$ and contributes a $\sqrt{n}$ factor as above;
 		\item for vertices not connected to any path between $U_\al$ and $V_\al$, it may be a vertex that is in either $U_\al\setminus V_\al$ or in $V_\al\setminus U_\al$ while not connected to any path between $U$ to $V$, and they contribute $n$ in one direction and is again fixed in another direction;
 		\item Floating vertices have its factor captured by the floating component for the blow-up, that it gives a factor $n$ in one direction and a $2|V(\al)|q_\al$ factor in the other.
 	\end{enumerate}
 \end{proof}
 
 
%\subsubsection{Floating components don't like a re-visit}
%
%From the discussion in the above subsection, dangling vertices and floating components contribute an extra factor when they are visited the second-time and forwards. In particular, each floating component (even contained in the SMVS) requires an extra $2|V(\al)|q_\al$ label when it is being visited the second time or onwards. A peculiar question at this point is whether each floating component contributes an extra factor of $\sqrt{2|V(\al)q_\al}$ or a factor of $2|V(\al)|q_\al$ to the final norm bound?  Specifically, can we rule out a floating component being visited more than twice (beyond necessity to avoid singleton decay)? If so, a $2|V(\al)|q_\al$ is only required when a floating component is visited the second time, and averaging with the first visit gives us a $\sqrt{2|V(\al)|q_\al}$ contribution to the final bound. 
%
%	For convenience, we restrict our attention to component with no dangling branch, i.e., degree-$1$ vertex, or a path of those.  We case on whether the component contains more than $1$ cycle. Let $C$ be a floating component.
%\paragraph{Monocycle component}
%In this case, we have $|E(C)|\leq |V(C)|$, and we first observe that via structure lemma, all edges must be either all $F$, all $R$ or all $H$ as any mix of edge-status results in surprise visit for a floating component. It suffices for us to observe that in this case, the component must be either all $F$ or all $R$ to obtain maximal-value as an all $H$ labeling may contribute a value of at most \[ 
%2|V(\al)|q_\al \cdot \sqrt{\frac{n}{d} }^{|E(C)|} 
%\] 
%while taking 
%
%
%\begin{claim}[$R$-edge-value bound]\label{claim: R-edge-val-bound}
%	The edge-value coming from $R$ edges is at most $\sqrt{n}^{|L(U_\al\setminus S_L , S_L)|}$.
%\end{claim}
%\begin{remark}
%	Note this is a strengthened bound than assigning each $R$ edge a $\sqrt{n}$ factor. This is useful for avoiding a blow-up in the labeling value due to $R$ cycle.
%\end{remark}
%\begin{proof}
%	Consider a BFS from $S_L$ to traverse the vertices in $L(U_\al\setminus S_L , S_L)$, and note that the claim is immediate if there is no edge leading to visited vertices, as each edge comes with a value at most $\sqrt{n}$, and we can charge each edge to the vertex it leads to. However, by design of our edge-value assignment scheme, each excess $R$ edge corresponds to some excess $F$ edge (which only gets assigned a factor $1$), hence they do not contribute extra edge-value. 
%\end{proof}
%\begin{claim}
%	Each vertex reachable from $S$ via an $F$ edge comes with a most a vertex cost of $n$, and it suffices for us to assume each $F$ edge is non-singleton.
%\end{claim}
%\begin{proof}
%	For any singleton $F$ edge, it comes with an edge value of $\sqrt{\frac{n}{d}}\cdot \frac{d}{n}\cdot \singdecay \leq \sqrt{\frac{d}{n}}\cdot \exp(-d)  $, while flipping it to an non-singleton edge gives us an $\exp(d)$ improvement (as non-singleton $F$ edge comes with a value of $\frac{1}{\sqrt{n}}$.
%	\end{proof}



	

\subsubsection{Bounding the block value for any separator}
	Let's now try to bound the block value $\edgeval(\calL)\cdot \vtxcost(\calL)$ for any locally optimal $\calL$, let $S$ be the corresponding separator,
  \begin{enumerate}
  	\item Each vertex outside $S$ contributes a factor of $\sqrt{n}$;
	\item Each vertex in $S$ that is not doubly constrained in the encoding process is arrived along an $H$ edge, and hence requires at most a $\sqrt{d}$ vertex factor if non-dangling, and a factor of $d$ if dangling;
	\item Each edge receiving an $H$ label is in $E(S)$ and contributes a value of at most $\sqrt{\frac{n}{d}}$;
	\item For dangling branches, we pick up an additional dangling factor $\dang(\al)$, that is an additional $2|V(\al)|q_\al$ for each dangling branch;
	\item For floating components, an extra label in $2|V(\al)|q$ for each component is sufficient for each component.
\end{enumerate} 

For intuition, we recommend the reader to ignore factors from excess $F$ edges, and dangling vertices. However as stated, the above bound is not easy to apply as it is not immediately clear what vertex factors are needed for encoding vertices inside $S$; fortunately, this can be simplified once we restrict our attention to a class of separators, \emph{irreducible} separators, without any loss in the SMVS value.
 
 We now unpack the factors from the above in a more illustrative manner, and show that it suffices for us to assume each vertex in $S$ is doubly constrained by $S_L$, and moreover, there is no dangling vertex inside $S$.
%\begin{observation}[$\sqrt{n}$ for each vertex outside $S$, and an extra $\sqrt{d}$ if dangling]
%	Charging the edge-value of the $R$ edge leading to that vertex in the BFS process from $S_L$ if the vertex is in $L(U_\al\setminus S_L, S_L)$, or the edge value of the non-excess $F$ edge that leads to the vertex in the BFS from $S$, and the vertex cost, each (non-dangling) vertex in $V(\al)\setminus S$ contributes a value of $\sqrt{n}$. Each vertex dangling picks up an extra $\sqrt{d}$ factor and contribute a total of $\sqrt{nd}$.
%\end{observation}
%\begin{observation}[$\sqrt{\frac{n}{d}}$ for each separator edge] Each edge inside the separator receives an $H$ label, and contributes a value of $\sqrt{\frac{n}{d}}$.
%\end{observation}
\subsubsection{Pruning superfluous $H$ edges}\label{sec:pruning-superfluous-H}

\begin{definition}[Irreducible SMVS]
	We call a separator $S$ an irreducible SMVS for a shape $\al$ if for any vertex $v\in S$ of degree $1$ in $E(S)$,  \begin{enumerate}
		\item There are two edge-disjoint paths $P_U, P_V$ from $v$ to $U_\al$ and $v$ to $V_\al$
		\item Both paths do not pass through any other vertex in $S$
	\end{enumerate}
\end{definition}

\begin{claim}
	For each locally optimal $\calL$ labeling that produces separator vertices in $S(\calL)$ not doubly constrained by $S_L(\calL)$, there is a labeling $\calL'$ with at least the same SMVS value while each vertex in $S(\calL')$ is doubly constrained by $S_L(\calL')$. Moreover, there is no dangling vertex in $S(\calL')$.
\end{claim}
\begin{proof} We start by considering non-dangling vertices in $S$.
	We first notice for any vertex in $S_L$ of degree $1$ in $S$, unless it is incident to an $F$ edge, we can pop it out of the separator and obtain the same value by turning the incident $H$ edge into an $R$ edge: the $H$ edge contributes at most a $\sqrt{d}$ vertex factor to indicate the destination of the edge and it contributes a factor of $\sqrt{\frac{n}{d}}$ through the edge-value, while we obtain the same value by picking the $\sqrt{n}$ value from the vertex being outside the separator. 
	
	Let $\calL'$ be the labeling obtained by applying the above procedure on $\calL$, and let $S = S(\calL')$ be its corresponding separator. Consider a BFS from $S_L$ to traverse vertices in $S\setminus S_L$, and note that each vertex in the separator not doubly constrained by $S_L$ has only one simple path to $S_L$, and it is not on any path from $S_L$ to a cycle. In other words, given $S_L$, each non-doubly constrained vertex forms a tree rooted at $S_L$. For each branch, starting from the leaf vertex, notice each vertex (if non-dangling) contributes to the block value via the edge that leads to that vertex from $S_L$ a factor of $\sqrt{\frac{n}{d}}$ and a vertex factor $\sqrt{d}$ for indicating the destination of the $H$ edge, giving a total of $\sqrt{\frac{n}{d}}\cdot \sqrt{d}=\sqrt{n}$. However, the same value can be attained by flipping the $H$ edge to an $F$ edge and pop this vertex out of the separator. 
	
	For each dangling vertex, the pop-out procedure is rather identical except we now need to take into account the dangling factor. Suppose it is indicated using a label in $d$, it contributes a value of $\sqrt{\frac{n}{d}}\cdot d=\sqrt{nd}$ while we can again pop the vertex out of the separator and obtain a value of $\sqrt{nd}$ with the extra $\sqrt{d}$ coming from the dangling factor $\dang$; analogously, we can generalzie this argument for long dangling branch inside the separator, we can again use the idea in Proposition~\ref{prop:long-high-mul-path}, and obtain a $\sqrt{2|V(\al)|q}$ bound as we would have 
%		For each dangling branch, notice each edge comes with a value of $\sqrt{\frac{n}{d}}^{\branch(i)}$, while each time a label in $2|V(\al)|q$ or a sequence of labels in $d$ is needed, giving us a total of 
\begin{align*}
		\sqrt{\frac{n}{d}}^{\branch(i)}\min(2|V(\al)|q, d^{\branch(i)}) &\leq 
	\sqrt{n}^{\branch(i)} \min(\frac{2|V(\al)q}{\sqrt{d}^{\branch(i)} }, \sqrt{d}^{\branch(i)}) \\&\leq \sqrt{n}^{\branch(i)}\min(\sqrt{2|V(\al)|q} ,\sqrt{d}^{\branch(i)})
	\end{align*}
	Note that this is the same value we would pick up from vertex factors if we pop out the entire dangling branch, and this completes our proof to the claim.
%	Recall that the factors of $\sqrt{n}^{\branch(i)}$ is already taken into account by the vertex factors of $\sqrt{n}$ for each vertex outside the separator, hence, each block's dangling blow-up is still at most $\min(\sqrt{2|V(\al)|q} ,\sqrt{d}^{\branch(i)})$ for each branch. Combining the argument for all dangling branches gives us the desired proposition.
%
%	
\end{proof}
%
%Wrapping up, the above claim allows us to assume each vertex in $S$ being doubly-constrained by $S_L$; analogously, applying this argument on $\calL^T$ allows us to assume $S\setminus S_R$ being doubly constrained by $S_R$. 
% \begin{align*}
%	\val(\calL)= \vtxcost(\calL)\cdot \edgeval(\calL) \leq \max_{S:\text{separator}}\sqrt{n}^{|V(\al)\setminus S|}\cdot \left(\sqrt{\frac{n}{d}}\right)^{|E(S)|}\cdot \sqrt{d}^{\dang}\cdot  \sqrt{d}^{|\exc(F)|}
%\end{align*}
%
%\subsubsection{Is there floating component inside $S$?}
%\begin{claim}
%	Let $S$ be the separator, $S\cap \float_\al = \emptyset$.
%\end{claim}
%\begin{proof}
%	Let $C$ be a floating component, and consider $C\cap S$. Pick an arbitrary vertex in $C\cap S$ to be the landing vertex for the corresponding floating component, for which we use a label in $2|V(\al)|q$. Notice the above pruning argument applies and we can assume any vertex in $C\cap S$ is doubly-constrained by any other vertex in $C\cap S$. Moreover, for each landing vertex, there is at most one nearby short-cycle, hence there is no extra encoding needed for identifying the vertices in $C\cap S$ beyond the landing vertex, giving us a block value of $ 
%	2|V(\al)|q\cdot  \sqrt{\frac{n}{d}}^{|E(C\cap S)| }
%	$.
%	
%	However, consider the separator obtained by popping out $C\cap S$, we pick up a value of $
%	\sqrt{n}^{|V(C\cap S)| }\cdot \sqrt{2|V(\al)|q}
%	$
%	where we note that any vertex doubly-constrained by the landing vertex of $C\cap S$ is also fixed (up to cyclic rotation) and there is no encoding factor needed beyond the landing factor. Ignoring the $\sqrt{2|V(\al)|q}$ gap, notice the separator value with $C\cap S$ is dominating unless $|E(C\cap S)|- |V(C\cap S)| \geq \frac{|E(C\cap S)|}{\log_d n}$.
%\end{proof}
%

\subsubsection{Not too many excess edges outside $S$}\label{sec:not-too-many-exc}
We remind the reader that $\sqrt{d}^{|\exc(F)|}$ is an artifact of our encoding since we encode a potential direction for future unforced return that may be incurred due to the excess edge, however, we point out that this is not too terrible a cost to pay as in any optimal labeling, there cannot be too many $\exc(F)$ edges, and we can handle the blow-up via edge-decay in the optimal labeling. \begin{proposition}
	Let $\calL$ be a locally optimal labeling, and $\exc(F)$ be the number of $F$ edges that lead to visited vertices when we consider a BFS from $S$,  \[ 
	\exc(F)< \lceil \frac{|F\setminus \exc(F)|}{\log_d n}\rceil
	\]
\end{proposition}
\begin{proof}
This follows from the optimality of SMVS, consider the new separator formed by including all vertices reached by $F$ edges, which gives us a change of $
\sqrt{n}^{-|F\setminus \exc(F)| } \cdot \sqrt{\frac{n}{d}}^{|F|}<1
$.
\end{proof}

	
\subsubsection{Wrapping up block value bound}
We are now ready to wrap up our bound for the block value.
\begin{proposition}
	For any irreducible locally optimal labeling $\calL$, let $S$ be its corresponding separator, \[		\vtxcost(\calL)\cdot \edgeval(\calL) \leq  (1+\eps)^{E(\al)}\cdot \sqrt{n}^{|V(\al)\setminus S|}\cdot \left(\sqrt{\frac{n}{d}}\right)^{|E(S)|}\cdot \dang(\al\setminus S)\cdot \float(\al )\cdot \sqrt{n}^{\mathsf{iso}(\al)}
	\]
	with \[ 
	\dang(\al\setminus S) \leq \prod_{b_i\in \branch(\al\setminus S)}\min \left(\sqrt{d}^{|b_i|}, 2|V(\al)|q_\al\right)
	\]
	and 
	\[
	\float(\al) = \left(2|V(\al)|q_\al \right)^{|\float_\al| }
	 \]
	 where $|\float_\al|$ is defined to be the number of floating components in $\al$, and $\iso$ the number of isolated vertices.
\end{proposition}
\begin{proof}
Recalling the factors accounted from above, 
	\begin{enumerate}
  	\item Each vertex outside $S$ contributes a factor of $\sqrt{n}$  (via \cref{sec:factors-of-root-n});
	\item Each vertex in $S$ is doubly constrained by the boundary of $S$ (via \cref{sec:pruning-superfluous-H});
	\item Each edge receiving an $H$ label is in $E(S)$ and contributes a value of at most $\sqrt{\frac{n}{d}}$;
	\item For dangling vertices, we pick up an additional dangling factor $\dang(\al\setminus S)$; each floating component comes with an extra $2|V(\al)|q_\alpha$ factor captured by $\float(\al)$;	\item  Each excess $F$ edge that leads to visited vertices incur an extra cost of $d$ for the potential unforced return it may induce, however, this is subsumed by edge decay (via \cref{sec:not-too-many-exc}).
	\end{enumerate} 

\end{proof}


\paragraph{Bounding the number of maximal value labelings}
To complete our norm bound, it remains for us to bound the number of maximal value labeling, and a naive bound would be $3^{E(\al)}$ by specifying the edge label for each edge, while we notice this can be improved to $3^{|V(\al)\setminus (\iso_\al\cup  U_\al\cap V_\al)|}$ as it suffices for us to indicate whether each vertex is inside the separator, and whether it is reached using an $H$ edge. Moreover, each vertex in $U_\al\cup V_\al$ is by definition inside the separator while vertex in $\iso_\al$ is bound to be outside the separator (otherwise giving a $2|V(\al)q/n$ gap from the maximal value). 

 The following corollary is then immediate once we maximize over any block labelings, \begin{corollary} 
For any $\eps>0$, any shape $\al$,we can bound its block value by\begin{align*}
	B_q(\al)&\coloneqq   \cdot 3^{|V(\al)\setminus (\iso_\al\cup  U_\al\cap V_\al)|} \cdot   \max_{\calL} \vtxcost(\calL)\cdot \edgeval(\calL) \\&\leq 3^{|V(\al)\setminus (\iso_\al\cup  U_\al\cap V_\al)|} \max_{S:\text{separator}}\cdot \sqrt{n}^{|V(\al)\setminus S|}\cdot \left(\sqrt{\frac{n}{d}}\right)^{|E(S)|} \cdot \dang(\al\setminus S)\cdot \float(\al)\cdot \sqrt{n}^{\iso_\al}
\end{align*}
\end{corollary}

\begin{lemma}\label{lem:shape-walk-val}
Given edge labeling on $t$-blocks $B_1,\dots, B_t$ for some $t\leq q_\al $, let $\vtxcost_t, \edgeval_t$ denote the vertex-cost and edge-value at the end of the $t$-th block,  \[ 
\vtxcost_{q} \cdot \edgeval_{q} \leq \sqrt{n}^{|U_\al|+|V_\al|}\cdot  B_q(\al)^{2q}
\]  
%Moreover, if there are $s$ singleton edges in the first $t$ blocks, the above bound can be improved to \[ 
%\vtxcost_{t} \cdot \edgeval_{t} \leq n^{|U_\al|}\left(\max_{S:\text{separator}}  \sqrt{n}^{2(|V(\al)|-|S|)}\left(\frac{n}{d}\right)^{|E(S)| }\right)^{t} (\singdecay)^s
%\]
\end{lemma}
\begin{proof}
	To see the above bound, first considering traversing from the direction of $U_\al\rightarrow V_\al$. And note that we can bound $\vtxcost_q\cdot \edgeval_q\leq n^{|U_\al|}\cdot B_q(\al)^{2q}$ by induction. Traversing the other way gives us $\vtxcost_q\cdot \edgeval_q \leq n^{|V_\al|} \cdot B_q(\al)^{2q}$. Taking the average then yields the desired bound.
		

%		 Taking the $\frac{1}{2q}$-th root gives us the desired upper bound of \[ 
%	 \max_{\calL:\text{labeling}} (\vtxcost(\calL)\cdot \edgeval(\calL))^{2q}\leq \max_{S:\text{separator}}\left(\sqrt{\frac{n}{d}}\right)^{|E(S)|}\cdot \sqrt{d}^{\dang}\cdot (2|V(\al)|q)^{\float }
%	 \]
%	 provided $n^{\frac{|U_\alpha|}{2q}}<1+o(1)$, which would suffice if we take $q=\Theta(|U_\al|\log^2 n)$. By symmetry, we can also apply this argument on $\al^T$, which would require us to have $n^{\frac{|V_\al|}{2q}|}<1+o(1)$, and hence we can take the average by setting $q=\Theta(\sqrt{|U_\al|\cdot |V_\al| }\log^2n )$.
\end{proof}


This completes our discussion for order-tuple indexed graph matrix. That being said, we work with a slightly more challenging setting in which our matrix is indexed by set, and this shall be our topic for the upcoming section.

%%

%\subsection{Wrapping up}
%We now show our main theorem from the above lemmas. For any $\eps>0$ and $q\in \N$, \begin{align*}
%	\Pr[\|M_\al\|> B_q(\al)+\epsilon ] &\leq \Pr[\Tr \left(M_\al M_\al^T \right)^q> (B_q(\al)+\epsilon)^{2q} ] \\
%	&\leq \frac{\E\left[\Tr\left(M_\al M_\al^T)^q\right)\right] }{(B_q(\al)+\eps)^{2q}}\\
%	&\leq \frac{n^{|U_\alpha|}B_q(\al)^{2q} }{(B_q(\al)+\eps)^{2q} }  &\text{(by main lemma )}\\
%	&\leq 
%\end{align*}


==> sparse_trace_method/new-prelim.tex <==
\section{Preliminaries}
\subsection{Graph Matrix Preliminaries}
\begin{definition}[Ordered-tuple indices]
	Each ordered-tuple index is represented by a set $S\subseteq [n]$ and an ordering $\calO_S$ of elements in $S$. The size of ordered-tuple indices is given by $|S|$.
\end{definition}
\begin{definition}[Graphical matrix for shape indexed by ordered-tuple]
Given a shape $\al$, we define graphical matrix (indexed by ordered-tuple) to be the matrix indexed by all possible ordered-tuples of $[n]$ with non-zero entries at $(S,\calO_S),(T,\calO_T)$ matrix ordered-tuple indices of size $|U_\al|$ and $|V_\al|$ s.t. \[ 
M_{\al,\calO}[(S,\calO_S),(T,\calO_T)] = \sum_{\substack{f:V(\al)\rightarrow [n] \text{injective},\\ f(U_\al )=(S, \calO_S), 
 f(V_\al)=(T,\calO_T)\\ f(U_\al\cap V_\al) = (S\cap T, \calO_{S\cap T} )}  } \prod_{e=\{i,j\}\in E(\al)} \chi_G(f(i),f(j))
\]
where $G$ is an underlying random graph sample, and $\calO_S, \calO_T$ are orderings for vertices in $S$ and $T$.
\end{definition}

Analogously, we can define the graphical matrix for shape indexed by set-indices.

\begin{definition}[Set-index]
	Each set index is represented by a set $S\subseteq [n]$. The size of set indices is given by $|S|$.
\end{definition}
\begin{definition}[Consistent ordering]
Given a ribbon $R $ with $U_R = S, V_R = T$, and $\calO_S, \calO_T, \calO_{S\cap T}$ an ordering for 
	$S$ and $T$, we call $(\calO_S, \calO_T ,\calO_{S\cap T})$ a consistent ordering if there are orderings $\calO_{S}$ and $\calO_{S\cap T}$ agree on the ordering for vertices in $S\cap T$, and similarly, $\calO_{T}$ and $\calO_{S\cap T}$ agree on the ordering for vertices in $S\cap T$.
\end{definition}

\begin{definition}[Graphical matrix for shape indexed by set]
Given a shape $\al$, we define graphical matrix (indexed by set) to be the matrix indexed by all possible subsets of $[n]$ with non-zero entries at $S,T$ matrix set-indices of size $|U_\al|$, $|V_\al|$ and $S\cap T$ a set index of size $|U_\al\cap V_\al|$ s.t. \[ 
M_\al[S,T] = \sum_{\substack{f:V(\al)\rightarrow [n] \text{injective},\\ \exists \calO_S s.t. f(U_\al)=(S, \calO_S),\\ \exists \calO_T s.t.
 f(V_\al)=(T,\calO_T) \\ f(U_\al\cap V_\al) = (S\cap T, \calO_{S\cap T}) }} \prod_{e=\{i,j\}\in E(\al)} \chi_G(f(i),f(j))
\]
where $G$ is an underlying random graph sample, and $\calO_S, \calO_T$ are orderings for vertices in $S$ and $T$ and $\calO_{S\cap T}$ an ordering for $S\cap T$ consistent with $\calO_S, \calO_T$.
\end{definition}
\begin{remark}
Throughout our work, we will use $M_\al$ to denote graphical matrix with set indices and $M_{\al, \calO}$ with ordered-tuple indices.
\end{remark}



%\begin{definition}[Tree-like shape]
%	We call a shape $\al$ tree-like if there is no short cycle in the shape $\al\circ\al^T$ and $\al^T\circ \al$, i.e., every vertex has only one path to $U_\al\cup V_\al$.
%\end{definition}
%\begin{definition}
%	We call a shape cyclic if it is not tree-like.
%\end{definition}
\subsection{Trace Method Preliminiaries}
\begin{definition}[Indicator functions]
	Let $\bdd[G]$ be the indicator function for bounded degree, i.e. $\bdd[G]=1$ if every vertex in $G$ has degree bounded by $d$, and $0$ otherwise; let $\cycle[G]$ be the indicator function for the absence of nearby $2$-cycle, i.e., $\cycle[G]=1$ if there is no nearby $2$-cycle in $G$, and $0$ otherwise.
\end{definition}
\begin{definition}[$2$-cycle free radius]
	Let $\kappa$ be the radius of $2$-cycle free neighborhood. It will be set as $\kappa \coloneqq 0.3\log_d n$.
\end{definition}
\begin{definition}[Edge and leg]
	We use ''edge'' to refer to the undirected edge in the underlying random graph sample, and ''leg'' to refer to a directed edge in the walk. \end{definition}

\begin{definition}[Singleton edge]
	We call an edge singleton if it is only used once in the walk.
\end{definition}
\begin{definition}[Surprise/excess leg]
We call a leg a surprise/excess leg if it uses a new edge to lead to a visited vertex in the walk. \end{definition}

\subsection{Shape terminology}
\begin{definition}[Floating vertex, and floating component]
	For a given shape $\al$, we call a connected component $Q\subseteq V(\al)$ a floating component if $Q$ is not connected to $U_\al \cup V_\al$. For each floating component, we arbitrarily pick a vertex to be the first vertex of the component in encoding. Let $E_\al(\float)\subseteq E_\al$ be the set of edges in a floating component.
\end{definition}
\begin{definition}[Simple path]
	We call a path simple if it does not traverse any edge more than once. However, it may traverse a vertex more than once.
\end{definition}
\begin{definition}[Dangling and non-dangling vertex]
	For a given shape $\al$, we call a vertex $v\in V(\al)$ a ''dangling'' vertex if it is not on any simple path from $U_\al\setminus V_\al $ to $V_\al\setminus U_\al$; otherwise, we call the vertex ''non-dangling''. We denote the set of dangling (and non-dangling) vertices of shape $\al$ by $V_\al(\dang)$ (and  $V_\al(\nd)$) respectively.
\end{definition}
\begin{definition}[Dangling branch]
	 Given a shape $\al$, let $\dang(\al)$ be the set of dangling vertices not on any path from $U_\al\setminus V_\al $ to $V_\al\setminus U_\al $ 
\end{definition}


%\begin{definition}[Dangling and non-dangling edge]
%	An edge is ''dangling'' if it is incident to a dangling vertex; otherwise, it is non-dangling. We denote the set of edges by $E_\al(\dang)$ and $E_\al(\nd)$ respectively. By construction, $E_\al(\dang)$ and $E_\al(\nd)$ partitions $E_\al\setminus E_\al(\float)$.
%\end{definition}
%\begin{definition}[Track and branch vertex]
%	For a given shape $\al$, fix $P$ a collection of non-backtracking vertex disjoint paths from $U_\al$ to $V_\al$, \begin{itemize}
%		\item Track vertex: a vertex is a ''track'' vertex if it is on a vertex-disjoint path in $P$;
%		\item Branch vertex: a vertex is a ''branch'' vertex if it is not on any vertex disjoint-path in $P$.
%	\end{itemize}
%  We denote the set of vertices by $V_\al(\branch)$ and $V_\al(\track)$ respectively. By construction, $V(\branch)$ and $V(\track)$ forms a partition of $V(\nd)$. 
%\end{definition}
%\begin{definition}[Track and branch edge]
%	For a given shape $\al$, fix $P$ a collection of non-backtracking vertex disjoint paths from $U_\al$ to $V_\al$, \begin{itemize}
%		\item Track edge: an edge on some vertex-disjoint path in $P$;
%		\item Branch edge: an edge not on any vertex disjoint-path in $P$.
%	\end{itemize}
%      We denote the set of edges by $E_\al(\branch)$ and $E_\al(\track)$ respectively. By construction, $E(\branch)$ and $E(\track)$ forms a partition of $E(\nd)$. 
%\end{definition}
%
%\begin{definition}[Constrained vertices and edges] 
%	For a given shape $\al$, and $P$ a collection of non-backtracking vertex disjoint paths, for a given set of edges $E\subseteq E(\branch)$, we call a vertex $v\in V_\al $ constrained by $E$ if \begin{itemize}
%		\item $v\in V(\branch)$ and $v$ is incident to an edge in $E$;
%		\item $v\in V(\track)$ and $v$ has at least $2$ paths in $E_\al$ to $V(E)$. 
%	\end{itemize}  
%	An edge is constrained by $E$ if it has both end-points in $E$. Let $R(E)\subseteq E_\alpha$ be the set of edges constrained by $E$.
%\end{definition}
%
\begin{definition}[Sparse MVS]
	For a given shape $\al$ with no floating and dangling vertex, we let $S$ the Sparse MVS be the maximizer of \[ 
	\max_{S:\text{ separator}} \sqrt{n}^{V(\al)-V(S)}\left(\sqrt{\frac{n}{d}} \right)^{E(S)}
	\]
	And we call the above quantity its corresponding SMVS-value.
\end{definition}
\begin{definition}[$S_L$ and $S_R$]
	For a given shape $\al$, for a vertex $v\in S$, \begin{enumerate}
		\item $v\in S_L$ if it can be reached from $U_\al$ without passing through any other vertex in $S$;
		\item $v\in S_R$ if it can be reached from $V_\al$ without passing through any other vertex in $S$;
	\end{enumerate}
\end{definition}

%\begin{proposition}
%	For each (non-dangling) vertex $v\in S_M$, it has at least $2$ paths of combined length at most $\log _d n$ to $S_L$ (possibly leading to the same vertex and thus forming a cycle), and similarly $2$ paths to $S_R$.
%\end{proposition}
%\begin{proof}
%	Fix a vertex $v\in S_M$, we first observe $v$ must be incident to at least $2$ edges in $E(S)$, otherwise removing $v$ from $S$ violates the maximality of $S$ since $v$ is non-dangling (causing a change of $\sqrt{n}\left(\sqrt{\frac{n}{d}} \right)^{-E(v)}\leq 1)  $. W.L.O.G., we can assume one edge incident to $v$ is on a path that leads to some vertex in $S_L$, it now remains to show the other edge is on a path that leads to some vertex in $S_L$ as well. 
%\end{proof}
\begin{definition}[Doubly constrained]
	Given a vertex $v$, and a set of vertices $S$, and a set of edges $E$, we say that $v$ is doubly-constrained by $S$ if $v$ has two (simple) paths to $S$, or $v$ is on a path from $S$ to a cycle  in $E$.  
\end{definition}
%\begin{proposition}
%	Fix an ordering of vertex-disjoint paths from $U_\alpha$ to $S_L$, $S_R$ to $V_\al$ (and analogously, $V_\al$ to $S_R$ and $S_L$ to $U_\al$), specifically for a fixed ordering of vertices in $S_L$ (and in $S_R$), for each vertex $v\in S_L$, let $D(v)\subseteq S\setminus S_L$ (and analogously $D(v)\subseteq S\setminus S_R$ for $v\in S_R$) be the set of vertices that turn doubly-constrained once $v$ is specified along with vertices in $S_L$ specified before $v$.
%\end{proposition}
%\begin{proposition}
%	For $S$ an SMVS, each vertex in $S\setminus S_L$ is doubly constrained by $S_L$, and each vertex in $S\setminus S_R$ is doubly constrained by $S_R$.
%\end{proposition}
%\begin{remark}
%	For convenience, we set dangling vertices not involved in any cycle to be outside the SMVS by default, as they contribute a factor of $\sqrt{nd}$ either way. 
%\end{remark}
%\begin{proof}
%	Fix a vertex $v\in S\setminus S_L$, we first observe $v$ must be incident to at least $2$ edges in $E(S)$, otherwise removing $v$ from $S$ violates the maximality of $S$ since $v$ is non-dangling (causing a change of $\sqrt{n}\left(\sqrt{\frac{n}{d}} \right)^{-E(v)}\leq 1)  $. W.L.O.G., we can assume one edge incident to $v$ is on a path that leads to some vertex in $S_L$. Consider the other edge, if it is on some path that leads to some vertex in $S_R\setminus S_L$, and the path does not lead to any cycle, removing the vertex $v$ as well as any other vertex on the path preserves the separator while it violates the maximality again. 
%\end{proof}
\begin{definition}[High-mul mirror walk]
	Given a length-$2$ block, for a given vertex $v\in V(\al)$, let $v^T\in V(\al)$ be the copy of vertex $v$ in $\al^T$; assume $v\in V(\al)$ receives label $L(v)\in [n]$ in the walk, if there is more than $1$ path of hig-mul edges from $v$ to $v^T\in V(\al^T)$, we call it a high-mul mirror walk if every vertex $u\in V(\al)$ on the high-mul path is receives the same label of its corresponding mirror vertex in $\al^T$, i.e. $L(u)=L(u^T)$.  
\end{definition}
\subsection{Block walk for graph matrices}
To bound the trace, it is useful to expand out the sum and notice each term can be described by a shape-walk as the following.
%\begin{definition}[Shape-walk for ordered-tuple indices]
%	Consider a mapping $P:V(\al, 2q)\rightarrow [n]$, we call it a shape-walk for ordered-tuple indices if it is locally injective in each $\al$ (and $\al^T$) block, and for each block $i\in [q]$, we have $U_{\al_i}=U_{\al^T_{i-1}}$, and $V_{\al_i}=V_{\al^T_{i}}$ with the equality hold as an ordered-tuple.
%	\end{definition}
\begin{definition}[Constraint-graph for ordered-tuple indices]
	Given a shape $\al$, and a $q\in \N$,  we define $V(\al,2q)$ to be the multigraph defined as the following,\begin{enumerate}
		\item Take $q$ copies of $\al_1,\dots,\al_q$ of $\al$, and $q$ copies of $\al_{1}^T,\dots, \al_q^T$ of $\al^T$;
		\item For each $i\in [q]$, we require the boundary to be consistent, i.e. $(V_{\al_i}, \calO_{V_{\al_i}}) = (V_{\al_i^T}, \calO_{V_{\al^T_i}})$, and $(U_{\al_i}, \calO_{U_{\al_i}}) = (U_{\al_{i-1}^T}, \calO_{V_{\al^T_{i-1}}})$ (where we denote $\al_0=\al_q$). 
		\item We call each $\al, \al^T$ block of the constraint graph a shape walk.
	\end{enumerate}
\end{definition}
\begin{definition}[Constraint-graph for set indices]
	Given a shape $\al$, and a $q\in \N$,  we define $V(\al,2q)$ to be the multigraph defined as the following,\begin{enumerate}
		\item Take $q$ copies of $\al_1,\dots,\al_q$ of $\al$, and $q$ copies of $\al_{1}^T,\dots, \al_q^T$ of $\al^T$;
		\item Each boundary $U_\al, V_\al$ is specified by an ordered tuple $(U_{\al_i},\calO_{U_{\al_i}})$ and $(V_{\al_i},\calO_{V_{\al_i}})$;
		\item For each $i\in [q]$, we require the boundary to be consistent as set, i.e. there exits a permutation $\sigma $ s.t. $\sigma(V_{\al_i},\calO_{V_{\al_i}})  = (V_{\al_i^T},\calO_{V_{\al_i^T}})$, and $\sigma(U_{\al_i}, \calO_{U_{\al_i}}) = (U_{\al_{i-1}^T},\calO_{U_{\al_{i-1}}}) $ (where we denote $\al_0=\al_q$);
		\item We call each $\al, \al^T$ block of the constraint graph a shape walk.
	\end{enumerate}
\end{definition}


	Each term in the summation of $\Tr\left[(M_\al M_\al)^{q}\right]$ is a shape-walk, and each ordered-tuple indexed shape walk is also a set-indexed shape-walk. The constraint graph for set indices can be decomposed into shape walks indexed by ordered-tuple with an additional permutation of the boundary set between blocks. 
	
With the observation above, we will start by working with graphical matrices indexed by ordered-tuples \cref{sec: maxval-labeling}, and then show how the permutation-jump on the boundary can be incorporated in \cref{sec:permutation-jump}. 
%\begin{definition}[Canonical walk]
%	A canonical walk $\calP$ is partition of constraint graphs s.t. for any $P,P'\in \calP$  if there is a permutation $\sigma:[n]\rightarrow [n]$ s.t. for each vertex $v\in V(\al,2q)$, $\sigma(P(v))=P'(v)$.
%\end{definition}
%\begin{observation}
%	Given a canonical walk $\calP$, let $\comb(P)$ be the number of distinct vertices visited in $\calP$, there are at most $n^{\comb(P)}$ shape-walks in the partition of $\calP$.
%\end{observation}

==> sparse_trace_method/order-return.tex <==
\subsection{(Non-dangling) Second-use return is forced} \label{sec:return-cost}
%For each vertex, consider the following quantity 
%\begin{proposition}
%	 Let $\calL$ be a maximal-value labeling, for any vertex $v\in V(\al)$ and any $H_v$ an $H$ component in $\calL$, \[ 
% \branch(H_v) \leq \dang(H_v) + 1
%\]
%\end{proposition}

In this subsection, we identify the cost of identifying a vertex arrived using some $R$ edge, i.e., edge that appears the second-time. On a high-level, the vertex-choice for the destination of such edge is fixed: for example, when we are traversing a tree from some root, each vertex only has $1$ edge that goes towards the root. That said, things might get slightly more complicated when the walk is no longer tree-like. Intuitively, any confusion for determining the vertex reached by an $R$ edge can be settled with a cost of $O(d)$ using degree bound, however, this would render us a trivial bound of $\sqrt{nd}$ analogous to row-sum bound. 

To get around with this, we note that any such confusion can be charged with a gap in the previous walk, which offers us a gap to encode auxiliary data for settling such confusion. Concretely, we relate the potential confuseion in determining destination of a return edge via \emph{surprise visit} \footnote{The argument in this section also relies upon another quantity \emph{missed-immediately-return} which can be seen as a proxy to surprise visits} , i.e., edges leading to visited vertices in the walk which correspond to some gap in our walk.

\begin{definition}[Potential-unforced-return factor $\pur$]
	At time $t$ (before the corresponding edge being processed), for each vertex $v$, let $\pur_t(v)$ be defined as the following,\begin{enumerate}
		\item Each return leg closed from $v$ contributes an $1$ to $\pur_t(v)$;
		\item Each unclosed $F$ edge currently incident to $v$ contributes an $1$;
		\item An extra $-1$ as we can maintain a counter for each vertex such that there is always one potential return-leg presumed to be forced.	\end{enumerate}
		Let $H_{v,t}$ be the component reachable using subsequent $H$ edges from $v$ at time $t$, and define \[ 
		\pur_t(H_v) \coloneqq \sum_{i\in H_{v,t}} \pur_t(i)
		\] 
\end{definition}
\begin{remark}
	The definition of $\pur_t(v)$ does not require $v$ to be on the boundary at time $t$ (similarly for $H_{v,t}$), while we are only interested at the desired invariant when it appears on the boundary.  
\end{remark}
%%\begin{definition}[Anchor vertex]
%	We call a vertex $v$ an anchor vertex if it opens up multiple $F$ edges at some single time-stamp in the walk.
%\end{definition}
\begin{definition}[Surprise visit counter] For a time-stamp $t$, for each vertex $v$ and $H_{v,t}$ defined above, let $s_t(v)$ be the number of surprise visits arriving at $v$ revealed by time $t$; we analogously define $s_t(H_v) = \sum_{i\in H_v} s_t(i)$.
\end{definition}
\subsection{Starting from the basic: a forced-return argument for $1$-in-$1$-out}

\begin{proposition}\label{prop: pur-invariant}
	Throughout the walk in which any vertex opens up at most $1$ edge each time it appears on the boundary,  we maintain the invariant \[ 
	\pur_t(H_{v,t}) \leq 2\cdot s_t(H_{v,t}) 
	\]
	for $H_{v,t}$ the $H$-component reachable from the current boundary vertex $v$.
	
%	In general, for a walk with no dangling vertex while a vertex (or an $H$ component) may open up more than $1$ $F$ edge at the boundary, we maintain the invariant \[ 
%	\pur_t(H_{v,t}) \leq 2\cdot s_t(H_{v,t}) + \mir_t(H_{v,t})
%	\]
\end{proposition}
\paragraph{Overview: unforced-return ignoring $H$ edges }
For starters, we observe for a single vertex $v$, if there is no $H$ edge being used throughout the walk and each vertex opens up at most $1$ edge on the boundary, \begin{enumerate}
%	\item Since each vertex opens up at most $1$ $F$ edge on the boundary, $\mir$ is $0$ throughout;
	\item When $v$ is first revealed, as base case, the return from $v$ must be using the edge that explores $v$, and we have $\pur(v)=0$;
	\item Each departure from $v$ may add $1$ potential-unforced-return edge as it adds an unclosed incidental $F$ edge to $v$, and departure from $v$ using $R$ edge does not change the $\pur$ factor at $v$;	\item However, the subsequent arrival may close an $F$ edge that is previously contributing as an unclosed $F$ edge incident to $v$ (though not necessarily the $F$ edge opened by the last departure), and hence $\pur(v)$ does not change from the last time when $v$ is at the boundary if arriving via an $R$ edge;
%\item In general, if it opens up $b_v>1$ many $F$ edges the last time on the boundary, notice each of the newly open legs that remains open while we arrive at vertex $v$ again (regardless of the arrival followed by $H$ or $R$ edge) is a missed immediate-return leg; 	%	\item  In general, if it opens up $b(v)$ $F$ edges that are not immediately closed in the last departure, and the subsequent arrival closes an open $F$ edge (to avoid surprise visit), we pick up a change of at most $b(v)-1$ for $\pur(v)$ (where this is an upper bound as multiple $F$ edges may get closed simultaneously in the arrival as well);

%
	\item The arrival, if using a new $F$ edge, is a surprise visit arriving at $v$ and contributes an $1$ to $s_t$ and an $1$ to $\pur$ on LHS;  the bound holds if we assign an increment of $2$ via the one single surprise visit.
	\end{enumerate}
	
	\paragraph{Incorporating $H$ edges}
	To extend our above argument for using $H$ edges, we give an argument based on $H$-component which may evolve over time. We first appeal to the following two claims building upon the prior observation that arriving at a vertex via an $R$ edge does not increase its $\pur$ factor compared to when it last appears on the boundary (for the case only a single edge may be opened up), \begin{claim}[Calling an $R$ edge does not change $\pur$ on vertices already in the current $H$-comp]
		Let $v$ be the current boundary at time $t$, let $H_{v,t}$ be the $H$-component of the boundary at time $t$, and an $R$ edge is called from $H_{v,t}$ (concretely from $v$) \[ 
		\sum_{i\in H_{v,t}} \pur_{t+1}(i) \leq \sum_{i\in H_{v,t}} \pur_t(i)
		\]  
		In other words, despite $H_{v,t}$ is not necessarily the same as $H_{v,t+1}$ since calling an $R$ edge may expand the current $H$ component, it does not increase $\pur$ factor restricted to the vertices in the current $H$ component.
	\end{claim}
	\begin{proof}
		To see the upper bound, observe that calling an $R$ edge from an $H$ component, restricted to the vertices already in the $H$ component prior to the closing of this $R$ edge, we simply have an edge contributing as an unclosed $F$ edge shifted to a closed return leg called from the component. The inequality follows when we close an $R$ edge between vertices already in the same $H$ component.
	\end{proof}
		\begin{claim}[Getting merged into an $H$ component via an $R$ edge does not change $\pur$ on the annexed vertices]
		Let $v$ be the boundary at time $t$, and let $t'$ be the subsequent time-mark such that $H_{v,t}$ is $H$-connected to the boundary (at $t'$) again and an $R$ edge is used at this step, i.e., $H_{v,t}\subseteq H_{u,t'}$, the $H_{v,t}$ component gets merged into a $H$ component via an $R$ edge at the current step for $u$ the boundary vertex at $t'$ followed by an $R$ edge \[ 
		\sum_{i\in H_{v,t}} \pur_{t'}(i) = \sum_{i\in H_{v,t}} \pur_t(i)
		\]
%		In general, if $H_{v,t}$ opens up $b(H_{v,t})> 1$ not-immediately-closed $F$ edges when it appears at the boundary last time, we have \[ 
%		\sum_{i\in H_{v,t}} \pur_{t'}(i) = \sum_{i\in H_{v,t}} \pur_t(i) + b(H_{v,t}) 
%		\]
	\end{claim}
	\begin{proof}
		Since we depart from $H_{v,t}$ at time $t$ via an $F$ edge, we have $\pur_{t_m}(H_{v,t}) = \pur_{t}(H_{v,t_m})+1$ for any $t<t_m<  t'$; however, since we arrive back at a vertex in $H_{v,t}$ at time $t'$ by closing an $R$ edge, we have $\sum_{j\in H_{v,t}} \pur_{t'}(j)  = \sum_{j\in H_{v,t}}\pur_{t'-1}(j)-1 = \sum_{j\in H_{v,t}}\pur_{t}(j)$, giving us the desired.
	\end{proof}
	
	We now proceed to prove the main proposition.
	\begin{proof}[Proof to  Proposition~\ref{prop: pur-invariant}]
	Suppose this is true throughout the walk so far, and we are currently at $H_{v,t}$, and move to $u$ from $v$ at time $t$, we need to show the above for $H_{u,t+1}$. By construction, it suffices for us to consider whether this is an $F/R$ edge.  Notice this is immediate if $v$ is a new vertex, as $H_{u,t+1} = \{u\}$, and there is no potential-unforced-return from $u$ at this time. Otherwise, if the $v\rightarrow u$ leg opens up a new surprise visit,
		\begin{enumerate}
		\item If $u\in H_{v,t}$, the new $F$ edge that gets open may contribute an $1$ to both $\pur_{t+1}(v)$ and $\pur_{t+1}(u)$ while $\pur$ factor of other vertices in $H_{v,t}$ does not get changed. That said, we pick up a gain of $2$ on the LHS, while the surprise visit also now contributes to $s_{t+1}(H_{v,t+1})$, giving an increment of $2$ on the RHS as well;	
		\item If $u\notin H_{v,t}$, let $t_u$ be the last time vertex $u$ appears at a boundary $H$ component, and call this component $H_{u,t_u}$, in addition to the factors contributing to $\pur_{t_u}(H_{u,t})$, the departure at time $t_u$  opens up $1$ $F$ edge from $H_{u,t_u}$. Plus the new surprise visit that we just open up, we have \begin{align*}
		\pur_{t+1}(H_{u,t+1}) &= \pur_{t_u}(H_{u,t_u}) +  2 \\&
		\leq 2\cdot s_{t_u}(H_{u,t_u}) +  2\\&=	 2\cdot s_{t+1}(H_{u,t}) 	
		\end{align*}
		where we observe that $s_{t+1}(H_{u,t}) = s_{t_u}(H_{u,t_u}) + 1$ as we just pick up a new surprise visit, and $H_{u,t_u} = H_{u,t}$ as a set of vertices.
		
%
%		and our arrival at $H_{u,t}$ via the surprise visit at time $t$ again contributes a gain of $2$ to the $RHS$ i.e., $\pur_{t+1}(H_{u,t}) = \pur_{t_u}(H_{u,t})+ b(H_{u,t_u})$, while we pick up a change of $2$ on the RHS as above.  
\end{enumerate}
		If $v\rightarrow u$ is an $R$ leg that closes some $F$ edge, let $t_u$ be defined as earlier,
		 \begin{enumerate}
		 	\item  $u\notin H_{v,t}$: This yields a merge of $H$ components, and we can partition $H_{u,t+1}$ into vertices $H$-reachable either via $u$ or $v$ at time $t$,  \begin{align*}
				\pur_{t+1}(H_{u,t+1})& = \sum_{i\in H_{v,t}} \pur_{t+1}(i) + \sum_{j\in H_{u,t}} \pur_{t+1}(j)
			\end{align*}
		By our claim that calling $R$ edge does not increase $\pur$ on the vertices in the current $H$ component, \begin{align*}
			 \sum_{i\in H_{v,t}} \pur_{t+1}(i)  \leq  \sum_{i\in H_{v,t}}\pur_t(i) =\pur_t(H_{v,t})\leq  2\cdot s_t(H_{v,t}) 
		\end{align*}
		Since $u\notin H_{v,t}$, for component $H_{u,t} = H_{u,t_u}$, it gets annexed into a new $H$-comp via an $F$ departure and a $R$ return, \[
		\sum_{j\in H_{u,t}}\pur_{t+1}(j) = \sum_{j\in H_{u,t}} \pur_{t_u}(j) = \pur_{t_{u}}(H_{u,t_u}) \leq 2\cdot s_{t_u}(H_{u,t_u}) 		 \] 
%		 If multiple $F$ edges get open up, among which $b(H_{v,t})$ are not immediately-return, we have \begin{align*}
%		 	\sum_{i\in H_{v,t}} \pur_{t'}(i) = \sum_{i\in H_{v,t}} \pur_t(i) + b(H_{v,t}) &\leq 2\cdot s_{t_u}(H_{u,t_u}) + \mir_{t_u}(H_{u,t_u})  +b(H_{v,t}) \\&= 2\cdot s_{t_u}(H_{u,t_u}) + \mir_{t+1}(H_{u,t_u}) 
%		 \end{align*}
%		 where we observe any edge in $b(H_{v,t})$ is a newly gained not-immediately-return leg. 
Combining the above yields 
\begin{align*}
		 	\pur_{t+1}(H_{u,t+1}) &\leq 2\cdot s_{t+1}(H_{v,t}) + 2\cdot s_{t+1}(H_{u,t_u})  = 2\cdot s_{t+1}(H_{u,t+1})  
		 \end{align*}
		 as $H_{v,t}$ and $H_{u,t_u}$ form a partition for $H_{u,t+1}$ for $u\notin H_{v,t}$, and the surprise visits inherit over time.
		 \item $u\in H_{v,t}$: This is a return within an $H$-component, and we have \[
		 \pur_{t+1}(H_{u,t}) \leq  \pur_{t}(H_{v,t})
		  \]
		  since calling a return leg within the same $H$ component does not increase $\pur$ factor (in fact, a decrease by $1$ as the corresponding $F$ edge contributes a factor $1$ to both endpoints in the $H$ component, while after being closed, it only contributes as a closed $R$ edge to one endpoint).
		  \end{enumerate}
	\end{proof}
	
\subsection{Upgrading towards $1$-in-many-out: branching}
\paragraph{Branching} The above argument crucially relies upon that each vertex can only encode at most $1$ edge when it is on the boundary each time, however, this is not true in the general setting for graph matrix, and particularly why rough matrix norm bounds depend crucially on \enquote{minimum vertex separator} of the underlying graph. That said, we note that the argument can be extended in a lightweight manner to the general case when the matrix is indexed by order-tuple, i.e., there is no permutation-jump involved in the walk.


For concreteness, we call a vertex an \emph{anchor} vertex if it encodes multiple (out-going) edges on the boundary at a single time in the walk. The crux of the argument observes that we can further constrain each such vertex to have each of its $F$ edge opens up in the branching to be closed before the vertex appears again on the boundary, as otherwise there is a gap from surprise visit that we can identify locally in the constraint graph, and this is captured by the counter $\mir$ to be defined momentarily.

\paragraph{Return bound for tuple-indexed walk}
Let's start with some definitions in this setting, and fix the traversal direction from $U_\al$ to $V_\al$.
\begin{definition}[Anchor vertex]
For a vertex $v$ in the shape $\al$ (or $\al^T$) and an edge-labeling $\calL$, we call it an \emph{anchor} vertex if it pushes out more than $1$ non-dangling edge, i.e., an edge on a simple path from $v$ to the next boundary.  \end{definition}
 \begin{definition}[Mirror copy]
 	For any vertex $v$ in $\al$ (or in $\al^T$), we let $\sigma(v) \in V(\al^T)$ or (in $V(\al)$) be the counterpart of $v$ obtained by shape-transpose. 
 \end{definition}
%For starters, we observe that the linearized constraint graph can decomposed as having $U_\al =V_\al$ vertex disjoint paths from $U_1$ to $V_q$ attaching path-segments between anchor vertex and its mirror copy. 

\begin{definition}[Missed-immediate-return factor counter $\mir$]
	For a vertex $v$ that opens up multiple $F$ edges from the boundary, let $\mir_t(v)$ be the number of $F$ edges it opens up as an anchor vertex so far in the walk that are not immediately closed when $v$ appears on the boundary again. Analogously, we define $\mir_t(H_{v,t})$ for the corresponding $H$-component.
\end{definition}
\begin{remark}
	For adjacency matrix or line graph, $\mir_t(v) = 0$ throughout the walk as each vertex may open up at most $1$ $F$ edge when at boundary.\end{remark}



For starters, consider the linearized constraint graph obtained by forgoing the trace-walk condition $U_1 = V_q$ (as an equality of order-tuples), and this is a graph of $q$ blocks of $\al$ and $\al^T$. We observe that the constraint graph can be encoded via the following process, and use this process to identify the charging of potential-surprised-visit with $\mir$ factor. For the following discussion, fix the traversal direction from $U_1$ to $V_q$.

\begin{mdframed}[frametitle = {Decomposing (linearized) constraint graph into path-segments}]
\begin{enumerate}
	\item We start with at most $U_\al=V_\al$ \emph{directed} vertex-disjoint paths from $U_1$ to $V_q$;
	\item Attach  \emph{directed} path-segments from an anchor vertex to its mirror copy in the subsequent block; 
	\item Attach path-segments between anchor vertices in the same block;
	\item Attach \emph{directed}(dangling) path-segment from an anchor vertex to a dangling vertex in the same block.
\end{enumerate}
\end{mdframed}


\begin{proposition}
	For each block, process the anchor-vertices pair according to their distance in increasing order in $\al\circ\al^T$. For each starting anchor vertex being processed, each path-segment crossing the boundary starting with $F$ edges is either immediately backtracking, or we can assign a surprise visit from the path segment (or its adjacent one) to the starting anchor vertex for its corresponding $\mir$ factor. Moreover, each surprise visit is assigned to at most $2$ $\mir$ factors.
\end{proposition}
\begin{proof}
		 We first observe that for any path-segment that departs from the starting anchor vertex with $F$ edge may only return to the anchor vertex (with label in $[n]$) within the path-segment at the corresponding mirror copy location (aka. the ending anchor vertex) if the starting anchor vertex (labeled in $[n]$) ever appears again the in the path segment. This follows from the injectiivty assumption: the starting anchor vertex may only appear in the current block, and unless there is a surprise visit in the segment, the path returning to the starting anchor vertex lands the starting anchor vertex (its label in $[n]$) at the ending anchor vertex location in the constraint graph. That said, for any anchor vertex that gets returned too early, aka. prior to the corresponding mirror copy location, the branch that returns to the current vertex gets assigned a surprise visit and each other path-segment that opens up new $F$ branches departing from the anchor vertex also gets assigned a surprise visit.		  
		 
		 	 Next, we observe that the return to the starting anchor vertex at its mirror location is mandatory for any segment starting with $F$. Suppose the current path-segment does not return, the starting anchor-vertex picks up $1$ $\mir$ factor from the path-segment. Suppose there is no surprise visit in the current segment (i.e., the $\mir$ factor from the segment is uncharged yet), we claim that this must be the first processed path-segment between the current pair of starting and ending vertices, as otherwise the current path-segment has to arrive at some known vertex at the mirror-copy location which gives a surprise visit to assign to the corresponding $\mir$ factor. However, notice for any anchor vertex with path-segment added to its mirror copy in its subsequent block, there are at least two edge-disjoint paths (given by distinct path segments) to its mirror copy. For concreteness, call the second path-segment processed the adjacent of the first segment. Notice these two path segments are disconnected in the graph sample once the starting anchor vertex is removed, while these two paths need to merge eventually at the mirror copy location. By assumption, the mirror copy is not the starting anchor vertex, hence there must be a surprise visit in the second path-segment and we can charge it to the $\mir$ factor of both the first and second path-segments. 
	 
	Furthermore, to see that a factor of $2$ is sufficient, notice each subsequent path-segment between the current pair of starting and ending anchor vertex either comes with a surprise visit or it is an immediate backtracking segment itself that does not contribute $\mir$ factor to the starting anchor vertex. This completes the proof to our proposition. 
	\end{proof}
	
%		
%\subsubsection{Forced return for walks with permutation-jump}
%In this section, we show ''return-being-forced'' without using injectivity assumption, as permutation-jump may now produce anchor vertices that branch out while each path-segment does not immeidately rejoin (or at all in the whole walk!) in the subsequent block. 
%
%For starters, we maintain an anchor vertex for each active path-segment (i.e., path with vertices in the current boundary) that identifies as the first vertex in the current path-segment without unclosed $F$ edge opened up by the current path-segment. The anchor vertex (and its extension, anchor component) will now serve as a joint connecting various path-segments.
%
%\begin{definition}[$R$-branch invasion]
%We call an $R$ leg a branch invasion at an anchor vertex (and component) if the corresponding $F$ edge is not opened-up by the current branch. 
%\end{definition}
%
%\begin{definition}[Active $F$-path]
%At any step in the walk, for any anchor component, call its path to any vertex in the current boundary an active $F$-path if the path departs from the anchor component via an $F$ edge.
%\end{definition}
%\begin{proposition}
%	For any path-segment, the active $F$-path from the anchor component is eventually closed in a reverse direction, unless there is a surprise visit in, or arriving at the active $F$-path.
%\end{proposition}
%
%\begin{proposition}
%	Swapping $R$ and $H$ label for path-segment invasion.
%\end{proposition}
%
%	\begin{proposition} Let $P_\al$ be a trace walk for shape $\al$,
%We can assign $\pur(P_\al) \coloneqq \sum_{H_{v,q}: \text{H-component at time }q} \pur(H_{v,q})$ factors to surprise visit such that \begin{enumerate}
%	\item each surprise visit is only charged $O(1)$ $\pur$ factors;
%	\item all but $\frac{|U_\al|+|V_\al|}{2} $ many (non-dangling) $\pur$ factors are assigned to some surprise visit.
%\end{enumerate} each surprise visit is only charged to $O(1)$ $\pur$ factors.
%\end{proposition}
%
%\begin{proof}
% For each $H$-component $H_v$, consider the final time $t$ it appears on the boundary in the walk, notice $\pur_t(H_v)$ by construction is an upper bound for the number of unforced-returns called from vertices in $H_v$ throughout the walk. We first see each surprise visit is not being assigned to too many $\pur$ factors. By Proposition~\ref{prop: pur-invariant}, there are two components of $\pur$ factors, (past) surprise visit and (future) missed-immediate-return. Before we start, observe the assignment for past surprise visits is immediate.
% 
% We now consider the assignment for $\mir$ factors. Call a vertex in the constraint graph an \emph{anchor vertex} if it splits out multiple $F$ edges when on the boundary, and we can restrict our attention to anchor vertex (as non-anchor vertex in the constraint graph does not contribute to $\mir$ factor). For starters, consider the linearized constraint graph obtained by forgoing the trace-walk condition $U_1 = V_q$ (as a set equality), and this is a graph of $q$ blocks of $\al$ with $\al^T$ glued with potentially non-trivial permutation jump. We observe the constraint graph can be encoded via the following process, and use this process to identify charging of potential-surprised-visit with $\mir$ factor. For the following discussion, fix the traversal direction from $U_1$ to $V_q$.
%
%\begin{mdframed}[frametitle = { Assigning $\mir$ factor to future surprise visit}]
%\begin{enumerate}
%	\item Attaching a segment: we can attach a (directed) path-segment between a start-vertex and an end-vertex such that the end-vertex is a vertex on an encoded path-segment unless it is a free vertex that is dangling vertex or in $V_q$;
%	\item For each path-segment that arrives at non-free end-point while starting with $F$ edges, we track whether the first edge on the path is closed when arriving at the end-point of the path-segment;
%	\item  If not,  there is at least one surprise visit on the path and we can assign it to the starting vertex as a $\mir$ factor.
%\end{enumerate}
%\end{mdframed}
%   We now observe that a vertex may only be an ''anchor'' vertex if it is the starting point of some path-segment, and each path-segment contributes at most one $\mir$ factor to the final $\pur$ factor via the potential $F$ edge it opens up at the starting vertex. It suffices for us to assign path-segments, and each path-segment that arrives at non-free end-point either dose not contribute to any $\mir$ factor, or contributes at least $1$ surprise visit.
%   
%   For each path segment, we claim that there is either a surprise visit that we can assign to along this segment, or the $F$ edge that opens up the segment is closed in a ''forced'' way, i.e., it does not contribute to any unforced return.
%   
%    To see that not too many $\mir$ factors are not accounted for, notice it must correspond to some free-path-segment, which is at most the number of dangling branches in the constraint graph with $|V_\al|$. Repeating this argument from the other direction gives us the $\frac{|U_\al|+|V_\al|}{2}$ bound.
% \end{proof}
% 
% 


%Branch-chasing
%
%
%
%Below is the branch-chasing argument
%\subsubsection{Branch-chasing using $R$ is free}
%\paragraph{Troubles for immediate-return based argument}
%To recap our prior argument, we essentially give a special treatment for \enquote{branching} vertices, i.e., those in the constraint graph that may encode multiple edges across the boundary, and we claim that for any such vertex, each $F$ edge that gets opened up when departing from this vertex must be immediately closed before this vertex appears again in the boundary: in particular, the branching vertex needs to match in its mirror-copy location unless there is a surprise visit that offers a gap for charging potential unforced return due to the vertex opening up multiple $F$ edges simultaneously in a single-shot. 
%
%However, this heuristic falls apart when we combine with permutation jump, as we no longer have injectivity assumption across the boundary: in particular, mirror copy is no longer well-defined. That said, we can consider a branching vertex that opens up simultaneously multiple $F$ branches, and one of them returns sooner than others, causing a potential confusion when calling an $R$ edge at the anchor vertex, that it may refer to any of the $F$ edges leading to the alive $F$ branch (and the $F$ edge leading to the anchor vertex before any of the $F$ branches get opened up). 
%
%
%\paragraph{Branch-chasing graph}
%We start by considering an auxiliary graph constructed as the following. It should be cautious that \emph{boundary} in the following section typically refers to the boundary of the walk unless otherwise specified. Notice each vertex on the boundary gives us a tiny constant decay via their edges. However, the core of our argument relies upon coloring the edges such that red edge is the only possible confusion, and furthermore, maintaining the invariant each vertex is not incident to \emph{too many red edges}.
% 
%\begin{mdframed}[frametitle = {Constructing and maintaining the branch-chasing graph}]
%\begin{enumerate}
%	\item This is a directed graph with each vertex receiving a label in $[n]$, moreover, we can color the edges into \emph{red} and \emph{black}, such that we are interested in the desired invariant each vertex is incident to only one out-going red edge unless there are further surprised visits assigned to this vertex;
%	\item Observe that there is no confusion if there the incident red-edge is \emph{unique};
%% 	\item In this graph, we are primarily interested in unclosed $F$ edges and vertices that split out multiple $F$ edges at a single time in the boundary;
%	\item We start with an empty graph and build the graph as the walk proceeds;
%	\item For each $F$ edge, we open up a \emph{directed black} edge from the original vertex to the vertex it arrives;
%	\item If the $F$ edge that gets opened up is a surprise visit, i.e., it leads to a previously explored vertex, we flip all the \emph{black} unclosed $F$ edges that have a directed path in the branch-chasing graph to the surprise destination to \emph{red}. 
%\end{enumerate}
%\end{mdframed}
%With this graph in hand, we first see how it may help us in deciding $R$ edges that arise in the chasing process when there are multitple walkers.
%\begin{observation}
%	 	If there is no dangling branch, any black edge is on a directed path to the current boundary of the walk, i.e., the boundary of the branch-chasing graph is equivalent to the walk boundary.
%\end{observation}
%\begin{corollary}
%	Each chase using black edge is fixed.
%\end{corollary}
%\begin{proof}
%	Despite each vertex may be incident to multiple black edges, notice the subgraph cut across by any black edge is a rooted tree, in particular, with some \emph{active} walker in the current boundary. We then consider the following process, at each (block) step in the walk,  it suffices for us to go through the vertices on the current boundary and query
%	\begin{enumerate}
%		\item whether it is an \enquote{branching} vertex looking for $R$ chase;
%		\item whether it is a vertex assigned to \enquote{beacon guidance} for $R$ chase;
%	\end{enumerate}
%	For each step, for each walker at some branching vertex looking for $R$ chase, the encoder can assign the  boundary vertex on the path promised by the out-going $R$ edge as the following,
%	\begin{enumerate}
%		\item For vertex $v$ looking for beacon-guidance, consider the subtree reached by the desired outgoing edge, assign beacon guidance for any branching vertex with $R$ chase query contained in the subtree;
%		\item Assign an arbitrary vertex in its subtree reached by the desired out-going edge not assigned for beacon-guidance to $v$. 	\end{enumerate}
%	
%	 To decode, since the branch-chasing graph (restricted to black edges) is a directed tree (forest), there exists some query node whose (out-going) subtree is query-node free; by out encoding, there is also promised to be at least one guidance node in that subtree, assign the outgoing edge pointing to the (potentially multiple) guidance beacon to the query-node. Remove their colors (temporarily), and repeat this process.
%\end{proof}
%\begin{remark}
%	It should be pointed out that we only aim to identify the edge-set used by $R$ chase from this process, as any further confusion is then resolved using edge-decay and automorphism factor.
%\end{remark}
%
%We now proceed to handle the potential confusion caused by surprise visit in the branch-chasing graph, i.e., red edges. Throughout the process, a surprise visit may turn black edges into red edges, and call this path the corresponding flip path of the surprise visit. 
%\begin{proposition}
%Consider the path of edges that have their colors flip, the \emph{flip path} passes through at most $2$ vertices that are incident to \emph{out-going} red edge before the current flip.
%\end{proposition}
%\begin{proof}
%	Without loss of generality, suppose the surprise visit proceeds from $a\rightarrow b$, we observe that any edge that gets flipped by this surprise visit. Let $u_a$ be the closest vertex on the flipped path to $a$ that is already incident to some out-going red edge before the current flip, and suppose there is some other vertex $v_a$ that also has a black path to $a$ before the current flip. We observe that it needs to pass through $u_a$ as the subgraph restricted to black edges is a directed tree. However, consider the supposedly black path from $v_a$ to $u_a$, we claim that it must be already be red before the current flip as $u_a$ has an out-going red-edge, which by construction, requires the $v_a$ to $u_a$ path to be flipped to red. Therefore, there can be at most $1$ vertex incident to  \emph{out-going} red edge before the current flip that has a flip-path to $a$; apply the above argument to the flip-path leading to $b$ then gives us the desired bound.
%\end{proof}
%\begin{corollary}
%	Assigning each surprise visit to two of the vertices its flipped path pass through that may be incident to more than $1$ out-going red edge captured by the factor $\red$,  we can maintain the following invariant for each vertex \[ 
%	\text{out-going red edges incident to $v$} \leq 1 + w_t(v)
%	\]
%	where $w_t(v)$ accounts the number of surprise visits assigned to vertex $v$ for creating new excess red edge originating from $v$.
%\end{corollary}
%
%% \begin{comment}
%% 
%% 	 \begin{mdframed}[frametitle = {Constructing and maintaining the branch-chasing graph}]
%%\begin{enumerate}
%%	\item This is a directed graph with each vertex receiving a label in $[n]$, moreover, we can color the vertices in the current boundary of the \emph{walk} using red and blue such that each blue vertex represents a vertex currently in the boundary serving as a beacon guidance, and a red vertex is an branching vertex currently in the boundary with possible $R$ chase query. One vertex may receive two colors at the same time.
%%	\item We start with an empty graph and build the graph as the walk proceeds;
%%	\item Push a vertex into the branch-chasing graph if it appears in the walk as some \emph{branching} vertex that splits out multiple edges simultaneously at the boundary (fix traversal direction from $U$ to $V$ w.l.o.g.);
%%	\item For each walker the \emph{branching} vertex splits out using $F$ edge (i.e., edge splits out from the branching vertex), add a vertex for the corresponding walker, and a directed edge from the branching vertex to the walker, which also receives a label in $[n]$; for each walker that departs using $H$ edges, maintain a vertex recording the current walker's location while no edge is added;
%%	\item For any walker on the boundary, update its current label in $[n]$ in its corresponding location at each step; if a walker vertex receives the same label in $[n]$ as a vertex that has a directed edge to itself, this corresponds to a return via closing the $F$ segment it used to depart from the last anchor vertex, remove the directed edge in-between, and collapse the two vertices;
%%	\item For any \emph{branching} vertex not currently on the boundary, if it has only one out-going directed edge, remove the vertex and merge its two incident directed edges into one (if one-in-one-out) with the same direction;
%%	\item If any vertex on the boundary witnesses a surprise visit, update the current vertex's label, remove the directed edge going into the current head of arm and if the new vertex is on any path between current anchor vertices (or current head of arm), make it a \emph{branching} vertex if not already, and replace the one directed edge that represents the active path passing through the surprise visit destination by two directed edges (passing through the new branching vertex).
%%\end{enumerate}
%%\end{mdframed}
%%
%%\begin{proposition}
%%	The branch-chasing graph is a tree (acyclic viewed as an undirected graph) throughout the walk, and each vertex in the branch-chasing graph receives a unique label in $[n]$.\end{proposition}
%%\begin{proof}
%%	Any surprise visit gets removed when it appears on the boundary.
%%\end{proof}
%%\begin{proposition}[Boundary equivalency] \label{prop:peaceful-merging}
%%	Throughout the walk, any $0$ out-degree vertex of the branch-chasing graph is in the walk boundary. In other words, any out-going edge from a branching vertex in the graph is on a directed path to the boundary. Moreover, a surprise visit may remove at most $1$ directed-edge in the branch-chase graph.
%%\end{proposition}
%%\begin{proof}
%%	We prove this by induction, and consider how the latest move may affect $v$ the boundary vertex of the branch-chasing graph.  By induction hypothesis $v$ is also at the boundary of the walk, and consider (potentially multiple) walkers from $v$, and process them sequentially (in arbitrary order). If there are multiple walkers currently at $v$, process them in order. 
%%	
%%	 If the current walker at $v$ moves to a new vertex using non-surprise $F/H$ edge, the walker has its label updated to the current destination in $[n]$, and potentially adding a directed edge (if $v$ has walkers-to-be processed or have other out-going edges in the branch-chase graph), while the current walker and $v$ (if remaining in the graph) both maintain the walk boundary status, and the potential out-going $F$ edge we add from $v$ points outwards to the boundary.
%%	 
%%%	  For a walker using surprise visit, let $p(v)$ be the parent of $v$ in the directed tree before this move, and we case on whether $v$ is currently a branching vertex in the branch-chasing graph, i.e., whether it has other walkers to be processed or out-going edges. If so, the surprise visit split out by the current arm removes the directed edge from $v$ to the current walker, while any other out-going edge from $v$ remains unaffected by this move, and hence still has a directed path to the current walk boundary. If $v$ does not have any more walker or out-going edges, observe that $v$ gets removed (ignored in the branch-chasing graph) after the surprise visit, while the invariant holds true for $p(v)$ as we create a new directed edge from $p(v)$ to the destination of the current head-of-arm, and other out-going edge from $p(v)$ remains unaffected.
%%	  
%%	  
%%	  For a walker using surprise visit, we first consider the out-going edges it may affect that are already present in the branch-chasing graph before the surprise visit. Let $p(v)$ be the parent of $v$ in the directed tree before this move: 
%%	  \begin{enumerate}
%%	  	\item The edge in the branch-chasing graph $p(v)\rightarrow v$ may be affected, but notice either $v$ gets removed from the branch-chasing graph after this surprise visit, or $v$ has other walkers or other out-going edge towards the current boundary, in which case the edge $p(v)\rightarrow v$ remains as pointing outwards to the boundary, and this is the only directed edge in the branch-chasing graph the walker can remove;
%%	  		  	\item Let the walker's surprise destination be $u$. Recall that if $u$ is currently passed through by some path-segment represented by some directed edge $a\rightarrow b$ in the branch-chasing graph, we divide the path-segment into two directed segments $a\rightarrow u \rightarrow b$. Notice the edge $a\rightarrow u$ is pointing outwards to the boundary as $u$ is on the boundary, and $u\rightarrow b $ is also pointing to the boundary by the invariant hypothesis on $a$ a \emph{branching vertex} in the branch-chasing graph;
%%	  	\item $v$ may remain in the branch-chasing graph as a \emph{branching vertex} after the surprise visit and any of its other out-going edges do not get affected by the current walker.
%%	  \end{enumerate} 
%%	  
%%	 \end{proof}
%%	 
%%\begin{corollary}
%%We can assign each surprise visit to at most $1$ directed edge in the branch-chasing graph such that for each vertex in the branch-chasing graph, each of its out-going directed-edge that gets removed without being closed from the reverse-direction is assigned $1$ factor of surprise visit. \end{corollary}	 
%%In other words, each return is either forced (via $1$-in-$1$-out argument) or can be assigned $1$ factor of surprise visit.
%%
%%	 
%%\begin{proposition}
%%	Each $R$ chase of a block (step) can be decoded as an edge-set for free, i.e., at a cost $O(2^{|U_\al|})$ (and $O(2^{|V_\al|}) $ for $\al^T$ block) where we call a step from an anchor vertex an $R$ chase if it uses an out-going $F$ edge from the branching vertex in the branch-chasing graph.
%%\end{proposition}
%%\begin{proof}
%%	At each (block) step in the walk, each out-going $F$ edge is on a path leading to some vertex in the walk boundary, it suffices for us to go through the vertices on the current boundary and query
%%	\begin{enumerate}
%%		\item whether it is an \enquote{branching} vertex looking for $R$ chase;
%%		\item whether it is a vertex assigned to \enquote{beacon guidance} for $R$ chase;
%%	\end{enumerate}
%%	For each step, for each anchor vertex looking for $R$ chase, the encoder can assign the  boundary vertex on the path promised by the out-going $R$ edge as the following,
%%	\begin{enumerate}
%%		\item For vertex $v$ looking for beacon-guidance, consider the subtree reached by the desired outgoing edge, assign beacon guidance for any branching vertex with $R$ chase query contained in the subtree;
%%		\item Assign an arbitrary vertex in its subtree reached by the desired out-going edge not assigned for beacon-guidance to $v$ (guaranteed by ~Proposition \ref{prop:peaceful-merging} ). 	\end{enumerate}
%%	
%%	 To decode, since the branch-chasing graph is a directed tree (forest), there exists some query node whose (out-going) subtree is query-node free; by encoding, there is also promised to be at least one guidance node in that subtree, assign the outgoing edge pointing to the (potentially multiple) guidance beacon to the query-node. Remove their colors (temporarily), and repeat this process.
%%	\end{proof}
%%
%% \end{comment}

\subsubsection{Return is still ''forced'' with dangling branches}
% We now put the above arguments together, concretely, we combine the argument for $1$-in-$1$-out and $R$-chase being free argument for walks with permutation-jump. We start by taking into account our prior observation of $R$-chase being free into $\pur$ factor, the potential function that controls the number of potential-unforced-returns throughout the walk. 
Before we dig into our final bound, we first see how having dangling edges may affect our forced return bound. Notice that having dangling edges indeed brings $\pur$ factor that does not get assigned to any surprise visit, however, our goal in this section is to show that beyond the ''anticpated'' $\pur$ factors, dangling edges do not contribute further confusion.

\paragraph{Attaching dangling branches and dangling factor assignment}
It should be pointed out that the return for each dangling branch is not necessarily fixed, and our goal here is to show each dangling branch, regardless of how many vertices the single branch may pass through, only incurs $1$ factor of potential-unforced-return.

 Let's start by recalling dangling branches (in a shape) can be encoded in the following manner: we can recursively attach a dangling branch to some identified vertex in the shape. And this begets our dangling factor assignment scheme:in each block-step, we assign each dangling factor to the vertex it attaches to, and update the $\pur$ function for each vertex on the newly attached segment via the $1$-in-$1$-out argument. At this point, it should be clear that the $\pur$ factor is associated with the number of dangling branches as opposed to dangling vertices. To formalize this intuition, we introduce \emph{attachment} edge, as this is the edge part of a dangling branch that comes with extra $\pur$ factor in our argument. Notice not all the edges in a dangling branch come with extra $\pur$ factor, and this is crucial for us in obtaining a norm bound with extra factor only depending on the number of dangling branches as opposed to the number of dangling vertices.
 
\begin{definition}[Attachment edge]
    Given a shape and a block-step walk of the corresponding shape, for each dangling branch, call the edge an attachment edge of the corresponding branch if its origin vertex is identified using $R/H$ edge while it spits out an $F$ edge as part of the dangling branch.
\end{definition}
 \begin{observation}
          For any dangling branch, at any block-step of the walk, there is at most one attachment edge unless there is a surprise visit locally along the branch. 
 \end{observation}
 We now introduce an edge-coloring scheme to take into account dangling branch's effects on $\pur$. For each dangling branch that gets encoded, we will color its $F$ edges as the following scheme,
 \begin{mdframed}[frametitle = {Coloring scheme for dangling branches}]
 \begin{enumerate}
     \item Following the encoding order that we start from some non-dangling vertex or landing vertex if floating and encode the edges along the dangling branch;
     \item We restrict our attention to $F$ edges along the dangling branch, and
     \item color each attachment edge \emph{yellow};
     \item color each non-attachment edge \emph{green} if it is not a surprise visit.
 \end{enumerate}
\end{mdframed} 
\begin{remark}
   An out-going green edge is an edge opened as part of dangling branched while it does not get assigned any dangling factor.
\end{remark}
\begin{definition}[Green edge assigment $\green(v)$]
	For any vertex $v$ at time $t$, we define the green edge counter as the number of surprise visits assigned to $v$ by time $t$.\end{definition}
For each $H$ component connected to $v$ at time $t$, we define \[ 
\green_t(H_{v,t}) = \sum_{v\in H_{v,t}} \green_t(v)  \,.
\]
%\begin{claim}
%For any $H$ component $H_v$ at time $t$, let $s_{\dang,t}(H_{v,t})$ be the number of surprise visits arriving at $v$ by time $t$ that is part of any dangling branch, we have \[ 
%\green_t(H_{v,t}) \leq s_{\dang,t}(H_{v,t} )
%\]
%\end{claim}
%\begin{proof}
%	The number of out-going green edges from $v$ may only change when $v$ pushes out non-attachment edge as part of some non-dangling branch, and unless this happens when $v$ is first encountered, in which case we have $0$ on the LHS and $1$ on the RHS, any increment on the LHS comes after a surprise visit arriving at $v$  
%\end{proof}
%

\begin{claim}
	Throughout the walk, for any vertex $v$ at time $t$, we maintain the invariant \[
	\# \text{out-going green edges from $v$ by time $t$} \leq  \green_t(v) + 1 	 \]
\end{claim}
%\begin{claim}
%%	For any dangling branch segment that passes through a sequence of vertices $\{v_i\}$, and suppose that for any vertex $v_i$ on the segment, we have $\green(v_i)=0$ before the segment is processed, we can assign surprise visits from the dangling segment such that $\green(v_i)=0$ continues to hold after the dangling segment is processed.
%%\end{claim}
\begin{proof}
	We prove this by induction on dangling branches. Notice this is true in the base case when each vertex first appears.We now process this by each dangling segment.  For starters, observe that this is also immediate if there is no surprise visit in the branch segment: let $v_0$ be the last ''seen'' vertex passed through by the dangling branch before the current block, that said, $v_0$ pushes out a yellow edge, and thus its invariant on $\green(v_0)$ continues to hold. For any vertex that is visited in the segment after $v_0$, since there is no surprise visit, each such vertex is new and the invariant holds immediately. 
	
	In the case there is some surprise visit, we can process the vertex in order of their distance to the attachment vertex of the current branch from shortest to farthest: for any vertex $v_i$ that pushes out a green $F$ edge while not its first green edge, let $e_i$ be the last $F$ edge before $v_i$ pushes out the $F$ edge in the dangling segment, and we note that $e_i$ is well-defined as otherwise this would be the first $F$ edge pushed out by the dangling branch, and hence be colored ''yellow''. Since $e_i$ is well-defined, we can further observe that this is a surprise visit and we assign it to $v_i$. 
\end{proof}

\subsection{Ultimate return bound}
We now put the above arguments together, concretely, we combine the argument for $1$-in-$1$-out and $R$-chase being free argument for walks with permutation-jump. Towards that end, we need to modify the definition of $\pur$ factor to take into account our prior observation that return is still forced if it is an $R$ chase,
\begin{definition}[Time $t$] We can associate each edge a particular time-mark. That said, we use time $t$ to represent the moment before the edge at the corresponding time-mark is used.	
\end{definition}
\begin{definition}[Upgraded $\pur$ factor] At time $t$ (before the edge of time $t$ is used), for each vertex $v$, let $\pur_t(v)$ be the counter for the following,\begin{enumerate}
		\item Each return leg closed from $v$ by time $t$ contributes an $1$ to $\pur_t(v)$;
		\item Each unclosed $F$ edge (that is not colored ''green'') currently incident to $v$, that also does not come with any immediate-return guarantee, contributes an $1$;
		\item An $-1$ as we can maintain a counter for each vertex such that there is always one potential return-leg presumed to be forced;
%		\item An extra $-1 \cdot 1_{v \text{ has seen outgoing red edge by } t} $ as we can maintain a counter for each vertex such that there is always one outgoing red edge presumed to be forced, and this is only needed when $v$ has outgoing red edge; 
		\item Each out-going green edge contributes an $1$;
		\item Each vertex contributes an $-1$ if it opens up any out-going green edge.
		\end{enumerate}
		Let $H_{v,t}$ be the component reachable using subsequent $H$ edges from $v$ at time $t$, and define \[ 
		\pur_t(H_v) \coloneqq \sum_{i\in H_{v,t}} \pur_t(i)
		\] 	
\end{definition}
\jnote{an attempt to reproduce and simplify the bound}
\begin{lemma}[Ultimate $\pur$ bound] Throughout the walk, we maintain the variant \[ 
\pur_t(H_{v,t}) \leq 2 s_t(H_{v,t})  + \mir_t(H_{v,t})+ \dang_t(H_{v,t}) + \green_t(H_{v,t}) 
\]
for $H_{v,t}$ the $H$-component reachable from the boundary vertex $v$ at the end of time $t$ (after the edge at time $t$ is used).
\end{lemma}
\begin{proof}
	Suppose the current edge being processed goes from $y$ to $v$, let $t$ be the last time mark $v$ appears in an $H$-component at the boundary, and let the corresponding component be $H_{v,t}$. Let $t'$ be the current time-mark, and we are to show the invariant for $H_{v,t'+1}$. For convenience, we introduce the shorthand \[ \Delta_{t_1, t_2}\circ f(a) \coloneqq f_{t_1}(a) -f_{t_2}(a)
		\]
		for our counter function $f \in \{s,\dang,\green\}$ and $t_1\geq  t_2$, and $a$ any vertex, or set of vertices.
 
	
	
	Following our prior observation, it suffices to consider $v,u$ to be in disjoint $H$-components before the edge $(u,v)$. And it suffices for us to show the following, \[ 
	\Delta_{t'+1, t} \circ \pur ( H_{v,t} )\leq  2\Delta_{t'+1, t}\circ H_{v,t}  + \Delta_{t+1, t}\circ \mir(H_{v,t}) +\Delta_{t+1, t}\circ \dang(H_{v,t})  + \Delta_{t+1,t} \circ \green( H_{v,t})
	\] 
	where we observe that each edge that contributes to $\pur_{t'+1}(H_{v,t})$ while not to $ \pur_t(H_{v,t})$ admits the following classification:\begin{enumerate}
		\item Notice this may be the edge used at time $t'$ if it is an $F$ edge, or an edge opened up in the last departure from $H_{v,t}$;
		\item We fist focus on edges opened up in the previous departure, for each such edge, depending on whether the edge opened up as part of some dangling branch, if this is a yellow edge (attachment edge), it is captured by $\Delta_{t+1, t}\circ \dang(H_{v,t})$;
		\item if this is a green edge, suppose it is opened up from vertex $v_t \in H_{v,t}$, we case on whether this is the first green edge opened up from $v_t$, if so, we have \[ 
		-1 \cdot 1_{v_t \text{has opened-up out-going green edge at time t+1}} - (-1)\cdot 1_{v_t \text{has opened-up out-going green edge at time t}}  + 1 = -1 +1 =0
		\]
		where the $+1$ comes from the particular green edge in inspection, and we observe \[ -1 \cdot 1_{v_t \text{has opened-up out-going green edge at time t}} = 0\,;\]
		\item if this is not the first green edge opened up from the source vertex, this is offset by the $ -1$ from the surprise visit in the dangling branch attached at the block of $t$ assigned to $v_t$;
		\item if this is not opened up as part of dangling branch, we case on whether the last departure from $H_{v,t}$ opens up multiple $F$ edges: if so each such	 edge either receives the immediate-return guarantee (in which case does not contribute to the $\pur$ factor), or it is offset by the corresponding factor from $\mir$;
		\item Otherwise, the last departure from $H_{v,t}$ may create one unclosed $F$ edge, and it is either offset by the arrival at $v$ again using $R$ edge at time $t'$, or this is a surprise visit and it suffices for us to offset the gain by assigning the surprise visit a factor $2$ on the RHS; 		\item Finally, inspecting the edges being used at time $t'$, note that W.L.O.G., we can assume there is at most one $F$ edge, as any subsequent ones are considered as surprise visits. Casing on whether this is an $F$ edge, if so, this is either a surprise visit in which case we pick up an increment of $1$ from RHS for each such edge from that gain of surprise visits, or $v$ is a new vertex and the hypothesis holds trivially for $H_{v,t'+1}$.
		\end{enumerate}
\end{proof}




%\begin{lemma}[Ultimate forced-return bound] Throughout the walk, we maintain the invariant \[
%\pur_t(H_{v,t}) \leq  s_t(H_{v,t})  + \mir_t(H_{v,t})+ \dang_t(H_{v,t}) +\green_t(H_{v,t})  \]
% for $H_{v,t}$ the $H$-component reachable from the boundary vertex $v$ at the end of time $t$ (after the edge at time $t$ is used),  where \begin{enumerate}
% 	\item 
%  $s_t$ is the surprise visit counter that counts the number of surprise visits arriving at $H_{v,t}$;
%   \item $\dang_t$ is the counter that counts the number of dangling branches attached to $H_{v,t}$, i.e., yellow edges;
% \end{enumerate}
%\end{lemma}
%\begin{proof}
%For clarity, in the case a vertex splits out multiple walkers at the block-step boundary at time $t$, we can process them in an arbitrary order, and notice each $F$ edge splits out does not affect the desired invariant at time $t$ since each such edge that appears in the branch-chasing graph with a walker on the boundary via local injectivity of graph matrix.
%
%% Suppose this is true for vertex $v$ when it last appears in an $H$-connected component on the boundary at time $t$, and we arrive at $v$ again at time $t'$ from $u$ using a leg $u\rightarrow v$ , we are to show the invariant at the end of current time-mark $t'$. We consider how $v$'s incidental $F$ edges may change from $t$ to the end of $t'$. Notice there may be multiple edges in the current step lead to $v$ at time $t'$, however, we can process the walkers in order and therefore assume in each time-mark only one edge is being used.
% 
% Suppose the current edge being used goes from $u$ to $v$, let time $t$ be the last time mark $v$ appears in the $H$ component at the boundary (before the edge at time $t$ gets used), and call the component $H_{v,t}$. We start by partitioning the unclosed $F$ edges incident to $H_{v,t}$ at time $t$ according to whether they contribute to $\pur_t(v)$, i.e. whether they appear as a directed edge going out from some vertex in $ H_{v,t}$ in the branch-chasing graph at time $t$. Let those that contribute (i.e. unprotected) be in $O_{t}(v)$ and the others (i.e. protected edges) be in $B_{t}(v)$.  Notice the last departure from $H_{v,t}$ (not necessarily from vertex $v$) at time $t$ may create one edge that is either in $B$ or in $O$ at time $t+1$. Our argument relies upon keeping track of how $B$ and $O$ may change between these two time-marks, and we now case on the status of the leg $u\rightarrow v$ at the current time-mark $t'$ (after the edge at $t'$ is used),
% \begin{comment}
%  \begin{enumerate}
% 	\item if the walker arrives via an $R$ edge, this edge does not contribute to any gain of $\pur_{t'}(H_{v,t})$ over $\pur_{t}(H_{v,t})$: 
%	 at time $t<t_m<t'$, there are two cases while either we close an edge that we use to depart from $H_{v,t}$, or the edge that we open at time $t$ remains open while we close a previously open edge $F$ at the return and therefore this edge is no longer contributing to the vertices in 
%		 any such leg alone does not contribute to any gain of $\pur_{t'}(H_{v,t})$ over $\pur_t(H_{v,t})$;
%	\item if the walker arrives via an $F$ edge, any such edge is a surprise visit and contributes to both the gain of  of $\pur_{t'}(H_{v,t})$ over $\pur_t(H_{v,t})$ and the gain of $s_{t'}(H_{v,t})$ over $s_t(H_{v,t})$; moreover, if the arriving walker also departs $H_{v,t}$ using $F$ edges at time $t$, i.e. it breaks an edge on branch-chase graph at the same time, and we pick up another factor of $1$ from $w_{t'}(H_{v,t})$;
%	\item there may be new non-surpirse $F$ edges (not part of dangling branches) open up from $v$ at time $t$ that now act as an incident $F$ edge to $v$, however, notice each such edge appears in the branch-chasing graph at time $t+1$ (i.e., right after edge in $t$ are encoded), and hence they either remain as an $F$ edge that points to the boundary on branch-chase graph, or they get removed while each removal assigns vertex $v$ a factor of surprise visit via a gain in $w_{t'}(H_{v,t})$ over $w_{t}(H_{v,t})$;
%	\item there may be surprise $F$ edges (not part of dangling branches) open up from $v$ at time $t$, though they never appear in the branch-chasing graph, while they contribute to the gain of  $w_{t'}(H_{v,t'})$ over $w_{t}(H_{v,t'})$ as a factor of hardwire surprise visits originating from this component; 
%	\item similarly for $F$ edges open before time $t$ that do not contribute to $\pur_t(H_{v,t})$ at time $t$  as they are part of the branch-chasing graph pointing to the boundary, that they either remain as an $F$ edge that points to the boundary on branch-chase graph, or they get removed while each removal assigns vertex $v$ a factor of surprise visit via a gain in $w(H_{v,t})$;
%	\item for new $F$ edges opened up at time $t$ by attaching dangling branches to $H_{v,t}$, they may now appear as unclosed $F$ edges that contribute to the gain of $\pur_{t'}(H_{v,t'})$, however, they also contribute to the gain of $\dang_{t'}(H_{v,t'})$ over $\dang_{t}(H_{v,t})$.
%\end{enumerate}
%\end{comment}
%
%\begin{enumerate}
%	\item Again, by construction, it suffices for us to consider the edge used at time $t'$ be $u\rightarrow v$ as either $F$ or $R$, since $H$ edge is automatically captured when we consider $H$-components;
%	\item If the walker arrives via an $R$ leg, and assume $v,u$ not in the same $H$ component before this leg as the other case is immediate via prior argument that calling an $R$ edge within the same component cannot increase $\pur$ factor. Therefore, it suffices for us to assume $u$ and $v$ being in disjoint $H$ components at time $t'-1$, i.e., before the use of the leg $u\rightarrow v$, and we can further restrict our attention to $H_{v,t'-1}$ as \[ 
%	\pur_{t'+1}\left(H_{v,t'}\right) = \pur_{t'+1}(H_{u,t'}) + \pur_{t'+1}(H_{v,t'}) \leq \pur_{t'}(H_{u,t'}) + \pur_{t'+1}(H_{v,t'})
%	\]
%	since calling an $R$ edge from an $H$-component cannot increase the $\pur$ factor on the original vertices, i.e. \[ 
%	\pur_{t'+1}(H_{u,t'})\leq \pur_{t'}(H_{u,t'}) 
%	\]
%	\item  Let $E_t$ be the edge that gets opened up at time $t$ when departing from $H_{v,t}$;
%	\item Consider the edges that may now contribute to $\pur_{t'}(H_{t,v})$ while not accounted for at time $t$, let this set of edges be $\Delta_{t'-t}(H_{v,t})$: they are either the edge $E_t$ if it is opened as a dangling edge, or an edge that shifts from $B_{t}$ to $O_{t'}$ (as well as potentially non-dangling $E_t$ that shifts from black to red), i.e., they are protected on the branch-chase graph at some time between $t$ and $t'-1$ as \emph{black} edges,  while no longer so at $t'$ since they are now \emph{red} edges; 	
%	\item For the edges that shift from black to red within the time interval $[t,t']$, we process them in an arbitrary order of their out-vertex in $a\in H_{v,t}$, and for each vertex's first edge being processed, we additionally case on whether the out-vertex $a$ has out-going red edge at time $t$: if not, the first edge flips $1_{a \text{ ever has outgoing red edge}}$ and this offsets the gain to the LHS; otherwise, any such edge assigns $a$ a factor of surprise visit via a gain in $w_{t'}(a)$ over $w_{t}(a)$, yielding  \begin{align*}
%	& |\Delta_{t'-t}(a) | \leq -1 \cdot \left( 1_{a \text{ has seen out-going red edge by } t' } - 1_{a \text{ has seen out-going red edge by } t } \right) + \left(w_{t'}(a) - w_{t}(a)\right)	
%%	&= -1 \cdot \left( 1_{a \text{ has seen out-going red edge by } t' } - 1_{a \text{ has seen out-going red edge by } t } \right) + \left(w_{t'}(a) - w_{t}(a)\right)	
%	\end{align*}
%	where we further observe $w_t(a) = w_{t+1}(a)$ as otherwise 
%	\item Furthermore, let $E_t$ be the edge that gets opened up at time $t$ when departing from $H_{v,t}$, notice the above bound can be improved to reserve the factor of $E_t$ should it shift to red from black, as we are only considering edges already revealed at time $t$, hence, introducing $w_t^{\setminus E_t}$ the short-hand that restricts the $w$ function to edge-recipient other than $E_t$, we can improve the above bound to \begin{align*}
%	&\text{number of revealed black out-going edges from $a$ shifted to red from $t$ to $t'$ } \\&\leq -1 \cdot \left( 1_{a \text{ has seen out-going red edge by } t' } - 1_{a \text{ has seen out-going red edge by } t } \right) + \left(w^{\setminus E_t}_{t'}(a) - w_{t}(a)\right)	
%	\end{align*}
%				\item As stated $E_t$ may contribute a gain of factor $1$ on the LHS via a gain in $\pur_{t'+1}(H_{v,t})$ if $E_t$ is not closed in the current arrival at $v$. Assuming not, we need to case on the status of the $E_t$ at time $t'$;
%		\item If the $R$ edge that gets closed contributed to $\pur_t(H_{v,t})$, i.e., $u\rightarrow v \in O_t(v)$,  (e.g. the edge is a surprise visit or a red out-going edge), this edge witnesses a drop of $1$ in $\pur_{t'+1}(v)$ over $\pur_t(v)$. On the other hand, the edge that gets open up at the departure from $v$ at time $t$ may now remain open at time $t'$ as an edge in $O$, contributing a $1$ to the $\pur$ factor. Combining the above, the $\pur_t(v)$ factor does not increase and we can additionally shift the color of $E_t$ from black to red without incurring any cost;
%	\item If the $R$ edge did not contribute to  $\pur_t(v)$, this is an $R$-chase, i.e., it is a \emph{black} edge incident to $v$ protected at time $t$, and it gets closed at time $t'$, and we need to case on the status of $E_t$, the edge that gets opened up at time $t$.
%%	\item If $E_t$ was opened up as a black edge, it either remains protected as a black edge or a sole red edge, hence does not contributing a gain to $\pur_{t'}(v)$, or it turns red while its gain is now offset by the gain in $w_{t'}(v)$ over $w_t(v)$ where we recall $w$ is the function that assigns surprise visits to vertices incident to excess red edges;
%	\item If $E_t$ was opened up as dangling edge, and moreover, as a dangling attachment edge, we pick up a gain in $\dang_{t'}(H_{v,t})$ over $\dang_t(H_{v,t})$ that can offset the gain from edge. Otherwise, $E_t$ is a  a green edge, i.e., part of some dangling branch while not an attachment edge, $E_t$ is then captured by the factor of $\green_t(v)$: it is either forced as the sole green edge, or it gets assigned surprise visit factors via the function $\green_t(v)$, letting $E_t$'s out-going vertex be $a$, we have \begin{align*}
%&1_{E_t \text{ is opened as a dangling edge} } \\& \leq \left(\underbrace{\dang_{t'}(a) - \dang_{t}(a)}_{\text{dangling attachment} } \right) + \bigg(-1\cdot 1_{E_t \text{ is the first out-going green edge from } a} + \left(\green_{t'}(a)- \green_t(a)\right) \bigg) 		
%	\end{align*} 
%%		\item  In this case, we conider whether  $E_t$ is a black edge at time $t'$: it either remains protected or it gets assigned a factor via a gain of surprise visit in $w_{t'}(H_{v,t'-1})$ over $w_t(H_{v,t})$ which offsets the gain of $1$ on the LHS from $E_t$;
%%	\item Notice the arguments are identical to the $1$-in-$1$-out if the edge that gets closed is not protected in time $t$, and we have $|O_t(v)| = |O_{t'}(v)|$ though they may differ as sets;	
%%\item Vertices in $H_{v,t}$ incident to green edges while not so anymore at time $t'$ may contribute a gain of factor $1$ in that gain of $\pur_{t'}(H_{v,t})$ over $\pur_t(H_{v,t})$, while noticing each such vertex gets assigned a drop of at least one green edge that ceases to contribute to  
%\item From the above, for the $H$-component restricted to vertices $H$-connected to $v$ at time $t'$, suppose an $R$ edge is used, (and noticing $H_{v,t'} = H_{v,t}$)
%	\begin{align*}
%		&\pur_{t'+1}(H_{v,t'}) - \pur_{t}(H_{v,t'}) \leq  \pur_{t'}(H_{v,t'}) - \pur_{t}(H_{v,t'})\\&\leq |\Delta_{t'-t}(H_{v,t})| +1_{E_t \text{ is opened up as a dangling edge}} \\&\leq \sum_{a \in H_{v,t} } -1 \cdot \left( 1_{a \text{ has seen out-going red edge by } t' } - 1_{a \text{ has seen out-going red edge by } t } \right) + \left(w_{t'}(a) - w_{t+1}(a)\right) \\
%		&+ \underbrace{\dang_{t'}(H_{v,t}) - \dang_{t}(H_{v,t})}_{\text{dangling attachment for } E_t} + \bigg(-1\cdot 1_{E_t \text{ is the first out-going green edge from } a} + \left(\green_{t'}(a)- \green_t(a)\right) \bigg) 	  \\
%		&\leq \sum_{a \in H_{v,t}} (w_{t'}(a) - w_t(a)) + (\dang_{t'}(a) - \dang_t(a)) + (\green_{t'}(a) - \green_t(a))
%		\\&= \sum_{a \in H_{v,t}} \Delta_{t'-t}\circ w(a) + \Delta_{t'-t}\circ \dang(a) + \Delta_{t'-t} \circ \green(a)
%				\end{align*}
%		where we introduce the short hands \[ 
%		\Delta_{t_1- t_2}\circ f(v) \coloneqq f_{t_1}(a) -f_{t_2}(a)
%		\]
%		for $f \in \{s,w,\dang,\green\}$ and $t_1> t_2$.
%%		Furthermore, recall we are considering the annexation of $H$-components (i.e. $v,u$ not $H$-connected at time $t'$) , combining with the factor of $H$-component restricted to $u$ at time $t'$ yields, \begin{align*}
%%			&\pur_{t'+1}(H_{v,t'+1}) = \pur_{t'+1}(H_{u,t'}) + \pur_{t'+1}(H_{v,t'})\\ &\leq \pur_{t'+1}(H_{u,t'})+  
%%		\end{align*} 
%	\ Combining with the component connected to $u$ at time $t'$ gives, (assuming $u,v$ again not in the same $H$-component at time $t'$) \begin{align*}
%		&\pur_{t'+1}(H_{v,t}) = \pur_{t'+1}(H_{u,t'}) + \pur_{t'+1}(H_{v,t'})\\
%		&\leq \pur_{t'}(H_{u,t'}) + \pur_{t}(H_{v,t'})  + \left(\pur_{t'+1}(H_{v,t}) - \pur_{t}(H_{v,t})\right) \\
%		&\leq s_{t'}(H_{u,t'}) + w_{t'}(H_{u,t'}) + \green_{t'}(H_{u,t'}) + s_{t}(H_{v,t}) + w_{t}(H_{u,t}) + \green_{t}(H_{u,t'}) \\
%		&+ s_{t'+1}(H_{v,t'})-s_{t}(H_{v,t'}) +\sum_{a \in H_{v,t}} \left(\Delta_{(t'+1)-t} \circ w(a) + \Delta_{(t'+1)-t}\circ \dang (a)  + 	\Delta_{(t'+1)-t}\circ \green(a) \right) \\
%		&\leq s_{t'+1}(H_{v,t'}) +  w_{t'+1}(H_{v,t'+1}) +  \dang_{t'+1}(H_{v,t'+1}) +  \green_{t'+1}(H_{v,t'+1})
%		 \end{align*}
%	where we use the property that the counter functions $\{s,w,\green, \dang \}$ is non-decreasing over time and factorizes over connected components. 
%	\item On the other hand, if the leg $u\rightarrow v$ is an $F$ edge, again assuming $u,v$ not being in the same $H$-component at time $t'$ and the other case is analogous, restricted to the $H_{v,t'}$, we have 
%	\begin{align*}
%		&\pur_{t'+1}(H_{v,t'}) - \pur_{t}(H_{v,t}) \leq |\Delta_{(t'+1) - t'}(H_{v,t})| + |\Delta_{t'-t}(H_{v,t})|   + 1_{E_t \text{is opened up as a dangling edge}} \\
%		&\leq |\Delta_{(t'+1) - t'}(H_{v,t})| + \sum_{a \in H_{v,t}}  \Delta_{t'-t}\circ w(a) + \Delta_{t'-t}\circ \dang(a) + \Delta_{t'-t} \circ \green(a)
%	\end{align*}
%	where we notice the factors restricted to last two terms are identical to the previous calculation when $R$ edge is used, and we can focus on the first term $|\Delta_{(t'+1) - t'}(H_{v,t})|$. Notice this set of edges are either the surprise visit we just opened up at time $t'$, or the edges that switch from black to red due to the current surprise visit (eg. potentially the edge $E_t$ that remains black at time $t'$ while now becoming red), and \begin{align*}
%		|\Delta_{(t'+1) - t'}(H_{v,t})| &\leq s_{t'+1}(H_{v,t'})-s_{t'}(H_{v,t'}) + \sum_{a\in H_{v,t'}} |\Delta_{(t'+1)-t'}(a)|
%			\end{align*}
%			Combining the above yields \begin{align*}
%		\pur_{t'+1}(H_{v,t'}) - \pur_{t}(H_{v,t}) 		\leq &s_{t'+1}(H_{v,t'})-s_{t}(H_{v,t'}) \\ +&\sum_{a \in H_{v,t}}  \Delta_{(t'+1)-t}\circ w(a) + \Delta_{(t'+1)-t}\circ \dang(a) + \Delta_{(t'+1)-t} \circ \green(a)
%			\end{align*}
%		Combining with the invariant for $H_{v,t}$ at time $t$ yields, \begin{align*}
%		\pur_{t'+1}(H_{v,t'+1}) &= \pur_{t'+1}(H_{v,t'}) \leq \pur_{t}(H_{v,t})	+ s_{t'+1}(H_{v,t'})-s_{t}(H_{v,t'}) \\ +&\sum_{a \in H_{v,t}}  \Delta_{(t'+1)-t}\circ w(a) + \Delta_{(t'+1)-t}\circ \dang(a) + \Delta_{(t'+1)-t} \circ \green(a)\\
%		&\leq s_{t'+1}(H_{v,t'+1}) + w_{t'+1}(H_{v,t'+1}) +  \dang_{t'+1}(H_{v,t'+1}) +  \green_{t'+1}(H_{v,t'+1})
%		\end{align*}
%
%%		%	\item if the walker arrives via an $F$ edge, any such edge is a surprise visit and contributes to both the gain of  of $\pur_{t'}(H_{v,t})$ over $\pur_t(H_{v,t})$ and the gain of $s_{t'}(H_{v,t})$ over $s_t(H_{v,t})$; moreover, if the arriving walker also departs $H_{v,t}$ using $F$ edges at time $t$, i.e. it breaks an edge on branch-chas
%\end{enumerate}
%\end{proof}

\paragraph{Putting things together for the final unforced return bound throughout the walk}
It suffices for us to consider each $H$-connected component when they last appear in the walk. Let $\{H_i,t_i\}$ be a sequence of $H$-connected components at the end of the walk, and time $t_i$ their last appearance time-mark, for a shape-walk $W$, we have \begin{align*}
	\pur(W) &\leq \sum_{H_i, t_i} \pur_{t_i}(H_{t_i})\\
	&\leq 2s_{t_i}(H_{i}) + \mir_{t_i}(H_i)+ \dang_{t_i}(H_{i}) +\green_{t_i}(H_i) \\
	&\leq 4\cdot s(W)+  \dang(W)
\end{align*} 
where we observe that each surprise visit may contribute a $2$ to the final bound via $s$ counter, and  a factor of $1$ via $\mir$ counter, a factor of $1$ via $\green$, and each $\dang$ attachment contributes a $1$ via $\dang$.

\begin{corollary}
Each surprise visit can cause at most $4$ unforced returns, i.e., it can be assigned to incur an extra vertex cost of at most $(2|V(\al)|q_\al)^{4}$ as each such confusion can be settled via a label in $2|V(\al)|q_\al$.
\end{corollary}
%\paragraph{Putting together unforced-return bound for set-indexed walk}

==> sparse_trace_method/preliminaries.tex <==
%\subsection{Preliminaries}
%\subsection{Preliminaries for norm bounds}

%
%\begin{definition}[Ordered-tuple indices]
%	Each ordered-tuple index is represented by a set $S\subseteq [n]$ and an ordering $\calO_S$ of elements in $S$. The size of ordered-tuple indices is given by $|S|$.
%\end{definition}
%\begin{definition}[Graphical matrix for shape indexed by ordered-tuple]
%Given a shape $\al$, we define graphical matrix (indexed by ordered-tuple) to be the matrix indexed by all possible ordered-tuples of $[n]$ with non-zero entries at $(S,\calO_S),(T,\calO_T)$ matrix ordered-tuple indices of size $|U_\al|$ and $|V_\al|$ s.t. \[ 
%M_{\al,\calO}[(S,\calO_S),(T,\calO_T)] = \sum_{\substack{f:V(\al)\rightarrow [n] \text{injective},\\ f(U_\al )=(S, \calO_S), 
% f(V_\al)=(T,\calO_T)\\ f(U_\al\cap V_\al) = (S\cap T, \calO_{S\cap T} )}  } \prod_{e=\{i,j\}\in E(\al)} \chi_G(f(i),f(j))
%\]
%where $G$ is an underlying random graph sample, and $\calO_S, \calO_T$ are orderings for vertices in $S$ and $T$.
%\end{definition}
%
%Analogously, we can define the graphical matrix for shape indexed by set-indices.
%
%\begin{definition}[Set-index]
%	Each set index is represented by a set $S\subseteq [n]$. The size of set indices is given by $|S|$.
%\end{definition}
%\begin{definition}[Consistent ordering]
%Given a ribbon $R $ with $U_R = S, V_R = T$, and $\calO_S, \calO_T, \calO_{S\cap T}$ an ordering for 
%	$S$ and $T$, we call $(\calO_S, \calO_T ,\calO_{S\cap T})$ a consistent ordering if there are orderings $\calO_{S}$ and $\calO_{S\cap T}$ agree on the ordering for vertices in $S\cap T$, and similarly, $\calO_{T}$ and $\calO_{S\cap T}$ agree on the ordering for vertices in $S\cap T$.
%\end{definition}
%
%\begin{definition}[Graphical matrix for shape indexed by set]
%Given a shape $\al$, we define graphical matrix (indexed by set) to be the matrix indexed by all possible subsets of $[n]$ with non-zero entries at $S,T$ matrix set-indices of size $|U_\al|$, $|V_\al|$ and $S\cap T$ a set index of size $|U_\al\cap V_\al|$ s.t. \[ 
%M_\al[S,T] = \sum_{\substack{f:V(\al)\rightarrow [n] \text{injective},\\ \exists \calO_S s.t. f(U_\al)=(S, \calO_S),\\ \exists \calO_T s.t.
% f(V_\al)=(T,\calO_T) \\ f(U_\al\cap V_\al) = (S\cap T, \calO_{S\cap T}) }} \prod_{e=\{i,j\}\in E(\al)} \chi_G(f(i),f(j))
%\]
%where $G$ is an underlying random graph sample, and $\calO_S, \calO_T$ are orderings for vertices in $S$ and $T$ and $\calO_{S\cap T}$ an ordering for $S\cap T$ consistent with $\calO_S, \calO_T$.
%\end{definition}
%\begin{remark}
%Throughout our work, we will use $M_\al$ to denote graphical matrix with set indices and $M_{\al, \calO}$ with ordered-tuple indices.
%\end{remark}
%
%

%\begin{definition}[Tree-like shape]
%	We call a shape $\al$ tree-like if there is no short cycle in the shape $\al\circ\al^T$ and $\al^T\circ \al$, i.e., every vertex has only one path to $U_\al\cup V_\al$.
%\end{definition}
%\begin{definition}
%	We call a shape cyclic if it is not tree-like.
%\end{definition}

%\paragraph{More terminologies for shapes}
%\begin{definition}[Floating vertex, and floating component]
%	For a given shape $\al$, we call a connected component $Q\subseteq V(\al)$ a floating component if $Q$ is not connected to $U_\al \cup V_\al$. For each floating component, we arbitrarily pick a vertex to be the first vertex of the component in encoding. Let $E_\al(\float)\subseteq E_\al$ be the set of edges in a floating component.
%\end{definition}
%\begin{definition}[Simple path]
%	We call a path simple if it does not traverse any edge more than once. However, it may traverse a vertex more than once.
%\end{definition}
%\begin{definition}[Dangling and non-dangling vertex]
%	For a given shape $\al$, we call a vertex $v\in V(\al)$ a ''dangling'' vertex if it is not on any simple path from $U_\al$ to $V_\al$; otherwise, we call the vertex ''non-dangling''. We denote the set of dangling (and non-dangling) vertices of shape $\al$ by $V_\al(\dang)$ (and  $V_\al(\nd)$) respectively.
%\end{definition}
%
%\begin{definition}[Dangling branch]
%	 Given a shape $\al$, for any non-dangling vertex $v$ incident to dangling vertices, consider the collection of dangling-vertices reachable from $v$ without passing through any other non-dangling vertex, by possibly removing excess edges that lead to visited vertices, this is a tree of dangling-vertices rooted at $v$, and we can pick an arbitrary order to go through the leaves, and identify a tree-path to the leaf such that each path-segment is a branch whose \begin{enumerate}
%	 	\item  branch-head is either a vertex in some previously identified branch or $v$;
%	 	\item  branch-tail is a leaf.
%	 \end{enumerate} 
%	 Moreover, we write $\dang(\al)$ as a collection of dangling branches in $\al$.
%\end{definition}	
%\begin{remark}
%	For clarity, the reader should keep in mind the example where each non-floating degree-$1$ vertex in $V(\al)\setminus U_\al\cup V_\al$ is dangling and a branch-tail.
%\end{remark} 
%\begin{definition}[Sparse MVS]
%	For a given shape $\al$ with no floating and dangling vertex, we let $S$ the Sparse MVS be the maximizer of \[ 
%	\max_{S:\text{ separator}} \sqrt{n}^{|V(\al)\setminus V(S)|}\left(\sqrt{\frac{n}{d}} \right)^{E(S)}
%	\]
%	And we call the above quantity its corresponding SMVS-value.
%\end{definition}
%\begin{definition}[$S_L$ and $S_R$]
%	For a given shape $\al$, for a vertex $v\in S$, \begin{enumerate}
%		\item $v\in S_L$ if it can be reached from $U_\al$ without passing through any other vertex in $S$;
%		\item $v\in S_R$ if it can be reached from $V_\al$ without passing through any other vertex in $S$;
%	\end{enumerate}
%\end{definition}
%\subsection{Block walk for graph matrix}
%To bound the trace, it is useful to expand out the sum and notice each term can be described by a shape-walk as the following.
%\begin{definition}[Constraint-graph for set indices]
%	Given a shape $\al$, and $q\in \N$,  we define $V(\al,2q)$ to be the graph defined as the following,\begin{enumerate}
%		\item Take $q$ copies of $\al_1,\dots,\al_q$ of $\al$, and $q$ copies of $\al_{1}^T,\dots, \al_q^T$ of $\al^T$;
%		\item Each boundary $U_{\al_i}, V_\al = U_{\al^T_i}, V_{\al^T_i}$ is specified by a subset in $[n]$;
%		\item For each $i\in [q]$, we require the boundary to be consistent as set, i.e. $U_{\al_i} = V_{\al^T_{i-1}}$ and $U_{\al^T_{i}} = V_{\al_i}$	 with each as a set equality;
%		\item Additionally, each such walk must be clsoed, i.e., $V_{\al^T_i} = U_1$ as a set-equality;
%		\item We call each $\al_i$ and $\al^T_i$ block a block-step in the walk.
%\end{enumerate}
%\end{definition}
%
%
%	Each term in the summation of $\Tr\left[(M_\al M_\al)^{q}\right]$ is a shape-walk consists of block steps, and bounding the value and the count of such walks shall be the main subject of our work.
%	
%\paragraph{Trace metod basics}
%\begin{definition}[Indicator functions]
%	Let $\bdd[G]$ be the indicator function for bounded degree, i.e. $\bdd[G]=1$ if every vertex in $G$ has degree bounded by $d$, and $0$ otherwise; let $\cycle[G]$ be the indicator function for the absence of nearby $2$-cycle, i.e., $\cycle[G]=1$ if there is no nearby $2$-cycle in $G$, and $0$ otherwise.
%\end{definition}
%\begin{definition}[$2$-cycle free radius]
%	Let $\kappa$ be the radius of $2$-cycle free neighborhood. It will be set as $\kappa \coloneqq 0.3\log_d n$.
%\end{definition}
%\begin{definition}[Edge and leg]
%	We use ''edge'' to refer to the undirected edge in the underlying random graph sample, and ''leg'' to refer to a directed edge in the walk. \end{definition}
%
%\begin{definition}[Singleton edge]
%	We call an edge singleton if it appears only once in the walk.
%\end{definition}
%\begin{definition}[Surprise visit]
%We call a leg a surprise leg/visit if it uses a new edge that leads to a previously visited vertex in the walk. \end{definition}


==> sparse_trace_method/sparse-norm-bound-conditioning.tex <==
\section{Sparse Norm Bounds under Conditioning }
In this section, we want to tighten the norm bound \ref{thm:sparse-norm-bounds} by conditioning on the high probability event where ultra-dense subgraph do not appear in the random graph sample from $G_{n,p}$. For simplicity, we will condition on the event that the graph does not have more than $2$-cycle in any $\ell$-neighborhood for $\ell\leq c\log^2n$.
\jnote{Let's address the $V^V$ later...}

\begin{definition}[$\ell$-forbidden shapes] Let $\al$ be a shape, we call it  $\ell$-forbidden if for any $i\in V(\al)$, $B_\ell(i; E(\al))$ witnesses at least $2$ cycle where  $B_\ell(i; E(\al))$ is the radius-$\ell$ neighborhood of $i$ induced by edges $E(\al)$. 
 \end{definition}

We first recall the following known norm bound,
\begin{theorem}[Sparse Norm Bounds]
For any shape $\alpha$ such that $U_{\alpha} \cap V_{\alpha} = \emptyset$ and any $q \in \mathbb{N}$, 
%$E\left[tr\left(\left(M_{\alpha}M_{\alpha}^T\right)^q\right)\right]$ is 
\[
\E\left[\tr\left(\left(M_{\alpha}M_{\alpha}^T\right)^q\right)\right] \leq n^{|V(\alpha)|}\left((4|V(\alpha|)^{|V(\alpha)|}\right)^{2q}\left(\max_{\text{separator } S}{n^{\frac{|V(\alpha)| - |S|}{2}}\left(\frac{3}{\sqrt{p}}\right)^{E(S)}q^{|S|-\frac{|L_S| + |R_S|}{2} + \frac{c(\alpha,S)}{2}}}\right)^{2q-2}.
\]
\end{theorem}

\begin{conjecture}For any shape $\alpha$ s.t. $U_\al \cap V_\al = \emptyset$ and any $q\in \N$, for any separator $S$, let $E(S)$ denote the number of edges inside $S$, and $\psi(S)$ the maximal subset of $E(S)$ s.t.  $G(V(S), \psi(S))$ is not $\ell$-forbidden,
\[
\E\left[\tr\left(\left(M_{\alpha}M_{\alpha}^T\right)^q\right)\right] \leq n^{|V(\alpha)|}\left((4|V(\alpha|)^{|V(\alpha)|}\right)^{2q}\left(\max_{\text{separator } S}{n^{\frac{|V(\alpha)| - |S|}{2}} 3^{E(S)} \left(\frac{1}{\sqrt{p}}\right)^{2\psi(S)-E(S)}q^{|S|-\frac{|L_S| + |R_S|}{2} + \frac{c(\alpha,S)}{2}}}\right)^{2q-2}.
\]
\jnote{this bound should be able to be tightened when there are extra excess edges outside $E(S)$, however, it might be tight when its a tree once we contract $S$ into a jumbo vertex}
\end{conjecture}

\subsection{Bounding Walk Value}
For a fixed walk $P$, let $S$ be the set of edges that only appear once, and $T$ the set of edges that appear at least twice,
we are interested in bounding $|\E\left[\val(P) \1[\calE]\right] |$ where $\calE$ is the event that the graph has no nearby $2$-cycle.
\begin{lemma} Let $\Psi=H_\Psi+J_\Psi \subseteq E(P)$ be the maximally unforbidden subgraph of $G(P)$ induced by multi-edges in $P$ (counting multiplicity), where $H_\Psi = \Psi\cap T$ and $J_\Psi = \Psi \cap S$, let $\cl(E)$ be the number of cycles induced by edges in $E$,
\[
 \left|\E\left[\val(P) \cdot\1\calE\right]\right|\leq 2^{|T|} \sqrt{\frac{n}{d}}^{S+\mul(T)}(\frac{d}{n})^{|S|+|H_\Psi|+\mul(\bar{H_\Psi}) } C(\log n)^2\gamma(S,T)2^{|S|}n^{-0.7(\frac{|S|}{\ell}-\cl(S\cup T))}
 \]
\end{lemma}
\begin{remark}
The important factor in the above claim is the exponential decay in terms of $|S|$, and we have decay surprise visit to handle the extra $n^{\cl(S\cup T)}$ as the number of surprise visits upper bounds the number of cycles.
\end{remark}
\begin{proof}
Given a walk $P$, let $G(P)$ be the edge-induced subgraph by $P$, and let $\psi(P)$ be again the maximally unforbidden graph of $G$ s.t. any $\ell$-neighbordhood of $G(P)$ is unforbidden. For convenience, we will also denote $\bar{H}=T\setminus H$ for $H\subseteq T$, and similarly $\bar{J}=S\setminus J$ for $J\subseteq S$. 
\begin{align*}
    &\left|\E\left[\val(P) \cdot\1\calE\right ]\right|\\ &= \left|\E[\prod_{e\in S\cup T} \left((\chi_e -\frac{d}{n}) \sqrt{\frac{n}{d}} \right)^{\mul(e)} \1{\calE}   \right|
    \\
    &= \sqrt{\frac{n}{d}}^{S+\mul(T)} \left|\E\left[\sum_{H\subseteq T, J\subseteq S} (1-\frac{d}{n})^{\mul(H)+\bar{H}}(\frac{d}{n})^{H+\mul(\bar{H})}(-1)^{\mul(\bar{H})+\bar{J} } (1-\frac{d}{n})^{J+\bar{J}}(\frac{d}{n})^{J+\bar{J}}\1{\calE |X_{H\cup J}=1, X_{\bar{H}\cup\bar{J}}=0 }\right]  \right|\\
    &\leq \sqrt{\frac{n}{d}}^{S+\mul(T)} \sum_{H\subseteq T} (\frac{d}{n})^{H+\mul(\bar{H})} \left|\E\left[ \sum_{J\subseteq S}(1-\frac{d}{n})^{J+\bar{J}}(\frac{d}{n})^{J+\bar{J}}(-1)^{\bar{J}}\1{\calE |X_{H\cup J}=1, X_{\bar{H}\cup\bar{J}}=0 } \right] \right|  \\
    &\leq   2^{T}\sqrt{\frac{n}{d}}^{S+\mul(T)}\max_{H\subseteq T}(\frac{d}{n})^{H+\mul(\bar{H})} \left|\E\left[ \sum_{J\subseteq S}(1-\frac{d}{n})^{|S|}(\frac{d}{n})^{|S|} (-1)^{\bar{J}}\1{\calE |X_{H\cup J}=1, X_{\bar{H}\cup\bar{J}}=0 } \right] \right| \\
    &= 2^{T}\sqrt{\frac{n}{d}}^{S+\mul(T)}\max_{H\subseteq T}  (\frac{d}{n})^{H+\mul(\bar{H})}(\frac{d}{n})^{|S|} \left| \sum_{J\subseteq S}(-1)^{\bar{J}}\Pr[\calE |X_{H\cup J}=1, X_{\bar{H}\cup\bar{J}}=0] \right|
    % &\leq  \left|\sum_{H\subseteq T, J\subseteq S}\prod_{e\in H\cup J} \left((1-\frac{d}{n})\sqrt{\frac{n}{d}}\right)^{\mul(e)} \prod_{e\in \bar{H}\cup \bar{J}}\left(-\frac{d}{n} \sqrt{\frac{n}{d}}\right)^{\mul(e)} \Pr[X_{H\cup J} = 1, X_{\bar{H}\cup \bar{J}}=0, \calE] \right|\\
    % &\leq \sqrt{n/d}^{S+\mul(T)} \left| \sum_{J\subseteq S} (1-\frac{d}{n})^{J}(-\frac{d}{n})^{S-J} \Pr[X_{T\cup J}=1, X_{S/J}=0, \calE]    \right|\\
    % &\leq \sqrt{n/d}^{S+\mul(T)} \left| \sum_{J\subseteq S} (1-\frac{d}{n})^{J}(-\frac{d}{n})^{S-J} (\frac{d}{n})^{J\cup T} (1-\frac{d}{n})^{S-J} \Pr[ \calE | X_{T\cup J}=1, X_{S/J}=0]  \right|\\
    % &\leq \sqrt{n/d}^{S+\mul(T)} (\frac{d}{n})^{S\cup T} \left|\E \sum_{J\subseteq S} (-1)^{S-J} \Pr[\calE| X_{T\cup J}=1, X_{S/J}=0]  \right|\\
    % &=\gamma(S,T) \left|\sum_{J\subseteq S} (-1)^{S-J} \Pr[\calE| X_{T\cup J}=1, X_{S/J}=0]   \right|
\end{align*}
It now remains to bound the quantity $(\frac{d}{n})^{H+\mul(\bar{H})}(\frac{d}{n})^{|S|} \left| \sum_{J\subseteq S}(-1)^{\bar{J}}\Pr[\calE |X_{H\cup J}=1, X_{\bar{H}\cup\bar{J}}=0] \right|$ for a fixed $H\subseteq T$.

To work with the distribution of $G_{n,p}$ conditioned on $X_{H\cup J}=1, X_{\bar{H}\cup \bar{J}}=0$, we appeal to the observation in Fan-Montanari, and consider an alternative distribution on  $G'$ a random graph sample where we sample edges outside $S\cup T$ w.p. $\frac{d}{n}$.
\begin{observation}
Consider $G'$ a random graph distribution where we sample edges outside $S\cup T$ w.p. $\frac{d}{n}$, then for any $J\subseteq S$, the following two distributions equal to each other, $$ \mu\{G' \cup H\cup J\} = \mu\{G|X_{H\cup J}=1, X_{\bar{H}\cup \bar{J}}=0\}$$ .
\end{observation}
\begin{observation}
Defining $f(g')=\sum_{J\subseteq S} (-1)^{S-J} \1{\calE|g'\cup J\cup T} $, then $$ 
\sum_{J\subseteq S} (-1)^{S-J} \Pr_{G\sim D_0}[\calE| X_{T\cup J}=1, X_{S/J}=0] = E_{g'\sim G'}[f(g')]
$$
\end{observation}
We now shift our attention to the $f$ function. Consider a fixed $g'$ sampled from $G'$, notice that if there is an edge $e\in S$ that is \textbf{unforced}, i.e., for any $J\subseteq S\setminus\{e\}$, $\1\{\calE[g'\cup \{e\}\cup \{J\} \cup \{T\} ]\} =\1\{\calE[g'\cup \{J\} \cup \{T\} ] \}$, then $f(g')=0$. 


\begin{definition}
 Given a subgraph $g'$ and edge set $A,B$, an edge $e\in S$ is forced w.r.t. $g\cup A\cup B$ if there exists $J\subseteq A\setminus \{e\}$, $\1{\calE|g'\cup \{e\}\cup \{A\} \cup \{B\} } \neq \1{\calE|g'\cup \{A\} \cup \{B\}  }$. 
\end{definition}

\begin{lemma}\label{lem: bounding-new-cycles}
$$\Pr_{g'\sim G'}[\text{ every edge in S is forced w.r.t. } g'\cup A\cup B] \leq  C(\log n)^2n^{-0.7(\frac{|S|}{\ell}-\cl(A\cup B) )}$$
\end{lemma}
\jnote{the log factor might not be exact}
\begin{proof}
We observe that this is the probability that each edge in $S$ is inside a cycle of length at most $\ell$ in $g'\cup S\cup T$ (that does not exist in $S\cup T$); and since there are $|S|$ edges in total, we have at least $\frac{|S|}{\ell}$ new cycles in $g'\cup S\cup T$. We now complete the proof by appealing to Lemma A.3 from Fan-Montanari.
\end{proof}
\begin{lemma}[Lemma A.3 of Fan-Montanari] Fix $d>1$. Let $S\subseteq \binom{n}{2}$ of size at msot $2\log^2n$. and let $\cl(S)$ denote the number of cycles induced by the edge set $S$, and let $\ell\leq 0.1\log_d n$. Let $G_0\cup S$ denote the random subgraph of the complete graph in which each edge outside of $S$ is present independently w.p. $\frac{d}{n}$ and each edge inside $S$ present w.p. $1$. Let $V\subseteq [n]$ be the set of vertices incident to at least one edge in $S$, then for some $C=C(d)>0, N_0=N_0(d)>0, n\geq N_0$ and any $0\leq t\leq (\log n)^2$,
\[ 
\Pr[\cl(B_\ell(V; G_0\cup S)\geq \cl(S)+t ]\leq C(\log n)^2n^{-0.7t}
\]
\end{lemma}
To wrap up the proof for the claim, we observe that if $\frac{S}{\ell}-\cl(S\cup T)<0$, then the bound is immediate as we can simply bound \[ 
 \left|\E\left[\val(P) \cdot\1\calE\right ]\right| =\gamma(S,T) \left|\sum_{J\subseteq S} (-1)^{S-J} \Pr_{G\sim D_0}[\calE| X_{T\cup J}=1, X_{S/J}=0]   \right|\leq  \gamma(S,T) 2^{S}
\]
On the other hand, if $\frac{S}{\ell}-\cl(S\cup T)\geq 0$, we will exploit Lemma \ref{lem: bounding-new-cycles}, and we have 
\begin{align*}
    \left|\E\left[\val(P) \cdot\1\calE\right ]\right| &=\gamma(S,T) \left|\sum_{J\subseteq S} (-1)^{S-J} \Pr_{G\sim D_0}[\calE| X_{T\cup J}=1, X_{S/J}=0]   \right|\\ 
    &\leq  \gamma(S,T) |\E_{g'}[f(g')]|\\
    &\leq \gamma(S,T) 2^{S}\Pr[f(g')\neq 0]\\
    &\leq \gamma(S,T) 2^{S} C(\log n)^2n^{-0.7(\frac{|S|}{\ell}-\cl(S\cup T))}
\end{align*}
\end{proof}
